Geometry of geodesics through Busemann measures in directed last-passage percolation

We consider planar directed last-passage percolation on the square lattice with general i.i.d. weights and study the geometry of the full set of semi-infinite geodesics in a typical realization of the random environment. The structure of the geodesics is studied through the properties of the Busemann functions viewed as a stochastic process indexed by the asymptotic direction. Our results are further connected to the ergodic program for and stability properties of random Hamilton-Jacobi equations. In the exactly solvable exponential model, our results specialize to give the first complete characterization of the uniqueness and coalescence structure of the entire family of semi-infinite geodesics for any model of this type. Furthermore, we compute statistics of locations of instability, where we discover an unexpected connection to simple symmetric random walk.

==> GeoWebPaper-Macros.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Packages go here
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{amsmath,amsfonts, amsthm,color,amssymb,mathrsfs,pgfplots,enumitem}   %F: enumitem is better than enumerate
%%% types of  labels:  [label=(roman*)]  \arabic*  \alph*    also under \itemize can use different symbols to mark items
\usepackage{times}
\RequirePackage[colorlinks,urlcolor=my-blue,linkcolor=my-red,citecolor=my-green]{hyperref}

\usepackage[numbers,comma,square,sort&compress]{natbib}
\usepackage{xargs}
\usepackage[colorinlistoftodos,prependcaption,textsize=footnotesize]{todonotes}
\usepackage{pdfcomment}
\usepackage{bm}
%\usepackage[left=1in,top=1in,right=1in,bottom=1in]{geometry}
\usepackage{scalerel}    %%%%  used first for scaling \bullet  
\usepackage{stmaryrd}   %%%% for integer interval notation 
\usepackage{mathabx}   %% made \widecheck work  
\usepackage{hyphenat}
\usepackage[utf8]{inputenc}
%\usepackage[notref,notcite]{showkeys}
%%%%  2019-03-22 Timo moved showkeys into the latex file itself in order to toggle it for printing. 
\usepackage{caption}
\usepackage{subcaption}
\usepackage{a4wide}
\usepackage{accents}
\usepackage{tikz}
\usetikzlibrary{arrows.meta,decorations.markings}
\usepackage{graphicx}
\usepackage{chngcntr}
\usepackage{float} %needed to fix the figures

\usepackage{rotating,centernot,cancel}    %% to manipulate symbols (Timo 2019-03-25) 

\numberwithin{figure}{section}
\numberwithin{equation}{section}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% New macros for this paper
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%General
\tikzset{middlearrow/.style={
        decoration={markings,
            mark= at position 0.6 with {\arrow{#1}} ,
        },
        postaction={decorate}
    }
}

\newcommand\aUset{\sV^{\,\w}} %The set of directions on which non-coalescence holds
%\newcommand\gpp{g_{\text{pp}}} %The shape function
\newcommand\gpp{g} %The shape function without pp subscript 
\newcommand\dgpp[1]{\widecheck{g}_{\text{pp}}^{#1}} %The shape function
\newcommand\T{T} %The shift, T
%\newcommand\cif{\xi_*} %The competition interface random variable
\newcommand\cid{\xi_*} %The competition interface random variable
\newcommand\adir{\zeta} 
\newcommand\wchk[1]{\widecheck{\omega}^{#1}} %Dual weights

%Busemann functions
\newcommand\B[1]{B^{#1}} %The Busemann function
\newcommand\BBbar[1]{{\overline B}^{#1}} %The Busemann function
\newcommand\Ubar{\overline U} %The Busemann function
\newcommand\dB[1]{u^{#1}} %The Busemann function
\newcommand\dBbar[1]{\overline{u}^{#1}} %The Busemann function

%Geodesics
\newcommand\geo[3]{\boldsymbol{\gamma}_{#1}^{\,#2,#3}} %Geodesic. Arguments are 1.) the index, 2.) the starting point, 3.) the direction
\newcommand\geobar[3]{{\overline{\boldsymbol{\gamma}}}_{#1}^{\,#2,#3}} %Geodesic. Arguments are 1.) the index, 2.) the starting point, 3.) the direction
\newcommand\geod[1]{\pi_{#1}} %A generic geodesic without a root or direction. The argument is the index.
%\newcommand\geod[1]{\boldsymbol{\gamma }_{#1}} %A generic geodesic without a root or direction. The argument is the index.


%Coalescence points
\newcommand\coal[1]{\mathbf{z}^{#1}} %Coalescence point. The argument is the direction.

%Split points
\newcommand\spt[2]{s_{#1}(#2)}


%The geodesic graphs and vertex sets 
\newcommand\G[1]{\mathcal{G}_{#1}} %The graph of geodesics. Argument is the direction.
\newcommand \dG[1]{\mathcal{G}^*_{#1}} %The dual graph to the graph of geodesics. Argument is the direction.
\newcommand\dGpp[1]{\widecheck{G}^{#1}} %The dual passage times
%\newcommand\dS[1]{\mathcal{T}_{#1}^{*}}
\newcommand\dS[1]{\mathcal{G}_{\cup#1}^{*}}   %% trying out another option

\def\Shock#1#2{{\bfS}^{#1}_{#2}}
\def\shock#1{{\bfS}_{#1}^*}      %%%% red points 
\def\ans#1#2{{\bfA}_{#1}^*(#2)}    %%%% ancestors 
\def\shockG#1{{\mathcal S}_{#1}^*}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Macros inherited from the DLR paper
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\addtolength{\hoffset}{-.8in} 
%\addtolength{\textwidth}{1.6in}
%\addtolength{\voffset}{-.3in} 
%\addtolength{\footskip}{.3in}
%\setlength{\oddsidemargin}{0in}
%\setlength{\evensidemargin}{0in}
%\setlength{\footskip}{0.2in}
%\setlength{\topmargin}{0.5in}
%\addtolength{\textheight}{.7in}
%\baselineskip=12pt   %%seems to make no difference? 
%\linespread{1.1}     %this works nicely to produce a more readable cropped 2-1


\RequirePackage{color}
\definecolor{my-link}{rgb}{0.5,0.0,0.0}
\definecolor{my-blue}{rgb}{0.0,0.0,0.6}
\definecolor{my-red}{rgb}{0.5,0.0,0.0}
\definecolor{my-green}{rgb}{0.0,0.5,0.0}
\definecolor{nicos-red}{rgb}{0.75,0.0,0.0}
\definecolor{really-light-gray}{gray}{0.8}
\definecolor{darkgreen}{rgb}{0.0,0.5,0.0}
\definecolor{darkblue}{rgb}{0.0,0.0,0.3}
\definecolor{nicosred}{rgb}{0.65,0.1,0.1}
\definecolor{light-gray}{gray}{0.7}

\definecolor{sussexg}{rgb}{0,0.7,0.7}
\definecolor{sussexp}{rgb}{0.4,0,0.4}
\definecolor{nicos-red}{rgb}{0.75,0.0,0.0}

\addtolength\marginparwidth{0.28in}

\newcommandx{\addmath}[2][1=]{\todo[linecolor=red,backgroundcolor=red!25,bordercolor=red,#1]{#2}}
\newcommandx{\fixtext}[2][1=]{\todo[linecolor=blue,backgroundcolor=blue!25,bordercolor=blue,#1]{#2}}
\newcommandx{\note}[2][1=]{\todo[linecolor=yellow,backgroundcolor=yellow!25,bordercolor=yellow,#1]{#2}}

%\pgfplotsset{compat=newest}
%\pgfplotsset{plot coordinates/math parser=false}
%\newlength\figureheight
%\newlength\figurewidth

%%%%%%   Symbols for plus and minus 
%\newcommand{\sig}{{\mbox{\larger$\square$}}}
%\newcommand{\gis}{\boxminus}
%\newcommand{\sig}{\boxempty}   % too large 
\newcommand{\sig}{{\scaleobj{0.8}{\boxempty}}} 
\newcommand{\sigg}{{\scaleobj{0.9}{\boxempty}}} 
%\newcommand{\sig}{{\raisebox{1pt}{\scaleobj{0.8}{\boxempty}}}}  
\newcommand{\gis}{{\raisebox{1pt}{\scaleobj{0.6}{\boxslash}}}}   
\newcommand{\giss}{{\raisebox{1pt}{\scaleobj{0.8}{\boxslash}}}}   
%\newcommand{\gis}{{\mbox{\larger$\diamond$}}}
%\newcommand{\sig}{\square}
%%%%    Try out also \ovoid and \ominus

\newcommand{\bbA}{\mathbb{A}}
\newcommand{\bbB}{\mathbb{B}}
\newcommand{\bbC}{\mathbb{C}}
\newcommand{\bbD}{\mathbb{D}}
\newcommand{\bbE}{\mathbb{E}}
\newcommand{\bbF}{\mathbb{F}}
\newcommand{\bbG}{\mathbb{G}}
\newcommand{\bbH}{\mathbb{H}}
\newcommand{\bbI}{\mathbb{I}}
\newcommand{\bbJ}{\mathbb{J}}
\newcommand{\bbK}{\mathbb{K}}
\newcommand{\bbL}{\mathbb{L}}
\newcommand{\bbM}{\mathbb{M}}
\newcommand{\bbN}{\mathbb{N}}
\newcommand{\bbO}{\mathbb{O}}
\newcommand{\bbP}{\mathbb{P}}
\newcommand{\bbQ}{\mathbb{Q}}
\newcommand{\bbR}{\mathbb{R}}
\newcommand{\bbS}{\mathbb{S}}
\newcommand{\bbT}{\mathbb{T}}
\newcommand{\bbU}{\mathbb{U}}
\newcommand{\bbV}{\mathbb{V}}
\newcommand{\bbW}{\mathbb{W}}
\newcommand{\bbX}{\mathbb{X}}
\newcommand{\bbY}{\mathbb{Y}}
\newcommand{\bbZ}{\mathbb{Z}}

%bold face
\newcommand{\bfA}{\mathbf{A}}
\newcommand{\bfB}{\mathbf{B}}
\newcommand{\bfC}{\mathbf{C}}
\newcommand{\bfD}{\mathbf{D}}
\newcommand{\bfE}{\mathbf{E}}
\newcommand{\bfF}{\mathbf{F}}
\newcommand{\bfG}{\mathbf{G}}
\newcommand{\bfH}{\mathbf{H}}
\newcommand{\bfI}{\mathbf{I}}
\newcommand{\bfJ}{\mathbf{J}}
\newcommand{\bfK}{\mathbf{K}}
\newcommand{\bfL}{\mathbf{L}}
\newcommand{\bfM}{\mathbf{M}}
\newcommand{\bfN}{\mathbf{N}}
\newcommand{\bfO}{\mathbf{O}}
\newcommand{\bfP}{\mathbf{P}}
\newcommand{\bfQ}{\mathbf{Q}}
\newcommand{\bfR}{\mathbf{R}}
\newcommand{\bfS}{\mathbf{S}}
\newcommand{\bfT}{\mathbf{T}}
\newcommand{\bfU}{\mathbf{U}}
\newcommand{\bfV}{\mathbf{V}}
\newcommand{\bfW}{\mathbf{W}}
\newcommand{\bfX}{\mathbf{X}}
\newcommand{\bfY}{\mathbf{Y}}
\newcommand{\bfZ}{\mathbf{Z}}

\newcommand{\bfa}{\mathbf{a}}
\newcommand{\bfb}{\mathbf{b}}
\newcommand{\bfc}{\mathbf{c}}
\newcommand{\bfd}{\mathbf{d}}
\newcommand{\bfe}{\mathbf{e}}
\newcommand{\bff}{\mathbf{f}}
\newcommand{\bfg}{\mathbf{g}}
\newcommand{\bfh}{\mathbf{h}}
\newcommand{\bfi}{\mathbf{i}}
\newcommand{\bfj}{\mathbf{j}}
\newcommand{\bfk}{\mathbf{k}}
\newcommand{\bfl}{\mathbf{l}}
\newcommand{\bfm}{\mathbf{m}}
\newcommand{\bfn}{\mathbf{n}}
\newcommand{\bfo}{\mathbf{o}}
\newcommand{\bfp}{\mathbf{p}}
\newcommand{\bfq}{\mathbf{q}}
\newcommand{\bfr}{\mathbf{r}}
\newcommand{\bfs}{\mathbf{s}}
\newcommand{\bft}{\mathbf{t}}
\newcommand{\bfu}{\mathbf{u}}
\newcommand{\bfv}{\mathbf{v}}
\newcommand{\bfw}{\mathbf{w}}
\newcommand{\bfx}{\mathbf{x}}
\newcommand{\bfy}{\mathbf{y}}
\newcommand{\bfz}{\mathbf{z}}


\newcommand{\mfa}{\mathfrak{a}}
\newcommand{\mfb}{\mathfrak{b}}
\newcommand{\mfc}{\mathfrak{c}}
\newcommand{\mfd}{\mathfrak{d}}
\newcommand{\mfe}{\mathfrak{e}}
\newcommand{\mff}{\mathfrak{f}}
\newcommand{\mfg}{\mathfrak{g}}
\newcommand{\mfh}{\mathfrak{h}}
\newcommand{\mfi}{\mathfrak{i}}
\newcommand{\mfj}{\mathfrak{j}}
\newcommand{\mfk}{\mathfrak{k}}
\newcommand{\mfl}{\mathfrak{l}}
\newcommand{\mfm}{\mathfrak{m}}
\newcommand{\mfn}{\mathfrak{n}}
\newcommand{\mfo}{\mathfrak{o}}
\newcommand{\mfp}{\mathfrak{p}}
\newcommand{\mfq}{\mathfrak{q}}
\newcommand{\mfr}{\mathfrak{r}}
\newcommand{\mfs}{\mathfrak{s}}
\newcommand{\mft}{\mathfrak{t}}
\newcommand{\mfu}{\mathfrak{u}}
\newcommand{\mfv}{\mathfrak{v}}
\newcommand{\mfw}{\mathfrak{w}}
\newcommand{\mfx}{\mathfrak{x}}
\newcommand{\mfy}{\mathfrak{y}}
\newcommand{\mfz}{\mathfrak{z}}


\newcommand{\mfG}{\mathfrak{G}}
\newcommand{\mfS}{\mathfrak{S}}

%script
\newcommand{\sA}{\mathcal{A}}
\newcommand{\sB}{\mathcal{B}}
\newcommand{\sC}{\mathcal{C}}
\newcommand{\sD}{\mathcal{D}}
\newcommand{\sE}{\mathcal{E}}
\newcommand{\sF}{\mathcal{F}}
\newcommand{\sG}{\mathcal{G}}
\newcommand{\sH}{\mathcal{H}}
\newcommand{\sI}{\mathcal{I}}
\newcommand{\sJ}{\mathcal{J}}
\newcommand{\sK}{\mathcal{K}}
\newcommand{\sL}{\mathcal{L}}
\newcommand{\sM}{\mathcal{M}}
\newcommand{\sN}{\mathcal{N}}
\newcommand{\sO}{\mathcal{O}}
\newcommand{\sP}{\mathcal{P}}
\newcommand{\sQ}{\mathcal{Q}}
\newcommand{\sR}{\mathcal{R}}
\newcommand{\sS}{\mathcal{S}}
\newcommand{\sT}{\mathcal{T}}
\newcommand{\sU}{\mathcal{U}}
\newcommand{\sV}{\mathcal{V}}
\newcommand{\sW}{\mathcal{W}}
\newcommand{\sX}{\mathcal{X}}
\newcommand{\sY}{\mathcal{Y}}
\newcommand{\sZ}{\mathcal{Z}}

\font \mymathbb = bbold10 at 11pt
\newcommand{\one}{\mbox{\mymathbb{1}}}
%\newcommand{\one}{\mathbf{1}}


\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\supp}{supp}

\def\esssup{\mathop{\mathrm{ess\,sup}}}
\def\range{\mathcal R}
\def\Uset{\mathcal U}
\def\fUset{\mathcal H}   % remove flat parts from \ri\Uset 
\newcommand{\dUset}[1]{\widecheck{\mathcal U}^{#1}}
%\def\Usetnice{\Uset_1}
\def\Usetnonuniq{\Uset_x^\w}
\def\Usetnonuniqz{\Uset_0^\w}
\def\Udense{\Uset_0}
\def\Ddense{\Diff_0}
\def\Usetnonuniqhat{\Uset_x^\what}
%\def\riUset{\Uset^\circ}

\newcommand{\fl}[1]{\lfloor{#1}\rfloor} 
\newcommand{\ce}[1]{\lceil{#1}\rceil}

\newcommand{\e}{\varepsilon}
\def\Diff{\sD}
\def\Cont{\sC}
\def\w{\omega}
\def\wbar{{\bar\w}}
\def\wtil{{\tilde\w}}
\newcommand{\ehat}{\widehat{e}}
\newcommand{\et}{\widehat{e}_1}   % e_1 + e_2 
\newcommand{\etstar}{\et^{\,*}}   %   (e_1 + e_2 )/2 
\newcommand{\ex}{\widehat{e}_2}   % e_2 - e_1 
\newcommand{\exstar}{\ex^{\,*}}   % (e_2 - e_1)/2  
\def\unif{\vartheta}
\def\Unif{\Gamma}
\def\eB{\kappa}
\def\EB{\cK}
\def\Bavg{\overline B}
\def\Gbar{\overline G}
\providecommand{\abs}[1]{\vert#1\vert}
\def\what{{\widehat\w}}
\def\wh{\widehat}
\def\wt{\widetilde}
\def\Omhat{\widehat\Omega}
\def\Omerg{\Omega^{\mathrm{???}}}
\def\Omreg{\Omega^{\mathrm{reg}}}
\def\Omjump{\Omega^{\mathrm{jump}}_0}
\def\OmCou{\Omega^{\mathrm{no3geo}}_0}
\def\Ombiinf{\Omega^{\mathrm{nobi}}_0}
\def\Omregjump{\Omega_0^{\mathrm{reg,jump}}}
\def\ddd{\displaystyle}
\def\fe{\Lambda}
\def\fepl{\fe_{\rm{pl}}}
\def\Zne{Z^{\rm NE}} 
\def\Qne{Q^{\rm NE}} 
\def\Zn{Z^{\rm N}} 
\def\xibar{\bar\xi}
\def\Abar{\overline A}
\def\zetabar{\bar\zeta}
\def\etabar{\bar\eta}
\def\hu{{\underline h}}
\def\ho{{\overline h}}
\def\ximin{{\underline\xi}}
\def\ximax{{\overline\xi}}
\def\ximinmin{\underline{\underline\xi}}
\def\ximaxmax{\overline{\overline\xi}}
\def\etaminmin{\underline{\underline\eta}}
\def\etamaxmax{\overline{\overline\eta}}
\def\zetaminmin{\underline{\underline\zeta}}
\def\zetamaxmax{\overline{\overline\zeta}}
\def\etamin{{\underline\eta}}
\def\etamax{{\overline\eta}}
\def\zetamin{{\underline\zeta}}
\def\zetamax{{\overline\zeta}}
\DeclareMathOperator{\ri}{ri}    %rel interior  
\DeclareMathOperator{\ext}{ext}    %extremes 
\DeclareMathOperator{\dist}{dist} 
%\def\xuDLR{x^{u,{\rm{DLR}}}}
\def\XDLR{\overline X^{\,x,\w}}
\def\Xtree{\widehat X^{\,\zeta,\w}}
\def\Xtreen{\widehat X^{\,\zeta,\w,(n)}}
%\def\backpix{{\overleftarrow{\pi}}^x} 
%\def\backpi{{\overset{\small\leftarrow}{\pi}}{}} 
\def\DLR{\mathrm{DLR}}
\newcommand{\siDLR}{\overrightarrow{\DLR}}
\newcommand{\biDLR}{\overleftrightarrow{\DLR}}
\def\CI{\phi}

\def\pici{\pi^{\rm{cif}}}
\def\ker{\kappa}
%\def\cid{\xi^*}
\def\Bci{B^*}
\def\Bcil{B^{*,\text\rm{(l)}}}
\def\Bcir{B^{*,\text\rm{(r)}}}
\def\Bbar{\overline B}
\def\Bbarci{\bar B^*}
%\def\cidm{\cid}
\def\cidmin{\underline\xi_{^{\scriptstyle*}}}
\def\cidmax{\overline\xi_*}
\def\ci{{\rm ci}}
\def\Pibar{\overline\Pi}
\def\Pici#1{\Pi^{\ci,\w,#1}}
\def\Picil#1{\Pi^{\ci,\w,\text\rm{(l)},#1}}
\def\Picir#1{\Pi^{\ci,\w,\text\rm{(r)},#1}}
\def\picix{\pi^{x,\ci}}
%\def\varphimin{\varphi^{{\text\rm{(l)}}}}
%\def\varphimax{\varphi^{{\text\rm{(r)}}}}
\def\cidl{\cid^{\text\rm{(l)}}}
\def\cidr{\cid^{\text\rm{(r)}}}
\def\cidlmin{\cidmin^{\text\rm{(l)}}}
\def\cidrmin{\cidmin^{\text\rm{(r)}}}
\def\cidlmax{\cidmax^{\text\rm{(l)}}}
\def\cidrmax{\cidmax^{\text\rm{(r)}}}
%\def\cTl{\cT^{\textrm{(l)}}}
%\def\thetal{\theta_*^{\text\rm{(l)}}}
%\def\thetar{\theta_*^{\text\rm{(r)}}}
%\def\Bcir{\overline B_*}
%\def\Bcil{\underline B_*}


\newcommand{\That}{\widehat{T}}
\def\Omtemphat{\widehat\Omega_0}
\def\Ommono{\Omega_{\rm{coc}}} %the Omega on which monotonicity (and other properties?) of cocycles holds
\def\Ommonohat{\widehat\Omega_{\rm{coc}}} %the Omega on which monotonicity (and other properties?) of cocycles holds
\def\Omcont#1{\Omega_{\rm{cont},#1}} %the Omega on which continuity holds at \xi
\def\Omconthat#1{\widehat\Omega_{\rm{cont},#1}} %the Omega on which continuity holds at \xi
\def\Omconstt#1{\Omega_{\rm{tilt},#1}} %the Omega on which h(B) is constant
\def\Omconsthat#1{\widehat\Omega_{\rm{tilt},#1}} %the Omega on which h(B) is constan
\def\Omback#1{\Omega_{#1,\downarrow0}} %the Omega on which the B-tree dies out
\def\OmBus{\Omega_{[\ximin,\ximax]}} %the Omega on which liminf and limsup bounds hold for Busemann limits for the given \xi
\def\Ombi{\Omega_{\rm{bi},[\ximin,\ximax]}} %the Omega on which liminf and limsup bounds hold for Busemann limits for the given \xi
\def\OmBuszeta{\Omega_{[\zetamin,\zetamax]}} %the Omega on which liminf and limsup bounds hold for Busemann limits for the given \zeta
\def\OmBusnice{\Omega_1} %the Omega on which Busemann limits exist on a dense set
\def\OmBusa{\Omega_a} %the Omega on which one force one solution holds 
\def\Omshape{\Omega_{\rm{shape}}} %the Omega on which the shape thms hold
\def\OmBushat{\widehat\Omega_{[\ximin,\ximax]}} %the Omega on which Busemann limit holds
\def\OmBushatzeta{\widehat\Omega_{[\zetamin,\zetamax]}} %the Omega on which liminf and limsup bounds hold for Busemann limits 
\def\OmBusallhat{\widehat\Omega_{\rm{Bus}}} %the Omega on which liminf and limsup bounds hold for Busemann limits for all \xi
\def\OmBusall{\Omega_{\rm{Bus}}} %the Omega on which liminf and limsup bounds hold for Busemann limits for all \xi
\def\Omexist{\Omega_{\rm{exist}}} %the Omega on which directedness of cocycle DLRs holds
\def\Omexistxi{\Omega_{\rm{exist},\xi}} %the Omega on which directedness of cocycle DLRs holds
\def\Omexisthat{\widehat\Omega_{\rm{exist}}} %the Omega on which directedness of cocycle DLRs holds
\def\Omdir{\Omega_{\rm{dir}}} %the Omega on which every DLR is directed
\def\Omdirhat{\widehat\Omega_{\rm{dir}}} %the Omega on which every DLR is directed
\def\OmBusPi{\Omega'_{[\ximin,\ximax]}} %the Omega on which DLR is Busemann for the given \xi
\def\OmBusPihat{\widehat\Omega'_{[\ximin,\ximax]}} %the Omega on which DLR is Busemann for the given \xi
\def\OmBusPiall{\Omega_{\rm{uniq}}} %the Omega on which Busemann limits will hold for all directions at once
\def\OmBusPiallhat{\widehat\Omega_{\rm{uniq}}} %the Omega on which Busemann limits will hold for all directions at once
\def\Omnondeg{\Omega_{\rm{nondeg}}}  %the Omega on which the only non-degenerate DLR solutions are \Pi^{e_i}
\def\OmBhat{\widehat\Omega_B}  %the Omega on which the DLR solution corresponding to B is directed
%\def\OmB{\Omega_B}  %the Omega on which the DLR solution corresponding to B is directed
%\def\Omreg{\Omega_{\rm{reg}}} % the Omega on which regular conditional probabilities are supported on the projection
\def\Omcif{\Omega_{\rm{cif}}} % the Omega on which regular conditional probabilities are supported on the projection
\def\Omnonuniq{\Omega_{\rm{ex}}} %the Omega on which Usetnonuniq does not intersect linear segments and includes non-diff points
\def\Omeihat{\widehat\Omega_{e_1,e_2}}


\def\WLLN{WLLN$_\xi$}
\def\SLLN{SLLN$_\xi$}
\def\proj{\pi}
\def\gDLR{\mathrm{gDLR}}
\def\cgDLR{\mathrm{cgDLR}}

\allowdisplaybreaks
%\allowdisplaybreaks[3]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Environment definitions go here
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{formal}[theorem]{Critical point derivation}
\newtheorem{experiment}[theorem]{Experimental Result}
\newtheorem{clam}[theorem]{Claim}
\newtheorem{condition}[theorem]{Condition}


\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
%\newtheorem{xca}[theorem]{Exercise}
\newtheorem{exercise}[theorem]{Exercise}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{conj}[theorem]{Conjecture}

%\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}
\newenvironment{remarks}{\begin{remark}\normalfont}{\end{remark}}
\newtheorem{quest}{Question}


%%%%%%%   the BEST  Timo macros (2018-01-19--)  %%%%%%%%

\newcommand{\nn}{\nonumber}

\DeclareMathOperator{\hull}{\overline{\text{co}}}
\DeclareMathOperator{\Span}{span}
\DeclareMathOperator{\bd}{bd}

\DeclareMathOperator{\sign}{sign} 
\DeclareMathOperator{\diam}{diam}
\DeclareMathOperator{\epi}{epi}
\DeclareMathOperator{\card}{card}
%\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\trace}{trace}
%\DeclareMathOperator{\dist}{dist}
\DeclareMathOperator{\var}{Var}
\DeclareMathOperator{\Var}{\mathbb Var}
  \DeclareMathOperator{\Cov}{Cov}  
  \DeclareMathOperator{\conv}{co}   %convex hull  


%\DeclareMathOperator{\proj}{Proj}
%\DeclareMathOperator{\ri}{ri}    %rel interior  
\DeclareMathOperator{\aff}{aff}   %affine hull  
\DeclareMathOperator{\effdom}{dom}   %eff domain 
\DeclareMathOperator{\id}{id}


\font \mymathbb = bbold10 at 11pt
\newcommand{\ind}{\mbox{\mymathbb{1}}}
%\def\ind{\mathbf{1}}
\def\deq{\overset{d}=} 
\def\dto{\overset{d}\to} 
\def\qedex{\hfill$\triangle$} 
\def\qedrm{\hfill$\triangle$} 
\def\iff{\Longleftrightarrow}
\def\implies{\Longrightarrow}
\def\rimplies{\Longleftarrow}

\newcommand{\bD}{\mathbb{D}}

\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}

\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}

\def\Z{\bbZ} 
\def\R{\bbR} 
\def\N{\bbN} 

\def\Xw{X}  %another letter for a weight 
\def\Yw{Y}  %another letter for a weight 
\def\Ywch{\wc\Yw}  %another letter for a weight 

\def\kvec{\mathbf{k}}  \def\mvec{\mathbf{m}}   \def\nvec{\mathbf{n}}
 \def\pvec{\mathbf{p}}
\def\xvec{\mathbf{x}}
\def\yvec{\mathbf{y}}
\def\zvec{\mathbf{z}}
\def\wvec{\mathbf{w}}
\def\Jvec{\mathbf{J}}
\def\Xvec{\mathbf{X}} \def\Yvec{\mathbf{Y}}  \def\Zvec{\mathbf{Z}} \def\thvec{\boldsymbol{\theta}}

\def\absorb{\triangleleft}

\def\timonote#1{{\color{darkgreen}{(#1)}}}
\def\E{\bbE}
\def\P{\bbP} %% environment measure 

 \def\wt{\widetilde}  \def\wh{\widehat} \def\wb{\overline} \def\wc{\widecheck}

\def\Bus#1{B^{#1}} 
\def\rBus#1{\wt B^{#1}}
\def\wtBus#1{\wt B^{#1}}
\newcommand\Busv[3]{\overline B^{\,#1,#2}_{#3}}

\def\RW{S}
\def\ZRW{Z}
\def\Zero{R}
\def\Zerobar{\overline\Zero}

%%%%%%%   Random measures with superscript "Bus" 
%\def\Bpp{\mathbf{n}^{\text{\rm Bus}}}  %  \Bpp = Busemann pt process of jump locations 
%\def\Bppa{{\boldsymbol\nu}^{\text{\rm Bus}}}   %  \Bppa = Busemann pt process of jump locations and jump sizes
%\def\Bppb{{\boldsymbol\mu}^{\text{\rm Bus}}}   %Busemann measure on edge k 
%\def\Bmeas{\mu^{\text{\rm Bus}}} 
%\def\Bmeasb{\boldsymbol{\nu}^{\text{\rm Bus}}} 
%\def\Bmm{m^{\text{\rm Bus}}}   %mean Busemann measure 

%%%%%  These random measures without superscript "Bus" 
\def\Bpp{\mathbf{n}}  %  \Bpp = Busemann pt process of jump locations 
\def\Bppa{{\boldsymbol\nu}}   %  \Bppa = Busemann pt process of jump locations and jump sizes
\def\Bppavar{\nu}   %  \Bppa = Busemann pt process of jump locations and jump sizes
\def\Bppb{{\boldsymbol\mu}}   %Busemann measure on edge k 
\def\Bmeas{\mu} 
\def\Bmeasb{\boldsymbol{\nu}} 
\def\Bmm{\lambda}   %mean Busemann point measure 
\def\umeas{u}   %measure of point locations of a purely atomic measure 

%\def\Hgraph{\cH}  %a graph 
\newcommand\Hgraph[1]{\mathcal{H}_{#1}}
\def\zclus{\bfK}    %notation for the backward cluster of z 
\def\cifset{\bfD}  %set of vertices with asymptotic cif direction in a set 
\def\xisim{\,\overset\xi\sim\,}    %equivalence relation  
%\def\zesim{\,\overset{[\zeta, \eta]}\sim\,}    %equivalence relation 
\def\zesim{ \overset{[\zeta, \eta]}\sim }    %equivalence relation without extra space

\def\depa{B}  %% departure processes from queues, also the generic variable for Busemanns in the description of the joint distribution. 
\def\serv{w}     %% service variables 

\def\level{\bbL}     %%%% levels on lattice 


  \def\evec{\mathbf{e}}  \def\uvec{\mathbf{u}}\def\vvec{\mathbf{v}}
   \def\avec{\mathbf{a}} \def\bvec{\mathbf{b}}

\newcommand\bnearrow{{\raisebox{1pt}{\scaleobj{0.5}{\mathbf\nearrow}}}}   %% \nearrow for a superscript so it doesn't look ridiculously big 
    
\def\caY{\cY^{\bnearrow}}  % a space of ordered n-tuples 
\def\caaY{\cY^{\bnearrow\!\bnearrow}}  % a space of ordered n-tuples 
\def\paramb{\tau}   %% needed a parameter -- not sure what a good letter choice is. 
   
\def\gdirv{\xi}    %geodesic direction 
\def\gdirc{\xi\cdot\evec}  %coordinate of a geodesic direction 

\def\Dop{D}    %%% D operator for departure process 
\def\Rop{R}  %% check weights or time in the back of the queue  
\def\Sop{S}    %%% S operator for sojourn time process 
\def\Daop{\cD}   %%n"bigger" operators 
\def\Taop{\cT}
\def\Saop{\cS} 
\def\rDop{{\overleftarrow\Dop}}    %%% reverse D operator for departure process 
\def\rRop{{\overleftarrow\Rop}}  %% check weights or time in the back of the queue  
\def\rSop{{\overleftarrow\Sop}}    %%% S operator for sojourn time process 
\def\fDop{{\overrightarrow\Dop}}    %%% forward D operator for departure process 
\def\fRop{{\overrightarrow\Rop}}  %%   forward
\def\fSop{{\overrightarrow\Sop}}    %%%   forward
\def\refl{\rho}   % reflection 

\def\OFP{(\Omega, \cF, P)} 
\def\OSP{(\Omega, \mfS, \P)}
   
   \newcommand{\lzb}{\llbracket}   %left Z bracket  
\newcommand{\rzb}{\rrbracket}   %right Z bracket 

\def\indep{\ \ \,{\raisebox{-1pt}{\text{\begin{rotate}{90}$\models$\end{rotate}}}}\ \, }  %independent random variables 
\def\nindep{\ \ \,{\raisebox{-1pt}{\text{\begin{rotate}{90}$\nvDash$\end{rotate}}}}\ \, }   %not independent random variables 

\newcommand\abullet{{\scaleobj{0.6}{\bullet}}}  %%%% smaller bullet to use inside functions 
\newcommand\bbullet{{\raisebox{0.5pt}{\scaleobj{0.6}{\bullet}}}} %% looks good for paths x_\bbullet 
\newcommand\brbullet{{\raisebox{-1pt}{\scaleobj{0.5}{\bullet}}}} %%  for subscript paths x_\brbullet   need negative raise 
\newcommand\cbullet{{\raisebox{1pt}{\scaleobj{0.6}{\bullet}}}}   %% looks good on Busemann process \Bus^\cbullet  as a subscript  

\newcommand\dbullet{{\scaleobj{0.7}{\bullet}}}   % same as \bbullet but without shift up

\newcommand\bcdot{{\scaleobj{1.8}{\cdot}}}
\newcommand\acdot{{\raisebox{-1pt}{\scaleobj{1.4}{\cdot}}}}  %%dot inside function 

%%%%%%%%   End Timo's macros %%%%%%%%%

%\usepackage{filemod}   
%\usepackage[short,nodayofweek,level,12hr]{datetime}   %%% clash

\overfullrule=5pt



==> JEMS Post-Accept Revision/Figs/cif-N5000L300.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
%
\definecolor{sussexg}{rgb}{0,0.7,0.7}
\definecolor{sussexp}{rgb}{0.4,0,0.4}
\definecolor{nicos-red}{rgb}{0.75,0.0,0.0}
%
\begin{tikzpicture}[scale=1.2]

\begin{axis}[%
%width=6.028in,
%height=4.754in,
%at={(1.011in,0.642in)},
%scale only axis,
%xmin=0,
%xmax=292,
%ymin=0,
%ymax=292,
unit vector ratio*=1 1 1,
axis line style={draw=none},
ticks=none,
axis x line*=bottom,
axis y line*=left
]

\addplot [color=nicos-red,  line width=1.0pt, forget plot]
  table[row sep=crcr]{%
0.5	0.5\\
1.5	0.5\\
1.5	1.5\\
2.5	1.5\\
2.5	2.5\\
3.5	2.5\\
4.5	2.5\\
4.5	3.5\\
5.5	3.5\\
6.5	3.5\\
7.5	3.5\\
8.5	3.5\\
8.5	4.5\\
8.5	5.5\\
8.5	6.5\\
8.5	7.5\\
9.5	7.5\\
10.5	7.5\\
10.5	8.5\\
11.5	8.5\\
12.5	8.5\\
13.5	8.5\\
14.5	8.5\\
15.5	8.5\\
15.5	9.5\\
16.5	9.5\\
17.5	9.5\\
18.5	9.5\\
19.5	9.5\\
20.5	9.5\\
21.5	9.5\\
22.5	9.5\\
23.5	9.5\\
24.5	9.5\\
25.5	9.5\\
25.5	10.5\\
26.5	10.5\\
27.5	10.5\\
28.5	10.5\\
29.5	10.5\\
30.5	10.5\\
31.5	10.5\\
32.5	10.5\\
33.5	10.5\\
34.5	10.5\\
35.5	10.5\\
36.5	10.5\\
37.5	10.5\\
38.5	10.5\\
38.5	11.5\\
38.5	12.5\\
38.5	13.5\\
38.5	14.5\\
39.5	14.5\\
40.5	14.5\\
41.5	14.5\\
42.5	14.5\\
42.5	15.5\\
43.5	15.5\\
44.5	15.5\\
45.5	15.5\\
46.5	15.5\\
47.5	15.5\\
47.5	16.5\\
48.5	16.5\\
49.5	16.5\\
50.5	16.5\\
51.5	16.5\\
52.5	16.5\\
53.5	16.5\\
54.5	16.5\\
55.5	16.5\\
56.5	16.5\\
57.5	16.5\\
58.5	16.5\\
59.5	16.5\\
59.5	17.5\\
60.5	17.5\\
60.5	18.5\\
61.5	18.5\\
62.5	18.5\\
63.5	18.5\\
64.5	18.5\\
65.5	18.5\\
66.5	18.5\\
67.5	18.5\\
68.5	18.5\\
69.5	18.5\\
70.5	18.5\\
70.5	19.5\\
71.5	19.5\\
72.5	19.5\\
73.5	19.5\\
74.5	19.5\\
75.5	19.5\\
76.5	19.5\\
77.5	19.5\\
78.5	19.5\\
79.5	19.5\\
80.5	19.5\\
81.5	19.5\\
82.5	19.5\\
83.5	19.5\\
84.5	19.5\\
85.5	19.5\\
85.5	20.5\\
86.5	20.5\\
87.5	20.5\\
88.5	20.5\\
88.5	21.5\\
89.5	21.5\\
89.5	22.5\\
90.5	22.5\\
91.5	22.5\\
91.5	23.5\\
92.5	23.5\\
93.5	23.5\\
94.5	23.5\\
95.5	23.5\\
96.5	23.5\\
97.5	23.5\\
98.5	23.5\\
99.5	23.5\\
100.5	23.5\\
100.5	24.5\\
101.5	24.5\\
101.5	25.5\\
102.5	25.5\\
103.5	25.5\\
104.5	25.5\\
105.5	25.5\\
106.5	25.5\\
107.5	25.5\\
108.5	25.5\\
109.5	25.5\\
110.5	25.5\\
111.5	25.5\\
111.5	26.5\\
112.5	26.5\\
113.5	26.5\\
114.5	26.5\\
115.5	26.5\\
116.5	26.5\\
117.5	26.5\\
117.5	27.5\\
118.5	27.5\\
118.5	28.5\\
118.5	29.5\\
119.5	29.5\\
119.5	30.5\\
120.5	30.5\\
121.5	30.5\\
122.5	30.5\\
123.5	30.5\\
124.5	30.5\\
125.5	30.5\\
126.5	30.5\\
126.5	31.5\\
127.5	31.5\\
128.5	31.5\\
128.5	32.5\\
129.5	32.5\\
130.5	32.5\\
131.5	32.5\\
132.5	32.5\\
133.5	32.5\\
134.5	32.5\\
135.5	32.5\\
136.5	32.5\\
137.5	32.5\\
138.5	32.5\\
139.5	32.5\\
140.5	32.5\\
141.5	32.5\\
142.5	32.5\\
143.5	32.5\\
144.5	32.5\\
145.5	32.5\\
146.5	32.5\\
147.5	32.5\\
148.5	32.5\\
149.5	32.5\\
150.5	32.5\\
151.5	32.5\\
152.5	32.5\\
153.5	32.5\\
154.5	32.5\\
155.5	32.5\\
156.5	32.5\\
157.5	32.5\\
158.5	32.5\\
159.5	32.5\\
160.5	32.5\\
161.5	32.5\\
162.5	32.5\\
163.5	32.5\\
164.5	32.5\\
165.5	32.5\\
166.5	32.5\\
167.5	32.5\\
167.5	33.5\\
168.5	33.5\\
169.5	33.5\\
169.5	34.5\\
170.5	34.5\\
171.5	34.5\\
172.5	34.5\\
173.5	34.5\\
174.5	34.5\\
175.5	34.5\\
176.5	34.5\\
177.5	34.5\\
178.5	34.5\\
179.5	34.5\\
180.5	34.5\\
181.5	34.5\\
181.5	35.5\\
182.5	35.5\\
183.5	35.5\\
183.5	36.5\\
183.5	37.5\\
183.5	38.5\\
184.5	38.5\\
185.5	38.5\\
186.5	38.5\\
187.5	38.5\\
188.5	38.5\\
189.5	38.5\\
190.5	38.5\\
191.5	38.5\\
191.5	39.5\\
192.5	39.5\\
193.5	39.5\\
194.5	39.5\\
195.5	39.5\\
196.5	39.5\\
197.5	39.5\\
198.5	39.5\\
199.5	39.5\\
200.5	39.5\\
201.5	39.5\\
202.5	39.5\\
203.5	39.5\\
204.5	39.5\\
205.5	39.5\\
206.5	39.5\\
207.5	39.5\\
208.5	39.5\\
209.5	39.5\\
210.5	39.5\\
211.5	39.5\\
212.5	39.5\\
213.5	39.5\\
214.5	39.5\\
215.5	39.5\\
216.5	39.5\\
217.5	39.5\\
218.5	39.5\\
219.5	39.5\\
220.5	39.5\\
220.5	40.5\\
220.5	41.5\\
221.5	41.5\\
222.5	41.5\\
223.5	41.5\\
223.5	42.5\\
224.5	42.5\\
225.5	42.5\\
225.5	43.5\\
226.5	43.5\\
227.5	43.5\\
228.5	43.5\\
229.5	43.5\\
230.5	43.5\\
231.5	43.5\\
232.5	43.5\\
233.5	43.5\\
234.5	43.5\\
235.5	43.5\\
236.5	43.5\\
237.5	43.5\\
238.5	43.5\\
239.5	43.5\\
240.5	43.5\\
241.5	43.5\\
241.5	44.5\\
242.5	44.5\\
243.5	44.5\\
244.5	44.5\\
245.5	44.5\\
246.5	44.5\\
247.5	44.5\\
};
\addplot [color=sussexp,  line width=1.0pt, forget plot]
  table[row sep=crcr]{%
0	0\\
1	0\\
2	0\\
3	0\\
4	0\\
5	0\\
6	0\\
7	0\\
8	0\\
9	0\\
10	0\\
11	0\\
12	0\\
13	0\\
14	0\\
14	1\\
15	1\\
16	1\\
17	1\\
18	1\\
19	1\\
20	1\\
21	1\\
22	1\\
23	1\\
24	1\\
25	1\\
26	1\\
27	1\\
28	1\\
29	1\\
30	1\\
30	2\\
31	2\\
32	2\\
33	2\\
34	2\\
35	2\\
36	2\\
37	2\\
38	2\\
39	2\\
40	2\\
41	2\\
42	2\\
43	2\\
44	2\\
45	2\\
46	2\\
47	2\\
48	2\\
49	2\\
50	2\\
51	2\\
52	2\\
53	2\\
54	2\\
55	2\\
56	2\\
57	2\\
58	2\\
59	2\\
60	2\\
61	2\\
62	2\\
63	2\\
64	2\\
64	3\\
65	3\\
66	3\\
67	3\\
68	3\\
69	3\\
70	3\\
71	3\\
72	3\\
73	3\\
74	3\\
75	3\\
76	3\\
77	3\\
78	3\\
79	3\\
80	3\\
81	3\\
82	3\\
83	3\\
84	3\\
85	3\\
86	3\\
87	3\\
88	3\\
89	3\\
90	3\\
91	3\\
92	3\\
93	3\\
94	3\\
95	3\\
96	3\\
97	3\\
98	3\\
99	3\\
100	3\\
100	4\\
101	4\\
102	4\\
103	4\\
104	4\\
105	4\\
106	4\\
107	4\\
107	5\\
108	5\\
109	5\\
110	5\\
111	5\\
112	5\\
113	5\\
114	5\\
115	5\\
115	6\\
116	6\\
117	6\\
117	7\\
117	8\\
117	9\\
118	9\\
119	9\\
120	9\\
121	9\\
122	9\\
123	9\\
124	9\\
125	9\\
126	9\\
127	9\\
128	9\\
129	9\\
130	9\\
131	9\\
132	9\\
132	10\\
133	10\\
134	10\\
135	10\\
136	10\\
137	10\\
138	10\\
138	11\\
138	12\\
139	12\\
140	12\\
140	13\\
140	14\\
141	14\\
142	14\\
143	14\\
144	14\\
145	14\\
146	14\\
147	14\\
148	14\\
149	14\\
150	14\\
150	15\\
151	15\\
152	15\\
153	15\\
154	15\\
155	15\\
156	15\\
157	15\\
158	15\\
159	15\\
160	15\\
161	15\\
161	16\\
162	16\\
163	16\\
164	16\\
165	16\\
166	16\\
167	16\\
168	16\\
168	17\\
169	17\\
170	17\\
171	17\\
172	17\\
173	17\\
174	17\\
174	18\\
175	18\\
176	18\\
177	18\\
178	18\\
179	18\\
180	18\\
181	18\\
182	18\\
183	18\\
184	18\\
185	18\\
186	18\\
187	18\\
188	18\\
189	18\\
190	18\\
191	18\\
192	18\\
193	18\\
194	18\\
195	18\\
196	18\\
197	18\\
198	18\\
199	18\\
200	18\\
201	18\\
202	18\\
203	18\\
204	18\\
204	19\\
205	19\\
206	19\\
207	19\\
208	19\\
209	19\\
210	19\\
211	19\\
212	19\\
213	19\\
214	19\\
215	19\\
216	19\\
217	19\\
218	19\\
219	19\\
220	19\\
221	19\\
221	20\\
221	21\\
222	21\\
223	21\\
223	22\\
224	22\\
225	22\\
226	22\\
227	22\\
228	22\\
229	22\\
229	23\\
230	23\\
230	24\\
230	25\\
231	25\\
232	25\\
232	26\\
233	26\\
234	26\\
234	27\\
235	27\\
236	27\\
237	27\\
238	27\\
239	27\\
240	27\\
240	28\\
240	29\\
241	29\\
242	29\\
242	30\\
243	30\\
244	30\\
245	30\\
246	30\\
247	30\\
248	30\\
249	30\\
249	31\\
250	31\\
250	32\\
251	32\\
252	32\\
253	32\\
253	33\\
254	33\\
255	33\\
256	33\\
257	33\\
257	34\\
258	34\\
};
\addplot [color=sussexg,  line width=1.0pt, forget plot]
  table[row sep=crcr]{%
0	0\\
0	1\\
0	2\\
1	2\\
1	3\\
1	4\\
1	5\\
1	6\\
1	7\\
2	7\\
2	8\\
3	8\\
3	9\\
4	9\\
5	9\\
5	10\\
6	10\\
7	10\\
7	11\\
7	12\\
7	13\\
8	13\\
9	13\\
10	13\\
11	13\\
12	13\\
13	13\\
13	14\\
14	14\\
14	15\\
14	16\\
14	17\\
14	18\\
15	18\\
16	18\\
17	18\\
18	18\\
19	18\\
20	18\\
21	18\\
22	18\\
23	18\\
24	18\\
25	18\\
25	19\\
25	20\\
26	20\\
27	20\\
27	21\\
27	22\\
27	23\\
27	24\\
28	24\\
29	24\\
29	25\\
30	25\\
30	26\\
31	26\\
32	26\\
33	26\\
34	26\\
35	26\\
36	26\\
36	27\\
37	27\\
38	27\\
39	27\\
40	27\\
41	27\\
42	27\\
43	27\\
44	27\\
45	27\\
46	27\\
47	27\\
48	27\\
49	27\\
49	28\\
49	29\\
50	29\\
51	29\\
52	29\\
52	30\\
53	30\\
54	30\\
54	31\\
54	32\\
55	32\\
56	32\\
57	32\\
58	32\\
59	32\\
60	32\\
60	33\\
61	33\\
61	34\\
62	34\\
63	34\\
64	34\\
65	34\\
66	34\\
66	35\\
66	36\\
66	37\\
66	38\\
66	39\\
66	40\\
66	41\\
66	42\\
67	42\\
68	42\\
69	42\\
70	42\\
71	42\\
72	42\\
73	42\\
74	42\\
75	42\\
76	42\\
76	43\\
77	43\\
77	44\\
77	45\\
78	45\\
79	45\\
80	45\\
81	45\\
82	45\\
83	45\\
84	45\\
85	45\\
86	45\\
87	45\\
88	45\\
89	45\\
90	45\\
91	45\\
92	45\\
93	45\\
94	45\\
95	45\\
96	45\\
97	45\\
98	45\\
99	45\\
100	45\\
101	45\\
102	45\\
103	45\\
103	46\\
103	47\\
104	47\\
105	47\\
106	47\\
107	47\\
108	47\\
109	47\\
110	47\\
111	47\\
112	47\\
113	47\\
114	47\\
115	47\\
116	47\\
116	48\\
116	49\\
117	49\\
117	50\\
117	51\\
118	51\\
119	51\\
120	51\\
121	51\\
122	51\\
123	51\\
124	51\\
124	52\\
125	52\\
126	52\\
126	53\\
126	54\\
127	54\\
128	54\\
128	55\\
129	55\\
130	55\\
130	56\\
131	56\\
131	57\\
131	58\\
131	59\\
131	60\\
131	61\\
132	61\\
133	61\\
133	62\\
134	62\\
135	62\\
135	63\\
136	63\\
136	64\\
136	65\\
137	65\\
137	66\\
138	66\\
139	66\\
140	66\\
140	67\\
140	68\\
140	69\\
141	69\\
141	70\\
141	71\\
142	71\\
142	72\\
143	72\\
144	72\\
145	72\\
146	72\\
147	72\\
147	73\\
148	73\\
149	73\\
150	73\\
150	74\\
151	74\\
151	75\\
152	75\\
153	75\\
153	76\\
153	77\\
154	77\\
154	78\\
155	78\\
156	78\\
157	78\\
158	78\\
159	78\\
160	78\\
160	79\\
160	80\\
160	81\\
160	82\\
161	82\\
161	83\\
162	83\\
163	83\\
163	84\\
163	85\\
164	85\\
165	85\\
166	85\\
167	85\\
168	85\\
169	85\\
169	86\\
169	87\\
170	87\\
171	87\\
172	87\\
173	87\\
174	87\\
175	87\\
176	87\\
177	87\\
178	87\\
179	87\\
180	87\\
181	87\\
181	88\\
182	88\\
183	88\\
184	88\\
185	88\\
186	88\\
186	89\\
187	89\\
188	89\\
189	89\\
190	89\\
191	89\\
192	89\\
193	89\\
194	89\\
195	89\\
196	89\\
197	89\\
197	90\\
198	90\\
198	91\\
199	91\\
200	91\\
201	91\\
};
\end{axis}
\end{tikzpicture}%

==> JEMS Post-Accept Revision/GeoWebPaper-AppA.tex <==
% !TEX root = GeoWebPaper.tex

\section{The geometry of geodesics: previously known results}\label{app:busgeo}


This appendix states   the properties of Busemann functions, geodesics, and competition interfaces which were discussed informally in Section \ref{sec:bus-brief}.   Theorem \ref{thm:Bus}  introduces the {\it Busemann process} with its main properties. It combines results that follow from 
Theorems 4.4 and 4.7, Lemmas 4.5(c) and 4.6(c), and Remark 4.11 in \cite{Jan-Ras-20-aop} and Lemmas 4.7 and 5.1 in \cite{Geo-Ras-Sep-17-ptrf-2}.

\begin{theorem}\label{thm:Bus}{\rm\cite{Jan-Ras-20-aop,Geo-Ras-Sep-17-ptrf-2}}
%Fix a countable dense subset $\Udense \subset\ri\Uset$. 
Let $\P_0$ be a probability measure on $\R^{\Z^2}$ under which the coordinate projections are i.i.d., have positive variance, and have $p>2$ finite moments.
There exists a Polish probability space $(\Omega,\sF,\bbP)$ with 
%ingredients {\rm(i)}--{\rm(iv)} listed next and for which 
\begin{enumerate}[label={\rm(\arabic*)}, ref={\rm\arabic*}]  \itemsep=3pt 
\item   a group $T=\{T_x\}_{x\in\bbZ^2}$  of $\sF$-measurable $\bbP$-preserving bijections $T_x:\Omega\to\Omega$,  
\item   a family $\{\w_x(\w) : x \in \bbZ^2\}$ of real-valued random variables $\w_x:\Omega\to\R$
such that  $\w_y(T_x \w) = \w_{x+y}(\w)$ for all $x,y \in \bbZ^2$, 
\item real-valued measurable functions $\B{\xi+}(x,y,\w)=\B{\xi+}_{x,y}(\w)$ and $\B{\xi-}(x,y,\w)=\B{\xi-}_{x,y}(\w)$ of $(x,y,\w,\xi)\in\Z^2\times\Z^2\times\Omega\times\ri\Uset$, 
\item  and  $T$-invariant events 
$\Omega_0^1 \subset \Omega$ and  $\Omega_\xi^1\subset\Omega_0^1$ for each  $\xi\in\ri\Uset$, with $\bbP(\Omega_0^1) = \P(\Omega_\xi^1)=1$, 
\end{enumerate} 
 such that properties \eqref{thm:cocyexist:a}--\eqref{thm:cocyexist:g} listed below hold. 

%%%%    EARLIER VERSION %%%%%%%%
%There exists a Polish probability space $(\Omega,\sF,\bbP)$, a group $T=\{T_x\}_{x\in\bbZ^2}$  of $\sF$-measurable $\bbP$-preserving bijections $T_x:\Omega\to\Omega$,  a family $\{\w_x(\w) : x \in \bbZ^2\}$ of real-valued random variables 
%such that  $\w_y(T_x \w) = \w_{x+y}(\w)$ for all $x,y \in \bbZ^2$, 
%%satisfying the hypotheses of the first paragraph of Section \ref{sub:setting}, 
%real-valued measurable functions $\B{\xi+}(x,y,\w)=\B{\xi+}_{x,y}(\w)$ and $\B{\xi-}(x,y,\w)=\B{\xi-}_{x,y}(\w)$ of $(x,y,\w,\xi)\in\Z^2\times\Z^2\times\Omega\times\ri\Uset$, and  $T$-invariant events 
%$\Omega_0^1 \subset \Omega$ and  $\Omega_\xi^1\subset\Omega_0^1$ for each  $\xi\in\ri\Uset$, with $\bbP(\Omega_0^1) = \P(\Omega_\xi^1)=1$  for each  $\xi\in\ri\Uset$, and such that the following hold.
%%for all $\w \in \Omega_0^1$ and all $x,y, z \in \bbZ^2$, the following hold. 
%%%%%%%%     EARLIER VERSION ENDS   %%%%%%%%%%   
\begin{enumerate}[label={\rm(\alph*)}, ref={\rm\alph*}]  \itemsep=3pt 
\item\label{thm:cocyexist:a} $\{\w_x:x\in\Z^2\}$ has distribution $\P_0$ under $\P$.
\item\label{thm:cocyexist:b} For any $I \subset \bbZ^2,$ the variables
\begin{align*}
\bigl\{(\w_x, \B{\xi\sig}(x,y,\w)): x \in I,y\ge x,\sigg\in\{-,+\},\xi\in \ri\Uset\bigr\}	
\end{align*}
are independent of $\{\w_x : x \in I^{<}\}$ where $I^<=\{x\in\Z^2:x\not\ge z\ \forall z\in I\}$.
\item\label{thm:cocyexist:c} For each $\xi\in\ri\Uset$,  $x,y\in\Z^2$, and $\sigg\in\{-,+\}$,
$\B{\xi\sig}(x,y)$ are  integrable and \eqref{E[h(B)]} holds.
\item\label{thm:cocyexist:foo} For each $\w\in\Omega$, $x,y\in\Z^2$, and $\sigg\in\{-,+\}$, 
if $\zeta,\eta\in\ri\Uset$ are such that $\nabla\gpp(\zeta\sigg)=\nabla\gpp(\eta\sigg)$, then $\B{\zeta\sig}(x,y,\w)=\B{\eta\sig}(x,y,\w)$.
\item\label{thm:cocyexist:d} For each $\w\in\Omega_0^1$,  $x,y,z\in\Z^2$, 
$\xi\in \ri\Uset$, and $\sigg\in\{-,+\}$ properties \eqref{cov-prop}, \eqref{coc-prop}, and \eqref{rec-prop2} hold. 
\item\label{thm:cocyexist:e} For each $\w\in\Omega_0^1$, monotonicity \eqref{mono} holds.
\item\label{thm:cocyexist:f} For each $\w\in\Omega_0^1$,  one-sided limits \eqref{Busemann-limits} hold.
\item\label{thm:cocyexist:h} For each $\w \in \Omega_0^1$ and each $x \in \bbZ^2$,
	\be\label{B:inf-lim} 
	\B{\xi\sig}(x,x+e_i)\to\infty \quad\text{as  }\ \xi\to e_{3-i}, \  \text{ for } \ i\in\{1,2\}. 
	\ee 
%\item For each $\w \in \Omega_\xi^1$ and each $x,y \in \bbZ^2$, %%THIS IS NOT CORRECT
%	\begin{align}\label{B:cont}
%	\lim_{\ri\Uset\ni\zeta \to \xi} \B{\zeta\sig}(x,y,\w) = \B{\xi}(x,y,\w).
%	\end{align}
\item\label{thm:ties} If $\P(\w_0\le r)$ is continuous in $r$, then for all $\xi\in\ri\Uset$, $\w\in\Omega_\xi^1$, $x\in\Z^2$, and $\sigg\in\{-,+\}$,
	\begin{align}\label{eq:ties}
	\B{\xi\sig}(x,x+e_1)\ne\B{\xi\sig}(x,x+e_2).
	\end{align}
\item\label{thm:cocyexist:erg} For all $\xi\in\ri\Uset$, $\w\in\Omega_\xi^1$, and $\sigg\in\{-,+\}$,
	\begin{align}\label{eq:erg-coc}
	\lim_{n\to\infty}\max_{x\in \,n\Uset\cap\Z^2_+}n^{-1}\abs{\B{\xi\sig}(0,x)-x\cdot\nabla\gpp(\xi\sigg)}=0.
	\end{align}
%The reasoning is this:  Thm 4.4 in DLR says there is a shape theorem with h(B). But then Lemma 4.5(c) says that if the mean of -h(B) is an extreme point of the superdifferential then h(B) is constant.  And in the case of B^{\xi\pm} Theorem 2.2(c) in shox says the mean of -h(B^{\xi\pm}) is \nabla\gpp(\xi\pm).  Lastly, our Lemma 4.6(c) in DLR says these are extremes in the superdifferential.
\item\label{thm:cocyexist:g} For all $\xi \in \Diff$, $\w\in\Omega_\xi^1$, and $x,y \in \bbZ^2$
	\begin{align}\label{B+=B-:temp}
	\B{\xi+}(x,y,\w)=\B{\xi-}(x,y,\w)=\B{\xi}(x,y,\w).
	\end{align} 
\item\label{thm:cocyexist:Busfn} If $\xi, \ximin, \ximax \in \sD$ then for all $\w \in \Omega_\xi^1$, the Busemann limit \eqref{eq:Busfn} holds.
\end{enumerate}	
\end{theorem}

%We can have \eqref{eq:ties}, \eqref{eq:erg-coc}, and \eqref{B+=B-:temp}, hold simultaneously for many directions $\xi$.  Namely, fix a countable dense set $\Udense\subset\Diff$. 
%Include in $\Diff$ all points that are endpoints of non-degenerate linear segments of $\gpp$, i.e.\ the countable set $\{\ximin,\ximax:\xi\in\ri\Uset,\ximin\ne\ximax\}\cap\Diff$. (This last set of points is needed only for a faster proof of Corollary \ref{cor:empty}.)
%Then for any event  $\Omega_0\subset\bigcap_{\xi\in\Udense}\Omega_\xi^1$ all three hold for all $\w\in\Omega_0$ and $\xi\in\Udense$.\medskip
%	\begin{align}\label{B+=B-}
%	\B{\xi+}(x,y,\w)=\B{\xi-}(x,y,\w)=\B{\xi}(x,y,\w)\qquad\text{for all }\w\in\Omega_0,\ \xi\in\Udense,\text{ and }x,y\in\Z^2.
%	\end{align} 
%\reversemarginpar\addmath{we will need this choice if we want to apply Theorem \ref{thm1}\eqref{thm1:cont} for multiple $\xi$'s at once. CHECK whether or not we do this}
%When the regularity condition \eqref{g-reg} is assumed, we will use the special choice $\Udense=\Ddense$. 


\begin{remark}[Weak limit construction of the Busemann process] 
\label{rmk:weak-lim} 
 Both articles \cite{Jan-Ras-20-aop,Geo-Ras-Sep-17-ptrf-2} on which we rely for Theorem \ref{thm:Bus} construct the process $\B{}$ as a weak limit point of  Ces\`aro averages of probability distributions of pre-limit objects.  This gives existence of the process on a probability space $\Omega$ that is larger than the product space $\R^{\Z^2}$ of the i.i.d.\ weights $\{\w_x\}$.  Article  \cite{Geo-Ras-Sep-17-ptrf-2} takes the outcome of the weak limit from existing literature in the form of a queueing fixed point, while \cite{Jan-Ras-20-aop}  builds the weak limit from scratch by considering the distribution of increments of point-to-line passage times, following the approach introduced in \cite{Dam-Han-14}.  

 To appeal to queueing literature,  \cite{Geo-Ras-Sep-17-ptrf-2}  assumes that   $\P(\w_0\ge c)=1$ for some real $c$.   A payoff is that each process $\{\B{\xi\sig}(x,y):x,y\in\Z^2\}$ is ergodic under either shift  $T_{e_i}$ \cite[Theorem 5.2(i)]{Geo-Ras-Sep-17-ptrf-2}.  The construction in \cite{Jan-Ras-20-aop} does not need the lower bound assumption but  gives only  the  $T$-invariance stated above in Theorem \ref{thm:Bus}\eqref{thm:cocyexist:a}.    
 
Theorem \ref{thm1} below quotes results from  \cite{Geo-Ras-Sep-17-ptrf-2} that were proved with the help of ergodicity. Remark \ref{rmk:erg3} explains how the required properties can be obtained without ergodicity. 
 \end{remark} 


%Note that part of the statement of Theorem \ref{thm:Bus} is the existence of a probability space on which the conclusions hold.  By Theorem 5.3 of \cite{Geo-Ras-Sep-17-ptrf-1}, under condition \eqref{g-reg}, the conclusions hold on every probability space supporting i.i.d.\ weights with marginal $\bbP_0$. In the language of stochastic analysis, the difference between these two statements is the usual distinction between weak and strong existence of solutions to stochastic equations.
%\smallskip


%\reversemarginpar\addmath{T: we should be explicit about the lack of ergodicity and how to mend it and what the implications/shortcomings are. Most readers will be surprised to be confronted by the fact that Bs are not ergodic even though we have iid weights. F: added this paragraph. Please read and edit.}
%The probability measure $\P$ is $T$-invariant, but is not shown to be ergodic under any of these shifts in general. One way to ensure $\P$ is ergodic under some shifts is to assume the existence of a real number $c$ such that $\P(\w_0\ge c)=1$ and apply \cite[Theorem 5.2(i)]{Geo-Ras-Sep-17-ptrf-1}. %  But in any case, 
%That result shows ergodicity of the process $\{\B{\xi\sig}(x,y):x,y\in\Z^2\}$ under $T_{e_i}$-shifts,  for fixed $\xi\in\ri\Uset$, $\sigg\in\{-,+\}$, and $i\in\{1,2\}$. %It is expected that this result should in fact still hold without the lower bound assumption on the weights. 
%This result does not guarantee joint ergodicity of the process or ergodicity under more general shifts.%, even for $(\B{\xi-},\B{\xi+})$, let alone for two different directions or under $T_x$ for an arbitrary $x\in\N^2$.  I

\begin{remark}[Strong existence and ergodicity of the Busemann process] 
\label{rk:ergodicity}
The regularity condition \eqref{g-reg} is equivalent to the  existence of a countable dense set $\Ddense\subset\Diff$ such that   $\zetamin,\zetamax\in\Diff$  for each $\zeta\in\Ddense$.
When \eqref{g-reg}  holds, \cite[Theorem 3.1]{Geo-Ras-Sep-17-ptrf-1} shows that for $\zeta$ in $\Ddense$, 
$\B{\zeta}(x,y)=\B{\zeta\pm}(x,y)$ 
can be realized as an almost sure limit of $G_{x,v_n}-G_{y,v_n}$ when  $v_n/n\to\xi$. The remaining values  $\B{\xi\sig}(x,y)$ 
%$\{\B{\xi\pm}(x,y):x,y\in\Z^2,\xi\in\ri\Uset\}$ 
can be obtained as  left and right limits from  $\{\B{\zeta}(x,y)\}_{\zeta\in\Ddense}$ as $\zeta\to\xi$. This way the  entire process $\{\B{\xi\sig}(x,y):x,y\in\Z^2,\xi\in\ri\Uset, \sigg\in\{-,+\}\}$ becomes    a measurable function of the i.i.d.\ weights $\{\w_x:x\in\Z^2\}$.  We can take $\Omega=\R^{\Z^2}$ and the Busemann process is  ergodic under any shift $T_x$ for $x\ne 0$. 
% and since these are i.i.d.\ under $\P_0$,  we have joint ergodicity of the full process under the shifts $T_x$, $x\in\Z^2\setminus\{0\}$.
\end{remark}

We record a simple observation here, 
 valid  under the continuous i.i.d.\ weights assumption \eqref{main-assump}:   there exists an event $\Omega_0^2$ with $\P(\Omega_0^2)=1$ such that $\forall \w\in\Omega_0^2$, 
\begin{align} 
\begin{split}
&\text{for every nonempty  finite subset $I\subset\Z^2$ and nonzero  integer coefficients $\{a_x\}_{x\in I}$, }\\ 
&\textstyle{\sum_{x\in I} a_x\w_x\ne 0.}
\end{split}\label{paths.2}  
\end{align} 
This condition implies the uniqueness of point-to-point geodesics mentioned under \eqref{G1}. 

 
The following theorem summarizes previous knowledge of  the structure of semi-infinite geodesics under assumption \eqref{main-assump}.  These results were partly summarized in Section \ref{sec:geod-brief}. 

\begin{theorem}{\rm\cite[Theorems 2.1, 4.3, 4.5, and 4.6]{Geo-Ras-Sep-17-ptrf-2}}\label{thm1}
%Assume \eqref{main-assump}. 
There exist $T$-invariant events $\Omega_0^3$ and $\Omega_\xi^3\subset\Omega_0^3$ for each $\xi\in\ri\Uset$, with $\P(\Omega_0^3)=1$, $\P(\Omega_\xi^3)=1$, and such that the following hold.
\begin{enumerate}[label={\rm(\alph*)}, ref={\rm\alph*}]  \itemsep=3pt 
	\item\label{thm1:exist}   For every $\w\in\Omega_0^3$,  for every $x\in\Z^2$, $\sigg\in\{-,+\}$, and  $\xi\in\ri\Uset$,
	$\geo{}{x}{\xi\sig}$ is $\Uset_{\xi\sig}$-directed and every 
	semi-infinite geodesic is $\Uset_\xi$-directed for some $\xi\in\Uset$.
	\item\label{thm1:coal} For every $\xi\in\ri\Uset$, for every $\w\in\Omega_\xi^3$, $x,y\in\Z^2$, and $\sigg\in\{-,+\}$, $\geo{}{x}{\xi\sig}$ and $\geo{}{y}{\xi\sig}$ coalesce,  i.e.\ there exists an integer $k\ge x\cdot\et\vee y\cdot\et$ such that $\geo{k,\infty}{x}{\xi\sig}=\geo{k,\infty}{y}{\xi\sig}$. 
	%This says that the graph $\G{\xi\sig}$ is one connected tree.
	\item\label{thm1:biinf}  For every $\xi\in\ri\Uset$, $\w\in\Omega_\xi^3$,  $x\in\Z^2$, and $\sigg\in\{-,+\}$, there exist at most finitely many $z\in\Z^2$ such that $\geo{}{z}{\xi\sig}$ goes through $x$. 
	%In other words, the tree $\G{\xi\sig}$ does not contain a bi-infinite up-right path.
	\item\label{thm1:direct}	If $\gpp$ is strictly concave,   then for any $\w\in\Omega_0^3$
		 every semi-infinite geodesic is $\xi$-directed for some $\xi\in\Uset$.
	\item\label{thm1:cont}%Suppose  $\P\{\w_0\le r\}$ is a continuous function of $r\in\R$.
% and $\gpp$ is %strictly concave and 		differentiable on $\ri\Uset$.   
If $\xi\in\ri\Uset$ is such that  $\Uset_\xi=[\,\ximin,\ximax\,]$ satisfies $\ximin, \xi,\ximax\in\Diff$, then for any $\w\in\Omega_\xi^3$ and $x\in\Z^2$ we have $\geo{}{x}{\xi+}=\geo{}{x}{\xi-}$. This is the unique $\Uset_\xi$-directed  semi-infinite  geodesic out of $x$  and, by part \eqref{thm1:coal}, all these geodesics coalesce. By part \eqref{thm1:biinf}, there are no bi-infinite $\Uset_\xi$-directed geodesics.
		  %For each $u\in\Z^2$ there are at most finitely many sites $v\in\Z^2$ such that the unique $\Uset_\xi$-directed  semi-infinite geodesic out of $v$ goes through $u$.
\end{enumerate}
\end{theorem}

\begin{remark}[Ergodicity in the proof of Theorem \ref{thm1}] \label{rmk:erg3} 
As mentioned in Remark \ref{rmk:weak-lim}, 
  \cite{Geo-Ras-Sep-17-ptrf-2}   uses ergodicity of cocycles.  But  the results quoted above in Theorem \ref{thm1} can be obtained  with stationarity, which comes   from  \cite{Jan-Ras-20-aop} without the restrictive assumption $\w_x\ge c$. 
  
 The proof of  directedness (Theorem \ref{thm1}\eqref{thm1:exist} above) given  in \cite[Theorem 4.3]{Geo-Ras-Sep-17-ptrf-2}
uses the shape theorem of ergodic cocycles stated in \cite[Theorem A.1]{Geo-Ras-Sep-17-ptrf-2}. This shape theorem  holds also in  the stationary setting, as stated above in \eqref{eq:erg-coc}.  This result comes from  \cite[Theorem 4.4]{Jan-Ras-20-aop} and it is proved in detail in  Appendix B of \cite{Jan-Ras-18-arxiv}.   Now the  proof of \cite[Theorem 4.3]{Geo-Ras-Sep-17-ptrf-2} goes through line-by-line after switching its references and applying \cite[Lemma 4.5(c)]{Jan-Ras-20-aop} to identify the correct centering for the cocycle. %The coalescence result is already proved in \cite{Geo-Ras-Sep-15} in the stationary case.

 Similarly, the non-existence of directed bi-infinite geodesics (Theorem \ref{thm1}\eqref{thm1:biinf} above) proved  in  \cite[Theorem 4.6]{Geo-Ras-Sep-17-ptrf-2} needs only stationarity after minor changes. Essentially the same argument is given in \cite[Lemma 6.1]{Jan-Ras-20-aop} in positive temperature, assuming only stationarity. %\textcolor{red}{explain more about non-existence of bi-infinites? that all one needs is a positive probability of having a positive density of triple points...}
 \end{remark} 
 
%The full measure events in parts \eqref{thm1:coal}, \eqref{thm1:biinf}, and \eqref{thm1:cont} depend on $\xi$. %and \eqref{thm1:cont} depends on $\xi$.
%An application of Fubini-Tonelli then shows that the claims in \eqref{thm1:coal} and \eqref{thm1:biinf} also hold on a full 
%$\P$-measure event and simultaneously 
%for all directions $\xi\in\ri\Uset$, except for a zero Lebesgue measure set of exceptional directions.
%\normalmarginpar\fixtext{edited the text a bit. read till the end of the section. text can probably be still be improved.} 
%It is conjectured that in fact, quite generally, there are no such exceptional directions in the case of part \eqref{thm1:biinf}. We state this as a condition that we assume in two of our results: parts \eqref{thm:shocks.d} and \eqref{thm:shocks.f} of Theorem \ref{thm:shocks} below.
We next record an easy consequence of the previous results, ruling out the existence of non-trivial semi-infinite geodesics which are either $e_1$- or $e_2$-directed.  %CHANGED HERE
\begin{lemma}\label{lem:notriv}
For $\w \in \Omega_0^1 \cap \Omega_0^2 \cap \Omega_0^3$, if $\gamma^x$ is a semi-infinite geodesic emanating from $x$ with $\gamma^x_n/n \to e_i$ for some $i \in \{1,2\}$, then $\gamma^x = \geo{}{x}{e_i}$.
\end{lemma}
\begin{proof}
We consider the case of $i=1$, with the case of $i=2$ being similar. Call $x \cdot \ehat = k$ and fix a sequence $\zeta_n \in \ri \Uset$ with $\zeta_n \to e_1$ as $n\to\infty$. By Theorem \ref{thm1}\eqref{thm1:exist}, $\geo{}{x}{\zeta_n}$ is $\Uset_{\zeta_n}$-directed. \cite[Theorem 2.4]{Mar-04} implies that $e_1 \notin \Uset_{\zeta_n}$. Then, by \eqref{paths.2}, if $\gamma^x$ is as in the statement, we must have $\geo{\ell}{x}{\zeta_n} \preceq \gamma_\ell^x \preceq x + (k-\ell) e_1 = \geo{\ell}{x}{e_1}$ for all $n \in \bbN$ and $\ell \geq k$. But Theorem \ref{thm:Bus}\eqref{thm:cocyexist:h} implies that for each fixed $\ell \geq k$,  $\geo{\ell}{x}{\zeta_n} = x + (k-\ell) e_1 = \geo{\ell}{x}{e_1}$ holds for all large enough $n$. The result follows.
\end{proof}



Under the assumption that $\gpp$ is differentiable on $\ri\Uset$,  Theorem \ref{thm1}\eqref{thm1:cont} holds for all $\xi\in\ri\Uset$. An application of the Fubini-Tonelli theorem gives that the claims in Theorem \ref{thm1}\eqref{thm1:coal} and Theorem \ref{thm1}\eqref{thm1:biinf} in fact hold on a single full $\P$-measure event simultaneously for Lebesgue-almost all directions $\xi\in\ri\Uset$.
It is conjectured that the claim in part \eqref{thm1:biinf} holds in fact on a single full-measure event, simultaneously, for all $\xi\in\ri\Uset$.\smallskip
% We state this as a condition that we will assume in two of our results: parts \eqref{thm:shocks.d} and \eqref{thm:shocks.f} of Theorem \ref{thm:shocks} below.
%%\begin{condition}\label{cond:biinf}
%\begin{align}\label{cond:biinf}
%\begin{minipage}{0.9\textwidth}
%There exists a $T$-invariant event $\Ombiinf$ with $\P(\Ombiinf)=1$ and such that for any $\w\in\Ombiinf$, the only bi-infinite geodesics are the trivial ones: $x+\Z e_i$ for $x\in\Z^2$ and $i\in\{1,2\}$.
%\end{minipage}
%\end{align}
%%\end{condition}
%Recently, \cite[Theorem 1]{Bas-Hof-Sly-18-} showed that condition \eqref{cond:biinf} holds if the weights $\{\w_x:x\in\Z^2\}$ are exponentially distributed i.i.d.\ random variables under $\P$. 



%%%%%%%   First attempt at streamlining 2019-08-06 -- not clear what is right path. 
%In the next theorem we state the directedness and coalescence of geodesics $\geo{}{x}{\xi\sig}$. Further properties appear in Appendix \ref{app:busgeo}. 
%
%\begin{theorem}{\rm\cite[Theorems 2.1, 4.3, 4.5, and 4.6]{Geo-Ras-Sep-17-ptrf-2}}\label{thm1}
%%Assume \eqref{main-assump}. 
%There exist $T$-invariant events $\Omega_0^3$ and $\Omega_\xi^3\subset\Omega_0^3$ for each $\xi\in\ri\Uset$, with $\P(\Omega_0^3)=1$, $\P(\Omega_\xi^3)=1$, and such that the following hold.
%\begin{enumerate}[label={\rm(\alph*)}, ref={\rm\alph*}]  \itemsep=3pt 
%	\item\label{thm1:exist}   For every $\w\in\Omega_0^3$,  for every $x\in\Z^2$, $\sigg\in\{-,+\}$, and  $\xi\in\ri\Uset$,
%	$\geo{}{x}{\xi\sig}$ is $\Uset_{\xi\sig}$-directed and every 
%	semi-infinite geodesic is $\Uset_\xi$-directed for some $\xi\in\Uset$.
%	\item\label{thm1:coal} For every $\xi\in\ri\Uset$, for every $\w\in\Omega_\xi^3$, $x,y\in\Z^2$, and $\sigg\in\{-,+\}$, $\geo{}{x}{\xi\sig}$ and $\geo{}{y}{\xi\sig}$ coalesce,  i.e.\ there exists an integer $k\ge x\cdot\et\vee y\cdot\et$ such that $\geo{k,\infty}{x}{\xi\sig}=\geo{k,\infty}{y}{\xi\sig}$. 
%	%This says that the graph $\G{\xi\sig}$ is one connected tree.
%\end{enumerate}
%\end{theorem}
%

 The next result is a small extension of Lemma 4.4 of \cite{Geo-Ras-Sep-17-ptrf-2}, achieved by an application of the monotonicity in \eqref{path-ordering}. %We provide the proof in the appendix.
%\normalmarginpar\addmath{maybe no need to provide a proof?}

%\addmath{NO ERGODICITY NEEDED}
\begin{theorem}\label{thm:extreme}
Assume the regularity condition \eqref{g-reg}. For any $\w\in\Omega_0^1\cap\Omega_0^2$, \eqref{eq:geoorder} holds.
\end{theorem}



The next theorem says that there are multiple geodesics that are directed in the same asymptotic direction $\cid$ as the competition interface, which itself can be characterized using the Busemann process. See Figure \ref{fig:cif2}.

\begin{theorem}{\rm\cite[Equation (5.2) and Theorems 2.6, 2.8, and 5.3]{Geo-Ras-Sep-17-ptrf-2}}\label{thm:cif}
%Assume \eqref{main-assump} and 
There exists a $T$-invariant event $\Omega_0^4$ such that $\P(\Omega_0^4)=1$ and the following hold for all $\w\in\Omega_0^4$.
\begin{enumerate}[label={\rm(\alph*)}, ref={\rm\alph*}]  \itemsep=3pt 
\item\label{thm:cif.a} There exists a unique point $\cid(\w)\in\ri\Uset$ such that \eqref{cid} holds.
\item\label{thm:cif.b} For any $\xi\in\ri\Uset$,   $\P(\cid=\xi)>0$ if and only if $\xi\in(\ri\Uset)\smallsetminus\Diff$.    
%\item\label{thm:cif.c} For any $\eta\prec\zeta$ in $\Uset$,  $\P([\eta,\zeta]\cap\,\aUset\neq\varnothing)\in\{0,1\}$. If $[\eta,\zeta]\cap(\ri\Uset)\subset\Diff$ and $\P\{[\eta,\zeta]\cap\,\aUset\neq\varnothing\}=1$,
%then the set of $\xi \in [\eta,\zeta]$ satisfying $\P\bigl\{\xi \text{ is an accumulation point of } \aUset\}=1$ is infinite and has no isolated points.
\item\label{thm:cif.c} For any $\zeta\prec\eta$ in $\ri\Uset$ with $\nabla\gpp(\zeta+)\ne\nabla\gpp(\eta-)$, for any $x\in\Z^2$, there exists $y\ge x$ such that $\cid(T_y\w)\in\,]\zeta,\eta[$. Consequently, any open interval outside  the closed  linear segments of   $\gpp$  contains $\cid$ with positive probability.  
\item\label{thm:cif.c1} For any $\xi\in(\ri\Uset)\smallsetminus\Diff$ and for any $x\in\Z^2$, there exists $y\ge x$ such that $\cid(T_y\w)=\xi$.
%\item\label{thm:cif.d} For any $x\in\Z^2$, $\geo{}{x}{\cid(T_x\w)+}$ takes a first step $e_1$, $\geo{}{x}{\cid(T_x\w)-}$ takes a first step $e_2$, and the two geodesics only intersect at $x$.
\end{enumerate}
	
If the regularity condition \eqref{g-reg} holds then the following also hold. 
	
\begin{enumerate}[label={\rm(\alph*)}, ref={\rm\alph*},resume]  \itemsep=3pt 
\item\label{cif-lln} We have the limit
\begin{align}\label{thm:cif:(i)}
\cid(\w)= \lim_{n\to\infty} n^{-1}\varphi_n^0(\w).  
\end{align}
%The   limit $\cid$ is almost surely an exposed point in $\ri\Uset$  {\rm(}recall definition \eqref{eq:epod}{\rm)}.  
\item\label{thm:cif:(ii)} $\cid(T_x\w)$ is the unique direction $\xi$ such that there are at least two $\Uset_\xi$-directed semi-infinite geodesics from $x$, namely $\geo{}{x}{\xi\pm}$, that separate at $x$ and never intersect thereafter.
%\item\label{thm:cif:(iii)}     $\Uset_*^x$ contains all $\xi\in(\ri\Uset)\smallsetminus\Diff$,  intersects every open interval outside the closed linear segments of $\gpp$, and is a countably infinite subset of $\{\cid(T_z\w):z\ge x\}$. 
\end{enumerate}
\end{theorem}

  Remark \ref{rmk:erg3} applies here as well. Ergodicity is invoked in the proofs of parts \eqref{thm:cif.b}, \eqref{thm:cif.c}  and \eqref{thm:cif.c1}  in \cite[Theorem 5.3(iii)--(iv)]{Geo-Ras-Sep-17-ptrf-2}   to apply the cocycle shape theorem.   In  our stationary setting this can be replaced with the combination of Theorem 4.4 and  Lemma 4.5(c) of \cite{Jan-Ras-20-aop}.

  

The following result for exponential weights, due to Coupier, states that there are no directions $\xi$ with three $\xi$-directed geodesics emanating from the same site.

\begin{theorem}\label{thm-Coupier}{\rm\cite[Theorem 1(2)]{Cou-11}}
Assume that under $\P$, the weights $\{\w_x:x\in\Z^2\}$ are exponentially distributed i.i.d.\ random variables. Then there exists a $T$-invariant event $\OmCou$ with $\P(\OmCou)=1$ and such that for any $\w\in\OmCou$, any $\xi\in\ri\Uset$, and any $x\in\Z^2$, there exist at most two $\xi$-directed semi-infinite geodesics out of $x$.
\end{theorem}


%Denote the event in the definition of condition \eqref{cond:biinf} by $\Ombiinf$.  
Fix a countable dense set $\Udense \subset \Diff$. 
The following event of full $\P$-probability is the basic setting for the proofs in Sections \ref{sec:bus}--\ref{sec:webpf}:  
	\begin{eqnarray}\label{Om0}
	&\Omega_0= \Omega_0^1 \cap \Omega_0^2\cap\Omega_0^4\cap\Bigl(\bigcap_{\xi\in\Udense}[\Omega_\xi^1\cap\Omega_\xi^3]\Bigr)\cap\Bigl(\bigcap_{\xi\in(\ri\Uset)\setminus\Diff}\Omega_\xi^3\Bigr).  %CHANGED HERE
	\end{eqnarray} 
When additional assumptions are needed, $\Omega_0$ will be further restricted.
%When the jump process condition \eqref{cond:jumpcond} holds we restrict to the smaller full $\P$-probability event $\Omjump$. 
%or on the smaller full $\P$-measure events $\Omjump$ (defined in \eqref{Omjump}), when the jump process condition \eqref{cond:jumpcond} holds, or $\Omjump\cap\OmCou$, when the weights are exponentially distributed, or 
%$\Omjump\cap\Ombiinf$, when both condition \eqref{cond:jumpcond} and the no bi-infinite geodesics condition \eqref{cond:biinf} hold. 
%\textcolor{red}{(any other combinations??)}
%The caveats are as follows. 
%\fixtext{F: added the ``or a condition that implies it''. Return to this whole paragraph later, once we figured out how we want to present the full-measure events.''}
%\note{C: How about if we have $\Omega_0$ be conditionally defined depending on whether certain events have full probability?}
%When the jump condition \eqref{cond:jumpcond}, or a condition that implies it, is assumed, it may be necessary to intersect this with another full measure set on which the condition holds. 
%For example, by \cite[Theorem 3.4]{Fan-Sep-20} \eqref{cond:jumpcond}, condition \eqref{cond:jumpcond} holds when the weights are exponentially distributed. Additionally, when the weights are exponentially distributed, we also intersect with $\OmCou$.



==> JEMS Post-Accept Revision/GeoWebPaper-AppB-D.tex <==
% !TEX root = GeoWebPaper.tex

\section{Auxiliary lemmas}
\label{a:aux} 


%We first record a simple observations 
% valid  under the continuous i.i.d.\ weights assumption \eqref{main-assump}.  Namely,  there exists an event $\Omega_0^2$ with $\P(\Omega_0^2)=1$ such that $\forall \w\in\Omega_0^2$: 
%\begin{align} 
%\begin{split}
%&\text{For all points $x\le y$ in $\Z^2$, there exists a unique path (the geodesic)  that }\\
%&\text{maximizes on the right-hand side of \eqref{G1}.}
%\end{split}\label{paths.1}\\[2pt]
%\begin{split}
%&\text{For every nonempty  finite subset $I\subset\Z^2$ and nonzero  integer coefficients $\{a_x\}_{x\in I}$, }\\ 
%&\textstyle{\sum_{x\in I} a_x\w_x\ne 0.}
%\end{split}\label{paths.2}  
%\end{align} 
%\begin{enumerate}[label={\rm(\roman*)}, ref={\rm\roman*}]  \itemsep=3pt 
%\item\label{paths.1} For all points $x\le y$ in $\Z^2$, there exists a unique geodesic path that maximizes on the right-hand side of \eqref{G1}.
%\item\label{paths.2} %For any points $x,y,z,z'\in\Z^2$ with, $x\le z$, $x\le z'$, $y\le z$,  $y\le z'$, and either $x\ne y$ or $z\ne z'$, we have  $G_{x,z}-G_{y,z}\ne G_{x,z'}-G_{y,z'}$.
%For any nonempty  finite $I\subset\Z^2$ and nonzero  integer coefficients $\{a_x\}_{x\in I}$,  
%$\sum_{x\in I} a_x\w_x\ne 0$.  
%\end{enumerate}\smallskip

%%%%%%%%   BELOW OLD LEMMA THAT USED REGULARITY TO GET \cid POINTS 
%
%As explained in Remark \ref{rk:ergodicity}, if the regularity condition \eqref{g-reg} is assumed, then the entire Busemann process $\bigl\{\B{\xi\sig}(x,y):x,y\in\Z^2,\sig\in\{-,+\},\xi\in\ri\Uset\bigr\}$ is measurable with respect to the $\sigma$-algebra generated by the i.i.d.\ weights $\{\w_x:x\in\Z^2\}$. 
%The following lemma is then a consequence of \eqref{E[h(B)]}, Theorem \ref{thm:cif}\eqref{thm:cif.b},
%the ergodicity of $\P$, and the fact that $(\ri\Uset)\setminus\Diff$ is countable.
%%1. \xi\notin\Diff implies \nabla\gpp(\xi\pm)\cdot(e_2-e_1) differ: if they are equal then 
%%(\nabla\gpp(\xi+)-\nabla\gpp(\xi-))\cdot e_1=(\nabla\gpp(\xi+)-\nabla\gpp(\xi-))\cdot e_2
%%the lhs is \le0 for all \xi and the rhs is \ge0 for all \xi.  so equality implies they are both 0. 
%%2. if Z_x is an ergdoic process with E[Z_0]\ne0, then the ergodic theorem implies that there are infinitely many x such that Z_x\ne0.
%
%\begin{lemma}%\label{lm:B+>B-}
%Assume that the regularity condition \eqref{g-reg} holds.
%Then there exists a $T$-invariant event $\Omreg\subset\Omega_0$ with $\P(\Omreg)=1$ and such that for any $\w\in\Omreg$ and any $\xi\in(\ri\Uset)\setminus\Diff$, there exist infinitely many $x\in\Z^2$ such that $\B{\xi+}(x+e_1,x+e_2)>\B{\xi-}(x+e_1,x+e_2)$ and there also exist infinite many $x\in\Z^2$ such that $\cid(T_x\w)=\xi$. 
%\end{lemma}

The next lemma follows from the shape theorem for cocycles \eqref{eq:erg-coc}. 

\begin{lemma}\label{lem:buselln}
Suppose $\gpp$ is differentiable on $\ri\Uset$. For any $\w \in \Omega_0$, $\xi\in\ri\Uset$, and  any $v\in\bbR^2$, $n^{-1}\B{\xi\pm}(0,\lfloor{nv}\rfloor)$ 
both converge to $v\cdot\nabla\gpp(\xi)$ as $n\to\infty$.
\end{lemma}


\begin{proof}
The claim is obvious for $v=0$. 
Suppose $v\in\bbR_+^2\setminus\{0\}$, the other cases being similar. 
%Take $\Omega_0'$ to be the intersection of $\Omega_0$, defined in \eqref{Om0}, and the $T$-invariant full measure event on which the \textcolor{red}{cocycle ergodic theorem for $\B{\zeta}$} holds for all $\zeta\in\Udense$. 
Take $\w\in\Omega_0$ and $\zeta,\eta\in\Udense$ with $\zeta\cdot e_1<\xi\cdot e_1<\eta\cdot e_1$.
Let $x_n=\lfloor{nv}\rfloor=m_ne_1+\ell_ne_2$. Then
		\begin{align*}
		\B{\xi+}(0,x_n)&=\B{\xi+}(0,m_ne_1)+\B{\xi+}(m_ne_1,x_n)\\
		&\le \B{\eta}(0,m_ne_1)+\B{\zeta}(m_n e_1,x_n)\\
		&\le \B{\eta}(0,m_ne_1)+\B{\zeta}(0,x_n)-\B{\zeta}(0,m_ne_1).
		\end{align*}
Divide by $n$, take it to $\infty$, and apply the \eqref{eq:erg-coc} to $\B{\zeta}$ and $\B{\eta}$ to get 
	\[\varlimsup_{n\to\infty} n^{-1}\B{\xi+}(0,x_n)\le (v\cdot e_1)e_1\cdot\nabla\gpp(\eta)+v\cdot\nabla\gpp(\zeta)-(v\cdot e_1)e_1\cdot\nabla g(\zeta).\]
	Take $\zeta$ and $\eta$ to $\xi$ to get
	\[\varlimsup_{n\to\infty} n^{-1}\B{\xi+}(0,x_n)\le v\cdot\nabla\gpp(\xi).\]
The lower bound on the liminf holds similarly and so we have proved the claim for $\B{\xi+}$. 
The same argument works for $\B{\xi-}$.
\end{proof}

The lemma below is proved by calculus. 

\begin{lemma}\label{a:lm:t500}    
%Let $n\ge2$.  Then for all $a,b\in(0,\infty)$, 
%\be\label{a:t498} 
%\frac{a^{n-1}b^n}{(a+b)^{2n-1}}   \le \frac{(1-\frac1n)^{n-1}}{(1-\frac1{2n})^{2n-1}} \cdot \biggl(\frac12\biggr)^{2n-1}  . 
%\ee
 Fix $c>0$.  Then for all $n\ge 1$ and all  $a,b$ such that $c\le a\le b\le a+\frac{c}n$, 
\be\label{a:t500} 
\frac{a^{n-1}b^n}{(a+b)^{2n-1}}   \ge \biggl(\frac12\biggr)^{2n-1} .  
\ee 
\end{lemma} 

\medskip 

\section{M/M/1 queues and  Busemann functions} \label{a:bus}

This appendix summarizes  results from \cite{Fan-Sep-20} that are needed for the proofs of the results of 
Section \ref{sec:exp}.   
Fix parameters  $0<\alpha<\beta$.   We formulate  a stationary M/M/1 queue in a particular way.   The inputs are two independent i.i.d.\ sequences:  an {\it inter-arrival process}  $I=(I_i)_{i\in\Z}$  with marginal distribution  $I_i\sim$ Exp$(\alpha)$ and   a {\it service process}  $Y=(Y_i)_{i\in\Z}$  with marginal distribution  $Y_i\sim$ Exp$(\beta)$.  Out of these inputs are produced two outputs: an {\it inter-departure process}   $\wt I=(\wt I_k)_{k\in\Z}$ and a {\it sojourn process}   $J=(J_k)_{k\in\Z}$,  through the following formulas.   Let $G=(G_k)_{k\in\Z}$ be any function on $\Z$ that satisfies $I_k=G_k-G_{k+1}$.   Define the function    $\wt G=(\wt G_k)_{k\in\Z}$ by 
\be\label{m:800}\begin{aligned} 
\wt G_k
=\sup_{m:\,m\ge k}  \Bigl\{  G_m+\sum_{i=k}^m Y_i\Bigr\}  
%=   G_k+ \sup_{m:\,m\ge k}  \Bigl\{  -(G_k-G_m) +\sum_{i=k}^m Y_i\Bigr\} \\
%&=   G_k+ \sup_{m:\,m\ge k}  \Bigl\{  -\sum_{i=k}^{m-1} I_i +Y_k +\sum_{i=k}^{m-1}  Y_{i+1} \Bigr\} \\
%&
=   G_k+Y_k + \sup_{m:\,m\ge k}  \sum_{i=k}^{m-1} (Y_{i+1}-I_i)  . 
\end{aligned} \ee
The convention for the empty sum is $\sum_{i=k}^{k-1} =0$. 
 Under the assumption on $I$ and $Y$,  the supremum in \eqref{m:800} is almost  surely  assumed at some finite $m$.     Then define the outputs by 
 \be\label{m:801}  \wt I_k =  \wt G_k - \wt G_{k+1}  \ee 
and  
  \be\label{m:J} J_k=\wt G_k -  G_k = Y_k + \sup_{m:\,m\ge k}  \sum_{i=k}^{m-1} (Y_{i+1}-I_i). % , \quad k\in\Z.   
    \ee
The outputs satisfy  the useful  iterative equations
  \be\label{m:IJ5}  
 \wt I_k=Y_k+(I_k-J_{k+1})^+
 \quad\text{and}\quad 
 J_k=Y_k+(J_{k+1}-I_k)^+ .  
  \ee
In particular, this implies  the inequality $\wt I_k\ge Y_k$. %and $J_k\ge Y_k$ 
    
 It is a basic fact about M/M/1 queues  that    $\wt I$ and $J$ are i.i.d.\ sequences with marginals $\wt I_k\sim$ Exp$(\alpha)$ and $J_k\sim$ Exp$(\beta-\alpha)$.  Furthermore, the three variables  $(Y_k, I_k, J_{k+1})$ on the right-hand sides of equations \eqref{m:IJ5}  are independent.   (See for example Appendix A in \cite{Fan-Sep-20}.)   But  $\wt I$ and $J$ are not independent of each other.  
    
The queueing interpretation goes as follows.  A  service station  processes a bi-infinite sequence of customers.   Queueing time runs backwards on the lattice $\Z$.   $I_i$ is the time between the arrivals of customers $i+1$ and $i$  ($i+1$ arrived before $i$)  and    $Y_i$ is the service time required by customer $i$.   $\wt I_k$ is the time between the departures of customers $k+1$ and $k$, with $k+1$ departing before $k$.  $J_k$ is the sojourn time of customer $k$, that is, the total time customer $k$ spent in the system from arrival to departure.  $J_k$ is the sum of the service time $Y_k$ and the waiting time of customer $k$, represented by the last member of \eqref{m:J}.  Because of our unusual convention with the backward indexing, even if $G_k$ is the moment of arrival of customer $k$, $\wt G_k$ is not the moment of departure.   The definition of $\wt G$  in \eqref{m:800} is natural in the present setting because it immediately ties in with LPP.    The convention in \cite{Fan-Sep-20} is different because in \cite{Fan-Sep-20} geodesics go south and west instead of north and east.
 
 The   joint distribution of successive  nearest-neighbor increments  of two Busemann functions on a horizontal or vertical line can now be described as follows. This is a special case of Theorem 3.2 in \cite{Fan-Sep-20}.  
 
 \begin{theorem}\label{th:B-q1}  Let   $\zeta\prec\eta$ in $\ri\Uset$ with parameters $\alpha=\alpha(\zeta)<\alpha(\eta)=\beta$ given by \eqref{u-a}.    Let $I=(I_i)_{i\in\Z}$    and    $Y=(Y_i)_{i\in\Z}$   be two independent i.i.d.\ sequences and define $\wt I=(\wt I_k)_{k\in\Z}$ as above through \eqref{m:800}--\eqref{m:801}.  

 
 \begin{enumerate}  [label={\rm(\alph*)}, ref={\rm(\alph*)}]   \itemsep=3pt  
\item\label{B1-1} Let $I_i\sim$ {\rm Exp}$(\alpha)$ and $Y_i\sim$ {\rm Exp}$(\beta)$.  Then the sequence %pair of sequences 
$(\B{\zeta}_{ke_1, (k+1)e_1}, \, \B{\eta}_{ke_1, (k+1)e_1})_{k\in\Z}$  has the same joint distribution as the pair $(\wt I, Y)$. 

  \item\label{B1-2}    Let    $I_i\sim$ {\rm Exp}$(1-\beta)$ and    $Y_i\sim$ {\rm Exp}$(1-\alpha)$.  Then the sequence  %pair of sequences 
  $(\B{\zeta}_{ke_2, (k+1)e_2}, \, \B{\eta}_{ke_2, (k+1)e_2})_{k\in\Z}$  has the same joint distribution as the pair $(Y, \wt I)$.      
  
  \end{enumerate} 

  \end{theorem}
 
Next we  derive a random walk representation for the sequence $\{\B{\zeta}_{ke_1, (k+1)e_1}- \B{\eta}_{ke_1, (k+1)e_1}\}_{k\in\Z}$ of (nonnegative) differences.   By Theorem \ref{th:B-q1} this sequence is equal in distribution to $\{\wt I_k-Y_k\}_{k\in\Z}$.   Define a two-sided randon walk $S$  with positive drift $E[I_{i-1}-Y_i]=\alpha^{-1}-\beta^{-1}$ by 
\be\label{BS}
S_n=\begin{cases}  -\sum_{i=n+1}^0 (I_{i-1}-Y_i), &n<0 \\[3pt]  0, &n=0\\[3pt] \sum_{i=1}^n (I_{i-1}-Y_i), &n>0.   \end{cases}
\ee
Then from \eqref{m:IJ5} and \eqref{m:J}, 
\begin{align*}
\wt I_k-Y_k = (I_k-J_{k+1})^+ = \biggl\{\,\inf_{n:\,n> k} \sum_{i=k+1}^{n} (I_{i-1}-Y_{i})\biggr\}^+ =  \bigl\{   \inf_{n:\,n> k}  (S_n-S_{k}) \bigr\}^+. 
\end{align*}
  From above we can record that  for $r>0$, 
\be\label{B4}
\P(  \B{\zeta}_{0, e_1}> \B{\eta}_{0, e_1}) =P(I_k>J_{k+1}) =  \frac{\beta-\alpha}{\beta}. 
\ee

 
  \begin{corollary}\label{cor:B-q2}  Let   $\zeta\prec\eta$ in $\ri\Uset$ with parameters $\alpha=\alpha(\zeta)<\alpha(\eta)=\beta$ given by \eqref{u-a}.    Let $S$ be the random walk in \eqref{BS} with step distribution {\rm Exp}$(\alpha)-{\rm Exp}(\beta)$.  Then the sequence $\{\B{\zeta}_{ke_1, (k+1)e_1}- \B{\eta}_{ke_1, (k+1)e_1}\}_{k\in\Z}$ has the same distribution as the sequence $ \bigl\{ \bigl( \,\ddd\inf_{n:\,n> k}   S_n-S_{k}\bigr)^+ \bigr\}_{k\in\Z}$.    \end{corollary} 
 
 \section{Random walk}\label{a:RW}
 
 Let $0<\alpha<\beta$ and let $\{X_i\}_{i\in\Z}$ be a doubly infinite sequence of i.i.d.\ random variables with marginal distribution $X_i \sim\text{Exp}(\alpha)-\text{Exp}(\beta)$ (difference of two independent exponential random variables).   Let $\theta$ denote the shift on the underlying canonical sequence space so that   $X_j=X_k\circ\theta^{j-k}$. 
  Let $\{S_n\}_{n\in\Z}$ be the  two-sided random walk   such that $S_0=0$ and $S_n-S_m=\sum_{i=m+1}^n X_i$ for all $m<n$ in $\Z$.  
%  defined by 
%\[  S_n=\begin{cases}  -\sum_{i=n+1}^0 X_i, &n<0 \\[3pt]  0, &n=0\\[3pt] \sum_{i=1}^n X_i, &n>0  \end{cases} \]
%so that the increments satisfy $S_n-S_m=\sum_{i=m+1}^n X_i$ for all $m<n$ in $\Z$.
 Let $(\lambda_i)_{i\ge 1}$ be the strict ascending ladder epochs of the forward walk.  That is, begin with $\lambda_0=0$,  and for $i\ge 1$  let 
\[  \lambda_i=\inf\{ n>\lambda_{i-1}:   S_{n} > S_{\lambda_{i-1}} \} . 
%\quad\text{and}\quad H_i=S_{T_{i}} -S_{T_{i-1}}. 
  \]
%and put $H_i=S_{T_{i}} -S_{T_{i-1}}$. 
 The positive drift of $S_n$ ensures that these variables are finite almost surely.   For $i\ge 1$  define the increments   $L_i=\lambda_i-\lambda_{i-1}$ and $H_i=S_{\lambda_{i}} -S_{\lambda_{i-1}}$.   The variables $\{L_i, H_i\}_{i\ge 1}$ are mutually independent with marginal distribution
 \be\label{expH1L1} \begin{aligned}
P(L_1=n, H_1>r) 
%&=  P(S_1<0, \dotsc, S_{n-1}<0, \, S_n>r)\\
%&=P(B_{n,r})
= C_{n-1}\,  \frac{\alpha^{n-1}\beta^n}{(\alpha+\beta)^{2n-1}}e^{-\alpha r}, \quad n\in\N, \, r\ge 0. 
\end{aligned}\ee 
Above $C_n=\frac{1}{n+1}{2n\choose n}$ for $n\ge0$ are the  Catalan numbers. 
 A small extension of the proof of Lemma B.3 in \cite{Fan-Sep-20} derives  \eqref{expH1L1}.  

  Let 
\be\label{d:expU}   W_0=\inf_{m>0} S_m . \ee   
Note that $W_0\circ\theta^n>0$ if and only if $S_n < \inf_{m>n} S_m$, that is, $n$ is a last exit time for the random walk. 
Define   successive last exit times  (in the language of Doney \cite{Don-89}) by 
\be\label{exp-si1}\begin{aligned} 
 \sigma_0&=\inf\{ n\ge0:  S_n < \inf_{m>n} S_m \}  % W_0\circ\theta^n >0\} 
 \\
\text{and for $i\ge 1$,}\qquad 
 \sigma_i&=\inf\{ n>\sigma_{i-1}:   S_n < \inf_{m>n} S_m \}. 
%= \inf\{ n>\sigma_{j-1}: W_0\circ\theta^n >0\} \\
%& =  \inf\Bigl\{ n>\sigma_{j-1}: \inf_{m>n} \sum_{i=n+1}^{m} Y_i  >0\Bigr\}
\end{aligned}\ee 
  

\begin{proposition}\label{pr:exp9}   %Assume $\alpha<\beta$.  
Conditionally on $W_0>0$ {\rm(}equivalently, on $\sigma_0=0${\rm)},  the pairs  $\{(\sigma_i-\sigma_{i-1}, S_{\sigma_i}-S_{\sigma_{i-1}})\}_{i\ge 1}$ are i.i.d.\ with  marginal distribution 
%$(\sigma_i-\sigma_{i-1}, S_{\sigma_i}-S_{\sigma_{i-1}})\deq(T_1, H_1)$.   
\be\label{exp85} \begin{aligned}
P(\sigma_i-\sigma_{i-1}=n, \, S_{\sigma_i}-S_{\sigma_{i-1}}>r\,\vert\,W_0>0) 
= C_{n-1}\,  \frac{\alpha^{n-1}\beta^n}{(\alpha+\beta)^{2n-1}}e^{-\alpha r}
\end{aligned}\ee 
for all $i\in\N$,  $n\in\N$,   and  $r\ge 0$. 
\end{proposition} 
 
\begin{proof} 
Let $0=n_0<n_1<\dotsm< n_\ell$ and $r_1,\dotsc,r_\ell>0$.   
  The dual random walk   $S^*_k=S_{n_\ell}-S_{n_\ell-k}$ for $0\le k\le n_\ell$ (p.~394 in Feller II \cite{Fel-71}) satisfies   $(S^*_k)_{0\le k\le n_\ell} \deq (S_k)_{0\le k\le n_\ell}$ and is independent of  $W_0\circ\theta^{n_\ell}$.   
  \begin{align*}
&P\bigl(\forall i=1,\dotsc,\ell:  \sigma_i-\sigma_{i-1}=n_i -n_{i-1} \text{ and }  S_{\sigma_i}-S_{\sigma_{i-1}}> r_i, \, W_0>0\bigr)\\  
&=
P\bigl(\forall i=1,\dotsc,\ell:  \sigma_i=n_i \text{ and }  S_{\sigma_i}-S_{\sigma_{i-1}}>r_i, \, W_0>0\bigr)\\
&=P\bigl( \forall i=1,\dotsc,\ell:  S_k>S_{n_i}>S_{n_{i-1}}+r_i \text{ for }  k\in\,\rzb n_{i-1}, n_i\lzb\, , \, W_0\circ\theta^{n_\ell} >0\bigr) \\
&= P\bigl( \forall i=1,\dotsc,\ell:  S^*_j< S^*_{n_\ell-n_i}<S^*_{n_\ell-n_{i-1}}-r_i \text{ for }  j\in\,\rzb n_\ell-n_i, n_\ell-n_{i-1} \lzb\, , \, W_0\circ\theta^{n_\ell} >0\bigr) \\
&=  P\bigl( \forall k=1,\dotsc,\ell:  \lambda_k=n_\ell-n_{\ell-k}\text{ and }  H_k>r_{\ell-k+1} \bigr)  \, P(W_0>0) \\
&=  P\bigl( \forall k=1,\dotsc,\ell:  L_k=n_{\ell-k+1}-n_{\ell-k}\text{ and }  H_k>r_{\ell-k+1} \bigr)  \, P(W_0>0)   .
%= C_{n-1}\,  \frac{\alpha^{n-1}\beta^n}{(\alpha+\beta)^{2n-1}}  \cdot  P(W_0>0) 
\end{align*} 
The claim follows from the independence of $\{L_k, H_k\}$ and \eqref{expH1L1}. 
%The event in the third probability above says that the ladder epochs of $S^*_{0,n_\ell}$ are $n_\ell-n_{\ell-1}, n_\ell-n_{\ell-2}, \dotsc, n_\ell$, with ladder height increments strictly above $r_\ell, r_{\ell-1},\dotsc, r_1$.  
\end{proof} 
 
% Next we extend Proposition \ref{pr:exp9} to negative times and also reformulate it. 
  From $\sigma_0$ as defined in \eqref{exp-si1},  extend  $\sigma_i$   to negative indices by defining, for $i=-1, -2, -3,\dotsc$, 
\be\label{exp:si1.1} 
\sigma_i=\max\bigl\{k<\sigma_{i+1}:     S_k< S_{\sigma_{i+1}}\bigr\} . 
\ee
For each $k\in\Z$ set 
\be\label{Wk}   W_k=   \inf_{n:\,n> k}   S_n-  S_{k} . \ee 
Then one can check that $\sigma_{-1}<0\le \sigma_0$, and for all $i,k\in\Z$, 
\be\label{78-63}  
S_{\sigma_i}=     \inf_{n:\,n> \sigma_{i-1}}   S_n  ,
\ee
\be\label{78-72}  W_{\sigma_i} 
=   \inf_{n:\,n> \sigma_i}   S_n- S_{\sigma_i} =  S_{\sigma_{i+1}}- S_{\sigma_i}, 
\ee
and 
%\be\label{78-64} \tau(i)=\min\bigl\{k>\tau(i-1):   \inf_{n:\,n> k}   S_n> S_{k}\bigr\}. 
%\ee
\be\label{78-65}  
 %  \inf_{n:\,n> k}   S_n>S_{k} 
  W_k>0   \ \iff\  k\in\{\sigma_i: i\in\Z\}. 
   \ee

\begin{theorem}\label{th:78-70} 
Conditionally on $\sigma_0=0$, equivalently, on $W_0>0$,   $\{\sigma_{i+1}-\sigma_i, W_{\sigma_i}: i\in\Z\}$ is an  i.i.d.\ sequence with marginal distribution 
\be\label{rw110} \begin{aligned} 
&P\bigl(\sigma_{i+1}-\sigma_i=n, \, W_{\sigma_i} >r\,\big\vert\,W_0>0\bigr) 
= C_{n-1}\,  \frac{\alpha^{n-1}\beta^n}{(\beta+\alpha)^{2n-1}}e^{-\alpha r} 
%\\   &\qquad\qquad= \frac1n\binom{2n-2}{n-1}\,  \frac{\alpha^{n-1}\beta^n}{(\beta+\alpha)^{2n-1}}e^{-\alpha r}\,,\quad n\in\N,\, r\in\R_+. 
\end{aligned} \ee
for all $i\in\N$,  $n\in\N$,   and  $r\ge 0$. 
\end{theorem}

%$\{\sigma_{i+1}-\sigma_i, \depa^2_{\sigma_i}-\depa^1_{\sigma_i}: i\ge0\}$

\begin{proof} 
 Define the processes $\Psi_+=\{\sigma_{i+1}-\sigma_i, W_{\sigma_i}: i\ge0\}$ and $\Psi_-=\{\sigma_{i+1}-\sigma_i, W_{\sigma_i}: i\le-1\}$.    $\Psi_+$ and  the conditioning  event    $W_0>0$ depend only on $(S_n)_{n\ge1}$,   while  $W_0>0$  implies   for $n<0$ that  $  \inf_{m:\,m>n} S_{m}= \inf_{m:\, n< m\le 0} S_{m}$.   $\Psi_+$ and $\Psi_-$ have been decoupled.  
 
Define another forward walk with the same step distribution  by $\wt S_k=-S_{-k}$ for $k\ge 0$.     Let $\lambda_0=0$,   $(\lambda_i)_{i\ge 1}$ be the successive ladder epochs and $H_i=\wt S_{\lambda_i}-\wt S_{\lambda_{i-1}}$   the successive ladder height increments for the $\wt S$ walk.  

We claim that on the event $\sigma_0=0$, 
\be\label{78-76} 
\lambda_{-i}=-\sigma_i \quad\text{and}\quad 
W_{\sigma_i}= H_{-i} \quad\text{for $i\le-1$.}  
\ee
First by definition, $\lambda_0=0=-\sigma_0$.  By the definitions and by induction, for $i\le -1$, 
\begin{align*}
\lambda_{-i} &=\min\{ k>\lambda_{-i-1}:  \wt S_k> \wt S_{\lambda_{-i-1}} \}
=\min\{ k>-\sigma_{i+1}:  S_{-k}< S_{\sigma_{i+1}} \} \\
%&=-\max\{ n<-\lambda_{-i-1}:  \wt S_{-n}> \wt S_{-\sigma_{i+1}} \} \\
&=-\max\{ n<\sigma_{i+1}:  S_{n}< S_{\sigma_{i+1}} \} 
= -\sigma_i 
\end{align*} 
where the last equality came from \eqref{exp:si1.1}.   Then from \eqref{78-72}, 
\begin{align*}  W_{\sigma_i} 
  =  S_{\sigma_{i+1}}- S_{\sigma_i}  =    -\wt S_{-\sigma_{i+1}}+\wt S_{-\sigma_i}
  =  -\wt S_{\lambda_{-i-1}}+\wt S_{\lambda_{-i}}= H_{-i}. 
\end{align*}
Claim \eqref{78-76} has been verified.  

Let   $\Psi'=\{ \lambda_{-i}-\lambda_{-i-1}, H_{-i}: i\le-1\}$,  a function of $(S_n)_{n\le -1}$.  
 By \eqref{78-76},    $\Psi_-=\Psi'$ on the event $\sigma_0=0$. 

Let $A$ and $B$ be suitable measurable sets of infinite sequences.  
\begin{align*}
&P( \Psi_+\in A, \Psi_-\in B\,\vert\,  W_0>0) =  \frac1{P(W_0>0)} P( \Psi_+\in A, \Psi'\in B, W_0>0) \\
&\qquad 
=\frac{P( \Psi_+\in A, W_0>0)}{P(W_0>0)} \, P(\Psi'\in B) 
=P( \Psi_+\in A\,\vert\,W_0>0)  P(\Psi'\in B). 
\end{align*} 
The conclusion follows.  By Proposition \ref{pr:exp9}, conditional on $W_0>0$, 
 $\Psi_+$ has the i.i.d.\ distribution \eqref{rw110}, which is the same as the i.i.d.\ distribution  \eqref{expH1L1} of $\Psi'$. 
\end{proof}




==> JEMS Post-Accept Revision/GeoWebPaper-Macros.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Packages go here
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{amsmath,amsfonts, amsthm,color,amssymb,mathrsfs,pgfplots,enumitem}   %F: enumitem is better than enumerate
%%% types of  labels:  [label=(roman*)]  \arabic*  \alph*    also under \itemize can use different symbols to mark items
\usepackage{times}
\RequirePackage[colorlinks,urlcolor=my-blue,linkcolor=my-red,citecolor=my-green]{hyperref}

\usepackage[numbers,comma,square,sort&compress]{natbib}
\usepackage{xargs}
\usepackage[colorinlistoftodos,prependcaption,textsize=footnotesize]{todonotes}
\usepackage{pdfcomment}
\usepackage{bm}
%\usepackage[left=1in,top=1in,right=1in,bottom=1in]{geometry}
\usepackage{scalerel}    %%%%  used first for scaling \bullet  
\usepackage{stmaryrd}   %%%% for integer interval notation 
\usepackage{mathabx}   %% made \widecheck work  
\usepackage{hyphenat}
\usepackage[utf8]{inputenc}
%\usepackage[notref,notcite]{showkeys}
%%%%  2019-03-22 Timo moved showkeys into the latex file itself in order to toggle it for printing. 
\usepackage{caption}
\usepackage{subcaption}
\usepackage{a4wide}
\usepackage{accents}
\usepackage{tikz}
\usetikzlibrary{arrows.meta,decorations.markings}
\usepackage{graphicx}
\usepackage{chngcntr}
\usepackage{float} %needed to fix the figures

\usepackage{rotating,centernot,cancel}    %% to manipulate symbols (Timo 2019-03-25) 

\numberwithin{figure}{section}
\numberwithin{equation}{section}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% New macros for this paper
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%General
\tikzset{middlearrow/.style={
        decoration={markings,
            mark= at position 0.6 with {\arrow{#1}} ,
        },
        postaction={decorate}
    }
}

\newcommand\aUset{\sV^{\,\w}} %The set of directions on which non-coalescence holds
%\newcommand\gpp{g_{\text{pp}}} %The shape function
\newcommand\gpp{g} %The shape function without pp subscript 
\newcommand\dgpp[1]{\widecheck{g}_{\text{pp}}^{#1}} %The shape function
\newcommand\T{T} %The shift, T
%\newcommand\cif{\xi_*} %The competition interface random variable
\newcommand\cid{\xi_*} %The competition interface random variable
\newcommand\adir{\zeta} 
\newcommand\wchk[1]{\widecheck{\omega}^{#1}} %Dual weights

%Busemann functions
\newcommand\B[1]{B^{#1}} %The Busemann function
\newcommand\BBbar[1]{{\overline B}^{#1}} %The Busemann function
\newcommand\Ubar{\overline U} %The Busemann function
\newcommand\dB[1]{u^{#1}} %The Busemann function
\newcommand\dBbar[1]{\overline{u}^{#1}} %The Busemann function

%Geodesics
\newcommand\geo[3]{\boldsymbol{\gamma}_{#1}^{\,#2,#3}} %Geodesic. Arguments are 1.) the index, 2.) the starting point, 3.) the direction
\newcommand\geobar[3]{{\overline{\boldsymbol{\gamma}}}_{#1}^{\,#2,#3}} %Geodesic. Arguments are 1.) the index, 2.) the starting point, 3.) the direction
\newcommand\geod[1]{\pi_{#1}} %A generic geodesic without a root or direction. The argument is the index.
%\newcommand\geod[1]{\boldsymbol{\gamma }_{#1}} %A generic geodesic without a root or direction. The argument is the index.


%Coalescence points
\newcommand\coal[1]{\mathbf{z}^{#1}} %Coalescence point. The argument is the direction.

%Split points
\newcommand\spt[2]{s_{#1}(#2)}


%The geodesic graphs and vertex sets 
\newcommand\G[1]{\mathcal{G}_{#1}} %The graph of geodesics. Argument is the direction.
\newcommand \dG[1]{\mathcal{G}^*_{#1}} %The dual graph to the graph of geodesics. Argument is the direction.
\newcommand\dGpp[1]{\widecheck{G}^{#1}} %The dual passage times
%\newcommand\dS[1]{\mathcal{T}_{#1}^{*}}
\newcommand\dS[1]{\mathcal{G}_{\cup#1}^{*}}   %% trying out another option

\def\Shock#1#2{{\bfS}^{#1}_{#2}}
\def\shock#1{{\bfS}_{#1}^*}      %%%% red points 
\def\ans#1#2{{\bfA}_{#1}^*(#2)}    %%%% ancestors 
\def\shockG#1{{\mathcal S}_{#1}^*}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Macros inherited from the DLR paper
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\addtolength{\hoffset}{-.8in} 
%\addtolength{\textwidth}{1.6in}
%\addtolength{\voffset}{-.3in} 
%\addtolength{\footskip}{.3in}
%\setlength{\oddsidemargin}{0in}
%\setlength{\evensidemargin}{0in}
%\setlength{\footskip}{0.2in}
%\setlength{\topmargin}{0.5in}
%\addtolength{\textheight}{.7in}
%\baselineskip=12pt   %%seems to make no difference? 
%\linespread{1.1}     %this works nicely to produce a more readable cropped 2-1


\RequirePackage{color}
\definecolor{my-link}{rgb}{0.5,0.0,0.0}
\definecolor{my-blue}{rgb}{0.0,0.0,0.6}
\definecolor{my-red}{rgb}{0.5,0.0,0.0}
\definecolor{my-green}{rgb}{0.0,0.5,0.0}
\definecolor{nicos-red}{rgb}{0.75,0.0,0.0}
\definecolor{really-light-gray}{gray}{0.8}
\definecolor{darkgreen}{rgb}{0.0,0.5,0.0}
\definecolor{darkblue}{rgb}{0.0,0.0,0.3}
\definecolor{nicosred}{rgb}{0.65,0.1,0.1}
\definecolor{light-gray}{gray}{0.7}

\definecolor{sussexg}{rgb}{0,0.7,0.7}
\definecolor{sussexp}{rgb}{0.4,0,0.4}
\definecolor{nicos-red}{rgb}{0.75,0.0,0.0}

\addtolength\marginparwidth{0.28in}

\newcommandx{\addmath}[2][1=]{\todo[linecolor=red,backgroundcolor=red!25,bordercolor=red,#1]{#2}}
\newcommandx{\fixtext}[2][1=]{\todo[linecolor=blue,backgroundcolor=blue!25,bordercolor=blue,#1]{#2}}
\newcommandx{\note}[2][1=]{\todo[linecolor=yellow,backgroundcolor=yellow!25,bordercolor=yellow,#1]{#2}}

%\pgfplotsset{compat=newest}
%\pgfplotsset{plot coordinates/math parser=false}
%\newlength\figureheight
%\newlength\figurewidth

%%%%%%   Symbols for plus and minus 
%\newcommand{\sig}{{\mbox{\larger$\square$}}}
%\newcommand{\gis}{\boxminus}
%\newcommand{\sig}{\boxempty}   % too large 
\newcommand{\sig}{{\scaleobj{0.8}{\boxempty}}} 
\newcommand{\sigg}{{\scaleobj{0.9}{\boxempty}}} 
%\newcommand{\sig}{{\raisebox{1pt}{\scaleobj{0.8}{\boxempty}}}}  
\newcommand{\gis}{{\raisebox{1pt}{\scaleobj{0.6}{\boxslash}}}}   
\newcommand{\giss}{{\raisebox{1pt}{\scaleobj{0.8}{\boxslash}}}}   
%\newcommand{\gis}{{\mbox{\larger$\diamond$}}}
%\newcommand{\sig}{\square}
%%%%    Try out also \ovoid and \ominus

\newcommand{\bbA}{\mathbb{A}}
\newcommand{\bbB}{\mathbb{B}}
\newcommand{\bbC}{\mathbb{C}}
\newcommand{\bbD}{\mathbb{D}}
\newcommand{\bbE}{\mathbb{E}}
\newcommand{\bbF}{\mathbb{F}}
\newcommand{\bbG}{\mathbb{G}}
\newcommand{\bbH}{\mathbb{H}}
\newcommand{\bbI}{\mathbb{I}}
\newcommand{\bbJ}{\mathbb{J}}
\newcommand{\bbK}{\mathbb{K}}
\newcommand{\bbL}{\mathbb{L}}
\newcommand{\bbM}{\mathbb{M}}
\newcommand{\bbN}{\mathbb{N}}
\newcommand{\bbO}{\mathbb{O}}
\newcommand{\bbP}{\mathbb{P}}
\newcommand{\bbQ}{\mathbb{Q}}
\newcommand{\bbR}{\mathbb{R}}
\newcommand{\bbS}{\mathbb{S}}
\newcommand{\bbT}{\mathbb{T}}
\newcommand{\bbU}{\mathbb{U}}
\newcommand{\bbV}{\mathbb{V}}
\newcommand{\bbW}{\mathbb{W}}
\newcommand{\bbX}{\mathbb{X}}
\newcommand{\bbY}{\mathbb{Y}}
\newcommand{\bbZ}{\mathbb{Z}}

%bold face
\newcommand{\bfA}{\mathbf{A}}
\newcommand{\bfB}{\mathbf{B}}
\newcommand{\bfC}{\mathbf{C}}
\newcommand{\bfD}{\mathbf{D}}
\newcommand{\bfE}{\mathbf{E}}
\newcommand{\bfF}{\mathbf{F}}
\newcommand{\bfG}{\mathbf{G}}
\newcommand{\bfH}{\mathbf{H}}
\newcommand{\bfI}{\mathbf{I}}
\newcommand{\bfJ}{\mathbf{J}}
\newcommand{\bfK}{\mathbf{K}}
\newcommand{\bfL}{\mathbf{L}}
\newcommand{\bfM}{\mathbf{M}}
\newcommand{\bfN}{\mathbf{N}}
\newcommand{\bfO}{\mathbf{O}}
\newcommand{\bfP}{\mathbf{P}}
\newcommand{\bfQ}{\mathbf{Q}}
\newcommand{\bfR}{\mathbf{R}}
\newcommand{\bfS}{\mathbf{S}}
\newcommand{\bfT}{\mathbf{T}}
\newcommand{\bfU}{\mathbf{U}}
\newcommand{\bfV}{\mathbf{V}}
\newcommand{\bfW}{\mathbf{W}}
\newcommand{\bfX}{\mathbf{X}}
\newcommand{\bfY}{\mathbf{Y}}
\newcommand{\bfZ}{\mathbf{Z}}

\newcommand{\bfa}{\mathbf{a}}
\newcommand{\bfb}{\mathbf{b}}
\newcommand{\bfc}{\mathbf{c}}
\newcommand{\bfd}{\mathbf{d}}
\newcommand{\bfe}{\mathbf{e}}
\newcommand{\bff}{\mathbf{f}}
\newcommand{\bfg}{\mathbf{g}}
\newcommand{\bfh}{\mathbf{h}}
\newcommand{\bfi}{\mathbf{i}}
\newcommand{\bfj}{\mathbf{j}}
\newcommand{\bfk}{\mathbf{k}}
\newcommand{\bfl}{\mathbf{l}}
\newcommand{\bfm}{\mathbf{m}}
\newcommand{\bfn}{\mathbf{n}}
\newcommand{\bfo}{\mathbf{o}}
\newcommand{\bfp}{\mathbf{p}}
\newcommand{\bfq}{\mathbf{q}}
\newcommand{\bfr}{\mathbf{r}}
\newcommand{\bfs}{\mathbf{s}}
\newcommand{\bft}{\mathbf{t}}
\newcommand{\bfu}{\mathbf{u}}
\newcommand{\bfv}{\mathbf{v}}
\newcommand{\bfw}{\mathbf{w}}
\newcommand{\bfx}{\mathbf{x}}
\newcommand{\bfy}{\mathbf{y}}
\newcommand{\bfz}{\mathbf{z}}


\newcommand{\mfa}{\mathfrak{a}}
\newcommand{\mfb}{\mathfrak{b}}
\newcommand{\mfc}{\mathfrak{c}}
\newcommand{\mfd}{\mathfrak{d}}
\newcommand{\mfe}{\mathfrak{e}}
\newcommand{\mff}{\mathfrak{f}}
\newcommand{\mfg}{\mathfrak{g}}
\newcommand{\mfh}{\mathfrak{h}}
\newcommand{\mfi}{\mathfrak{i}}
\newcommand{\mfj}{\mathfrak{j}}
\newcommand{\mfk}{\mathfrak{k}}
\newcommand{\mfl}{\mathfrak{l}}
\newcommand{\mfm}{\mathfrak{m}}
\newcommand{\mfn}{\mathfrak{n}}
\newcommand{\mfo}{\mathfrak{o}}
\newcommand{\mfp}{\mathfrak{p}}
\newcommand{\mfq}{\mathfrak{q}}
\newcommand{\mfr}{\mathfrak{r}}
\newcommand{\mfs}{\mathfrak{s}}
\newcommand{\mft}{\mathfrak{t}}
\newcommand{\mfu}{\mathfrak{u}}
\newcommand{\mfv}{\mathfrak{v}}
\newcommand{\mfw}{\mathfrak{w}}
\newcommand{\mfx}{\mathfrak{x}}
\newcommand{\mfy}{\mathfrak{y}}
\newcommand{\mfz}{\mathfrak{z}}


\newcommand{\mfG}{\mathfrak{G}}
\newcommand{\mfS}{\mathfrak{S}}

%script
\newcommand{\sA}{\mathcal{A}}
\newcommand{\sB}{\mathcal{B}}
\newcommand{\sC}{\mathcal{C}}
\newcommand{\sD}{\mathcal{D}}
\newcommand{\sE}{\mathcal{E}}
\newcommand{\sF}{\mathcal{F}}
\newcommand{\sG}{\mathcal{G}}
\newcommand{\sH}{\mathcal{H}}
\newcommand{\sI}{\mathcal{I}}
\newcommand{\sJ}{\mathcal{J}}
\newcommand{\sK}{\mathcal{K}}
\newcommand{\sL}{\mathcal{L}}
\newcommand{\sM}{\mathcal{M}}
\newcommand{\sN}{\mathcal{N}}
\newcommand{\sO}{\mathcal{O}}
\newcommand{\sP}{\mathcal{P}}
\newcommand{\sQ}{\mathcal{Q}}
\newcommand{\sR}{\mathcal{R}}
\newcommand{\sS}{\mathcal{S}}
\newcommand{\sT}{\mathcal{T}}
\newcommand{\sU}{\mathcal{U}}
\newcommand{\sV}{\mathcal{V}}
\newcommand{\sW}{\mathcal{W}}
\newcommand{\sX}{\mathcal{X}}
\newcommand{\sY}{\mathcal{Y}}
\newcommand{\sZ}{\mathcal{Z}}

\font \mymathbb = bbold10 at 11pt
\newcommand{\one}{\mbox{\mymathbb{1}}}
%\newcommand{\one}{\mathbf{1}}


\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\supp}{supp}

\def\esssup{\mathop{\mathrm{ess\,sup}}}
\def\range{\mathcal R}
\def\Uset{\mathcal U}
\def\fUset{\mathcal H}   % remove flat parts from \ri\Uset 
\newcommand{\dUset}[1]{\widecheck{\mathcal U}^{#1}}
%\def\Usetnice{\Uset_1}
\def\Usetnonuniq{\Uset_x^\w}
\def\Usetnonuniqz{\Uset_0^\w}
\def\Udense{\Uset_0}
\def\Ddense{\Diff_0}
\def\Usetnonuniqhat{\Uset_x^\what}
%\def\riUset{\Uset^\circ}

\newcommand{\fl}[1]{\lfloor{#1}\rfloor} 
\newcommand{\ce}[1]{\lceil{#1}\rceil}

\newcommand{\e}{\varepsilon}
\def\Diff{\sD}
\def\Cont{\sC}
\def\w{\omega}
\def\wbar{{\bar\w}}
\def\wtil{{\tilde\w}}
\newcommand{\ehat}{\widehat{e}}
\newcommand{\et}{\widehat{e}_1}   % e_1 + e_2 
\newcommand{\etstar}{\et^{\,*}}   %   (e_1 + e_2 )/2 
\newcommand{\ex}{\widehat{e}_2}   % e_2 - e_1 
\newcommand{\exstar}{\ex^{\,*}}   % (e_2 - e_1)/2  
\def\unif{\vartheta}
\def\Unif{\Gamma}
\def\eB{\kappa}
\def\EB{\cK}
\def\Bavg{\overline B}
\def\Gbar{\overline G}
\providecommand{\abs}[1]{\vert#1\vert}
\def\what{{\widehat\w}}
\def\wh{\widehat}
\def\wt{\widetilde}
\def\Omhat{\widehat\Omega}
\def\Omerg{\Omega^{\mathrm{???}}}
\def\Omreg{\Omega^{\mathrm{reg}}}
\def\Omjump{\Omega^{\mathrm{jump}}_0}
\def\OmCou{\Omega^{\mathrm{no3geo}}_0}
\def\Ombiinf{\Omega^{\mathrm{nobi}}_0}
\def\Omregjump{\Omega_0^{\mathrm{reg,jump}}}
\def\ddd{\displaystyle}
\def\fe{\Lambda}
\def\fepl{\fe_{\rm{pl}}}
\def\Zne{Z^{\rm NE}} 
\def\Qne{Q^{\rm NE}} 
\def\Zn{Z^{\rm N}} 
\def\xibar{\bar\xi}
\def\Abar{\overline A}
\def\zetabar{\bar\zeta}
\def\etabar{\bar\eta}
\def\hu{{\underline h}}
\def\ho{{\overline h}}
\def\ximin{{\underline\xi}}
\def\ximax{{\overline\xi}}
\def\ximinmin{\underline{\underline\xi}}
\def\ximaxmax{\overline{\overline\xi}}
\def\etaminmin{\underline{\underline\eta}}
\def\etamaxmax{\overline{\overline\eta}}
\def\zetaminmin{\underline{\underline\zeta}}
\def\zetamaxmax{\overline{\overline\zeta}}
\def\etamin{{\underline\eta}}
\def\etamax{{\overline\eta}}
\def\zetamin{{\underline\zeta}}
\def\zetamax{{\overline\zeta}}
\DeclareMathOperator{\ri}{ri}    %rel interior  
\DeclareMathOperator{\ext}{ext}    %extremes 
\DeclareMathOperator{\dist}{dist} 
%\def\xuDLR{x^{u,{\rm{DLR}}}}
\def\XDLR{\overline X^{\,x,\w}}
\def\Xtree{\widehat X^{\,\zeta,\w}}
\def\Xtreen{\widehat X^{\,\zeta,\w,(n)}}
%\def\backpix{{\overleftarrow{\pi}}^x} 
%\def\backpi{{\overset{\small\leftarrow}{\pi}}{}} 
\def\DLR{\mathrm{DLR}}
\newcommand{\siDLR}{\overrightarrow{\DLR}}
\newcommand{\biDLR}{\overleftrightarrow{\DLR}}
\def\CI{\phi}

\def\pici{\pi^{\rm{cif}}}
\def\ker{\kappa}
%\def\cid{\xi^*}
\def\Bci{B^*}
\def\Bcil{B^{*,\text\rm{(l)}}}
\def\Bcir{B^{*,\text\rm{(r)}}}
\def\Bbar{\overline B}
\def\Bbarci{\bar B^*}
%\def\cidm{\cid}
\def\cidmin{\underline\xi_{^{\scriptstyle*}}}
\def\cidmax{\overline\xi_*}
\def\ci{{\rm ci}}
\def\Pibar{\overline\Pi}
\def\Pici#1{\Pi^{\ci,\w,#1}}
\def\Picil#1{\Pi^{\ci,\w,\text\rm{(l)},#1}}
\def\Picir#1{\Pi^{\ci,\w,\text\rm{(r)},#1}}
\def\picix{\pi^{x,\ci}}
%\def\varphimin{\varphi^{{\text\rm{(l)}}}}
%\def\varphimax{\varphi^{{\text\rm{(r)}}}}
\def\cidl{\cid^{\text\rm{(l)}}}
\def\cidr{\cid^{\text\rm{(r)}}}
\def\cidlmin{\cidmin^{\text\rm{(l)}}}
\def\cidrmin{\cidmin^{\text\rm{(r)}}}
\def\cidlmax{\cidmax^{\text\rm{(l)}}}
\def\cidrmax{\cidmax^{\text\rm{(r)}}}
%\def\cTl{\cT^{\textrm{(l)}}}
%\def\thetal{\theta_*^{\text\rm{(l)}}}
%\def\thetar{\theta_*^{\text\rm{(r)}}}
%\def\Bcir{\overline B_*}
%\def\Bcil{\underline B_*}


\newcommand{\That}{\widehat{T}}
\def\Omtemphat{\widehat\Omega_0}
\def\Ommono{\Omega_{\rm{coc}}} %the Omega on which monotonicity (and other properties?) of cocycles holds
\def\Ommonohat{\widehat\Omega_{\rm{coc}}} %the Omega on which monotonicity (and other properties?) of cocycles holds
\def\Omcont#1{\Omega_{\rm{cont},#1}} %the Omega on which continuity holds at \xi
\def\Omconthat#1{\widehat\Omega_{\rm{cont},#1}} %the Omega on which continuity holds at \xi
\def\Omconstt#1{\Omega_{\rm{tilt},#1}} %the Omega on which h(B) is constant
\def\Omconsthat#1{\widehat\Omega_{\rm{tilt},#1}} %the Omega on which h(B) is constan
\def\Omback#1{\Omega_{#1,\downarrow0}} %the Omega on which the B-tree dies out
\def\OmBus{\Omega_{[\ximin,\ximax]}} %the Omega on which liminf and limsup bounds hold for Busemann limits for the given \xi
\def\Ombi{\Omega_{\rm{bi},[\ximin,\ximax]}} %the Omega on which liminf and limsup bounds hold for Busemann limits for the given \xi
\def\OmBuszeta{\Omega_{[\zetamin,\zetamax]}} %the Omega on which liminf and limsup bounds hold for Busemann limits for the given \zeta
\def\OmBusnice{\Omega_1} %the Omega on which Busemann limits exist on a dense set
\def\OmBusa{\Omega_a} %the Omega on which one force one solution holds 
\def\Omshape{\Omega_{\rm{shape}}} %the Omega on which the shape thms hold
\def\OmBushat{\widehat\Omega_{[\ximin,\ximax]}} %the Omega on which Busemann limit holds
\def\OmBushatzeta{\widehat\Omega_{[\zetamin,\zetamax]}} %the Omega on which liminf and limsup bounds hold for Busemann limits 
\def\OmBusallhat{\widehat\Omega_{\rm{Bus}}} %the Omega on which liminf and limsup bounds hold for Busemann limits for all \xi
\def\OmBusall{\Omega_{\rm{Bus}}} %the Omega on which liminf and limsup bounds hold for Busemann limits for all \xi
\def\Omexist{\Omega_{\rm{exist}}} %the Omega on which directedness of cocycle DLRs holds
\def\Omexistxi{\Omega_{\rm{exist},\xi}} %the Omega on which directedness of cocycle DLRs holds
\def\Omexisthat{\widehat\Omega_{\rm{exist}}} %the Omega on which directedness of cocycle DLRs holds
\def\Omdir{\Omega_{\rm{dir}}} %the Omega on which every DLR is directed
\def\Omdirhat{\widehat\Omega_{\rm{dir}}} %the Omega on which every DLR is directed
\def\OmBusPi{\Omega'_{[\ximin,\ximax]}} %the Omega on which DLR is Busemann for the given \xi
\def\OmBusPihat{\widehat\Omega'_{[\ximin,\ximax]}} %the Omega on which DLR is Busemann for the given \xi
\def\OmBusPiall{\Omega_{\rm{uniq}}} %the Omega on which Busemann limits will hold for all directions at once
\def\OmBusPiallhat{\widehat\Omega_{\rm{uniq}}} %the Omega on which Busemann limits will hold for all directions at once
\def\Omnondeg{\Omega_{\rm{nondeg}}}  %the Omega on which the only non-degenerate DLR solutions are \Pi^{e_i}
\def\OmBhat{\widehat\Omega_B}  %the Omega on which the DLR solution corresponding to B is directed
%\def\OmB{\Omega_B}  %the Omega on which the DLR solution corresponding to B is directed
%\def\Omreg{\Omega_{\rm{reg}}} % the Omega on which regular conditional probabilities are supported on the projection
\def\Omcif{\Omega_{\rm{cif}}} % the Omega on which regular conditional probabilities are supported on the projection
\def\Omnonuniq{\Omega_{\rm{ex}}} %the Omega on which Usetnonuniq does not intersect linear segments and includes non-diff points
\def\Omeihat{\widehat\Omega_{e_1,e_2}}


\def\WLLN{WLLN$_\xi$}
\def\SLLN{SLLN$_\xi$}
\def\proj{\pi}
\def\gDLR{\mathrm{gDLR}}
\def\cgDLR{\mathrm{cgDLR}}

\allowdisplaybreaks
%\allowdisplaybreaks[3]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Environment definitions go here
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{formal}[theorem]{Critical point derivation}
\newtheorem{experiment}[theorem]{Experimental Result}
\newtheorem{clam}[theorem]{Claim}
\newtheorem{condition}[theorem]{Condition}


\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
%\newtheorem{xca}[theorem]{Exercise}
\newtheorem{exercise}[theorem]{Exercise}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{conj}[theorem]{Conjecture}

%\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}
\newenvironment{remarks}{\begin{remark}\normalfont}{\end{remark}}
\newtheorem{quest}{Question}


%%%%%%%   the BEST  Timo macros (2018-01-19--)  %%%%%%%%

\newcommand{\nn}{\nonumber}

\DeclareMathOperator{\hull}{\overline{\text{co}}}
\DeclareMathOperator{\Span}{span}
\DeclareMathOperator{\bd}{bd}

\DeclareMathOperator{\sign}{sign} 
\DeclareMathOperator{\diam}{diam}
\DeclareMathOperator{\epi}{epi}
\DeclareMathOperator{\card}{card}
%\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\trace}{trace}
%\DeclareMathOperator{\dist}{dist}
\DeclareMathOperator{\var}{Var}
\DeclareMathOperator{\Var}{\mathbb Var}
  \DeclareMathOperator{\Cov}{Cov}  
  \DeclareMathOperator{\conv}{co}   %convex hull  


%\DeclareMathOperator{\proj}{Proj}
%\DeclareMathOperator{\ri}{ri}    %rel interior  
\DeclareMathOperator{\aff}{aff}   %affine hull  
\DeclareMathOperator{\effdom}{dom}   %eff domain 
\DeclareMathOperator{\id}{id}


\font \mymathbb = bbold10 at 11pt
\newcommand{\ind}{\mbox{\mymathbb{1}}}
%\def\ind{\mathbf{1}}
\def\deq{\overset{d}=} 
\def\dto{\overset{d}\to} 
\def\qedex{\hfill$\triangle$} 
\def\qedrm{\hfill$\triangle$} 
\def\iff{\Longleftrightarrow}
\def\implies{\Longrightarrow}
\def\rimplies{\Longleftarrow}

\newcommand{\bD}{\mathbb{D}}

\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}

\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}

\def\Z{\bbZ} 
\def\R{\bbR} 
\def\N{\bbN} 

\def\Xw{X}  %another letter for a weight 
\def\Yw{Y}  %another letter for a weight 
\def\Ywch{\wc\Yw}  %another letter for a weight 

\def\kvec{\mathbf{k}}  \def\mvec{\mathbf{m}}   \def\nvec{\mathbf{n}}
 \def\pvec{\mathbf{p}}
\def\xvec{\mathbf{x}}
\def\yvec{\mathbf{y}}
\def\zvec{\mathbf{z}}
\def\wvec{\mathbf{w}}
\def\Jvec{\mathbf{J}}
\def\Xvec{\mathbf{X}} \def\Yvec{\mathbf{Y}}  \def\Zvec{\mathbf{Z}} \def\thvec{\boldsymbol{\theta}}

\def\absorb{\triangleleft}

\def\timonote#1{{\color{darkgreen}{(#1)}}}
\def\E{\bbE}
\def\P{\bbP} %% environment measure 

 \def\wt{\widetilde}  \def\wh{\widehat} \def\wb{\overline} \def\wc{\widecheck}

\def\Bus#1{B^{#1}} 
\def\rBus#1{\wt B^{#1}}
\def\wtBus#1{\wt B^{#1}}
\newcommand\Busv[3]{\overline B^{\,#1,#2}_{#3}}

\def\RW{S}
\def\ZRW{Z}
\def\Zero{R}
\def\Zerobar{\overline\Zero}

%%%%%%%   Random measures with superscript "Bus" 
%\def\Bpp{\mathbf{n}^{\text{\rm Bus}}}  %  \Bpp = Busemann pt process of jump locations 
%\def\Bppa{{\boldsymbol\nu}^{\text{\rm Bus}}}   %  \Bppa = Busemann pt process of jump locations and jump sizes
%\def\Bppb{{\boldsymbol\mu}^{\text{\rm Bus}}}   %Busemann measure on edge k 
%\def\Bmeas{\mu^{\text{\rm Bus}}} 
%\def\Bmeasb{\boldsymbol{\nu}^{\text{\rm Bus}}} 
%\def\Bmm{m^{\text{\rm Bus}}}   %mean Busemann measure 

%%%%%  These random measures without superscript "Bus" 
\def\Bpp{\mathbf{n}}  %  \Bpp = Busemann pt process of jump locations 
\def\Bppa{{\boldsymbol\nu}}   %  \Bppa = Busemann pt process of jump locations and jump sizes
\def\Bppavar{\nu}   %  \Bppa = Busemann pt process of jump locations and jump sizes
\def\Bppb{{\boldsymbol\mu}}   %Busemann measure on edge k 
\def\Bmeas{\mu} 
\def\Bmeasb{\boldsymbol{\nu}} 
\def\Bmm{\lambda}   %mean Busemann point measure 
\def\umeas{u}   %measure of point locations of a purely atomic measure 

%\def\Hgraph{\cH}  %a graph 
\newcommand\Hgraph[1]{\mathcal{H}_{#1}}
\def\zclus{\bfK}    %notation for the backward cluster of z 
\def\cifset{\bfD}  %set of vertices with asymptotic cif direction in a set 
\def\xisim{\,\overset\xi\sim\,}    %equivalence relation  
%\def\zesim{\,\overset{[\zeta, \eta]}\sim\,}    %equivalence relation 
\def\zesim{ \overset{[\zeta, \eta]}\sim }    %equivalence relation without extra space

\def\depa{B}  %% departure processes from queues, also the generic variable for Busemanns in the description of the joint distribution. 
\def\serv{w}     %% service variables 

\def\level{\bbL}     %%%% levels on lattice 


  \def\evec{\mathbf{e}}  \def\uvec{\mathbf{u}}\def\vvec{\mathbf{v}}
   \def\avec{\mathbf{a}} \def\bvec{\mathbf{b}}

\newcommand\bnearrow{{\raisebox{1pt}{\scaleobj{0.5}{\mathbf\nearrow}}}}   %% \nearrow for a superscript so it doesn't look ridiculously big 
    
\def\caY{\cY^{\bnearrow}}  % a space of ordered n-tuples 
\def\caaY{\cY^{\bnearrow\!\bnearrow}}  % a space of ordered n-tuples 
\def\paramb{\tau}   %% needed a parameter -- not sure what a good letter choice is. 
   
\def\gdirv{\xi}    %geodesic direction 
\def\gdirc{\xi\cdot\evec}  %coordinate of a geodesic direction 

\def\Dop{D}    %%% D operator for departure process 
\def\Rop{R}  %% check weights or time in the back of the queue  
\def\Sop{S}    %%% S operator for sojourn time process 
\def\Daop{\cD}   %%n"bigger" operators 
\def\Taop{\cT}
\def\Saop{\cS} 
\def\rDop{{\overleftarrow\Dop}}    %%% reverse D operator for departure process 
\def\rRop{{\overleftarrow\Rop}}  %% check weights or time in the back of the queue  
\def\rSop{{\overleftarrow\Sop}}    %%% S operator for sojourn time process 
\def\fDop{{\overrightarrow\Dop}}    %%% forward D operator for departure process 
\def\fRop{{\overrightarrow\Rop}}  %%   forward
\def\fSop{{\overrightarrow\Sop}}    %%%   forward
\def\refl{\rho}   % reflection 

\def\OFP{(\Omega, \cF, P)} 
\def\OSP{(\Omega, \mfS, \P)}
   
   \newcommand{\lzb}{\llbracket}   %left Z bracket  
\newcommand{\rzb}{\rrbracket}   %right Z bracket 

\def\indep{\ \ \,{\raisebox{-1pt}{\text{\begin{rotate}{90}$\models$\end{rotate}}}}\ \, }  %independent random variables 
\def\nindep{\ \ \,{\raisebox{-1pt}{\text{\begin{rotate}{90}$\nvDash$\end{rotate}}}}\ \, }   %not independent random variables 

\newcommand\abullet{{\scaleobj{0.6}{\bullet}}}  %%%% smaller bullet to use inside functions 
\newcommand\bbullet{{\raisebox{0.5pt}{\scaleobj{0.6}{\bullet}}}} %% looks good for paths x_\bbullet 
\newcommand\brbullet{{\raisebox{-1pt}{\scaleobj{0.5}{\bullet}}}} %%  for subscript paths x_\brbullet   need negative raise 
\newcommand\cbullet{{\raisebox{1pt}{\scaleobj{0.6}{\bullet}}}}   %% looks good on Busemann process \Bus^\cbullet  as a subscript  

\newcommand\dbullet{{\scaleobj{0.7}{\bullet}}}   % same as \bbullet but without shift up

\newcommand\bcdot{{\scaleobj{1.8}{\cdot}}}
\newcommand\acdot{{\raisebox{-1pt}{\scaleobj{1.4}{\cdot}}}}  %%dot inside function 

%%%%%%%%   End Timo's macros %%%%%%%%%

%\usepackage{filemod}   
%\usepackage[short,nodayofweek,level,12hr]{datetime}   %%% clash

\overfullrule=5pt



==> JEMS Post-Accept Revision/GeoWebPaper-Sec1.tex <==
% !TEX root = GeoWebPaper.tex

%Should mention that the previous state of the art largely had to restrict attention to semi-infinite geodesics which are `typical' but only for a fixed direction. \textcolor{red}{mention prominently the curious fact about the appearance of bi-infinite shock paths!}

\section{Introduction} 

\subsection{Random growth models} Irregular or random growth is a ubiquitous phenomenon in nature,   from the growth of tumors, crystals, and bacterial colonies to the propagation of forest fires and the spread of water through a porous medium. Models of random growth have been a driving force in probability theory over the last sixty years and a wellspring of important ideas \cite{Auf-Dam-Han-17}. 

The mathematical analysis of such models began in the early 1960s with the introduction of the {\it Eden model} by Eden \cite{Ede-61} and {\it first-passage percolation} (FPP) by Hammersley and Welsh \cite{Ham-Wel-65}.  
About two decades later, early forms of a directed variant of FPP,  {\it directed last-passage percolation}  (LPP), appeared in a paper by Muth \cite{Mut-79} in connection with {\it series of queues in tandem}. 
Soon after, Rost \cite{Ros-81} introduced a random growth model, now known as the {\it corner growth model} (CGM), in connection with the {\it totally asymmetric simple exclusion process} (TASEP), a model of interacting particles. 
A decade later, the CGM arose naturally from LPP in queueing theory in the work of Szczotka and Kelly \cite{Szc-Kel-90} and Glynn and Whitt \cite{Gly-Whi-91}.
Around the same time, the third author \cite{Sep-98-mprf-1} connected the CGM and LPP to  Hamilton-Jacobi equations and Hopf-Lax-Oleinik semigroups.%, bringing in yet another analytical tool to the model.
%The CGM acquired even more analytical tools, through further connections to subjects like statistical physics, integrable systems, 
%and representation theory; \addmath{is this a good reference? any others?}
%see the review \cite{Dam-Ras-Sep-16}.    

 Much of this early work was primarily concerned with the deterministic asymptotic shape and large deviations of the randomly growing interface.   The breakthrough  of Baik, Deift, and Johansson  \cite{Bai-Dei-Joh-99}  showed that   the  fluctuations of the Poissonian LPP model   have the same  limit as the fluctuations of the largest eigenvalue of  the {\it Gaussian unitary ensemble}  derived by Tracy and Widom in \cite{Tra-Wid-94}.   This result was extended to  the exactly solvable versions of the CGM  by  Johansson  in \cite{Joh-00}.  These results  marked the CGM and the related LPP and TASEP models as members of the {\it Kardar-Parisi-Zhang}  (KPZ) universality class.  This  universality class is conjectured to describe the statistics of a growing interface   observed when a rapidly mixing stable state invades a rapidly mixing metastable state.  This subject  has been a major focus of   probability theory and statistical physics over the last three decades.  Recent surveys appear in  \cite{Cor-12,Cor-16,Hal-Tak-15,Qua-Spo-15,Qua-12}.


\subsection{Geodesics} A common feature of many models of random growth is  a natural metric-like interpretation  in which there exist paths that can be thought of as geodesics. In these interpretations, the growing interface can be viewed as a sequence of balls of increasing radius and centered at the origin. This connection is essentially exact in the case of FPP, which  describes a random pseudo-metric on $\bbZ^d$. Related models like the CGM and stochastic Hamilton-Jacobi equations have natural extremizers through their Hopf-Lax-Oleinik semi-groups, which share many of the properties of geodesics. For this reason and following the convention in the field, we will call all such paths geodesics.

Considerable effort has been devoted to understanding the geometric structure of semi-infinite geodesics in models of random growth. In the mathematical literature, this program was largely pioneered in the seminal work of Newman and co-authors \cite{New-95, Lic-New-96, How-New-97, How-New-01}, beginning with his paper in the 1994 Proceedings of the ICM \cite{New-95}. Under strong hypotheses on the curvature of the limit shape, that early work showed that all such geodesics must be asymptotically directed and that for Lebesgue-almost every fixed direction, from each site of the lattice, there exists a unique semi-infinite geodesic with that asymptotic direction and all these geodesics coalesce.  In special cases where the curvature  hypotheses are met, Newman's program was subsequently implemented in LPP models  \cite{Cat-Pim-11,Cat-Pim-12,Cat-Pim-13,Fer-Pim-05, Wut-02} and  certain stochastic Hamilton-Jacobi equations \cite{Bak-Li-19,Bak-16,Bak-Cat-Kha-14}. In all  the results of the last twenty-five years, the obstruction of needing to work on direction-dependent events of full probability  has been a persistent issue. A description of the overall geometric structure of semi-infinite geodesics has remained elusive. 

It is known that the picture described by these now-classical methods cannot be complete, because uniqueness fails for countably infinitely many random directions \cite{Geo-Ras-Sep-17-ptrf-2,Fer-Mar-Pim-09,Cou-11}. In the CGM, these special directions are the asymptotic directions of {\it competition interfaces}.    These  are dual lattice paths that separate geodesics rooted at a fixed site. Competition interface directions are distinguished by the existence of (at least)  two geodesics that emanate from the same site,  have  the same asymptotic direction, but  separate immediately in their first step. Once these two geodesics separate they never intersect again.  So in these directions  coalescence also fails. 

%Aside from this, essentially nothing else is known. 

Borrowing ideas from classical metric geometry, Newman introduced the tool of Busemann functions into the field in \cite{New-95}. In Newman's work, these Busemann functions are defined as directional limits of differences of metric distances or passage times. Following Newman's work and the subsequent seminal work of Hoffman in \cite{Hof-08}, Busemann functions have become a  principal tool for studying semi-infinite geodesics. The existence of the Busemann limits, however, relies on strong hypotheses on the limit shape.  Modern work primarily uses generalized Busemann functions, which exist without assumptions on the limit shape \cite{Dam-Han-14,Dam-Han-17,Geo-Ras-Sep-17-ptrf-1,Geo-Ras-Sep-17-ptrf-2,Ahl-Hof-16-}.

\subsection{Busemann measures} The present paper  introduces a new framework that relates geometric properties of geodesics to analytic properties of a measure-valued stochastic process called the {\it Busemann process} or {\it Busemann measures}. 
These Busemann measures are  Lebesgue-Stieltjes measures of generalized Busemann functions on the space of spatial directions, and  the Busemann process is the associated family of distribution functions.   This  approach enables a study of the entire family of semi-infinite geodesics on a single event of full probability. %This is the first time this has been achieved. 

We  describe, in terms of the supports of the Busemann measures, the random exceptional directions in which uniqueness or coalescence of geodesics fails. Many of these  results hold without further assumptions on the weight distribution. 
This work also identifies key hypotheses %on the Busemann process which 
that are  equivalent to desirable coalescence and uniqueness properties of geodesics. 
We expect that our methods will apply in related models including FPP and stochastic Hamilton-Jacobi equations.
%
%
%
%Subsequently, more analytical tools were brought to these models from subjects like integrable probability and representation theory and LPP played a central  role in the significant progress in the understanding of the KPZ class, 
%achieved over the last two decades; see the reviews \cite{Cor-12,Cor-16,Qua-12,Bor-Pet-14}.
%
%
%\textcolor{red}{Another important question concerns the geometry of the minimizing paths (maybe a quick general description of what a growth model is, so that it is clear what minimizing paths have to do with this?). The geometry of geodesics is in fact related to both the shape and fluctuation questions.  
%This is the subject of our paper. This program was spearheaded by Newman's seminal paper \cite{New-95}. For a long time the focus was on fixed directions. We are interested in completing the picture by studying all directions at once. And we in fact do complete the picture in the exponential case.  Then the rest of the intro...}
%\textcolor{red}{We bring classical objects like Poisson process and random walk as opposed to the KPZ non-classical objects}
 %
% In this model, the vertices of the lattice $\bbZ^2$ are populated by i.i.d.\ random weights. The passage time between two coordinatewise ordered vertices  is the maximal  sum of the weights collected by  an  admissible path between the two vertices. A precise definition appears in \eqref{G1} below.   Admissible paths are those that take only nearest-neighbor  steps up or to the right.  Maximizing paths   are called  geodesics.  These exist  trivially because there are only finitely many admissible paths  between any pair of  ordered vertices.  We restrict to the case where the weights have a continuous distribution so that the point-to-point geodesic is almost surely unique.   
%
% This model describes a randomly growing subset  of the lattice, and hence is  also known as  the {\it corner growth model}.  A fundamental result, which is stated carefully in \eqref{sh-th} below, is that  to leading order  this randomly growing  cluster  has a deterministic asymptotic shape.
%
%To simplify this introductory   discussion, consider the case where the limit shape is differentiable and strictly concave. This hypothesis holds in the model with exponential weights and is expected to hold generally. Under this regularity hypothesis, it is known \cite{Geo-Ras-Sep-17-ptrf-1,Geo-Ras-Sep-17-ptrf-2,Fer-Pim-05,Cou-11}  that all semi-infinite geodesics are asymptotically directed and that in  each fixed  direction   there is a unique semi-infinite geodesic 
%  from each lattice site,  and all these geodesics with the  same direction coalesce. See also \cite{Dam-Han-14,Dam-Han-17,Lic-New-96,How-New-01,New-95,Cat-Pim-11} for similar results in related models. 
%
%On the other hand, it is also known \cite{Geo-Ras-Sep-17-ptrf-2,Fer-Mar-Pim-09,Cou-11} that at least countably infinitely many directions exist where coalescence fails. These special directions are the asymptotic directions of competition interfaces, which are dual lattice paths that separate geodesics rooted at a fixed  site according to whether their first step is up or to the right. Competition interface directions are distinguished by the existence of (at least)  two different geodesics rooted at the same site, with the same asymptotic direction. %; because of this, in addition to coalescence not holding, we say that geodesic uniqueness fails in these directions.  
%%:
%Aside from this, essentially nothing else is known. Indeed, as far as we know, there are not even conjectures about the behavior of the model in the exceptional directions where coalescence fails. Nevertheless, natural questions abound: How many exceptional directions exist? Can coalescence of geodesics with the same asymptotic direction fail, but uniqueness still hold? For a given exceptional direction, how many disjoint semi-infinite geodesics with that asymptotic direction exist? What is the geometric structure of the graph of these geodesics?
%On the other hand, it is also known \cite{Geo-Ras-Sep-17-ptrf-2,Fer-Mar-Pim-09,Cou-11} that uniqueness fails for countably infinitely many directions. These special directions are the asymptotic directions of competition interfaces, which are dual lattice paths that separate geodesics rooted at a fixed  site according to whether their first step is up or to the right. Competition interface directions are distinguished by the existence of (at least)  two different geodesics emanating from the same site and having the same asymptotic direction. Once these two geodesics separate, they never intersect again. Hence, coalescence also fails. 
%Aside from this, essentially nothing else is known. 
%Nevertheless, natural questions abound: What is the size of the set of exceptional directions for which coalescence fails? In particular, can coalescence of geodesics with the same asymptotic direction fail, but uniqueness still hold? For a given exceptional direction, how many disjoint semi-infinite geodesics with that asymptotic direction exist? What is the geometric structure of the graph of these geodesics?
%As far as we know, there are not even conjectures about the answers to these questions.
%
%In the present paper, we introduce a new general framework that relates geometric properties of geodesics to analytic properties of a measure-valued stochastic process called the {\it Busemann process} or {\it Busemann measures}. 
%These Busemann measures are  Lebesgue-Stieltjes measures of Busemann functions on the space of spatial directions, with the Busemann process being the associated family of distribution functions.   Busemann functions themselves are limits of differences of passage times. They have become central objects in the study of first- and last-passage percolation since the pioneering work of Newman \cite{New-95} and Hoffman \cite{Hof-08}.   Busemann functions in growth models  are  analogues of the similarly named    objects  in metric geometry.
%The Busemann process is indexed by a parameter that encodes an asymptotic spatial  direction. 
 %The process is built from Busemann functions, which themselves are limits of differences of passage times, analogously to the objects with the same name in metric geometry.
%
%This approach  enables a study of the full family of semi-infinite geodesics on a single event of full probability for the first time. We can describe, in terms of the supports of the Busemann measures,  the random  exceptional directions in which uniqueness or coalescence of geodesics fails. Many of our results hold without further assumptions on the weight distribution,  but our work also identifies key hypotheses   under which desirable properties hold and  that merit further study.  

In the exactly solvable case with i.i.d.\ exponential weights, when the new results  are combined with previous work from   \cite{Cou-11, Fer-Pim-05, Geo-Ras-Sep-17-ptrf-2}, this yields  a complete characterization of the uniqueness and coalescence structure of all semi-infinite geodesics    on a single event of full probability.  Here is a  summary: 
\begin{enumerate}[label={\rm(\roman*)}, ref={\rm\roman*}]  \itemsep=3pt 
\item Every semi-infinite geodesic has an asymptotic direction.
\item 
 There exists a random countably infinite dense set of interior directions in which  there are {\it exactly two} geodesics  from each lattice site, a left geodesic and a right geodesic. These two  families of left and right geodesics can be constructed from the Busemann process.   Each family   forms a tree of coalescing geodesics.
  
  \item   In every other interior direction there is a unique geodesic from each lattice point, which again can be constructed from the Busemann process. In each such  direction these geodesics coalesce to form a tree. 
%Moreover, these families of semi-infinite geodesics which are built from the Busemann process are the only semi-infinite geodesics. 
\item\label{summary:v} The countable set of  directions of non-uniqueness is exactly  the set of asymptotic directions of competition interfaces 
from all lattice points, in addition to being the set of  discontinuity directions of the Busemann process.
\item In a direction $\xi$ of non-uniqueness, finite geodesics out of a site $x$ with endpoints going in direction $\xi$ converge to the left (resp.\ right) semi-infinite geodesic out of $x$ with asymptotic direction $\xi$ if and only if the endpoints eventually stay to the left (resp.\ right) 
of the competition interface rooted at the point where the left and right semi-infinite geodesics out of $x$ split.  
\item In a direction $\xi$ of uniqueness, finite geodesics out of a site $x$ with endpoints going in direction $\xi$ converge to the  semi-infinite geodesic out of $x$ with asymptotic direction $\xi$.
\end{enumerate}
This gives the first complete accounting of semi-infinite geodesics in a model which lies in the KPZ class.\smallskip

\subsection{Instability points} Passage times in LPP solve a variational problem  that is a   discrete version of the stochastic Burgers  Hopf-Lax-Oleinik semigroup.  
Through this connection, this paper  is also related  to the ergodic program for the %inviscid 
  stochastic Burgers equation  initiated by Sinai in \cite{Sin-92}. 
  As mentioned in point \eqref{summary:v} above, the exceptional directions in which coalescence fails correspond to directions at which the Busemann process has jump discontinuities.  % as a function of the asymptotic direction.  
  This means that the Cauchy problem at time $-\infty$ is not well-posed for certain initial conditions  that correspond to these exceptional directions. 
  In this case, it is reasonable to expect that solving the Cauchy problem with the initial condition given at time $t_0$ and sending $t_0\to-\infty$ gives multiple limits at 
  the space-time locations where the Busemann process has jump discontinuities. Thus we call these locations points of instability.
  %Thus, multiple semi-infinite optimal Lagrangian paths emanate from the spatial locations where the Busemann process has jump discontinuities. 
 %These locations then play the role of shocks in the present discrete setting.  
  In situations where the Cauchy problem is well-posed, points of instability correspond to shock locations. 
  The structure of shocks in connection with the Burgers program has been a major line of research \cite{E-etal-00,Bec-Kha-07,Bak-16}, with a conjectured relationship between shock statistics and the KPZ universality phenomenon (Bakhtin and Khanin \cite{Bak-Kha-18}). These conjectures are open. 
  
 % We study shocks in random exceptional directions, while \cite{E-etal-00,Bec-Kha-07,Bak-16,Bak-Kha-18} consider only fixed deterministic directions.  

%Our results are also connected to the ergodic program for the %inviscid 
%  stochastic Burgers equation  initiated by Sinai in \cite{Sin-92}. Passage times in LPP solve a variational problem  that is a   discrete version of a  Hopf-Lax-Oleinik semigroup.  In this interpretation, spatial locations where the Busemann process has jump discontinuities as a function of the asymptotic direction play the role of shocks.  The structure of shocks in connection with the Burgers program has been a major line of research \cite{E-etal-00,Bec-Kha-07,Bak-16}, with a conjectured relationship between shock statistics and the KPZ universality phenomenon (see Bakhtin and Khanin \cite{Bak-Kha-18}). These conjectures are entirely open. The shocks we study are associated to semi-infinite geodesics %(maximizers) 
%with asymptotic directions which are 
%exceptional in the sense that they are the directions in which coalescence fails. Those considered in \cite{E-etal-00,Bec-Kha-07,Bak-16,Bak-Kha-18} are for fixed directions.  


%In connection to the aforementioned dynamical systems point of view, 
%To the best of our knowledge, this is the first paper to consider the structure of shocks in exceptional directions. 
%\addmath{how to convey that we study things that happen a.s., but we are interested in exceptional directions because the picture is different there}


 Past works \cite{E-etal-00,Bec-Kha-07,Bak-16,Bak-Kha-18} considered shocks in  fixed deterministic directions, where the Cauchy problem at time $-\infty$ is shown to be well-posed almost surely and  these shocks are the only points of instability.  
 %We study instabilities in random exceptional directions.  
 %\textcolor{red}{point out here that for fixed directions, shocks are the only instabilities!}
  Our model is in a non-compact space setting, where these problems have been especially difficult to study. In exceptional directions, 
  points of instability turn out to have a markedly different structure from what has been seen previously in fixed directions.  Among the new phenomena are that points of instability form bi-infinite paths that both branch and coalesce. 
Bi-infinite shock paths have previously been observed only when  the space is compact  and the asymptotic direction is fixed. 
Branching shocks have not been observed.
%An example of the new phenomena we observe is that all shocks are bi-infinite in our setting. Existence of bi-infinite shocks has only previously been observed in compact space settings and for typical directions. 

 In the exponential model we  compute non-trivial  statistics of points of instability. 
 %This has not been achieved previously in a model of this type. 
 Among  our  results  is an unexpected connection with simple symmetric random walk: conditional on a $\xi$-directed path of instability points passing through the origin, the distribution of the locations of $\xi$-points of instability on the $x$-axis  %in the exponential model 
has the same law as the zero set of simple symmetric random walk sampled at even times. 

%\textcolor{red}{Do we want to mention that our shocks are bi-infinite, even though our setting is not compact, and that the shocks not only coalesce, but also branch out? could point fo Figure \ref{fig:shocks2b}.}

%In this paper, 
%\note{F: don't we want to give some examples of HOW we resolve some of these questions? I kind'a liked Timo's paragraph on this.}
%we resolve all of these questions and more in the exponential model and introduce tools which allow for the study of these and similar questions for general models. It is natural to expect that analogues of the tools we introduce also exist in related models like first passage percolation. The main idea of the present project is to relate analytic questions about regularity of the stochastic process of Busemann process as a function of the direction to geometric properties of geodesics. As will be seen in the sequel, most of our results are equivalences, showing the intimate connection between geometric properties of geodesics and analytic properties of the Busemann process.

%\fixtext{C: There will be something about it, but I think that's going to be the hardest part of the intro to write well.}
%\textcolor{red}{F: I still think we should mention the web of shocks in the intro. Also, previous work needs to be mentioned... }

%To add:
%Clean up the geodesics stuff
%Something about shocks.
%Identification with the zero set of simple symmetric random walk. We are able to compute some non-trivial statistics of shocks, which suggest a tantalizing Brownian connection in the scaling limit. In particular, we show that conditional on having a shock line crossing the horizontal line at zero, the other locations where shocks cross the horizontal line have the same law as the zero set of simple symmetric random walk. This is a particularly striking result, as previous


%\subsection{Geodesics and Busemann functions}  We study directed last-passage percolation (LPP) with nearest-neighbor steps  on the planar square lattice $\Z^2$.  
%



%In the general LPP model, we give an exact characterization of when it is possible for there to exist geodesics rooted at sites $x$ and $y$ with the same asymptotic direction which either do not coalesce or do not intersect, in terms of the Busemann process.  
%It is natural to expect that the same structure as is studied here appears in related models like first passage percolation, where all  the necessary ingredients are  present.

%\textcolor{red}{Mention something about shocks.. Some text is below.. Maybe the long version should have an appendix about shocks in PDE etc (at least eventually, not necessarily in v1 that we want to post soon).}

%\subsection{Organization of the paper} 

%\timonote{Below the old text.  Cover up as soon as what's valuable for now has been extracted.}  

%introduce the acronym LPP

%mention that the general results should extend to the FPP case because all the structure is there already. 
%we work with LPP because it has a solvable model and therefore we can go much further.
%mention that Coupier's results are for rooted things

%mention that the equivalence of the Busemann process being a jump process and coalescence of $\pm$ geodesics gives a new technique of proving coalescence.  for a fixed direction, this gives a new proof of coalescence.  but this gives more: a route to classifying the whole coalescence business for all directions at once.\bigskip

%\textcolor{red}{About shocks:} I could not work out the analogue of the energy dissipation argument in LPP. The main issue is that I am not sure how to define a solution out of the $\B{\xi\pm}$ for which the $\B{\xi\pm}$ would be giving the SPATIAL left- and right-limits. We cannot take spatial limits in a discrete space!!  
%BUT, here are a few points in favor of still calling the red points ``unstable shocks'':\bigskip

%1. The objects that seem to still be present in the discrete setting are the semi-infinite geodesics (the minimizers of the HLO variational formula). 
%This is in fact the way Yura defines shocks: first one defines a semi-infinite minimizer out of every (deterministic) point and then uses monotonicity to define leftmost and rightmost paths out of every point.  The exceptional space points that have different leftmost and rightmost paths are shocks. 

%This construction is for a fixed direction AND it does not make sense in a discrete-space setting.  In our setting, we do get though leftmost and rightmost minimizers by squeezing. These are precisely the $\xi\pm$ geodesics.  The advantage of doing things this way is that this works both in discrete and continuous spaces.  Note one subtlety though in the continuous space setting: there are two things that may happen.   If $\B{\xi\pm}$ are different, we get two different leftmost and rightmost geodesics and hence we get a shock.  But it may happen that at some (exceptional) points $\B{\xi\pm}$ match and yet we have two different leftmost and rightmost geodesics!  (I expect this will happen in a zero temperature setting, where it may happen that $\B{\xi+}=\B{\xi-}$ but they are discontinuous at some [random] points.)    So the red graph is a graph of shocks, but not all shocks are in the red graph!      This does not happen in the discrete case, since there is not enough space to get the other kinds of shocks (no multiple geodesics, if $\B{\xi\pm}$ match.)

%The difference between the red graph shocks and the other kind of shocks is their stability.  I presume that again the set $\aUset$ will be countable and dense. We will see the red graph type shocks only for $\xi\in\aUset$. But the other type of shocks should be present for all $\xi\in\ri\Uset$ (in zero temperature, and should not occur for any $\xi$, in positive temperature). My guess is that this second type of shocks does not have bi-infinite paths and it may even be the case that there is continuity in $\xi$ for these paths.   If so, then these are stable shocks while the red graph gives unstable shocks.

%We won't have to do any speculation about the other type of shocks in LPP since they do not occur in the discrete space setting. So we can just justify how the red graph disappears and reappears as you move $\xi$ and call our shocks unstable, leaving out that there are probably also stable shocks in the continuum setting.\medskip

%I should say that our red points are unstable shocks in the above sense if you add to the above the fact that characteristics and minimizers should really live on dual path spaces (in PDEs one solves an initial condition problem and the other a terminal condition problem, and so one can construct one from the other by a similar path duality to the one Timo has in his paper).\bigskip    

%2. In the PDE setting, assuming things are bounded and smooth enough, plugging in the leftmost and rightmost minimizers into the action, at a shock point, will produce the left- and right-limits $u(t,x\pm)$. Since our $\B{\xi\pm}$ do come from the leftmost and rightmost $\xi\pm$ geodesics, which we just said play the roles of leftmost and rightmost minimizers, we can think of them as the analogues of the SPATIAL left- and right-limits.  But then our red points ARE shocks because they are the points of discontinuity of the gradients.\bigskip

%{\bf Note:} That subtlety about the two different types of shocks does actually show up in the discrete space case too when one tries to work out the energy dissipation business:  it seems that even in the fixed direction case, the points where the dual graphs coalesce dissipate kinetic energy.  So in principle they should be considered shock points. The same happens even for the exceptional $\xi$'s.   Points $x^*$ that are not red and such that $x^*+e_1$ and $x^*+e_2$ both point to $x^*$ in the dual graph do seem to dissipate kinetic energy. They seem to belong to the ``stable shocks.''   But this argument is incomplete because like I said above, I cannot figure out how to work out the energy dissipation business when we have two different $\B{\xi\pm}$.
%\subsection{Previous work}
%\textcolor{red}{Still need text here. What works do we want to mention??}

%\subsection{Instructions for reading the paper} We state many almost sure results by naming full-probability events $\Omega^i_j$  on which the claimed properties hold.  The  reader need not try to keep track of these events, except  to follow the proofs to the letter.  The only important distinction is that when there is a separate full-probability event for each spatial direction $\xi$, the event is denoted by $\Omega^i_\xi$.  


\subsection{Organization of the paper}
%Section \ref{sec:busgeo} summarize  currently known results on Busemann functions and existence, uniqueness and coalescence of geodesics.  
%Section \ref{s:Bmeas} introduces Busemann measures and studies their relationship with the geometry of semi-infinite geodesics. 
%The outline of the paper is as follows. 
Section \ref{sec:busgeo} defines the model and summarizes the currently known results  on Busemann functions and existence, uniqueness, and coalescence of geodesics.
Section \ref{s:Bmeas}  contains  our main results on Busemann measures and the geometry of geodesics for general weight distributions.  Section \ref{sec:LPPDS}  connects  our general results to dynamical systems and studies
the web of instability  defined by the discontinuities of the Busemann process. Section \ref{sec:exp} specializes to the  exponential case  to compute non-trivial statistics of the Busemann process.  Proofs come  in Sections \ref{sec:bus}--\ref{sec:exp-pf}, with some auxiliary results relegated to  Appendices \ref{a:aux}--\ref{a:RW}.  Appendix \ref{app:busgeo} collects the inputs we need from previous work.

\subsection{Setting and notation} \label{sub:setting}
Throughout this paper, $(\Omega, \sF,\bbP)$ is a Polish probability space equipped with a group $T=\{T_x\}_{x\in\Z^2}$ of $\sF$-measurable $\bbP$-preserving bijections $T_x:\Omega\to\Omega$
%,  $x\in\bbZ^2$, 
such that $T_0=$ identity and  $T_xT_y=T_{x+y}$.
% for all $x,y\in\bbZ^2$. 
%Let $T$ denote the collection $\{T_x:x\in\Z^2\}$. 
$\bbE$ is expectation relative to $\bbP$.
A generic point in this space is denoted by $\w \in \Omega$. We assume that there exists a family $\{\w_x(\w) : x \in \bbZ^2\}$ of real-valued random variables called {\it weights} such that  
	\begin{align}\label{main-assump}
	\begin{split}
	&\text{$\{\w_x\}$ are i.i.d.\ with a continuous distribution under $\bbP$,  $\Var(\w_0)>0$,}\\[-2.5pt]
	&\text{and $\exists p>2$\,: $\bbE[\abs{\w_0}^p] < \infty$.}
	\end{split}
	\end{align}
%$\{\w_x\}$ are i.i.d.\ under $\bbP$, $\Var(\w_0)>0$, and $\exists p>2$\,: $\bbE[\abs{\w_0}^p] < \infty$.
We require further that  $\w_y(T_x \w) = \w_{x+y}(\w)$ for all $x,y \in \bbZ^2$.   $\P_0$  denotes the marginal distribution of $\{\w_x:x\in\Z^2\}$ under $\P$.   
Continuous distribution means that  $\P_0(X\le r)$ is a continuous function of $r\in\R$.   $X\sim\text{ Exp}(\alpha)$ means that the random variable $X$ satisfies $P(X>t)=e^{-\alpha t}$ for $t>0$ (rate $\alpha$ exponential distribution). 

The canonical setting is the one where $\Omega=\R^{\Z^2}$ is endowed with the product topology, Borel $\sigma$-algebra $\sF$, and the natural shifts, $\w_x$ are the coordinate projections, and $\P=\P_0$ is a product shift-invariant measure.

The standard basis vectors of $\bbR^2$ are  $e_1= e_+ = (1,0)$ and $e_2=e_-=(0,1)$. The $e_\pm$ notation will   conveniently  shorten some statements.  
Additional special vectors are   $\et = e_1 + e_2$, $\etstar=\et/2$, $\ex=e_2-e_1$, and $\exstar=\ex/2$.  In the dynamical view of LPP,  $\et$ is the  time coordinate and  $\ex$  the  space coordinate.  See Figure \ref{fig:evecs}.
%of  a right-handed coordinate system.  
The spatial  level at time  $t\in \bbZ$ is denoted by  $\level_t = \{x \in \bbZ^2 : x \cdot \et = t\}$.     The half-vectors $\etstar$ and $\exstar$ connect   $\Z^2$  with its dual lattice $\Z^{2*}=\etstar+\Z^2$.

\begin{figure}[h]
 	\begin{center}
 		 \begin{tikzpicture}[scale=1,>=stealth]
%			\draw[line width=1.5pt,->](0,0)--(0,1);		 
%			\draw[line width=1.5pt,->](0,0)--(1,0);		 
%			\draw[line width=1.5pt,->](.03,-.03)--(1.03,.97);		 
%			\draw[line width=1.5pt,->](-.03,.03)--(.47,.53);		 
%			\draw[line width=1.5pt,->](-.03,-.03)--(-1.03,.97);		 
%			\draw[line width=1.5pt,->](.03,.03)--(-0.47,0.53);		 
%			\draw[fill=black](0,0) circle(3pt);
			\begin{scope}
			\draw(0,-0.5)--(0,1.5);
			\draw(1,-0.5)--(1,1.5);
			\draw(-1,-0.5)--(-1,1.5);
			\draw(-1.5,0)--(1.5,0);
			\draw(-1.5,1)--(1.5,1);
			\draw[line width=1.5pt,->](0,0)--(0,1);		 
			\draw(0.2,1)node[above]{\small$e_2=e_-$};
			\draw[line width=1.5pt,->](0,0)--(1,0);		 
			\draw(1.65,0)node[above]{\small$e_1=e_+$};
			\draw[line width=1.5pt,->](0,0)--(1,1);		 
			\draw(1.2,1)node[above]{\small$\et$};
			\draw[line width=1.5pt,->](0,0)--(-1,1);		 
			\draw(-1.2,1)node[above]{\small$\ex$};
			\draw[fill=black](0,0) circle(3pt);
			\draw(0,-.2)node[left]{\small$0$};
			\end{scope}

			\begin{scope}[shift={(4,0)}]
			\draw(0,-0.5)--(0,1.5);
			\draw(1,-0.5)--(1,1.5);
			\draw(-1,-0.5)--(-1,1.5);
			\draw(-1.5,0)--(1.5,0);
			\draw(-1.5,1)--(1.5,1);
			\draw[dashed](-1.5,0.5)--(1.5,0.5);
			\draw[dashed](-.5,-0.5)--(-.5,1.5);
			\draw[dashed](.5,-0.5)--(.5,1.5);
			\draw[line width=1.5pt,->](0,0)--(0.5,0.5);		 
			\draw(0.8,0.5)node[above]{\small$\etstar$};
			\draw[line width=1.5pt,->](0,0)--(-0.5,0.5);		 
			\draw(-0.7,0.5)node[above]{\small$\exstar$};
			\draw[fill=black](0,0) circle(3pt);
			\draw(0,-.2)node[left]{\small$0$};
			\end{scope}
			
			\begin{scope}[shift={(7,0)}]
			\draw(0,-0.5)--(0,1.5);
			\draw(1,-0.5)--(1,1.5);
			\draw(-.5,0)--(1.5,0);
			\draw(-.5,1)--(1.5,1);
			\draw[line width=1.5pt](1,0)--(0,1);
			\draw(0.7,0.7)node{\small$\Uset$};
			\draw[fill=black](0,0) circle(3pt);
			\draw(0,-.2)node[left]{\small$0$};
			\draw(0.2,1)node[above]{\small$e_2$};
			\draw(1.2,0)node[above]{\small$e_1$};
			\end{scope}
			
		\end{tikzpicture}
 	 \end{center}
 	\caption{\small  An illustration of the  vectors $e_1$, $e_2$, $e_{\pm}$, $\et$, $\ex$, $\etstar$,  $\exstar$, and the set $\Uset$. The dashed lines in the middle plot are edges of the dual lattice $\Z^{2*}=\bbZ^2+\etstar$.}
 \label{fig:evecs}
 \end{figure}



A statement with $\pm$ and possibly also $\mp$  is a conjunction of two statements: one for the top signs, and another one for the bottom signs.  We employ $\sigg$ to represent an arbitrary element of $\{-,+\}$.

% To avoid confusion with such statements we also employ the notational convention that $\sigg$ is an element of $\{-,+\}$. %,and 
%\note{looks like we never need the opposite sign.}
%if the opposite sign is needed in the same statement, it is denoted by $\giss$.

%${\scaleobj{0.5}{\boxminus}}$ 

 %   $\boxempty$    $\ovoid$ 


We  use  $\R_+=[0,\infty)$, $\Z_+=\Z\cap\R_+$  and $\N=\{1,2,3,\dotsc\}$.   For $x,y\in\R^2$, inequalities such as $x\le y$ and $x< y$, 
and operations such as $x\wedge y=\min(x,y)$ and $x\vee y=\max(x,y)$
are understood coordinatewise.  (In particular, $x<y$ means $x\cdot e_i<y\cdot e_i$ for both $i=1,2$.)  For $x\le y$ in $\Z^2$, $\lzb x, y\rzb$ denotes the rectangle $\{z\in\Z^2:x\le z\le y\}$. 
For integers $i\le j$, $\lzb i,j\rzb$ denotes the interval $[i,j]\cap\Z$.  For $m\le n$ in $\Z\cup\{-\infty,\infty\}$ we denote a sequence $\{a_i:m\le i\le n\}$ by $a_{m,n}$. 

A path $\geod{m,n}$ in $\bbZ^2$ with $\geod{i+1}- \geod{i} \in \{e_1,e_2\}$ for all $i$ is called an {\it up-right} path. 
Throughout, paths are indexed so that $\geod{k}\cdot\et=k$.


For vectors $\zeta,\eta \in \bbR^2$, denote  open and closed line segments by  $]\zeta,\eta[\, = \{t\zeta + (1-t)\eta : 0 < t < 1\}$ and  $[\zeta,\eta] = \{t \zeta + (1-t) \eta : 0 \leq t \leq 1\}$, with the consistent definitions for  $]\zeta,\eta]$ and $[\zeta,\eta[$.   $\Uset = [e_2,e_1]$ with  relative interior $\ri \Uset = ]e_2,e_1[$. See Figure \ref{fig:evecs}. A left-to-right ordering of points $\zeta,\eta\in\R^2$ with $\zeta\cdot\et=\eta\cdot\et$ is defined by $\zeta \prec \eta$ if $\zeta \cdot e_1 < \eta \cdot e_1$ and $\zeta \preceq \eta$ if $\zeta \cdot e_1  \leq \eta \cdot e_1$.   This leads to notions of left and right limits: if  $\zeta_n \to \xi$ in $\Uset$, then $\zeta_n \nearrow \xi$ if $\zeta_n \prec \zeta_{n+1}$ for all $n$, while $\zeta_n \searrow \xi$ if $\zeta_{n+1} \prec \zeta_n$  for all $n$. 
%Given a sequence $\zeta_n \in \Uset$, we say that $\zeta_n \nearrow \xi$ if $\zeta_n \prec \zeta_{n+1}$ for all $n$ and $\zeta_n \to \xi$ as $n\to\infty$. Similarly, given a sequence $\eta_n \in \Uset$, we say $\eta_n \searrow \xi$ if $\eta_{n+1} \prec \eta_n$ for all $n$ and $\eta_n \to \xi$ as $n \to \infty$. 


The support $\supp\mu$ of a signed Borel measure $\mu$  is the smallest closed set whose complement has zero measure under the total variation measure $\abs\mu$.   
%Let $\bbX$ be a topological space equipped with the Borel $\sigma$-algebra and let $\mu$ be a non-negative Borel measure on $\bbX$. The support of $\mu$ is a closed subset of $\bbX$ and is denoted by $\supp \mu$. It is the set of points $x \in \bbX$ with the property that every open set $O$ with $x \in O$ has $\mu(O) >0$. If $\mu$ is a non-positive measure, then the support of $\mu$ is defined to be $\supp (-\mu)$ in the sense just described. 
%
%If $\mu$ is a signed measure on a measurable space $(\bbX,\cX)$, the total variation measure of $\mu$ is a positive measure on $(\bbX,\cX)$, which we denote by $|\mu|$. It is defined by $|\mu|(A) = \sup \sum_i |\mu(A_i)|$, where the supremum is over countable measurable partitions $\{A_i\} \subset \bbX$ of $A$. 
\medskip



==> JEMS Post-Accept Revision/GeoWebPaper-Sec2.tex <==
% !TEX root = GeoWebPaper.tex

%\section{The geometry of geodesics: known results}\label{sec:busgeo}
\section{Preliminaries on last-passage percolation}\label{sec:busgeo}

This section introduces   the background required for the main results in Sections \ref{s:Bmeas}--\ref{sec:exp}.  To avoid excessive technical detail at this point,  precise  statements of  previous  results needed for the proofs later in the paper  are deferred to Appendix \ref{app:busgeo}.  


\subsection{The shape function} \label{s:shape} 
Recall the assumption \eqref{main-assump}.
For $x \leq y$ in $\bbZ^2$ satisfying $x \cdot \et = k$ and $y \cdot \et = m$,  denote by $\Pi_x^y$ the collection of up-right paths $\geod{k,m}$ which satisfy $\geod{k} = x$ and $\geod{m} = y$. 
The {\it last-passage time} from $x$ to $y$ is defined by 
\be\label{G1} 
G_{x,y} = G(x,y)=\max_{\geod{k,m} \in \Pi_x^y} \sum_{i=k}^{m-1} \w_{\geod{i}}. 
\ee
A maximizing path is called a (point-to-point or finite) {\it geodesic} and denoted by $\gamma^{x,y}$.
%A geodesic is a path $\geod{k,m} \in \Pi_x^y$ with the property that 
%\begin{align*}
%G_{x,y} &= \sum_{i=k}^{m} \w_{\geo{i}{}{}}. 
%\end{align*}
%Geodesics between sites $x \in \bbZ^2$ and $y\in \bbZ^2$ satisfying $x \leq y$ always exist since there are only finitely many such paths. 
%The hypothesis that the weights are continuous implies that there is a event of full probability on which all (finite) geodesics are unique. 
Under the i.i.d.\ continuous distribution assumption \eqref{main-assump},  $\gamma^{x,y}$   is almost surely  unique. 

%\subsection{The shape function}
The shape theorem \cite{Mar-04} says there exists a non-random  function $\gpp:\bbR_+^2 \to \bbR$ such that with probability one
\be\label{sh-th} 
\lim_{n\to\infty} \;\max_{x\, \in \,\bbZ^2_+ : \, |x|_1 = n} \frac{\abs{G_{0,x} - \gpp(x)}}{n} = 0.
\ee
This {\it shape function} $\gpp$  is symmetric, concave, and homogeneous of degree one. By homogeneity, $\gpp$  is determined by its values on $\Uset$. 
%For $\xi \in \bbR_+^2$,   the superdifferential of $g$ at $\xi$ is %the set 
%\begin{align*}
%\partial \gpp(\xi) &= \{h \in \bbR^2 : \forall \zeta \in \bbR_+^2, \, \gpp(\zeta) \le   \gpp(\xi) + h \cdot (\zeta-\xi)\}.
%\end{align*}
%A quick computation checks that if $h \in \partial \gpp(\xi)$ then $h\cdot\xi = \gpp(\xi)$. See \cite[Lemma 2.1]{Jan-Ras-18-arxiv}.
%
%Differentiability of $\gpp$ at $\xi$ is equivalent to $|\partial \gpp(\xi)| = 1$ \cite[Theorem 25.2]{Roc-70}. In this case, $\partial \gpp(\xi) = \{\nabla \gpp(\xi)\}$. 
%We introduce the image of $\Uset$ under the superdifferential map
%\begin{align*}
%\partial \gpp (\Uset) &= \{h \in \bbR^2 : \exists \xi \in \Uset :h \in \partial \gpp(\xi)\}
%\end{align*}
Concavity implies the existence of one-sided derivatives:
\begin{align*}
\nabla \gpp(\xi \pm) \cdot e_1 = \lim_{\e \searrow 0} \frac{\gpp(\xi \pm \e e_1) - \gpp(\xi)}{\pm \e} \qquad{ and }\qquad \nabla \gpp(\xi \pm) \cdot e_2 = \lim_{\e \searrow 0} \frac{\gpp(\xi \mp \e e_2) - \gpp(\xi)}{\mp \e}.
\end{align*}
By \cite[Lemma 4.7(c)]{Jan-Ras-18-arxiv} 
%these are the two extreme points of the convex set $\partial \gpp(\xi).$ Therefore 
differentiability of $\gpp$ at $\xi\in\ri\Uset$ is the same as $\nabla \gpp(\xi+) = \nabla \gpp(\xi -)$.
Denote the directions of differentiability by
\be\label{df:D} %\begin{align*}
\Diff = \{\xi \in \ri \sU : \gpp \text{ is differentiable at }\xi\}.
\ee%\end{align*}

For $\xi \in \ri \Uset$,  define the maximal linear segments of $g$ with slopes given by  the    right $(\sigg=+)$ and the  left $(\sigg=-)$ derivatives of $g$ at $\xi$  to be
\begin{align*}
\Uset_{\xi\sig} = \bigl\{\zeta \in \ri\Uset : \gpp(\zeta) - \gpp(\xi) = \nabla \gpp(\xi\sigg) \cdot (\zeta - \xi)\bigr\},\quad\sigg\in\{-,+\}. 
\end{align*}
%It is possible that either or both of these sets can degenerate to a point. 
We say $g$ is {\it strictly concave} at $\xi\in\ri\Uset$ if $\Uset_{\xi-}=\Uset_{\xi+}=\{\xi\}$.  Geometrically this means that $\xi$ does not lie on a nondegenerate closed linear segment of $\gpp$. 
The usual notion of strict concavity on an open  subinterval of $\Uset$ is the same as having this pointwise 
strict concavity at   all $\xi$ in the interval.

\begin{figure}[h]
\begin{center}
\begin{tikzpicture}[>=latex,scale=1]
\begin{scope}
\draw[line width=1pt] (-1.19,0.6)--(1.19,1.2);
\draw[ line width=0.5pt,dashed](0,0.89)--(0,0);
\draw(0,-.25)node{$\xi$};
\end{scope}
\begin{scope}[shift={(3,0)}]
\draw[line width=1pt] (-1.19,0)--(0,1.2)--(1.19,0);
\draw[ line width=0.5pt,dashed](0,1.19)--(0,0);
\draw(0,-.25)node{$\xi$};
\end{scope}
\begin{scope}[shift={(6,0)}]
\draw[line width=1pt] (-1.19,0)--(0.01,1.2);
\draw[line width=1pt] (1.19,0) arc (20:70:2cm);
\draw[ line width=0.5pt,dashed](0.01,1.2)--(0.01,0);
\draw(0,-.25)node{$\xi$};
\end{scope}
 \begin{scope}[shift={(9,0)}]
\draw[line width=1pt] (1.19,0) arc (20:70:2cm);
\draw[line width=1pt] (-1.19,0) arc (160:110:2cm);
\draw[ line width=0.5pt,dashed](0,1.2)--(0,0);
\draw(0,-.25)node{$\xi$};
\end{scope}
\begin{scope}[shift={(11.5,0)}]
\draw[line width=1pt] (2,0) arc (10:170:1.35cm);
\draw[ line width=0.5pt,dashed](0.65,1.13)--(0.65,0);
\draw(0.7,-.25)node{$\xi$};
\end{scope}
\end{tikzpicture}
\end{center}
\caption{\small   In the first three graphs $\gpp$ is not strictly concave at $\xi$ while in the last two it is.}
\label{fig:conc} \end{figure}

For a given $\xi\in\ri\Uset$, let $\ximin\preceq\ximax$ denote the endpoints of the (possibly degenerate) interval 
\begin{align*}
\Uset_{\xi} &= \Uset_{\xi-} \cup \Uset_{\xi +} = [\hspace{0.5pt}\ximin,\ximax\hspace{0.8pt}].  
\end{align*}
%Martin's shape function asymptotic  at the boundary \cite[Theorem 2.4]{Mar-04} implies that $\gpp$  is not   linear on any nondegenerate interval with one endpoint $e_i$. Thus we set  $\Uset_{e_i} = \{e_i\}$ for $i \in \{1,2\}$.   
If $\xi\in\Diff$ then $\Uset_{\xi-}=\Uset_{\xi+}=\Uset_{\xi}$ while if $\xi\notin\Diff$ then $\Uset_{\xi-}\cap\,\Uset_{\xi+}=\{\xi\}$. Set $\Uset_{e_i}=\{e_i\}$, for $i\in\{1,2\}$.\smallskip

Additional control over the geometry of geodesics is provided by this regularity condition:
%\begin{condition}\label{g-reg}
\begin{align}\label{g-reg}
\begin{split}
&\text{The shape function $\gpp$ is strictly concave at all $\xi\notin\Diff$ or, equivalently, $\gpp$ is differentiable}\\[-2.5pt]
&\text{at the endpoints of its linear segments.}
\end{split}
\end{align}
%\end{condition}

Condition \eqref{g-reg} holds obviously  if $\gpp$ is either differentiable or strictly concave. Both of these latter properties are true  for exponential  weights   and are conjectured to be valid more generally for continuously distributed  weights. Under % the regularity condition 
\eqref{g-reg},   if both $ \Uset_{\xi-}$  and $\Uset_{\xi +}$ are nondegenerate intervals,  then   $ \Uset_{\xi-}=\Uset_{\xi +}=\Uset_{\xi}$ (leftmost graph in Figure \ref{fig:conc}). 

%\textcolor{red}{Mention that the only known model that satisfies condition \eqref{g-reg} and continuous weights is the exponential one, and give the formula for the shape. Also mention that we will be explicit whenever a result requires this condition. And that this condition is conjectured to be always the case, under e.g.\ continuous weights.}



\subsection{The Busemann process}
%\subsection{The Busemann process, semi-infinite geodesics and competition interfaces}
\label{sec:bus-brief}
Under regularity condition \eqref{g-reg}, it is known that for each fixed 
$\xi \in \Diff$     %CHANGED HERE
 and $x,y \in \bbZ^2$, there is a $\xi$-dependent event of full probability on which the limit
\begin{align}
\B{\xi}(x,y) = \lim_{n\to\infty} (G_{x,v_n} - G_{y,v_n})  \label{eq:Busfn}
\end{align}
exists and agrees for all sequences $v_n \in \bbZ^2$ such that $\abs{v_n}\to\infty$ and  $v_n/n \to \xi$.  Similar  limits appear in metric geometry under the name of {\it Busemann functions}.

The goal of this paper  is to  study the LPP model  without a priori hypotheses on the shape function.  Hence  the  limit in \eqref{eq:Busfn} cannot serve as a starting point. Instead we work with a stochastic process of {\it generalized} Busemann functions, indexed by $\xi \in \ri \Uset$,  constructed through a weak limit procedure on an extended probability space. See Remark \ref{rmk:weak-lim} for a brief discussion of the construction of this process in \cite{Jan-Ras-20-aop}, which is based in part on ideas from \cite{Dam-Han-14, Geo-Ras-Sep-17-ptrf-1}. This  process agrees with  \eqref{eq:Busfn} when the limit in  \eqref{eq:Busfn}  exists. 
% and has many  properties   implied by \eqref{eq:Busfn} even when  the limit does not exist. % Theorem \ref{thm:Bus}  in Appendix \ref{app:busgeo} collects these properties. In particular, it shows that there

The construction in \cite{Jan-Ras-20-aop} produces  a probability space  $(\Omega, \sF, \bbP)$ with a group of shifts $T =\{T_x : x \in \bbZ^2\}$ that satisfies  the requirements of Section \ref{sub:setting} and a stochastic process  $\bigl\{\B{\xi\sigg}(x,y): x,y \in \bbZ^2,\, \xi \in \ri \Uset, \,\sigg \in \{-,+\}\bigr\}$ on $\Omega$, which we   call the {\it Busemann process}. We record here those properties of this process that  are needed for Sections \ref{s:Bmeas}--\ref{sec:exp}. 
% understanding our results in Sections \ref{s:Bmeas}--\ref{sec:exp}  and leave the rest to the appendix. 

In general, there is a $T$-invariant full probability  event on which the following hold. For all $\xi \in \ri \Uset$, $x,y,z \in \bbZ^2$, and $\sigg \in \{-,+\}$:
 \begin{align}
	&\B{\xi\sig}(x+z,y+z,\w)=\B{\xi\sig}(x,y,T_z\w),\label{cov-prop}\\
	&\B{\xi\sig}(x,y,\w)+\B{\xi\sig}(y,z,\w)=\B{\xi\sig}(x,z,\w),\label{coc-prop}\\
	&\min\bigl\{\B{\xi\sig}(x,x+e_1,\w),\B{\xi\sig}(x,x+e_2,\w)\bigr\}=\w_x,\quad\text{and}\label{rec-prop2}\\
	&\E\bigl[ \B{\xi\sig}(x,x+e_i)\bigr] = \nabla\gpp(\xi\sigg)\cdot e_i.\label{E[h(B)]}
\end{align}

Properties \eqref{cov-prop}--\eqref{coc-prop} express that each $\B{\xi\sig}$ is a {\it covariant cocycle}.   The {\it weights recovery} property \eqref{rec-prop2}  is the key  that relates these cocycles to the LPP process. 
 \eqref{E[h(B)]} shows that the Busemann process is naturally parametrized by the superdifferential of the shape function $\gpp$.
 The following monotonicity  is inherited from the path structure: for all $x \in \bbZ^2$ and $\xi,\xi' \in \ri\Uset$ with $\xi\prec\xi'$,
\begin{align}\label{mono}
\begin{split}
&\B{\xi-}(x,x+e_1,\w) \ge \B{\xi+}(x,x+e_1,\w)\ge \B{\xi'-}(x,x+e_1,\w)\ge \B{\xi'+}(x,x+e_1,\w)\quad\text{and} \\
&\B{\xi-}(x,x+e_2,\w) \le \B{\xi+}(x,x+e_2,\w)\le \B{\xi'-}(x,x+e_2,\w)\le \B{\xi'+}(x,x+e_2,\w).
\end{split}
\end{align} 
%All of these properties are elementary when the limit \eqref{eq:Busfn} exists.

As a consequence of monotonicity and the cocycle property \eqref{coc-prop}, left and right limits exist. The signs in $\B{\xi\pm}$   correspond to   left and  right continuity: for all $x,y \in \bbZ^2$,   $\xi \in \ri \Uset$, and  $\sigg \in \{-,+\}$, 
	\begin{align}\label{Busemann-limits}
	\begin{split}
	\B{\xi-}(x,y,\w)=\lim_{\ri\Uset\,\ni\, \zeta \nearrow \xi}\B{\zeta\sig}(x,y,\w)\quad\text{and}\quad
	\B{\xi+}(x,y,\w)=\lim_{\substack{\ri\Uset\,\ni\,\zeta \searrow \xi}}\B{\zeta\sig}(x,y,\w).
	\end{split}
	\end{align}
When $\B{\xi+}(x,y,\w)=\B{\xi-}(x,y,\w)$ we drop the $+/-$ distinction and 
write $\B{\xi}(x,y,\w)$.


%We will work on the probability space constructed in Theorem \ref{thm:Bus} and so the 
%The standing assumption for the rest of the paper will be the following:
%	\begin{assumption}\label{main-assump}
%%	\text{Assume the setting of Theorem \ref{thm:Bus} and that $\P(\w_0\le r)$ is continuous in $r$.}
%	  $\P_0$ is a probability measure on $\R^{\Z^2}$ under which the coordinate projections are i.i.d.\ with a positive variance, $p>2$ finite moments, and a continuous distribution, i.e.\ $\P_0(\w_0\le r)$ 
%	is continuous in $r$.    The processes $\{\w_x:x\in\Z^2\}$ and $\{\B{\xi\sig}(x,y):x,y\in\Z^2, \sigg\in\{-,+\}, \xi \in \ri \Uset\}$ are defined on the measure-preserving system $(\Omega,\sF,\bbP,T)$ with properties \eqref{cov-prop}--\eqref{Busemann-limits} above, and $\{\w_x\}$ has distribution $\P_0$. 
%	%  $(\Omega,\sF,\bbP,T)$, $\{\w_x:x\in\Z^2\}$, and $\{\B{\xi\sig}(x,y):x,y\in\Z^2, \sigg\in\{-,+\}, \xi \in \ri \Uset\}$   are as constructed in Theorem \ref{thm:Bus}.
%	\end{assumption}

Theorem \ref{thm:Bus}  in Appendix \ref{app:busgeo} contains the complete list of the properties of the Busemann process that  are  used in the proofs in Sections \ref{sec:bus}--\ref{sec:webpf}. 

\subsection{Semi-infinite geodesics}\label{sec:geod-brief}

A path $\geod{k,\infty}$ with $\geod{i+1}- \geod{i} \in \{e_1,e_2\}$ for all $i\ge k$ is called a {\it semi-infinite geodesic emanating from, or rooted at}, $x$ if $\geod{k}=x$ and for any $m,n \in \bbZ_+$ with $k\le m \leq n$, the restricted path $\geod{m,n}$ is a geodesic between $\geod{m}$ and $\geod{n}$.  A path $\geod{-\infty,\infty}$ with $\geod{i+1}- \geod{i} \in \{e_1,e_2\}$ for all $i$ is called a {\it bi-infinite geodesic} if $\geod{m,n}$ is a geodesic for any $m\le n$ in $\Z$.
Due to the fact that the set of admissible steps is $\{e_1,e_2\}$, from each site $x$,  there are always two trivial semi-infinite geodesics, namely $x+\Z_+ e_1$, which we denote by $\geo{}{x}{e_1}$, and $x+\Z_+ e_2$, which we denote by $\geo{}{x}{e_2}$. There are two trivial bi-infinite geodesics going through $x$, namely $x+\Z e_1$ and $x+\Z e_2$, which we do not introduce notation for. %CHANGED HERE

A semi-infinite geodesic $\geod{k,\infty}$, or a bi-infinite geodesic $\geod{-\infty,\infty}$, is  {\it directed}  into a set $\cA\subset\Uset$ if the limit points of $\geod{n}/n$ as $n\to\infty$  are all in $\cA$.  When $\cA=\{\xi\}$ the condition becomes $\lim_{n\to\infty} \geod{n}/n=\xi$ and we  say $\geod{k,\infty}$ is {\it $\xi$-directed}.\smallskip


Using the Busemann process, we construct a semi-infinite path $\geo{}{x}{\xi\sig}$  for each $\xi\in\ri\Uset$, both signs $\sigg\in\{-,+\}$,  and all  $x \in \bbZ^2$,  via these rules: the initial point is  $\geo{m}{x}{\xi\sig}=x$ where $m=x\cdot\et$, and for $n\ge m$
\be\label{d:bgeo}\begin{aligned}
\geo{n+1}{x}{\xi\sig} &= \begin{cases}
\geo{n}{x}{\xi\sig} + e_1, & \text{ if } \B{\xi\sig}(\geo{n}{x}{\xi\sig},\geo{n}{x}{\xi\sig} + e_1) < \B{\xi\sig}(\geo{n}{x}{\xi\sig},\geo{n}{x}{\xi\sig} + e_2),\\
 \geo{n}{x}{\xi\sig} + e_2, & \text{ if } \B{\xi\sig}(\geo{n}{x}{\xi\sig},\geo{n}{x}{\xi\sig} + e_1) > \B{\xi\sig}(\geo{n}{x}{\xi\sig},\geo{n}{x}{\xi\sig}+ e_2),\\
\geo{n}{x}{\xi\sig} + e_{\sig},& \text{ if } \B{\xi\sig}(\geo{n}{x}{\xi\sig},\geo{n}{x}{\xi\sig} + e_1) = \B{\xi\sig}(\geo{n}{x}{\xi\sig},\geo{n}{x}{\xi\sig}+ e_2).
\end{cases}
\end{aligned}
\ee
As above, we dispense with the $\pm$ distinction when $\geo{}{x}{\xi+}=\geo{}{x}{\xi-}$.  These geodesics inherit an ordering from \eqref{mono}:   for all $x\in\Z^2$, $n\ge x\cdot\et$, and $\zeta\prec\eta$ in $\ri\Uset$,
	\begin{align}\label{path-ordering}
	\geo{n}{x}{\zeta-}\preceq\geo{n}{x}{\zeta+}\preceq\geo{n}{x}{\eta-}\preceq\geo{n}{x}{\eta+}.
	\end{align}

Similarly, the geodesics inherit one-sided continuity from \eqref{Busemann-limits}  in the sense of convergence of finite length segments: 
for all $x \in \bbZ^2$,   $\xi \in \ri \Uset$ and $\sigg\in\{-,+\}$, if $k = x \cdot \et$ and $m \geq k$ is an integer, then
\be\label{pmgeolim}
\lim_{\ri\Uset\,\ni\,\eta \searrow \xi} \geo{k,m}{x}{\eta\sig}  =  \geo{k,m}{x}{\xi+}\quad \text{and}\quad\lim_{\ri\Uset\,\ni\,\zeta \nearrow \xi} \geo{k,m}{x}{\zeta\sig} =  \geo{k,m}{x}{\xi-}.
\ee 

 An elementary  argument given in 
\cite[Lemma 4.1]{Geo-Ras-Sep-17-ptrf-2}
shows that properties \eqref{coc-prop} and \eqref{rec-prop2} combine to imply that these paths are all semi-infinite geodesics and that, moreover, for all choices of $x \in \bbZ^2$,  $n\ge x\cdot\et$,  $\sigg\in\{-,+\}$, and $\xi\in\ri\Uset$, we have 
\begin{align} \label{eq:buspass}
G(x,\geo{n}{x}{\xi\sig}) &= \B{\xi\sig}(x,\geo{n}{x}{\xi\sig}).
\end{align} 


%\textcolor{red}{Mention that under condition \eqref{g-reg}, it is enough to just assume the setting in the first paragraph of Section \ref{sub:setting} and continuous weights. I.e.\ in this case, the Busemann process does not require extending the space any further.}


%\begin{proof}
%We prove the $\xi+$ limit, with the $\xi-$ limit being similar. It suffices to show that at  each site $x$ with $k=x\cdot\et$, for any sequence $\eta_n\searrow\xi$, for $n$ sufficiently large,  $\geo{k+1}{x}{\eta_n-}=\geo{k+1}{x}{\xi+}$. Suppose first that $\B{\xi+}(x,x+e_1) > \B{\xi+}(x,x+e_2)$. Then by \eqref{Busemann-limits} there exists $n_0$ so that for all $n \geq n_0, \B{\eta_n-}(x,x+e_1)> \B{\eta_n-}(x,x+e_2)$, in which case $\geo{k+1}{x}{\eta_n-} = \geo{k+1}{x}{\xi+}=x+e_2$. The case of $\B{\xi+}(x,x+e_1) < \B{\xi+}(x,x+e_2)$ is similar. Now suppose that $\B{\xi+}(x,x+e_1) = \B{\xi+}(x,x+e_2)= \w_{x}$. Then by monotonicity \eqref{mono}, we have $\w_x \leq\B{\eta_n-}(x,x+e_1) \leq \B{\xi+}(x,x+e_1) = \w_x$ for all $n$. It follows that $\geo{k+1}{x}{\eta_n} = \geo{k+1}{x}{\xi+}=x+e_1$.
%\end{proof}


Below  are the  main properties of these  Busemann geodesics  $\geo{}{x}{\xi\sig}$ under assumption \eqref{main-assump}, from  article \cite {Geo-Ras-Sep-17-ptrf-2}.  (Theorem \ref{thm1}  in Appendix \ref{app:busgeo} provides  a more  precise accounting.) 
\begin{enumerate}[label={\rm(\roman*)}, ref={\rm\roman*}]  \itemsep=3pt 
\item Every semi-infinite geodesic is $\Uset_\xi$-directed for some $\xi\in\Uset$.
\item $\geo{}{x}{\xi\sig}$ is $\Uset_{\xi\sig}$-directed for each $x \in \bbZ^2$ and each $\xi \in \Uset$.
\item \label{pt:unique} If $\xi,\ximin,\ximax \in \Diff$, then there is a $\xi$-dependent event of full probability on which $\geo{}{x}{\xi-} = \geo{}{x}{\xi+}$ for all $x \in \bbZ^2$.
\item\label{pt:coal}  There is a $\xi$-dependent event of full probability on which $\geo{}{x}{\xi\sig}$ and $\geo{}{y}{\xi\sig}$ coalesce for each $\sig \in \{+,-\}$. That is, for each $x,y \in \bbZ^2$, there exists an $\w$-dependent $K \in \bbN$ such that for all $k \geq K$,  $\geo{k,\infty}{x}{\xi\sig}= \geo{k,\infty}{y}{\xi\sig}$. 
\end{enumerate}
% structure of semi-infinite geodesics under \eqref{main-assump}. 

%\smallskip

The regularity condition \eqref{g-reg} guarantees that $\geo{}{x}{\xi-}$ and $\geo{}{x}{\xi+}$ are extreme among the $\Uset_\xi$-directed geodesics out of $x$ in the sense that for any $x\in\Z^2$,  $\xi\in\ri\Uset$,  and any $\Uset_\xi$-directed semi-infinite geodesic $\geod{}$ emanating from $x$, we have 
\begin{equation}\label{eq:geoorder}	
	\geo{n}{x}{\xi-} \preceq \geod{n} \preceq \geo{n}{x}{\xi+} 
	%\geo{n}{x}{\xi-} \cdot e_1 \leq \geod{n} \cdot e_1 \leq \geo{n}{x}{\xi+} \cdot e_1 
\end{equation}
for all $n\ge x\cdot\et$. We record this fact as Theorem \ref{thm:extreme} in Appendix \ref{app:busgeo}. 
%Extremality gives  control of    general semi-infinite geodesics through   $\geo{}{x}{\xi+}$ and $\geo{}{x}{\xi-}$. 



Under the regularity condition \eqref{g-reg} and $\xi,\ximin,\ximax\in\Diff$, part \eqref{pt:unique} combined with \eqref{eq:geoorder} implies that there is a $\xi$-dependent event of full probability on which there is a unique $\Uset_\xi$-directed geodesic from each $x \in \bbZ^2$. Moreover, by part \eqref{pt:coal}, all of these geodesics coalesce. On the other hand, under the same condition, it is known that 
there are exceptional random directions at which both uniqueness and coalescence fail. We discuss these directions in the next subsection.

 %Among the main goals of this paper is the  study  of the structure of semi-infinite geodesics in such exceptional directions and in particular to prove results about the structure of all semi-infinite geodesics on a single event of full probability.
%%%%%  Timo's comment: I think this has been said enough? Or not? 



% without direction dependence in the event of full probability on which the result holds.

%\timonote{Clumsy transition here.  First it's ``(c) and (e)'' but then "this". F: Better now?  T: No, because the new assumption introduced below only addresses (c), not (c) and (e). F: OK now??} 
%\note{only a small number of our results!! we could say exactly to what purpose we would use this.}

%Henceforth, we redefine $\Omega_\xi$ to denote the smaller full-measure event $\Omega'_\xi$ and redefine $\Omega_0$ to denote $\Omega'''_0\cap\bigcap_{\xi\in\Udense}\Omega'_\xi$.
%Below, we will repeat this abuse of notation several times, where we use 
%$\Omega_\xi$ to denote full-measure events that may depend on $\xi$ and then use $\Omega_0$ to denote 
%a full-measure event that does not depend on the direction $\xi$ and is contained in $\bigcap_{\xi\in\Udense}\Omega_\xi$.




%\textcolor{red}{Say something about the spanning tree for a fixed $\xi$? Say something about the dual graph and the shock-like structure? (in which case, we can add the figures)  Maybe not...}

\subsection{Non-uniqueness  of directed semi-infinite geodesics}
\label{s:mult-geo} 
%\subsection{Multiple directed semi-infinite geodesics and the Busemann measures}
%\addmath{WARNING: under differentiability, not \eqref{g-reg}.  if there are corners, then there are multiple geodesics!}
%Under the regularity condition \eqref{g-reg} Theorems \ref{thm:extreme} and \ref{thm1} give existence, uniqueness, and coalescence of $\Uset_\xi$-directed geodesics for a fixed $\xi\in\ri\Uset$, where uniqueness also requires $\xi \in \Diff$.  The uniqueness result in Theorem \ref{thm1}\eqref{thm1:cont} holds only on a full-measure event that depends on the direction $\xi$.   
For a fixed site $x \in \bbZ^2$, a natural direction in which non-uniqueness occurs is  the {\it competition interface direction}, which we denote by $\cid(T_x\w)$.  At the origin, $\cid(\w)\in\ri\Uset$ is   the unique direction such that 
	\begin{align}\label{cid}
	\B{\zeta\pm}(e_1,e_2)<0\quad\text{if}\quad\zeta\prec\cid(\w)
	\quad\text{and}\quad
	\B{\zeta\pm}(e_1,e_2)>0\quad\text{if}\quad\zeta\succ\cid(\w).
	\end{align}
Theorem \ref{thm:cif} records the main properties of competition interface directions, including the existence and uniqueness of such a direction.

Under  the regularity condition \eqref{g-reg}, we also have the following alternative description of $\cid(\w)$. Fix a site $x\in\Z^2$.  The uniqueness of finite geodesics implies that the collection of geodesics from $x$ to all points  $y \in x+ \bbZ^2_+$ form a tree $\sT_x$ rooted
at $x$ and spanning $x+\bbZ_+^2$. The subtree rooted at $x+e_1$ is separated from the subtree rooted at $x+e_2$  by a path $\{\varphi_n^x:n\ge x\cdot\et\}$ on the dual lattice $\etstar+\Z^2$, known as the {\it competition interface}. See Figure \ref{fig:cif1}.

\begin{figure}[H]
\begin{center}

\begin{tikzpicture}[>=latex,scale=0.5]

\draw(-0.37,-0.35)node{$x$};
\draw(-1.3,1)node{$x+e_2$};
\draw(1.5,-0.5)node{$x+e_1$};

% TREE

\draw[line width=1pt](9,0)--(0,0)--(0,9);     %width of tree lines
\draw[line width=1pt](2,0)--(2,4)--(5,4)--(5,7)--(7,7)--(7,9)--(9,9);
\draw[line width=1pt](1,0)--(1,3);
\draw[line width=1pt](0,4)--(1,4)--(1,5)--(2,5)--(2,7);
\draw[line width=1pt](2,5)--(4,5)--(4,6);
\draw[line width=1pt](3,5)--(3,6)--(3,8)--(5,8)--(5,9)--(6,9);
\draw[line width=1pt](3,7)--(4,7);
\draw[line width=1pt](6,7)--(6,8);
\draw[line width=1pt](0,6)--(1,6)--(1,8)--(2,8)--(2,9)--(3,9);
\draw[line width=1pt](4,8)--(4,9);
\draw[line width=1pt](0,9)--(1,9);
\draw[line width=1pt](5,4)--(7,4)--(7,5)--(9,5)--(9,8);
\draw[line width=1pt](6,4)--(6,6)--(7,6);
\draw[line width=1pt](8,5)--(8,8);
\draw[line width=1pt](2,1)--(8,1)--(8,2)--(9,2);
\draw[line width=1pt](2,2)--(4,2)--(4,3)--(6,3);
\draw[line width=1pt](9,0)--(9,1);

%copyright purposes
\draw[line width=1pt](5,0)--(5,1);
\draw[line width=2pt,color=white](4,1)--(5,1);

%copyright purposes 2
\draw[line width=1pt](4,3)--(4,4);
\draw[line width=2pt,color=white](3,4)--(4,4);

\draw[line width=1pt](5,1)--(5,2)--(7,2)--(7,3);
\draw[line width=1pt](8,2)--(8,4)--(9,4);
\draw[line width=1pt](3,2)--(3,3);
\draw[line width=1pt](8,3)--(9,3);

%%% Competition interface

\draw[line width=2.0pt,color=nicosred](.5,.5)--(0.5,3.5)--(1.5,3.5)--(1.5, 4.5)--(4.5,4.5)--(4.5,7.5)--(5.5,7.5)--(5.5,8.5)--(6.5,8.5)--(6.5, 9.5);   %width of comp int
%\draw[line width=3.5pt, densely dotted](.5,.5)--(0.5,3.5)--(1.5,3.5)--(1.5, 4.5)--(4.5,4.5)--(4.5,7.5)--(5.5,7.5)--(5.5,8.5)--(6.5,8.5)--(6.5, 9.5);    %style of comp int line
%\draw[line width=3.5pt, dashed](.5,.5)--(0.5,3.5)--(1.5,3.5)--(1.5, 4.5)--(4.5,4.5)--(4.5,7.5)--(5.5,7.5)--(5.5,8.5)--(6.5,8.5)--(6.5, 9.5);
\foreach \x in {0,...,9}{
             \foreach \y in {0,...,9}{
\draw[ fill =sussexp](\x,\y)circle(1.7mm);    %size of bullet
}} 


\foreach \x in{0,...,6}{
		\draw[ fill =sussexg](\x, 9)circle(1.7mm);    %size of bullet		
				}

\foreach \x in{0,...,5}{
		\draw[ fill =sussexg](\x, 8)circle(1.7mm);    %size of bullet		
				}

\foreach \x in{0,...,4}{
		\foreach \y in {5,6,7}{
		\draw[fill =sussexg](\x, \y)circle(1.7mm);    %size of bullet		
				}}

\foreach \x in{0,...,1}{
		\draw[ fill =sussexg](\x, 4)circle(1.7mm);    %size of bullet		
				}

\foreach \x in{0,...,0}{
		\foreach \y in {1,2,3}{
		\draw[fill =sussexg](\x, \y)circle(1.7mm);    %size of bullet		
				}}

\draw[fill=white](0,0)circle(1.7mm); 

\end{tikzpicture}

\end{center}
\caption{\small   The geodesic tree $\mathcal{T}_x$ rooted at $x$.  
The competition interface  (solid line)  emanates from $x+\etstar$ and separates 
the   subtrees of $\mathcal{T}_x$ rooted at $x+e_1$   and $x+e_2$.}
\label{fig:cif1}
\end{figure}

Under condition \eqref{g-reg}, the competition interface satisfies $\varphi_n^x/n \to \cid(T_x\w)$, given by \eqref{cid}. Moreover, each of these two trees contains at least one semi-infinite geodesic with asymptotic direction $\cid(T_x\w)$. Indeed, $\cid(T_x\w)$ is the unique direction with the property that there exist at least two semi-infinite geodesics rooted at $x$, with asymptotic direction $\cid(T_x\w)$, and which differ in their first step. See Figure \ref{fig:cif2}. Theorem \ref{thm-Coupier} records the fact that when the weights are exponentially distributed, there are no directions $\xi$ with three $\xi$-directed geodesics emanating from the same point.


\begin{figure}[H]
\centering
\begin{subfigure}{0.38\textwidth}
\includegraphics[width=\textwidth]{Figs/cif1-standalone.pdf}
\end{subfigure}
\begin{subfigure}{0.59\textwidth}
\input{Figs/cif-N5000L300.tex}
\end{subfigure}
%\input{Figs/cif-N5000L5000.tex}
\caption{\small  The competition interface (middle path) separating the two $\cid$-directed geodesics. The left picture is a small portion of the right one. In the picture on the right the $x$-axis appears to be stretched, but the scales of the axes are in fact identical.}
\label{fig:cif2}
\end{figure}





==> JEMS Post-Accept Revision/GeoWebPaper-Sec3.tex <==
% !TEX root = GeoWebPaper.tex

\section{Busemann measures, exceptional directions, and coalescence points}\label{s:Bmeas} 
%\subsection{Preliminaries} 
The central theme of   this paper is the relationship between analytic properties of the Busemann process and the geometric properties of the geodesics $\geo{}{\abullet}{\xi\sig}$ for   $\xi \in \ri \Uset$ and $\sigg\in\{-,+\}$. 
%A major role will be played by directions of discontinuity of the Busemann process. 
It will be convenient in what follows to have a bookkeeping tool for the locations at which the Busemann processes are not locally constant. A natural way to record this information is through the supports of the associated Lebesgue-Stieltjes measures. 



%We begin with the observation that the Busemann processes have locally bounded total variation, which justifies the construction of these measures.
%
%\begin{corollary}
%There exists a $T$-invariant Borel set $\Omega_0 \subset \Omega$ with $\bbP(\Omega_0) = 1$ such that, for all $\w \in \Omega_0$ and  $x,y \in \bbZ^2$, the processes $\xi \mapsto \B{\xi\pm}(x,y)$ are of locally bounded total variation.
%\end{corollary}
%\begin{proof}
%By \textcolor{red}{(cocycle property)}, it suffices to prove this result for $\xi \mapsto \B{\xi\pm}(x,x+e_i)$, $i \in \{1,2\}$, which are monotone functions.  
%\end{proof}
As functions of the direction parameter $\xi$, $\B{\xi-}_{x,x+e_i}$  and $\B{\xi+}_{x,x+e_i}$ are respectively left- and right-continuous versions of the same monotone function and satisfy the cocycle property \eqref{coc-prop}. As a consequence, 
for each $x,y\in\Z^2$, $\sigg\in\{-,+\}$, $\xi\mapsto\B{\xi\sig}(x,y)$ has locally bounded total variation.  
%The functions $\xi \mapsto \B{\xi\pm}(x,y)$ have  locally bounded total variation and 
%they agree at $\xi$ in the   dense set $\Udense$. 
Hence on each compact subset  $K$ of $\ri \Uset$ there exists a signed Lebesgue-Stieltjes measure  $\mu_{x,y}^{K}$  with the property that whenever 
%$\zeta,\eta \in K$ satisfy 
$\zeta \prec \eta$ and $[\zeta, \eta]\subset K$,
\be\label{Bmeas}\begin{aligned}
\mu_{x,y}^{K}(\,]\zeta, \eta])  = \B{\eta+}_{x,y} - \B{\zeta +}_{x,y}
\quad\text{and}\quad
\mu_{x,y}^{K}([\zeta , \eta [\,)= \B{\eta-}_{x,y} - \B{\zeta -}_{x,y}.
\end{aligned}\ee
%Recall the dense set $\Udense$, chosen after Theorem \ref{thm:Bus}. The concavity of $\gpp$ implies that $\ri\Uset\setminus\Diff$ is at most countable and hence $\Udense$ is dense in $\ri\Uset$. Then \eqref{B+=B-:temp} implies that in fact $\mu_{x,y}^{K,\pm}$ are the same measure, which we will denote by $\mu_{x,y}^K$.

The restriction to compact sets is a technical point: in general, $\B{\xi+}_{x,y}$ and $\B{\xi-}_{x,y}$  are signed sums of monotone functions and thus correspond to formal linear combinations of positive measures. 
By the limit in \eqref{B:inf-lim}, 
%Theorem \ref{thm:Bus}\eqref{thm:cocyexist:f},  
each of these positive measures assigns infinite mass to the interval $\ri\Uset$ and if any two of the measures come with different signs, the formal linear combination will not define a signed measure on all of $\ri\Uset$. We will ignore this technical point in what follows and write $\mu_{x,y}(\bbullet)$ for the value of this measure and $|\mu_{x,y}|(\bbullet)$ for the value of the total variation measure whenever they are unambiguously defined. In that vein, we define the \emph{support of the measure $\mu_{x,y}$} on $\ri\Uset$ as 
\begin{align}
\supp{\mu_{x,y}} &= \bigcup_{\zeta,\,\eta\,\in\,\ri\Uset: \, \zeta\prec\eta}
%{\substack{\zeta,\eta\,\in\,\ri\Uset\\ \zeta\prec\eta}}
\supp{\mu_{x,y}^{[\zeta,\eta]}},
\end{align}
where $\supp{\mu_{x,y}^{[\zeta,\eta]}}$ is, as usual, the 
%\reversemarginpar\addmath{do we need a reference to any of this? C: I vote no.}
support of the (well-defined) total variation measure $\abs{\mu_{x,y}^{[\zeta,\eta]}}$. Naturally, this definition agrees with the standard notion of the support of a measure when $\mu_{x,y}$ is a well-defined positive or negative measure on $\Uset$. 

\subsection{Coalescence and the Busemann measures}
%These Busemann measures and their supports are the fundamental tools in our analysis of geodesics. 
%In all of the following results, $\Omega_0$ is a $T$-invariant event of full measure which is constructed in equation \eqref{Om0} of Appendix \ref{app:busgeo}.
%\fixtext{polish. this applies to the next section too. is this the right spot? or should we repeat/remind in the next section?}
%All of the following results hold on a single event of full measure. In particular, the event does not depend on the directions $\zeta,\eta,\xi\in\ri\Uset$ that appear in the statements.
%\begin{theorem}\label{thm:nonint}
%%There exists a $T$-invariant event $\Omega_0$ with $\P(\Omega_0)=1$ and such that for all $\w \in \Omega_0$, the following are equivalent.
%%\begin{enumerate}[label={\rm(\alph*)}, ref={\rm\alph*}]  \itemsep=3pt 
%%\item $\xi \in \supp|\mu_{x,y}|$
%%\item For some choice of path $\geod{}^x \in \{\geo{}{x}{\xi+},\geo{}{x}{\xi-}\}$ and some choice of  path $\geod{}^y \in \{\geo{}{y}{\xi+}, \geo{}{y}{\xi-}\}$, $\geod{}^x \cap \geod{}^y = \varnothing$.
%%\end{enumerate}
%%There exists a $T$-invariant event $\Omega_0$ with $\P(\Omega_0) = 1$ and such that 
%For all $\w \in \Omega_0$ and all $x,y \in \Z^2$, %satisfying $x \cdot e_1 \leq y \cdot e_1$ and $x \cdot e_2 \geq y \cdot e_2$, 
%a $\xi\in\ri\Uset$ is in $\supp{\mu_{x,y}}$ if and only if %$\geo{}{x}{\xi-} \cap \geo{}{y}{\xi+} = \varnothing$. 
%either $\geo{}{x}{\xi-} \cap \geo{}{y}{\xi+} = \varnothing$ or $\geo{}{x}{\xi+} \cap \geo{}{y}{\xi-} = \varnothing$.
%%If furthermore Condition \eqref{cond:jumpcond} holds, then $\xi\in\supp{\mu_{x,y}}$ is also equivalent to $\B{\xi+}(x,y,\w)\ne\B{\xi-}(x,y,\w)$.
%\end{theorem}


%Now, throw away all the countably many null sets that were introduced so far and thus define %\note{Switched this to eqnarray to deal with the issue with the eqref not working correctly. The label is Om0, not sure why it isn't showing.}
%	\begin{eqnarray}\label{Om0}
%	\begin{split}
%	&\qquad\qquad\Omega_0=\Omega_0^2\cap\Omega_0^3\cap\Omega_0^5\cap\bigcap_{\xi\in\Udense}(\Omega_\xi^1\cap\Omega_\xi^4)\quad\text{and}\\%	&\Omreg=\Omega_0\cap\Omega_0^4,\quad\text{if Condition \eqref{g-reg} is assumed},\\
%	&\qquad\qquad\Omjump=\Omega_0\cap\Omega_0^6\cap\Omega_0^7,\quad\text{if condition \eqref{cond:jumpcond} (or a condition implying it) is assumed.}
%%	&\Omregjump=\Omega_0\cap\Omega_0^4\cap,\quad\text{if both Conditions \eqref{g-reg} and \eqref{cond:jumpcond} are assumed}.
%	%&\Omexp_0=\Omjump_0\cap\Omega_0^4,\quad\text{if $\{\w_x:x\in\Z^2\}$ are i.i.d.\ exponentially distributed.}
%	\end{split}
%	\end{eqnarray} 

The first  result below relates membership in the support with the existence of disjoint Busemann geodesics. 
\begin{theorem}\label{thm:nonint}
The following  holds with $\P$-probability one. For all $x\ne y$ in $\Z^2$ and $\xi\in\ri\Uset$  statements \eqref{thm:nonint.a} and \eqref{thm:nonint.b} below are equivalent: 
\begin{enumerate}[label={\rm(\roman*)}, ref={\rm\roman*}] \itemsep=3pt 
\item\label{thm:nonint.a} $\xi \in \supp{\mu_{x,y}}$.
\item\label{thm:nonint.b}  Either $\geo{}{x}{\xi-} \cap \geo{}{y}{\xi+} = \varnothing$ or $\geo{}{x}{\xi+} \cap \geo{}{y}{\xi-} = \varnothing$.
\end{enumerate}
Under the regularity condition \eqref{g-reg}, \eqref{thm:nonint.a} and \eqref{thm:nonint.b} are equivalent to
\begin{enumerate}[label={\rm(\roman*)}, ref={\rm\roman*},resume] \itemsep=3pt 
\item\label{thm:nonint.c}There exist $\Uset_\xi$-directed semi-infinite geodesics $\geod{}^x$ and $\geod{}^y$ out of $x$ and $y$, respectively,
%\begin{align*}
%&\ximin\cdot e_1 \leq \varliminf_{n\to\infty} \frac{\geod{n}^x \cdot e_1}{n} \leq \varlimsup_{n\to\infty} \frac{\geod{n}^x \cdot e_1}{n}  \leq \ximax \cdot e_1,  \\
%&\ximin\cdot e_1 \leq \varliminf_{n\to\infty} \frac{\geod{n}^y \cdot e_1}{n} \leq \varlimsup_{n\to\infty} \frac{\geod{n}^y \cdot e_1}{n}  \leq \ximax \cdot e_1, %\text{ and }
%\end{align*}
such that $\geod{}^x \cap \geod{}^y = \varnothing$.
\end{enumerate}
\end{theorem}

The difference between statements \eqref{thm:nonint.b} and \eqref{thm:nonint.c} is that if $\xi\not\in\supp{\mu_{x,y}}$ then \eqref{thm:nonint.b} leaves open the possibility that even though $\geo{}{x}{\xi-}$ and $\geo{}{y}{\xi+}$ intersect and   $\geo{}{x}{\xi+}$ and $\geo{}{y}{\xi-}$ intersect,  there may be other $\Uset_\xi$-directed geodesics out of $x$ and $y$  that do not intersect. This is because without the regularity condition \eqref{g-reg}, we currently do not know whether  \eqref{eq:geoorder} holds, that is, whether $\geo{}{x}{\xi+}$ is 
the rightmost and $\geo{}{x}{\xi-}$ the  leftmost $\Uset_\xi$-directed geodesic out of $x$.
%extreme among $\Uset_\xi$-directed geodesics out of $x$.


The subsequent  several results relate the support of Busemann measures to the coalescence geometry of geodesics.   For $x,y\in\Z^2$,   $\xi\in\ri\Uset$, and signs   $\sigg\in\{-,+\}$, define 
  the {\it coalescence point}  of  the geodesics $\geo{}{x}{\xi\sig}$ and $\geo{}{y}{\xi\sig}$
by 
\be\label{df:coal-z} \begin{aligned}
\coal{\xi\sig}(x,y) &= \begin{cases}
\text{first point in $\geo{}{x}{\xi\sig}\cap \geo{}{y}{\xi\sig}$}, & \text{if } \geo{}{x}{\xi\sig}\cap \geo{}{y}{\xi\sig} \neq \emptyset \\[3pt] 
\infty, &  \text{if } \geo{}{x}{\xi\sig}\cap \geo{}{y}{\xi\sig}= \emptyset.  
\end{cases}
\end{aligned}\ee
The  first point $z$ in $\geo{}{x}{\xi\sig}\cap \geo{}{y}{\xi\sig}$ is identified uniquely by choosing  the common point $z=\geo{k}{x}{\xi\sig}=\geo{k}{y}{\xi\sig}$ that  minimizes $k$. 
In the expression above,  $\infty$ is the point added in the one-point compactification of $\Z^2$. 
%where we have taken the convention that $\coal{\xi\sig}(x,y) = \infty$ if the geodesics rooted at $x$ and $y$ do not coalesce. 
If the two geodesics  $\geo{}{x}{\xi\sig}$ and  $\geo{}{y}{\xi\sig}$ ever meet, they coalesce due to the local rule in \eqref{d:bgeo}. We write $\coal{\xi}{(x,y)}$ when $\coal{\xi-}(x,y)=\coal{\xi+}(x,y)$. 

As $\Z^2\cup\{\infty\}$-valued functions,  $\xi\mapsto\coal{\xi+}(x,y)$ is right-continuous and $\xi\mapsto\coal{\xi-}(x,y)$ is left-continuous.  Namely, 
a consequence of \eqref{pmgeolim} is that for $\xi \in \ri \Uset$ and $\sigg\in\{-,+\}$, 
\begin{align}\label{coal-lim}
\lim_{\ri\Uset\,\ni\,\eta \searrow \xi} \coal{\eta \sig}(x,y) = \coal{\xi+}(x,y). 
\end{align}
If $\coal{\xi+}(x,y) = \infty$ this limit still holds in the sense that then $\abs{\coal{\eta \sig}(x,y)}\to\infty$.   The analogous statement holds for convergence from the left to  $\coal{\xi-}(x,y)$. 
%These limits are understood in the extended sense if $\coal{\xi+}(x,y) = \infty$ or $\coal{\xi-}(x,y)=\infty.$ 

The next theorem states that an interval of directions outside the support of a Busemann measure corresponds to geodesics following common initial segments to a common coalescence point. 

\begin{theorem}\label{thm:1path}   With probability one,   simultaneously  for all $\zeta\prec\eta$ in $\ri\Uset$ and all $x,y\in\Z^2$,  statements  \eqref{thm:1path.a}, \eqref{thm:1path.b}, and \eqref{thm:1path.c} below are equivalent:   
\begin{enumerate}[label={\rm(\roman*)}, ref={\rm\roman*}] \itemsep=3pt 
\item\label{thm:1path.a} $\abs{\mu_{x,y}}(\,]\zeta, \eta[\,)=0$.
\item\label{thm:1path.b}   Letting $k=x\cdot\et$ and $\ell=y\cdot\et$,  there exist a point $z$ with $z\cdot\et=m\ge k\vee\ell$  and path segments $\pi_{k,m}$ and $\wt\pi_{\ell,m}$  with these properties:   $\pi_k=x$, $\wt\pi_\ell=y$,  $\pi_m=\wt\pi_m=z$, and  for all $\xi\in\,]\zeta, \eta[$ and $\sigg\in\{-,+\}$ we have   $\geo{k,m}{x}{\xi\sig}=\pi_{k,m}$ and $\geo{\ell,m}{y}{\xi\sig}=\wt\pi_{\ell,m}$.  
\item\label{thm:1path.c} Letting $k=x\cdot\et$ and $\ell=y\cdot\et$,  there exists a point $z$ with $z\cdot\et=m\ge k\vee\ell$ so that for all $\xi\in\,]\zeta, \eta[$ and $\sigg\in\{-,+\}$, $\coal{\xi\sig}(x,y)=z$.
\end{enumerate}
\end{theorem} 

%Given the relevance of the support of the Busemann measures, 
%t is natural to wonder about its  structure.
%% looks like. An argument, given in Section \ref{sec:bus}, 
% The next lemma implies that the support   is always nowhere dense. % We record this fact in the following lemma. 
 
 The next lemma verifies that intervals that satisfy statement \eqref{thm:1path.a} of Theorem \ref{thm:1path}  almost surely make up a  random  dense open subset of $\ri\Uset$. 
% Recall that $\Udense$ is an arbitrary countable dense subset of points of differentiability of $\gpp$.

\begin{lemma}\label{lm:isolated}   
 Let $\Udense\subset\ri\Uset$ be a fixed countable dense set of points of differentiability of $\gpp$.
Then the  following holds with $\P$-probability one: 
for every $x,y\in\Z$ and every $\xi\in\Udense$, there exist $\zeta\prec\xi\prec\eta$ in $\ri\Uset$ such that  $\abs{\mu_{x,y}}(\,]\zeta, \eta[\,)=0$. 
%$]\zeta,\eta[\,\cap\supp{\mu_{x,y}}=\varnothing$.
\end{lemma}



%For $x,y\in\Z^2$,   $\xi\in\ri\Uset$, and signs   $\sigg\in\{-,+\}$, define 
%the {\it coalescence level} $\ell^{\xi\sig}(x,y)$ of the $\geo{}{x}{\xi\sig}$ and $\geo{}{y}{\xi\sig}$ geodesics as
%the smallest $\ell\ge x\cdot\et\vee y\cdot\et$ such that $\geo{\ell}{x}{\xi\sig}=\geo{\ell}{y}{\xi\sig}$, if such an $\ell$ exists, 
%and $\infty$ otherwise.
%\be\label{df:coal-l}  
%\ell^{\xi\sig}(x,y)=\inf\{x\cdot\et: x \in \geo{}{x}{\xi\sig}\cap \geo{}{y}{\xi\sig}\}
%\ee
%with the convention that the infimum of an empty set is $\infty$. 

%%%%%  OLD def. of coalescence pt. 
%\be\label{df:coal-z} \begin{aligned}
%\coal{\xi\sig}(x,y) &= \begin{cases}
%\geo{\ell^{\xi\sig}}{x}{\xi\sig}=\geo{\ell^{\xi\sig}}{y}{\xi\sig}, & \text{if } \geo{}{x}{\xi\sig}\cap \geo{}{y}{\xi\sig} \neq \emptyset, \\[3pt] 
%\infty, &  \text{if } \geo{}{x}{\xi\sig}\cap \geo{}{y}{\xi\sig}= \emptyset, 
%\end{cases}
%\end{aligned}\ee

A  natural question is whether the measure is Cantor-like with no isolated points of support, or   if the support   consists entirely of isolated points, or if both are possible.  These features also turn out to have counterparts in coalescence properties. 
  For a set $\cA\subset\Uset$  say that $\xi$ is a {\it  limit point of $\cA$ from the right} 
if $\cA$ intersects $]\xi, \eta[$ for each $\eta\succ\xi$, with a similar definition for limit points from the left.


\begin{theorem}\label{thm:supp-tri}
The following  holds with probability one. For all $x,y \in \bbZ^2$ and $\xi \in \ri \Uset$:
\begin{enumerate} [label={\rm(\alph*)}, ref={\rm\alph*}]   \itemsep=3pt 
\item\label{thm:supp-tri:1} $\xi\notin\supp{\mu_{x,y}}$ $\Longleftrightarrow$ $\coal{\xi+}(x,y)=\coal{\xi-}(x,y) \in \bbZ^2$.
\item\label{thm:supp-tri:2} $\xi$ is an isolated point of $\supp{\mu_{x,y}}$ $\Longleftrightarrow$ $\coal{\xi+}(x,y) \neq \coal{\xi-}(x,y)$ but both $\coal{\xi\pm}(x,y) \in \bbZ^2$.
\item\label{thm:supp-tri:3} $\xi$ is a limit point of $\supp{\mu_{x,y}}$ from the right $\Longleftrightarrow$ $\coal{\xi+}(x,y)=\infty$.  Similarly,  $\xi$ is a limit point of $\supp{\mu_{x,y}}$ from the left  $\Longleftrightarrow$ $\coal{\xi-}(x,y)=\infty$. 
 \end{enumerate}
\end{theorem}

%\begin{theorem}\label{th:isopt}
%%Let $\Omega_0$ be the full measure event in Proposition \ref{pr:supp2}.
%%There exists a $T$-invariant Borel set $\Omega_0 \subset \Omega$ with $\bbP(\Omega_0) = 1$ so that 
%For all $\w \in \Omega_0$, all $x,y \in \bbZ^2$, and $\xi \in \ri \Uset$, the following are equivalent.
%\begin{enumerate} [label={\rm(\alph*)}, ref={\rm\alph*}]   \itemsep=3pt 
%\item\label{prop:isopt:1} $\coal{\xi+}(x,y), \coal{\xi-}(x,y) \in \bbZ^2$ and $\coal{\xi+}(x,y) \neq \coal{\xi-}(x,y)$.
%\item\label{prop:isopt:2} $\xi$ is an isolated point of $\supp{\mu_{x,y}}$.
% \end{enumerate}
%\end{theorem}
%
%
%\begin{proposition} \label{pr:supp2}
%%There is a $T$-invariant event $\Omega_0$ with $\bbP(\Omega_0)=1$ and such that 
%%Let $\Omega_0$ be the full measure event from Proposition \ref{pr:supp1}.
%For all $\w \in \Omega_0$ and all $x,y \in \bbZ^2$, the following are equivalent:
%\begin{enumerate} [label={\rm(\alph*)}, ref={\rm\alph*}]   \itemsep=3pt 
%\item\label{eq110}  $\xi \not\in \supp{\mu_{x,y}}$.
%\item\label{eq111} $\coal{\xi-}(x,y) = \coal{\xi+}(x,y) \in \bbZ^2$.
%\item\label{eq112} $\B{\xi-}(x,y) = \B{\xi+}(x,y)$ and $\coal{\xi-}(x,y), \coal{\xi+}(x,y) \in \bbZ^2$. 
%\end{enumerate}
%\end{proposition}


 This motivates  
the following condition on the Busemann process   which  will be invoked in some  results in the sequel: 
%\begin{condition}\label{cond:jumpcond}
\begin{align}\label{cond:jumpcond}
\begin{minipage}{0.9\textwidth}
There exists a full $\P$-probability event on which every point of $\supp{\mu_{x,y}}$ is isolated, for all $x,y\in\Z^2$. 
%\P\Bigl\{\forall x,y\in\Z^2:\text{ every point of $\supp{\mu_{x,y}}$ is isolated}\Bigr\}=1.
\end{minipage}
\end{align}\smallskip
%\end{condition}
Equivalently, condition \eqref{cond:jumpcond} says that   $\xi \mapsto \B{\xi\pm}(x,y)$ is a  jump process whose jumps do not accumulate on $\ri \Uset$. For this reason, we  refer to \eqref{cond:jumpcond} as the  {\it jump process condition}.
%In particular,   $\aUset$ is countable. 
%\normalmarginpar\addmath{would be better to put this right after the condition is stated. but we need $\Omega_0$ for the statement!!}
%We cite the jump process condition \eqref{cond:jumpcond} explicitly in all statements   that require it.
It is shown in \cite[Theorem 3.4]{Fan-Sep-20} that \eqref{cond:jumpcond} holds 
when the weights $\w_x$ are i.i.d.\ exponential random variables.  
In addition to Lemma \ref{lm:isolated}, this is a further  reason to expect that \eqref{cond:jumpcond} holds very generally. 
%which further justifies highlighting it.  
%This and the following lemma suggest  that  \eqref{cond:jumpcond}  should hold more generally.

Under condition \eqref{cond:jumpcond}  Theorem \ref{thm:supp-tri} extends to a global  coalescence statement.  
 
\begin{theorem}\label{thm:+-coal}
%Assume \eqref{main-assump}. 
%There is an event of full $\bbP$ probability on which s
Statements \eqref{thm:+-coal.a} and  \eqref{thm:+-coal.b} below are equivalent.
\begin{enumerate}[label={\rm(\roman*)}, ref={\rm\roman*}] \itemsep=3pt 
\item\label{thm:+-coal.a} The jump process condition \eqref{cond:jumpcond} holds.
\item\label{thm:+-coal.b} This holds with $\P$-probability one: for all $x,y\in\Z^2$, all $\xi\in\ri\Uset$, and both signs $\sigg\in\{-,+\}$, the geodesics $\geo{}{x}{\xi\sig}$ and $\geo{}{y}{\xi\sig}$ coalesce.
\end{enumerate}
\end{theorem}


%When condition \eqref{cond:jumpcond} or a condition implying it is assumed, our results will hold on the smaller 
%$T$-invariant full measure event:
%	\begin{eqnarray}\label{Omjump}
%	\Omjump=\Omega_0\cap\Omega_0^5\cap\Omega_0^6.
%	\end{eqnarray} 
%All of our results will hold on one of the following $T$-invariant full $\P$-measure events: $\Omega_0$, $\Omjump$, $\Omega_0\cap\Ombiinf$, $\Omjump\cap\Ombiinf$, and $\Omjump\cap\OmCou$, depending on the assumptions of the result.\smallskip
%The results that  assume the weights are exponentially distributed 
%will hold on $\Omjump_0\cap\OmCou$ or $\Omjump_0\cap\Ombiinf$.\smallskip
%In the course of some of the proofs we will also need the following $T$-invariant full $\P$-measure events that depend on $\xi\in\ri\Uset$:
%	\begin{align}\label{Omxi}
%	\begin{split}
%	&\Omega_\xi=\Omega_0\cap\Omega_\xi^1\cap\Omega_\xi^3\quad\text{and}\\
%	&\Omjump_\xi=\Omega_\xi\cap\Omega_0^5,\quad\text{if Condition \eqref{cond:jumpcond} is assumed.}
%	\end{split}
%	\end{align}

We introduce  the random  set of exceptional directions obtained by taking the union of the supports of  the Busemann measures:
%We denote the set of points which lie in the support of some Busemann measure by $\aUset$:
\begin{align} 
\aUset &= \bigcup_{x,\,y\,\in\,\bbZ^2} \supp{\mu_{x,y}} \;\subset\;\ri\Uset. \label{df:aUset}
\end{align}
It turns out that not all pairs $x,y$ are necessary for the union.  It suffices  to take  pairs of adjacent points  along horizontal or vertical lines, or along  any  bi-infinite path  with nonpositive local slopes.  
\begin{lemma}\label{lm:downright}
%Assume \eqref{main-assump}.
%There exists a $T$-invariant event $\Omega_0$ with $\P(\Omega_0)=1$ and such that 
The following holds for $\P$-almost every $\w$.  
Let $x_{-\infty,\infty}$ be any bi-infinite path in $\Z^2$ such that  $\forall i\in\Z$,  $(x_{i+1}-x_i)\cdot e_1\ge 0$ and $(x_{i+1}-x_i)\cdot e_2\le 0$ and not both are zero. Then 
%For any path $x_{-\infty,\infty}$ with $x_{i+1}-x_i\in\{e_1,-e_2\}$ for all $i\in\Z$, we have
	\[\aUset= \bigcup_{i\in\Z} \supp\mu_{x_i,x_{i+1}}.\]
\end{lemma}

 

%Under the regularity condition \eqref{g-reg}, $\aUset$ is almost surely dense outside the closed linear segments of $\gpp$ and 
%\note{F edited this a bit. $\aUset$ does not contain all of $\Diff^c$, without ergodicity}
%has atoms exactly at the directions of non-differentiability.
%but is random otherwise.
%It is {\it a priori} not clear from \eqref{cid} if  $\cid\in\aUset$. 
%Theorems \ref{thm1}\eqref{thm1:exist}, \ref{thm:cif}\eqref{thm:cif:(ii)}, and \ref{thm:nonint} (applied to the points ${x+e_1,x+e_2}$) imply that $\cid(T_x\w)\in\supp{\mu_{x+e_1,x+e_2}}\subset\aUset$.  

  The remainder of this section addresses   (i) characterizations of $\aUset$ and  (ii) its significance for  uniqueness and coalescence of geodesics. 
  The first item relates the exceptional directions to asymptotic directions of competition interfaces. 
  
  \begin{theorem}\label{thm:Vcid} 
  The following hold for $\P$-almost every $\w$.
\begin{enumerate}[label={\rm(\alph*)}, ref={\rm\alph*}] \itemsep=3pt 
\item\label{thm:Vcid.1} 
 For   all $x\in\Z^2$, $  \supp \mu_{x,x+e_1} \cap \supp \mu_{x,x+e_2}=\{\cid(T_x\w)\} $.   In particular, 
 $\aUset\supset\{\cid(T_x\w): x\in\Z^2\}$.  
   \item\label{thm:Vcid.2} 
 Under the jump process condition \eqref{cond:jumpcond},  
$\aUset=\{\cid(T_x\w): x\in\Z^2\}$. 
%$\xi \in \aUset$ if and only if there exists $x \in \bbZ^2$ such that $\xi = \cid(\T_x\w)$.
\end{enumerate}

  \end{theorem} 
  
  
The next issue is the relationship between   $\aUset$ and  regularity properties of $\gpp$.   Recall the definition \eqref{df:D} of $\Diff$ as the set of differentiability points of $\gpp$.   Let $\fUset$ be the subset of $\ri\Uset$ that remains after removal of all open linear segments of $\gpp$ and removal of  those endpoints of linear segments that are differentiability points.  Equivalently, $\fUset$ consists of those $\xi\in\ri\Uset$ at which $\gpp$ is either non-differentiable or strictly concave. 

\begin{theorem}\label{th:V1}  $ $ 
\begin{enumerate}[label={\rm(\alph*)}, ref={\rm\alph*}] \itemsep=3pt 
\item\label{th:V1.a} Let  $\xi\in\ri\Uset$. Then  $\xi\in\Diff$ if and only if $\P(\xi\in\aUset)=0$. %Equivalently,    if and only if $\P(\xi\in\supp{\mu_{x,x+e_i}})=0$ for any {\rm(}and hence all{\rm)} $x\in\Z^2$ and $i\in\{1,2\}$. 
If  $\xi\notin\Diff$ then 
\[  \P(\exists x:  \,\cid(T_x\w) =\xi) = \P(\xi\in\aUset)= 1.  \]  

\item\label{th:V1.b} For $\P$-almost every $\w$, the set  $\{\cid(T_x\w): x\in\Z^2\}$ and the set  $\aUset$ are  dense subsets of $\fUset$. 

%\item\label{th:V1.c}  %Under  the regularity condition \eqref{g-reg},  $(\ri\Uset)\setminus\Diff\subset\aUset$ for $\P$-almost every $\w$.
%Assume the regularity condition \eqref{g-reg}. Then  for $\P$-almost every $\w$, $\aUset$ contains all points of non-differentiability of $\gpp$.
\end{enumerate}
\end{theorem}

% Under  the regularity condition \eqref{g-reg}, parts \eqref{th:V1.a} and \eqref{th:V1.c} imply a sharp dichotomy for every $\xi\in\ri\Uset$:   $\P(\xi\in\aUset)=0$ or $1$ depending on whether $\xi\in\Diff$ or not.  
 
   
%%%%%    OLD THEOREM V1 BEFORE THE TECHNICAL STATEMENTS BECAME LEMMAS IN THE PROOF SECTION  %%%%%%%%%
%\begin{theorem}\label{th:V1}
%%\normalmarginpar\note{In the language of Daley and Vere-Jones, $\xi$ is a fixed atom of the random measure (Def. 9.3.I in Volume 2), in case we want to mention this.}
%For any $\xi\in\ri\Uset$ we have $\xi\in\Diff$ if and only if $\P(\xi\in\aUset)=0$ which itself holds if and only if $\P(\xi\in\supp{\mu_{x,x+e_i}})=0$ for any {\rm(}and hence all{\rm)} $x\in\Z^2$ and $i\in\{1,2\}$. 
%
%The following hold for $\P$-almost every $\w$.
%\begin{enumerate}[label={\rm(\alph*)}, ref={\rm\alph*}] \itemsep=3pt 
%\item\label{th:V1.0} 
%Let $\zeta\prec\eta$ in $\ri\Uset$.  Then $\,]\zeta,\eta[\,\cap\,\aUset\ne\varnothing$ if and only if $\nabla\gpp(\zeta+)\ne\nabla\gpp(\eta-)$. 
%  \item\label{th:V1.0'} 
%Let $\zeta\prec\eta$ in $\ri\Uset$.  If $\nabla\gpp(\zeta-)=\nabla\gpp(\eta-)$, then $[\zeta,\eta[\,\cap\,\aUset=\varnothing$. Similarly, if 
%$\nabla\gpp(\zeta+)=\nabla\gpp(\eta+)$, then $]\zeta,\eta]\cap\,\aUset=\varnothing$. 
%\end{enumerate}
%\end{theorem}
%%%%%%%%%%%%%   END OLD THEOREM V1 %%%%%%%%%%%%

The next  theorem identifies  $\aUset$ as   the set of
directions with multiple semi-infinite geodesics.  
As before,  the regularity condition \eqref{g-reg} allows us to talk about general $\Uset_\xi$-directed semi-infinite geodesics, instead of only the Busemann geodesics $\geo{}{x}{\xi\sig}$.  
% Under  the jump process condition \eqref{cond:jumpcond} the $+$ and $-$ geodesics coalesce (Theorem \ref{thm:+-coal}), and consequently the $\pm$  geodesics must agree or separate. 

%\newpage

\begin{theorem}\label{th:V2}
%Assume \eqref{main-assump}.
%There exists a $T$-invariant event $\Omega_0$ with $\P(\Omega_0)=1$ and such that 
The following hold for $\P$-almost every $\w$.
\begin{enumerate}[label={\rm(\alph*)}, ref={\rm\alph*}] \itemsep=3pt 
\item\label{th:V2.a}  
$\xi\in(\ri\Uset)\setminus\aUset$ if and only if the following is true: $\geo{}{x}{\xi+}=\geo{}{x}{\xi-}$ for all $x\in\Z^2$ and all these geodesics coalesce.
\item\label{th:V2.b} Under the regularity condition \eqref{g-reg}, $\xi\in(\ri\Uset)\setminus\aUset$ if and only if the following is true: there exists a unique $\Uset_\xi$-directed semi-infinite geodesic out of every $x\in\Z^2$ and all these geodesics coalesce.
\item\label{th:V2.c}  Under  the jump process condition \eqref{cond:jumpcond} the existence of $x\in\Z^2$ such that $\geo{}{x}{\xi+}=\geo{}{x}{\xi-}$ 
implies that $\geo{}{y}{\xi+}=\geo{}{y}{\xi-}$ for all $y\in\Z^2$,  all these geodesics coalesce, and $\xi\in(\ri\Uset)\setminus\aUset$.
\item\label{th:V2.d} Assume  both the regularity condition \eqref{g-reg} and the jump process condition \eqref{cond:jumpcond}.  Suppose there exists   $x\in\Z^2$  such that $\geo{}{x}{\xi+}=\geo{}{x}{\xi-}$.  Then  there is a unique $\Uset_\xi$-directed semi-infinite geodesic out of every $x\in\Z^2$,  all these geodesics coalesce, and $\xi\in(\ri\Uset)\setminus\aUset$.   
\end{enumerate}
\end{theorem}

By the uniqueness of finite geodesics, 
two   geodesics emanating from the same site $x$ cannot intersect after they separate. Consequently, non-uniqueness of semi-infinite directed geodesics implies the existence of non-coalescing semi-infinite directed geodesics.   
 When both  conditions \eqref{g-reg} and \eqref{cond:jumpcond} hold, Theorem \ref{th:V2}\eqref{th:V2.d}  
shows the converse:   uniqueness     implies   coalescence. 
%However,   non-coalescence does not automatically imply non-uniqueness simply because unique geodesics may fail to coalesce. 
%The converse may, {\it a priori}, not hold. In principle, it might happen that for a given direction $\xi$, out of each site there exists a unique $\Uset_\xi$-directed geodesic, and yet some of these geodesics do not coalesce.
%Using uniqueness of finite geodesics, one quickly sees that non-uniqueness of semi-infinite geodesics with the same asymptotic direction rooted at a single site implies that coalescence of geodesics with that asymptotic direction cannot hold. The converse is not clear: one could imagine, for example, infinitely many disjoint geodesics with the same asymptotic direction.  
%\note{C: Added. Please read. F: reworded..}

We close this section with a theorem that collects those previously established properties of geodesics which hold when both the regularity condition \eqref{g-reg} and the jump process condition \eqref{cond:jumpcond} are in force. 
Lemma \ref{lm:capst-aux} justifies that the geodesics in part \eqref{th:capst.d} are $\xi$-directed rather than merely   $\Uset_\xi$-directed.  
 
\begin{theorem}\label{th:capst}   Assume  the regularity condition \eqref{g-reg} and the jump process condition \eqref{cond:jumpcond}.   The following hold for $\P$-almost every $\w$.
\begin{enumerate}     [label={\rm(\alph*)}, ref={\rm\alph*}]   \itemsep=3pt  
\item\label{th:capst.a} $\xi \in \aUset$ if and only if there exist $x,y \in \bbZ^2$ with $\B{\xi-}(x,y) \neq \B{\xi+}(x,y)$.
\item\label{th:capst.b} $\xi \in \aUset$ if and only if there exists $x \in \bbZ^2$ such that $\xi = \cid(\T_x\w)$.
\item\label{th:capst.c} If $\xi \in (\ri\Uset) \backslash \aUset$, then for each $x \in \bbZ^2$,    
$\geo{}{x}{\xi}=\geo{}{x}{\xi-}=\geo{}{x}{\xi+}$ and this   is the  unique  $\Uset_\xi$-directed semi-infinite geodesic out of $x$. 
%$\geod{}^{x,\xi}$ rooted at $x$ and that satisfies 
%\begin{align}\label{xi-lln}
%\lim_{n\to\infty} \frac{\geod{n}^{x,\xi}}{n} = \xi.
%\end{align}
For any $x,y \in \bbZ^2$, $\geo{}{x}{\xi}$ and $\geo{}{y}{\xi}$ coalesce.
\item\label{th:capst.d} If   $\xi \in \aUset$, then from   each  $x \in \bbZ^2$  there exist at least two   $\xi$-directed semi-infinite  geodesics   that  separate eventually, namely  $\geo{}{x}{\xi-}$ and $\geo{}{x}{\xi+}$. 
  For each pair $x,y \in \bbZ^2$,  $\geo{}{x}{\xi-}$ and $\geo{}{y}{\xi-}$ coalesce and $\geo{}{x}{\xi+}$ and $\geo{}{y}{\xi+}$ coalesce. 
\end{enumerate}

\end{theorem} 

\smallskip

 

%Similarly to Theorem \ref{thm:nonint},  without the regularity condition \eqref{g-reg}, parts \eqref{th:V2.a} and \eqref{th:V2.c} in Theorem \ref{th:V2} leave open the possibility that even though $\geo{}{x}{\xi\pm}$ agree, there may be other $\Uset_\xi$-directed geodesics.


\subsection{Exponential case}
We   specialize to the case where 
	\begin{align}\label{exp-assump}
	\text{$\{\w_x : x \in \bbZ^2\}$ are i.i.d.\ mean one exponential random variables.}
	\end{align} 
%\eqref{exp-assump} is the standing assumption for this section.  
 Rost's classic result \cite{Ros-81} gives the shape function 
%It is shown in \cite[Theorem 3.4]{Fan-Sep-20}  that Condition \eqref{cond:jumpcond} holds under \eqref{exp-assump}. Also, under \eqref{exp-assump}, it is \addmath{reference?} known that 
	\begin{align}\label{exp-shape}
	\gpp(\xi)=%\E[\w_0]
	\bigl(\sqrt{\xi\cdot e_1}+\sqrt{\xi\cdot e_2}\,\bigr)^2,\quad\xi\in\R_+^2.
	\end{align}
 The regularity condition \eqref{g-reg} is satisfied as  $\gpp$ is strictly concave and differentiable on $\ri \Uset$.   The supports $\supp\mu_{x,y}$ are unions of inhomogeneous Poisson processes and hence   the jump process condition \eqref{cond:jumpcond} is satisfied.   This comes from  \cite[Theorem 3.4]{Fan-Sep-20} and is described in Section \ref{sub:palm} below. These two observations imply that the conclusions of Theorem \ref{th:capst} hold. With some additional work, we can go beyond the conclusions of Theorem \ref{th:capst} in this solvable setting.
 % The distribution of the Busemann  measures $\mu_{x,x-e_1}$ for horizontal edges  is  described below in \eqref{Bppa4}.  
 % Thus  Theorem \ref{th:capst} holds in the exponential model. 
%Before moving to the statement of our results in the exponential model, we introduce the notation $\spt{\xi}{x}$ for 

Let $\spt{\xi}{x}$ denote  the location where the $\xi+$ and $\xi-$ geodesics out of $x$ split:
\begin{align}
\spt{\xi}{x} &= \begin{cases}
\text{last point in  } \geo{}{x}{\xi-} \cap \geo{}{x}{\xi+} & \text{ if }\geo{}{x}{\xi-} \neq \geo{}{x}{\xi+}, \\
\infty & \text{ if } \geo{}{x}{\xi-} = \geo{}{x}{\xi+}.
\end{cases}
\end{align}

For part \eqref{th:exp1.c} in the next theorem, recall the finite geodesic $\gamma^{x,y}$ defined below \eqref{G1} and the  competition interface path $\varphi^x$ introduced in Section \ref{s:mult-geo}.   Convergence of paths means that any finite segments eventually coincide. 
  
\begin{theorem}\label{th:exp1}
Assume \eqref{exp-assump}.  Then the conclusions of Theorem \ref{th:capst} hold with $\Uset_\xi=\{\xi\}$ for all $\xi \in \ri \Uset$.  Additionally,  the following  hold $\P$-almost surely. 
\begin{enumerate}     [label={\rm(\alph*)}, ref={\rm\alph*}]   \itemsep=3pt  
\item\label{th:exp1.a} If  $\xi \in \aUset$ then from  each  $x \in \bbZ^2$ there emanate exactly two semi-infinite $\xi$-directed  geodesics that eventually separate, namely  $\geo{}{x}{\xi-}$ and $\geo{}{x}{\xi+}$. 
\item\label{th:exp1.b} For any $\xi \in \ri \Uset$ and any three $\xi$-directed semi-infinite geodesics rooted at any three points, at least two of the geodesics coalesce.
%Nowhere on the lattice do there exist three non-coalescing semi-infinite geodesics with the same asymptotic direction in $\ri\Uset$.   
\item\label{th:exp1.c} Let  $x\in\Z^2$, $\xi\in\ri\Uset$, and let $\{v_n\}_{n\ge m} $ be any sequence on $\Z^2$ such that $v_n\cdot\et=n$ and  $v_n/n \to \xi$.  If  $v_n \prec \varphi_n^{\spt{\xi}{x}}$ for all sufficiently large $n$, then $\gamma^{x,v_n} \to \gamma^{x,\xi-}$ as $n\to\infty$. If $\varphi_n^{\spt{\xi}{x}} \prec v_n$ for all sufficiently large $n$ then $\gamma^{x,v_n} \to \gamma^{x,\xi+}$ as $n\to\infty$.
\item\label{th:exp1:d} For each $x \in \bbZ^2$, the entire collection of semi-infinite geodesics emanating from $x$ is exactly $\bigl\{\geo{}{x}{e_1},\geo{}{x}{e_2},\geo{}{x}{\xi \sigg} : \xi \in \ri \Uset, \sigg \in \{+,-\}\bigr\}$. %CHANGED HERE 
\end{enumerate}
\end{theorem} 

%%%%%%    OLD EXPONENTIAL THEOREM  %%%%%
%\begin{theorem}\label{th:exp1}
%Assume \eqref{exp-assump}.
%%There is a $T$-invariant event $\Omega_0$ with $\bbP(\Omega_0) = 1$ and  such that  
%The following statements hold for $\P$-almost every $\w$.
%\begin{enumerate}     [label={\rm(\alph*)}, ref={\rm\alph*}]   \itemsep=3pt  
%\item\label{th:exp1.a} $\xi \in \aUset$ if and only if there exist $x,y \in \bbZ^2$ with $\B{\xi+}(x,y) \neq \B{\xi-}(x,y)$.
%\item\label{th:exp1.b} $\xi \in \aUset$ if and only if there exists $x \in \bbZ^2$ such that $\xi = \cid(\T_x\w)$.
%\item\label{th:exp1.c} If $\xi \in (\ri \sU) \backslash \aUset$, then for each $x \in \bbZ^2$,    
%$\geo{}{x}{\xi}=\geo{}{x}{\xi+}=\geo{}{x}{\xi-}$ and this   is the  unique semi-infinite $\xi$-directed geodesic out of $x$. 
%%$\geod{}^{x,\xi}$ rooted at $x$ and that satisfies 
%%\begin{align}\label{xi-lln}
%%\lim_{n\to\infty} \frac{\geod{n}^{x,\xi}}{n} = \xi.
%%\end{align}
%For any $x,y \in \bbZ^2$, $\geo{}{x}{\xi}$ and $\geo{}{y}{\xi}$ coalesce.
%\item\label{th:exp1.d} Let  $\xi \in \aUset$.   Then for each  $x \in \bbZ^2$ there exist exactly two semi-infinite $\xi$-directed  geodesics emanating from $x$.  % and satisfying \eqref{xi-lln}.
%These two   are exactly $\geo{}{x}{\xi+}$ and $\geo{}{x}{\xi-}$
%%. For each $x \in \bbZ^2$, $\geo{}{x}{\xi+}$ and $\geo{}{x}{\xi-}$ 
%that eventually separate.  For each pair $x,y \in \bbZ^2$,  $\geo{}{x}{\xi+}$ and $\geo{}{y}{\xi+}$ coalesce and $\geo{}{x}{\xi-}$ and $\geo{}{y}{\xi-}$ coalesce. 
%\end{enumerate}
%\end{theorem}
%%%%%%%%%%  END OLD EXP THEOREM  %%%%%%%

Theorem \ref{th:exp1} resolves a number of previously open problems on the geometry of geodesics in the exponential model. It shows that in all but countably many exceptional directions, the collection of geodesics with that asymptotic direction  coalesce and form a tree. These exceptional directions are identified both with the directions of discontinuity of the Busemann process and the asymptotic directions of competition interfaces.   Moreover, in each exceptional direction $\xi\in \aUset$, ahead of each lattice site $x$, there is a $\xi$-directed  competition interface at which the $\xi-$ and $\xi+$ geodesics out of $x$ split. These are the only two $\xi$-directed geodesics rooted at $x$. Strikingly, each of the two families of $\xi-$ and $\xi+$ geodesics has the same structure as the collection of  geodesics in a typical direction: each family forms a tree of coalescing semi-infinite paths.

 
%In particular, almost surely, there is no direction in $\ri\Uset$  in which there are three or more disjoint semi-infinite geodesics  from any three lattice sites.  The reason is that among three geodesics, two must have the same sign $+$ or $-$ and hence these two coalesce.  

 Theorem \ref{th:exp1} utilizes  Theorem \ref{thm-Coupier}, due to Coupier \cite{Cou-11}, that rules out three geodesics that have the same direction,  emanate from a common vertex, and eventually separate.    It appears that the modification argument of \cite{Cou-11} cannot rule out three non-coalescing geodesics from distinct roots, and so  Theorem \ref{th:exp1}\eqref{th:exp1.b}   significantly extends Theorem \ref{thm-Coupier}. 
 
Finally, Theorem \ref{th:exp1} gives a complete description of the coalescence structure of finite geodesics to semi-infinite geodesics in the exponential model. Part \eqref{th:exp1.c} says that if we consider a sequence of lattice sites $v_n$ with asymptotic direction $\xi$, then the geodesic from $x$ to $v_n$ will converge to the $\xi-$ geodesic out of $x$ if and only if $v_n$ eventually stays to the left of the competition interface emanating from the site $\spt{\xi}{x}$ where the $\xi-$ and $\xi+$ geodesics out of $x$ separate. Similarly it will converge to the $\xi+$ geodesic if and only if it stays to the right of that path. The competition interface lives on the dual lattice, so for large $n$ every point  $v_n$ is either to the left or to the right of the competition interface. The coalescence structure of semi-infinite geodesics to arbitrary sequences $v_n$ with $v_n/n \to \xi$ then follows by passing to subsequences.

 The results of Section \ref{s:Bmeas}  are proved in Section \ref{sec:bus}, except   Lemma \ref{lm:downright} which is proved  at the end of Section \ref{shockgraphs:pfs}.



 


==> JEMS Post-Accept Revision/GeoWebPaper-Sec4.tex <==
% !TEX root = GeoWebPaper.tex

\section{Last-passage percolation as a dynamical system} \label{sec:LPPDS}

After the general description of uniqueness and coalescence of Section \ref{s:Bmeas}, we take a closer look at the spatial structure of the set of lattice points where particular values or ranges of values from the set  $\aUset$ of exceptional directions appear. (Recall its definition \eqref{df:aUset}.)  
As mentioned in the introduction, there is a connection to instability in noise-driven conservation laws.  The next section explains this  point of view.  

\subsection{Discrete Hamilton-Jacobi equations}\label{s:HJ}
We take a dynamical point of view of LPP.   Time proceeds in the negative diagonal direction $-\et=-e_1-e_2$ and the spatial axis is $\ex=e_2-e_1$.  For each $t\in\Z$, the spatial level at time $t$ is $\level_{t}=\{x\in\Z^2: x\cdot \et=t\}$.    For $x\in\Z^2$ and $A\subset\Z^2$ let $\Pi_x^A$ denote the set of up-right paths $\pi_{k,m}$ such  that  $\pi_k=x$ and $\pi_m\in A$, where $k=x\cdot\et$ and $m$ is any integer $\ge k$ such that $A\cap\level_m\ne\varnothing$.  For each $\xi\in\ri\Uset$ and sign $\sigg\in\{-,+\}$,    the Busemann function $\B{\xi\sig}$ satisfies the following equation:   for all $t\le t_0$ and $x\in\level_{t}$, 
\be\label{hj8} 
\B{\xi\sig}(x,0)= \max\Bigl\{ \, \sum_{i=t}^{t_0-1} \w_{\pi_i} +  \B{\xi\sig}(\pi_{t_0}, 0)  :  \pi\in\Pi_x^{\level_{t_0}} \Bigr\} . 
\ee
The unique   maximizing path  in \eqref{hj8} is the geodesic segment  $\geo{t,t_0}{x}{\xi\sig}$.  

Equation  \eqref{hj8} can be viewed as a discrete Hopf-Lax-Oleinik semigroup.   
For example, equation \eqref{hj8} is an obvious  discrete analogue of the variational formula (1.3) of \cite{Bak-Cat-Kha-14}.  At first blush  the two formulas appear different because  (1.3) of \cite{Bak-Cat-Kha-14} contains a  kinetic energy term.  However, this term is not needed in \eqref{hj8} above  because all admissible steps are of size one and all paths between  levels $\level_{t}$ and $\level_{t_0}$ have equal length (number of steps).   

Through this analogy with a Hopf-Lax-Oleinik semigroup we can regard  $\B{\xi\sig}(\bbullet\,,0)$   as a global solution of a discrete stochastic Hamilton-Jacobi equation started in the infinite past ($t_0\to\infty$) and driven by the noise $\w$.  The spatial difference $\B{\xi\sig}(x+e_1, x+e_2)=\B{\xi\sig}(x+e_1, 0)-\B{\xi\sig}(x+e_2,0)$ can then be viewed as a global solution of a discretized stochastic Burgers equation.  %Article  \cite{Jan-Ras-19-pams-} presents  a more detailed view of this connection. 
%Theorem 3.2(f)

%\subsection{Flow of Busemann measures} 

By Lemma \ref{lem:buselln}, if $\gpp$ is differentiable on $\ri\Uset$, then  
$\B{\xi+}$ and $\B{\xi-}$ both satisfy for each $x \in \bbZ^2$
\begin{align*}
\lim_{\abs{n}\to\infty} \frac{\B{\xi\pm}\left(x,x+n\ex \right)}{n} &= \nabla \gpp(\xi)\cdot\ex.
\end{align*} 
Thus, $\B{\xi\pm}$ are two solutions with the same value of the conserved quantity.
%Lemma 3.1 in \cite{Jan-Ras-19-pams-} shows that the asymptotic velocity is the conserved quantity of this discrete stochastic Burgers equation. 
Under the jump process condition \eqref{cond:jumpcond}, $\xi \in \supp \mu_{x+e_1,x+e_2}$ if and only if $\B{\xi+}(x+e_1,x+e_2) \neq \B{\xi-}(x+e_1,x+e_2)$.  
This means that the locations $x$ where $\xi \in \supp \mu_{x+e_1,x+e_2}$ are precisely the space-time points at which the two solutions $\B{\xi\pm}$ differ. 
It is reasonable to expect then that these points are locations of instability in the following sense. The spatial differences of the solution to the stochastic Hamilton-Jacobi equation started at time $t_0$ with a linear initial condition dual to $\xi$,
	\[\max\{G_{x+e_1,y}-y\cdot\nabla\gpp(\xi):y\cdot\et=t_0\}-\max\{G_{x+e_2,y}-y\cdot\nabla\gpp(\xi):y\cdot\et=t_0\},\]
has at least two limit points $\B{\xi\pm}(x+e_1,x+e_2)+(e_1-e_2)\cdot\nabla\gpp(\xi)$ as $t_0\to\infty$.  
This is supported by simulations and is hinted at by Theorem \ref{th:exp1}\eqref{th:exp1.c}.

%By Theorem \ref{thm:nonint}, $\xi \in \supp \mu_{x+e_1,x+e_2}$ if and only if $\geo{}{x+e_2}{\xi-}\cap\geo{}{x+e_1}{\xi+}=\varnothing$. 
%This is analogous to two distinct Lagrangian minimizers from the infinite past terminating at a shock. 
%% that two minimizers terminate at a shock point in a scalar conservation law.
%%On the other hand, under condition \eqref{g-reg}, the family $\{\B{\xi+}(x,y) : x,y \in \bbZ^2\}$ generates the rightmost  $\Uset_{\xi}$-directed geodesics out of each site. Similarly $\{\B{\xi-}(x,y) : x,y \in \bbZ^2\}$ generates the leftmost geodesics. This is analogous to the picture one sees in the continuous space Burgers equation by taking spatial left and  right limits.  In this sense, we can think of the condition $\B{\xi+}(x+e_1,x+e_2) \neq \B{\xi-}(x+e_1,x+e_2)$ as being analogous to the left and right gradients of a solution differing at these sites, which is the usual definition of a shock in the continuous setting.  Even without condition \eqref{cond:jumpcond}, \medskip
%Significant attention has been devoted to understanding the statistics and structure of shocks in the continuous  stochastic Burgers equation \cite{Sin-92,E-etal-00,Bec-Kha-07,Bak-Kha-18,Bak-16}.
%%going back to the seminal work of Sinai in \cite{Sin-92}. Shocks have also attracted substantial attention in recent years \cite{E-etal-00,Bec-Kha-07,Bak-Kha-18,Bak-16}. 
%%\cite{Kha-Zha-17} (higher dimentions, compact setting)
%%
%Our interest in the present section is to introduce a natural notion of a shock in our setting, which essentially agrees with the previous description. 
With these points in mind, we now define what we mean by instability points and then turn to studying their geometric structure. Proofs of the results of this section appear in Section \ref{sec:webpf}. 

%Now suppose in addition that the jump process condition \eqref{cond:jumpcond} holds. Let $h(\xi)=-\nabla\gpp(\xi)$ and for $h\in\R^2$ define the point-to-line passage time from $x\in\Z^2$ with $x\cdot\et\le n$ to level $n\in\Z$, with {\it tilt} (or {\it external field}) $h$ by
%	\begin{align*}
%	G_{x,(n)}^{h} &= \max_{y:y\cdot\et=n} (G_{x,y}+h\cdot y).
%	\end{align*}
%The point-to-line analogue of \cite[Theorem 6.1]{Geo-Ras-Sep-17-ptrf-1} (which generalizes (3.3) therein) can be generalized to hold for all directions $\xi\in\ri\Uset$ simultaneously, outside one null set of weights $\w$. See \cite[Theorem 4.14]{Jan-Ras-20-aop} and \cite[Lemma 4.11]{Sep-18} for, respectively, the positive-temperature (general weights) and zero-temperature (exponential weights) point-to-point versions of such a theorem. \textcolor{red}{(Chris and I are planning to have a statement in the 1F1S paper... So we can eventually point to that!)}  The result is that, for $\P$-almost every $\w$, for all $\xi\in\ri\Uset$ and $x\in\Z^2$,
%	\begin{align*}
%	\B{\xi-}(x+e_1,x+e_2)&\le\varliminf_{n\to\infty}(G_{x+e_1,(n)}^{h(\xi)}-G_{x+e_2,(n)}^{h(\xi)})  \\
%	&\le\varlimsup_{n\to\infty}(G_{x+e_1,(n)}^{h(\xi)}-G_{x+e_2,(n)}^{h(\xi)}) 
%	\le \B{\xi+}(x+e_1,x+e_2).
%	\end{align*}
%Under the jump process condition \eqref{cond:jumpcond}, $\xi\in\aUset$ is equivalent to $\B{\xi-}(x+e_1,x+e_2)<\B{\xi+}(x+e_1,x+e_2)$. 
%But then, we have
%	\[ \varlimsup_{n\to\infty}(G_{x+e_1,(n)}^{h(\zeta)}-G_{x+e_2,(n)}^{h(\zeta)}) \le \B{\zeta+}(x+e_1,x+e_2) \le \B{\xi-}(x+e_1,x+e_2)<\B{\xi+}(x+e_1,x+e_2)\]
%	and
%	\[ \varliminf_{n\to\infty}(G_{x+e_1,(n)}^{h(\eta)}-G_{x+e_2,(n)}^{h(\eta)}) \ge \B{\eta-}(x+e_1,x+e_2) \ge \B{\xi+}(x+e_1,x+e_2)>\B{\xi-}(x+e_1,x+e_2)\]
%for any $\zeta,\eta\in\ri\Uset$ with $\zeta\prec\xi\prec\eta$.  
%
%This shows that the infinite horizon problem (the one where we push the constant initial condition to the remote past and try to take a limit) is 
%\addmath{need to say that $\B{\xi\pm}(x+e_1,x+e_2)$ is the analogue of the solution at $x^*$}
%unstable at the shock points $x^*\in\shock{\xi}$, because the limits are discontinuous as the we vary the parameter (the direction), crossing $\xi$.    
%%Then, the solution is unstable in the sense that no matter how close we get $\zeta$ to $\xi$, the limit with tilt $h(\zeta)$ will remain separated by at least $B_{x^*}-\B{\xi-}_{x^*}>0$. The other case is similar.    
%On the other hand, if $x^*\not\in\shock{\xi}$, then $\B{\xi\pm}(x+e_1,x+e_2)$ match and under the jump process condition \eqref{cond:jumpcond}, $\B{\zeta\pm}(x+e_1,x+e_2)=\B{\xi}(x+e_1,x+e_2)$ for $\zeta$ close enough to $\xi$.  Therefore, 
%we have 
%	\[ \lim_{n\to\infty}(G_{x+e_1,(n)}^{h(\zeta)}-G_{x+e_2,(n)}^{h(\zeta)}) = \B{\xi}(x+e_1,x+e_2)\]
%for all such $\zeta$ and we see that the solution is stable at $x^*$.\smallskip
%
%In words, $\aUset$ is exactly the set of directions for which the One-Force One-Solution (1F1S) principle fails, and for these directions, $\shock{\xi}$ is exactly the set of points at which this principle does not hold. \note{This is not correct, right? Showing that 1F1S actually fails would require us starting with a fixed initial condition and showing that the limit fails to hold.}


\subsection{Webs of instability}\label{sec:web} 
For a direction  $\xi \in \ri \Uset$ and a sign $\sigg\in\{-,+\}$,   let $\G{\xi\sig}$ be the directed graph whose vertex set is  $\bbZ^2$ and  whose  edge  set includes  $(x, x+e_i)$  whenever $\geo{m+1}{x}{\xi\sig} = x + e_i$. Here $m=x\cdot\et$  and we consider both $i\in\{1,2\}$.   These are the directed graphs of $\xi\sigg$ geodesics defined by  \eqref{d:bgeo}. By construction, each $\G{\xi\sig}$ is a disjoint union of trees, i.e.\ a forest, and for each $x \in \Z^2$, the geodesic $\geo{}{x}{\xi\sig}$ follows the directed edges of   $\G{\xi\sig}$. 
%By Theorem \ref{thm:+-coal}, under the jump process condition \eqref{cond:jumpcond} each  $\G{\xi\sig}$ is a  tree. 
%Theorem \ref{thm1}\eqref{thm1:biinf} says that for a fixed $\xi\in\ri\Uset$ and $\w\in\Omega_\xi^3$, $\G{\xi\sig}$ does not contain any bi-infinite up-right paths.
%\timonote{Think about removing last two sentences.} 	

Recall the vectors    $\etstar=\et/2= (e_1 + e_2)/2$  and $\exstar=\ex/2=(e_2-e_1)/2$. 
Let $\dG{\xi\sig}$ be the directed graph whose vertex set is the dual lattice $\Z^{2*}=\etstar+\bbZ^2$ and whose edge set is defined by this rule:  for each $x\in\bbZ^2$,  on the dual lattice $x+\etstar$ points to $x+\etstar-e_i$ in $\dG{\xi\sig}$ if and only if on the original lattice  $x$ points to $x+e_i$ in $\G{\xi\sig}$.   Pictorially this means that $\dG{\xi\sig}$ contains all the  south and west  directed nearest-neighbor  edges of  $\Z^{2*} $  that do not  cross an edge of $\G{\xi\sig}$.     See Figure \ref{fig:trees} for an illustration.

\begin{figure}[h]
\centering
 		 \begin{tikzpicture}[scale=1,>=stealth]
			\begin{scope}
			\draw(0,-.5)--(0,1.5);
			\draw(1,-.5)--(1,1.5);
			\draw(-.5,0)--(1.5,0);
			\draw(-.5,1)--(1.5,1);
			\draw[color=darkblue,line width=2pt,->](0,0)--(0,1);
			\draw[color=nicos-red,line width=1pt,->](.5,.5)--(.5,-.5);
			\draw[fill=black](0,0) circle(2pt);
			\draw(-.05,-0.15)node[left]{$x$};
			\draw[fill=white](.5,.5) circle(2pt);
			\draw(0.5,0.62)node[right]{$x^*=x+\etstar$};
			\end{scope}
			
			\begin{scope}[shift={(0,2.5)}]
			\draw(0,-.5)--(0,1.5);
			\draw(1,-.5)--(1,1.5);
			\draw(-.5,0)--(1.5,0);
			\draw(-.5,1)--(1.5,1);
			\draw[color=darkblue,line width=2pt,->](0,0)--(1,0);
			\draw[color=nicos-red,line width=1pt,->](.5,.5)--(-.5,.5);
			\draw[fill=black](0,0) circle(2pt);
			\draw(-.05,-.15)node[left]{$x$};
			\draw[fill=white](.5,.5) circle(2pt);
			\draw(0.5,0.62)node[right]{$x^*=x+\etstar$};
			\end{scope}			
		\end{tikzpicture}
		\hspace{2cm}
\includegraphics[trim={5.4cm 15.6cm 7.5cm 3.6cm},clip,width=5cm]{Figs/trees-standalone}%\hspace{1.5cm}
%\includegraphics[trim={5.4cm 15.6cm 7.5cm 3.6cm},clip,width=4cm]{Figs/trees2-standalone}
\caption{\small  Left plot: An illustration of the duality relation between the edges of $\G{\xi{\scriptscriptstyle{\boxempty}}}$ (black/thick) and those of $\dG{\xi{\scriptscriptstyle{\boxempty}}}$ (red/thin). Right plot: An illustration of a (blue/thick) north-east directed  geodesic graph $\G{\xi{\scriptscriptstyle{\boxempty}}}$   and its (red/thin) south-west directed  dual $\dG{\xi{\scriptscriptstyle{\boxempty}}}$.}
%\caption{\small  An illustration of a (blue/thick) north-east directed  geodesic graph $\G{\xi\sig}$   and its (red/thin) south-west directed  dual $\dG{\xi\sig}$.}
%Two simulations of the (blue/thick)  geodesic graphs ($\G{\xi+}$ or $\G{\xi-}$) and its (red/thin) dual. 
%Weights are i.i.d.\ exponential(1). $\xi=(e_1+e_2)/2$ on the left and $\xi=(2e_1+e_2)/3$ on the right. }
\label{fig:trees}\end{figure}


For  $\zeta\preceq\eta$ in $\ri\Uset$ let  the graph 
%\addmath{use $\dG{\cup[\zeta, \eta]}$ instead?}
$\dS{[\zeta,\eta]}$ be the union of  the graphs $\dG{\xi\sig}$ over $\xi\in[\zeta,\eta]$ and $\sigg\in\{-,+\}$.
 That is, the vertex set of  $\dS{[\zeta,\eta]}$ is $\Z^{2*}$, and the edge set of  $\dS{[\zeta,\eta]}$ is the union of the  edge sets of $\dG{\xi\pm}$ over $\xi\in[\zeta,\eta]$.   From each point $x^*\in\Z^{2*}$   a directed edge of $\dS{[\zeta,\eta]}$ points to $x^*-e_1$ or $x^*-e_2$ or both.  Due to  the monotonicity \eqref{mono} of the Busemann functions,   $\dS{[\zeta,\eta]}$ is  the union of just the two  graphs $\dG{\zeta-}$ and $\dG{\eta+}$.  In particular,   $x^*$ points to $x^*-e_2$ in $\dS{[\zeta,\eta]}$ if and only if $x^*-\etstar$ points to $x^*+\exstar$ in $\G{\zeta-}$, and 
 $x^*$ points to $x^*-e_1$ in $\dS{[\zeta,\eta]}$ if and only if $x^*-\etstar$  points to $x^*-\exstar$ in $\G{\eta+}$.
%due to the monotonicity that forces horizontal arrows in $\G{\xi-}$ to be also in $\G{\xi+}$ and a similar story for vertical arrows.


Identify the space-time point % $x^* \in \etstar+\bbZ^2$ 
$x+ \etstar \in\bbZ^{2*}$
on the dual lattice with the diagonal edge that connects $x+e_1$ and $x+e_2$
%$x^*+\exstar$ and $x^*-\exstar$ 
on the primal lattice (see Figure \ref{fig:dual}).
 %For example, $0^*=(e_1+e_2)/2$.  %%% Timo: thought this was unnecessary here. 
 %\addmath{dispense with the $A$-shock point and just focus on the type of $A$ we actually use?}
% For a subset $A\subset\ri\Uset$, $\w\in\Omega$, and $x \in \bbZ^2$, we say there is an $A$-{\it shock point} in configuration $\w$  at the dual lattice point $x^*=x+\etstar$ whenever   $A\cap\supp\mu_{x+e_1,x+e_2}\neq\varnothing$. 
Call the dual lattice point $x^*=x+\etstar$  a $[\zeta, \eta]$-{\it instability point}  if $[\zeta, \eta]\cap\supp\mu_{x+e_1,x+e_2}\neq\varnothing$.   
%As mentioned earlier in \eqref{mu=|mu|}, $\supp{\mu_{x+e_1,x+e_2}}=\supp\mu_{x+e_1,x+e_2}$.
%For $\zeta\prec\eta$ we 
%say $x^*$ is a $(\zeta,\eta)$-shock point if it is a $A$-shock point with $A=\{t\zeta+(1-t)\eta:0<t<1\}$. 
If $\zeta=\eta=\xi$,  call  $x^*$  a {\it $\xi$-instability point}.   
Denote the set of $[\zeta,\eta]$-instability points   by $\shock{[\zeta,\eta]}$,  with  $\shock{\xi}=\shock{[\xi,\xi]}$.  
$\shock{[\zeta,\eta]}$ is the union of $\shock{\xi}$ over $\xi\in[\zeta,\eta]$.
    Theorem \ref{thm:nonint} and the ordering \eqref{path-ordering}  of geodesics give the following characterization in terms of disjoint geodesics, alluded to in Section \ref{s:HJ}. 

\begin{figure}%[h]
 	\begin{center}
 		 \begin{tikzpicture}[scale=1,>=stealth]
			\draw(0,1)--(1,0);
			\draw[fill=black](1,0) circle(2pt);
			\draw[fill=black](0,1) circle(2pt);
			\draw[fill=black](0,0) circle(2pt);
			\draw[fill=white](.5,.5) circle(2pt);
			\draw(0,-0.5)--(0,1.5);
			\draw(1,-0.5)--(1,1.5);
			\draw(-.5,0)--(1.5,0);
			\draw(-.5,1)--(1.5,1);
			\draw[dashed](-.5,0.5)--(1.5,0.5);
			\draw[dashed](.5,-0.5)--(.5,1.5);
			\draw(0,-.2)node[left]{$x$};
			\draw(.45,.75)node[right]{$x^*$};
			\draw(0,1.2)node[left]{$x+e_2$};
			\draw(1,-.2)node[right]{$x+e_1$};
			
		\end{tikzpicture}
 	 \end{center}
 	\caption{\small  The edge $(x+e_1,x+e_2)$ is identified with the dual point $x^*=x+\etstar$.}
 \label{fig:dual}
 \end{figure}



\begin{lemma}\label{lem:shockequiv} 
The following holds for $\bbP$-almost every $\w$.   Let $\zeta\preceq\eta$, including the case $\zeta=\eta=\xi$.     Let $x\in\Z^2$ and   $x^*=x+\etstar$.   Then $x^*\in\shock{[\zeta,\eta]}$    if and only if $\geo{}{x+e_2}{\zeta-}\cap\geo{}{x+e_1}{\eta+}=\varnothing$. 
\end{lemma}

%%%%%%%%     OLD VERSION WITH (a)-(b)  %%%%%%
%\begin{lemma}\label{lem:shockequiv} 
%The following holds for $\bbP$-almost every $\w$ and every $x\in\Z^2$.  Let  $x^*=x+\etstar$.  
%\begin{enumerate}     [label={\rm(\alph*)}, ref={\rm\alph*}]   \itemsep=3pt  
%\item For $\zeta\prec\eta$ in $\ri\Uset$,  $x^*\in\shock{[\zeta,\eta]}$    if and only if $\geo{}{x+e_2}{\zeta-}\cap\geo{}{x+e_1}{\eta+}=\varnothing$. 
%\item  For $\xi\in\ri\Uset$,  $x^*\in\shock{\xi}$  if and only if $\geo{}{x+e_2}{\xi-}\cap\geo{}{x+e_1}{\xi+}=\varnothing$.
%\end{enumerate} 
%\end{lemma}
%%%%%%%%     OLD VERSION WITH (a)-(b)  %%%%%%



 

%$\xi$-shock points are in a sense analogous to the locations of shocks in (bi-infinite in time) global solutions of Burgers equation. 




%x^* is a [\zeta,\eta]-shock iff \supp\mu_{x+e_1,x+e_2} intersects [\zeta,\eta] iff 
%\exists\xi\in[\zeta,\eta] s.t. \xi\in\supp\mu_{x+e_1,x+e_2} iff \exists \xi\in[\zeta,\eta] s.t. x^* is a \xi-shock. 
  Let  the {\it instability graph} $\shockG{[\zeta,\eta]}$ be the subgraph of $\dS{[\zeta,\eta]}$  with vertex set $\shock{[\zeta,\eta]}$ and those  directed edges of $\dS{[\zeta,\eta]}$  that point  from some  $x^*\in\shock{[\zeta,\eta]}$ to  a point 
$x^*-e_i\in\shock{[\zeta,\eta]}$, for either  $i\in\{1,2\}$.  (The proof of  Theorem  \ref{thm:shock1} in Section \ref{shockgraphs:pfs}  shows that {\it every} edge of $\dS{[\zeta,\eta]}$ that emanates from a point of $\shock{[\zeta,\eta]}$ is in fact an edge of  $\shockG{[\zeta,\eta]}$.)   

In the  case $\zeta=\eta=\xi$ write  $\shockG{\xi}$ for   $\shockG{[\xi,\xi]}$.  Explicitly,  the vertices of $\shockG{\xi}$ are dual points $x+\etstar$ such that $\xi\in\supp\mu_{x+e_1,x+e_2}$ and the edges are those of $\dG{\xi-}\cup\dG{\xi+}$ that connect these points.  

The graph $\shockG{[\zeta,\eta]}$ is also the edge union of the graphs $\shockG{\xi}$  over $\xi\in[\zeta, \eta]$. To see this, let $x^*=x+\etstar$.  If $\xi=\cid(T_x\w)\in[\zeta, \eta]$ then  $\shockG{\xi}$ contains both edges from $x^*$ to $x^*-e_1$ and $x^*-e_2$, as does $\shockG{[\zeta,\eta]}$.    If $\cid(T_x\w)\notin[\zeta, \eta]$ then in  $\shockG{\xi}$ and in $\shockG{[\zeta,\eta]}$, $x^*$ points to   the same vertex $x^*-e_i$.  

%Write $\shock{\xi}$ and $\shockG{\xi}$ for $\shock{[\xi,\xi]}$ and $\shockG{[\xi,\xi]}$. 
%It follows   that   $\shock{[\zeta,\eta]}$ is the union of $\shock{\xi}$ over $\xi\in[\zeta,\eta]$.

 \begin{remark}
By the continuity \eqref{pmgeolim} and the fact that the support of a measure is a closed set we get that almost surely, 
for any $\zeta\preceq\eta$ in $\ri\Uset$ and for any finite box $[-L,L]^2\cap\Z^2$, $\shockG{[\zeta',\eta']}=\shockG{[\zeta,\eta]}$ on the entire box, for $\zeta'\prec\zeta$ close enough to $\zeta$ and $\eta'\succ\eta$ close enough to $\eta$.
This explains why the two top graphs in Figure \ref{fig:shocks2b} are identical and are in fact equal to $\shockG{\xi}$.
 \end{remark} 


The message of the  next theorem is that  instability points exist for all exceptional directions in $\aUset$, and these  instability points arrange themselves on  bi-infinite directed paths  in the instability graphs.


\begin{theorem}\label{thm:shock1}
The following holds for $\bbP$-almost every $\w$. Pick any $\zeta\preceq\eta$ in $\ri\Uset$ such that  $[\zeta,\eta]\cap\,\aUset\ne\varnothing$, including   the case $\zeta=\eta=\xi$.    Then the  instability graph $\shockG{[\zeta,\eta]}$ is an infinite directed graph.   Furthermore,  $\shockG{[\zeta,\eta]}$ equals the union of the bi-infinite directed paths of the graph $\dG{\cup[\zeta,\eta]}$.   In the backward {\rm(}north and east{\rm)} orientation, each such path is $[\zetamin,\etamax]$-directed. 
\end{theorem} 

In particular,   if $x^*\in\shock{[\zeta,\eta]}$ and $m=x^*\cdot\et$,  there exists a bi-infinite sequence $\{x^*_n\}_{n\in\Z}\subset\shock{[\zeta,\eta]}$ such that $x^*_m=x^*$ and for each $n$,   $x^*_n\cdot\et=n$ and  $x^*_n$ points to  $x^*_{n-1}$   in the graph $\shockG{[\zeta,\eta]}$.  As $n\to\infty$,  the limit points of $n^{-1}x^*_n$ lie in $[\zetamin,\etamax]$. 


%%%%%%%%  OLD VERSION  %%%%%%%
%\begin{theorem}\label{thm:shock1}
%The following holds for $\bbP$-almost every $\w$. Pick any $\zeta\preceq\eta$ in $\ri\Uset$ such that  $[\zeta,\eta]\cap\,\aUset\ne\varnothing$, including   the case $\zeta=\eta=\xi$.    Then the  shock graph $\shockG{[\zeta,\eta]}$ is an infinite directed graph. Every point of $\shock{[\zeta,\eta]}$ lies on a bi-infinite directed path in the graph $\shockG{[\zeta,\eta]}$.  That is, if $x^*\in\shock{[\zeta,\eta]}$ and $m=x^*\cdot\et$,  there exists a bi-infinite sequence $\{x^*_n\}_{n\in\Z}\subset\shock{[\zeta,\eta]}$ such that $x^*_m=x^*$ and for each $n$,   $x^*_n\cdot\et=n$ and  $x^*_n$ points to  $x^*_{n-1}$   in the graph $\shockG{[\zeta,\eta]}$.  Every such path is $[\zetamin,\etamax]$-directed:  as $n\to\infty$,  the limit points of $n^{-1}x^*_n$ lie in $[\zetamin,\etamax]$. 
%\end{theorem} 

%%%%%%%%  EVEN  OLDER VERSION  %%%%%%%
%\begin{enumerate}[label={\rm(\alph*)}, ref={\rm\alph*}] \itemsep=3pt 
%\item\label{thm:shocks.0} Shock points exist: $\shock{[\zeta,\eta]}\neq\varnothing$.
%\item\label{thm:shocks.a} Any path that starts at a shock point $x^*\in\shock{[\zeta,\eta]}$ and takes steps in $\{-e_1,-e_2\}$ along edges of the graph $\dS{[\zeta,\eta]}$  remains entirely in the graph $\shockG{[\zeta,\eta]}$.   In particular,  each $x^*\in\shock{[\zeta,\eta]}$ is the starting point of an infinite directed  path in $\shockG{[\zeta,\eta]}$. 
%has all its vertices in $\shock{[\zeta,\eta]}$ and is hence a path in $\shockG{[\zeta,\eta]}$. 
%\item\label{thm:shocks.b} For any point $x^*\in\shock{[\zeta,\eta]}$, there exists a semi-infinite  up-right path $x^*_{m,\infty}$ of points in $\shock{[\zeta,\eta]}$ emanating from $x^*_m=x^*$ and such that for all $n\ge m$, $x^*_{n+1}-x^*_n\in\{e_1,e_2\}$ and $x^*_{n+1}$ is a parent of $x^*_n$ in $\shockG{[\zeta,\eta]}$. All such paths are $[\zetamin,\etamax]$-directed. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%    faulty convergence lemma commented away 
% The next  lemma states a  convergence property. 
%See Figures \ref{fig:shocks2a} and \ref{fig:shocks2b} for an illustration.
%
%\begin{lemma}
%%There exists a $T$-invariant event $\Omega_0$ with $\P(\Omega_0)=1$ and such that 
%The following holds for $\bbP$-almost every $\w$. 
%%For any $\zeta\preceq\zeta'\preceq\eta'\preceq\eta$ in $\ri\Uset$, $\shock{[\zeta',\eta']}\subset\shock{[\zeta,\eta]}$, $\dS{[\zeta',\eta']}\subset\dS{[\zeta,\eta]}$, and $\shockG{[\zeta',\eta']}\subset\shockG{[\zeta,\eta]}$. 
%For any $L\in\N$ and $\zeta\prec\eta$ in $\ri\Uset$ there exists an $\e>0$ such that if $\abs{\zeta'-\zeta}_1<\e$ and $\abs{\eta'-\eta}_1<\e$, then $\shock{[\zeta',\eta']}=\shock{[\zeta,\eta]}$, $\dS{[\zeta',\eta']}=\dS{[\zeta,\eta]}$, and $\shockG{[\zeta',\eta']}=\shockG{[\zeta,\eta]}$ inside the finite square  $[-L,L]^2\cap\Z^{2*}$. 
%\end{lemma}
%the proof uses monotonicity and the fact that the support is a closed set
%%%%%%%%    faulty convergence lemma end  %%%%%%%%%%

\begin{figure}[h]
\centering
\includegraphics[width=0.45\textwidth]{Figs/shocks_n500-1.pdf}\ \ \ 
\includegraphics[width=0.45\textwidth]{Figs/shocks_n500-2.pdf}
\includegraphics[width=0.45\textwidth]{Figs/shocks_n500-3.pdf}\ \ \ 
\includegraphics[width=0.45\textwidth]{Figs/shocks_n500-4.pdf}
\caption{\small  Four nested down-left pointing  $\shockG{[\zeta,\eta]}$ graphs in the square  $[-100,100]^2$. Top to bottom, left to right, in reading order, 
%$[\zeta,\eta]$ equals  $[(0.096,0.904),(0.772,0.228)]$, $[(0.219,0.781),(0.595,0.405)]$, $[(0.318,0.682),(0.476,0.524)]$, and $[(0.355,0.645),(0.436,0.564)]$.  
$[\zeta\cdot e_1,\eta\cdot e_1]$ equals  $[0.096,0.772]$, $[0.219,0.595]$, $[0.318,0.476]$, and $[0.355,0.436]$.  
Two further nested subgraphs appear in Figure \ref{fig:shocks2b}.  
In the simulation the weights were exponentially distributed and we chose the direction $\xi$ to be a jump point of the Busemann process on the edge $(0,e_1)$.}
%In the simulation we chose the direction $\xi$ to be the jump of the Busemann process on the edge $(0,e_1)$ 
%such that $\xi\cdot e_1$ is maximal in $[0,0.6]$.} %\textcolor{red}{(to guarantee $\alpha$ is far from $1$, to control the truncation for the vertical edges.)}}
\label{fig:shocks2a}\end{figure}

\begin{figure}[h]
\centering
\includegraphics[width=0.45\textwidth]{Figs/shocks_n500-5.pdf}\ \ \ 
\includegraphics[width=0.45\textwidth]{Figs/shocks_n500-6-2.pdf}
\includegraphics[width=0.45\textwidth]{Figs/shocks_n500-zoom2.pdf}\ \ \  
\includegraphics[width=0.45\textwidth]{Figs/shocks_n500-zoom1.pdf}
\caption{\small  Continuing with the simulation setting of Figure \ref{fig:shocks2a}, the top two pictures  are $\shockG{[\zeta,\eta]}$ graphs in $[-100,100]^2$ with 
%$[\zeta,\eta]=[(0.374,0.626),(0.417,0.583)]$ (left) and $[(0.393,0.607),(0.397,0.603)]$ (right). 
$[\zeta\cdot e_1,\eta\cdot e_1]=[0.374,0.417]$ (left) and $[0.393,0.397]$ (right). 
The two graphs are in fact identical.  The  pictures on the second row zoom into the framed squares of the  top right picture, the left one into the square $[-20,20]^2$ and  the right  one into $[-10,10]^2$.  Besides the down-left pointing red $\shockG{[\zeta,\eta]}$ graphs, the bottom pictures include   the up-right pointing graphs $\G{\zeta-}$ (green/lighter) and $\G{\eta+}$ (purple/darker).  Whenever $\G{\zeta-}$  and $\G{\eta+}$ separate at $x$,    green points up and purple points right, and  $\shockG{[\zeta,\eta]}$ has a branch point at $x+\etstar$.   The blue/green trees that occupy the islands surrounded by red paths are described in Section \ref{sec:Busflow}. 
% The weights and the direction $\xi$ in this simulation are the same as the ones in Figure \ref{fig:shocks2a}. Thus, the graphs on the first row are subgraphs of the ones in Figure \ref{fig:shocks2a}.
}
\label{fig:shocks2b}\end{figure}


% About the graph.   $\G{\zeta-}$ (green/lighter) and $\G{\eta+}$ (purple/darker).  These point together except when green up and purple right.  

Next we   describe  the branching and coalescing of the bi-infinite directed paths that make up   the  graph $\shockG{[\zeta,\eta]}$.  
If there is a  directed path  in the graph $\shockG{[\zeta,\eta]}$  from $y^*$ to $x^*$, then   $y^*$ is an {\it ancestor} of $x^*$ and  equivalently  $x^*$ is a {\it descendant} of $y^*$.  
%If the path from $y^*$ to $x^*$ is  a single edge, in which case  $x^*\in\{y^*-e_1,y^*-e_2\}$,  we say that $y^*$ is a {\it parent} of $x^*$ and $x^*$ is an {\it offspring} of $y^*$.
Let $\ans{[\zeta,\eta]}{x^*}$ denote the set of ancestors of $x^*$ in the graph $\shockG{[\zeta,\eta]}$.  Abbreviate again  $\ans{\xi}{x^*}=\ans{[\xi,\xi]}{x^*}$.\smallskip  
%, i.e.\ the points $y^*\in\shock{\xi}$ such that $x^*\absorb y^*$.

A point $x^*\in\shock{[\zeta,\eta]}$ is   a {\it branch point}  in the  graph $\shockG{[\zeta,\eta]}$  if  $x^*$  is an ancestor of both $x^*-e_1$ and $x^*-e_2$.  Branch points are dual to those where $\zeta-$ and $\eta+$ geodesics separate. Similarly, $x^*\in\shock{[\zeta,\eta]}$ is a {\it coalescence point} if both $x^*+e_1$ and $x^*+e_2$ are ancestors of $x^*$.   Figures \ref{fig:shocks2a} and \ref{fig:shocks2b} display  simulations that illustrate the branching and coalescing. 


For the sharpest branching and coalescing properties in the next theorem, we invoke again the regularity condition \eqref{g-reg}  and  the jump process condition \eqref{cond:jumpcond}, and additionally the non-existence of non-trivial bi-infinite geodesics: 

 %\begin{condition}\label{cond:biinf}
\begin{align}\label{cond:biinf}
\begin{minipage}{0.9\textwidth}
There exists a full $\bbP$-probability event on which the only bi-infinite geodesics are the trivial ones: $x+\Z e_i$ for $x\in\Z^2$ and $i\in\{1,2\}$.
\end{minipage}
\end{align}
%\end{condition}
Condition  \eqref{cond:biinf} is known to hold  in the exponential case %\cite[Theorem 1]{Bas-Hof-Sly-18-}.  
  \cite{Bal-Bus-Sep-20,Bas-Hof-Sly-18-}. 

 
%to competition interface roots, of which there are infinitely many. 
%\timonote{Need more precise language, for isn't every vertex a root of a competition interface? F: OK now?}  
%Under the jump process condition \eqref{cond:jumpcond}, any two shock points have  a common ancestor. 
%%\note{F edited the text here a bit. Please read}
%Under the no bi-infinite geodesics condition \eqref{cond:biinf}  any two shock points also share a common descendant.  If both \eqref{cond:jumpcond} and \eqref{cond:biinf} hold,  there are infinitely many coalescence points.  
%
 
\begin{theorem}\label{thm:shocks}
The following hold for $\bbP$-almost every $\w$ and all $\zeta\preceq\eta$ in $\ri\Uset$ such that  $[\zeta,\eta]\cap\,\aUset\ne\varnothing$.  The case $\zeta=\eta=\xi$ is included unless otherwise stated.
\begin{enumerate}[label={\rm(\alph*)}, ref={\rm\alph*}] \itemsep=3pt 
%%%%%%   Parts commented out below moved to a separate theorem 2019-11-23 %%%%%%%
%\item\label{thm:shocks.0} Shock points exist: $\shock{[\zeta,\eta]}\neq\varnothing$.
%\item\label{thm:shocks.a} Any path that starts at a shock point $x^*\in\shock{[\zeta,\eta]}$ and takes steps in $\{-e_1,-e_2\}$ along edges of the graph $\dS{[\zeta,\eta]}$  remains entirely in the graph $\shockG{[\zeta,\eta]}$.   In particular,  each $x^*\in\shock{[\zeta,\eta]}$ is the starting point of an infinite directed  path in $\shockG{[\zeta,\eta]}$. 
%%has all its vertices in $\shock{[\zeta,\eta]}$ and is hence a path in $\shockG{[\zeta,\eta]}$. 
%\item\label{thm:shocks.b} For any point $x^*\in\shock{[\zeta,\eta]}$, there exists a semi-infinite  up-right path $x^*_{m,\infty}$ of points in $\shock{[\zeta,\eta]}$ emanating from $x^*_m=x^*$ and such that for all $n\ge m$, $x^*_{n+1}-x^*_n\in\{e_1,e_2\}$ and $x^*_{n+1}$ is a parent of $x^*_n$ in $\shockG{[\zeta,\eta]}$. All such paths are $[\zetamin,\etamax]$-directed. 
\item\label{thm:shocks.c} $x^*$ is a branch point in $\shockG{[\zeta,\eta]}$
if and only if $\cid(T_{x^*-\etstar}\w)\in[\zeta,\eta]$.
\item\label{thm:shocks.d} If $\zeta\prec\eta$, then any $x^*,y^*\in\shock{[\zeta,\eta]}$ have a common descendant: $\exists z^*\in\shock{[\zeta,\eta]}$ such that $x^*,y^*\in\ans{[\zeta,\eta]}{z^*}$. If we assume the no bi-infinite geodesics condition \eqref{cond:biinf}, then the same statement holds also for the case $\zeta=\eta=\xi$.
\item\label{thm:shocks.e} Assume the jump process condition \eqref{cond:jumpcond}.  
Then any $x^*,y^*\in\shock{[\zeta,\eta]}$ have a common ancestor 
$z^*\in\ans{[\zeta,\eta]}{x^*}\cap\ans{[\zeta,\eta]}{y^*}$. 
\item\label{thm:shocks.f} Suppose  $\zeta\prec\eta$ are such that $]\zeta,\eta[\,\cap\aUset\ne\varnothing$.  Then  for any $z\in\Z^2$ there is a coordinatewise strictly ordered infinite sequence $z<z_1^*<z_2^*< \dotsm<z_n^*<\dotsm$   such that each $z_n^*$ is a   branch point in $\shockG{[\zeta,\eta]}$.  
There are also  infinitely many coalescence points in $\shockG{[\zeta,\eta]}$. 
\item\label{thm:shocks.g} If the jump process condition \eqref{cond:jumpcond} holds and $\xi\in\aUset$, then  for any $z\in\Z^2$ there is a coordinatewise strictly ordered infinite sequence $z<z_1^*<z_2^*< \dotsm<z_n^*<\dotsm$   such that each $z_n^*$ is a   branch point in $\shockG{\xi}$. 
%\timonote{Should this somehow be combined with \eqref{thm:shocks.e}?} 
If additionally the no bi-infinite geodesics condition \eqref{cond:biinf} holds, then there are infinitely many coalescence points in $\shockG{\xi}$.
%This is because if say $\xi\in[\zeta,\eta]\cap\supp{\mu_{x+e_1,x+e_2}}$, then there are infinitely many points where the $\xi\pm$ geodesics split.)}
%\timonote{Should we include the injective mapping from branch points to coalescence points? Or should this actually go into \eqref{thm:shocks.d}?} 
\end{enumerate}
\end{theorem}

\begin{remark}\label{rk:erg2}
If regularity condition \eqref{g-reg} holds, then part \eqref{thm:shocks.f} holds for $\zeta\prec\eta$ with $[\zeta,\eta]\cap\aUset\ne\varnothing$. %and $\w$ in the full measure set $\Omreg$, where $\Omreg$ was introduced in Lemma \ref{lm:B+>B-}. 
The proof of this is given right after that of Theorem \ref{thm:shocks} in Section \ref{shockgraphs:pfs}.
\end{remark}

Given that there are infinitely many instability points when instability points exist, it is natural to wonder what their density on the lattice is. We identify the following trichotomy.
%either $\xi\not\in\aUset$, or 
%$\xi \in \aUset \cap \Diff$ and the $\xi$-shock points have zero density, or $\xi \in(\ri\Uset)\setminus\Diff\subset\aUset$ and the $\xi$-shock points have positive density.

\begin{proposition} \label{prop:trichotomy}
Assume the regularity condition \eqref{g-reg}.
Then for $\bbP$-almost every $\w$ and all $\xi\in\ri\Uset$, exactly one of the following three scenarios happens: 
\begin{enumerate}[label={\rm(\alph*)}, ref={\rm\alph*}]
\item $\xi\not\in\aUset$ and hence there are no $\xi$-instability points.
\item $\xi\in\aUset\cap\Diff$ and there are infinitely many $\xi$-instability points but they have zero density.
\item $\xi\not\in\Diff$ and $\xi$-instability points have positive density.
\end{enumerate}
\end{proposition}
%(\ri\Uset)\setminus\Diff\subset\aUset\subset\ri\Uset

%\subsection{Mass transport along the shocks}
%
%\textcolor{red}{also, where does the picture with equivalence classes belong?}
We return to this question in Section \ref{sec:exp} in the solvable case of exponential weights, where we can say significantly more.



\subsection{Flow of Busemann measure} \label{sec:Busflow}
 This section views the instability graph $\shockG{[\zeta,\eta]}$ as a description of the south-west directed  flow of Busemann measure on the dual lattice. 
 As discussed in Section \ref{s:HJ}, we can think of the function $\B{\xi\sig}(x+e_1, x+e_2)$ %=\B{\xi\sig}(x+e_1, 0)-\B{\xi\sig}(x+e_2,0)$ 
  as a global solution of a discretized stochastic Burgers equation.  We can assign the value $\B{\xi\sig}(x+e_1, x+e_2)$ to the dual point $x^*=x+\etstar$ that represents the diagonal edge $(x+e_1, x+e_2)$.  Then the cocycle property \eqref{coc-prop} gives us a flow of Busemann measure along the south and west pointing edges of the dual lattice $\Z^{2*}$. 
 First decompose   the Busemann measure of the  edge $(x+e_1, x+e_2)$ as a sum  $\mu_{x+e_1, x+e_2}=\mu_{x+e_1, x}+\mu_{x,x+e_2}$ of two positive measures.  This is justified by  the cocycle property \eqref{coc-prop}. 
Then  stipulate that measure $\mu_{x+e_1, x}$ flows south from $x^*$ to $x^*-e_2$ and contributes to Busemann measure $\mu_{x-\ex, x}$,  while measure $\mu_{x,x+e_2}$ flows west from $x^*$ to $x^*-e_1$ and contributes to Busemann measure $\mu_{x, x+\ex}$.   See Figure \ref{fig:flow}.
%Again the cocycle property \eqref{coc-prop}  ensures that 

\begin{figure}[h]
 	\begin{center}
 		 \begin{tikzpicture}[scale=1.2,>=stealth]
			\draw(0,-.5)--(0,3.5);		 
			\draw(1,-.5)--(1,3.5);		 
			\draw(2,-.5)--(2,3.5);		 
			\draw(3,-.5)--(3,3.5);		 
			\draw(-.5,0)--(3.5,0);		 
			\draw(-.5,1)--(3.5,1);		 
			\draw(-.5,2)--(3.5,2);		 
			\draw(-.5,3)--(3.5,3);	
			\draw(0,2)--(2,0);
			\draw(1,2)--(2,1);
			\draw(1,3)--(3,1);
			\draw[line width=1.5pt,->](1.4,1.5)--(0.6,1.5);	 
			\draw[line width=1.5pt,->](1.5,1.4)--(1.5,0.6);	 
			\draw[line width=1.5pt,->](2.4,1.5)--(1.6,1.5);	 
			\draw[line width=1.5pt,->](1.5,2.4)--(1.5,1.6);	 
			\draw[fill=white](1.5,1.5) circle(2pt);
			\draw(1.55,1.35)node[left]{\small$x^*$};
			\draw[fill=white](0.5,1.5) circle(2pt);
			\draw[fill=white](1.5,0.5) circle(2pt);
			\draw[fill=white](2.5,1.5) circle(2pt);
			\draw[fill=white](1.5,2.5) circle(2pt);
			\draw[fill=black](1,1) circle(2pt);
			\draw(1,0.8)node[left]{\small$x$};
			\draw[fill=black](2,0) circle(2pt);
			\draw(2,.15)node[right]{\small$x-\ex$};
			\draw[fill=black](0,2) circle(2pt);
			\draw(0,2.2)node[left]{\small$x+\ex$};
			\draw[fill=black](1,2) circle(2pt);
			\draw(1.05,2.2)node[left]{\small$x+e_2$};
			\draw[fill=black](2,1) circle(2pt);
			\draw(2,1.15)node[right]{\small$x+e_1$};
			\draw[fill=black](2,2) circle(2pt);
			\draw(2,2.2)node[right]{\small$x+\et$};
			\draw[fill=black](3,1) circle(2pt);
			\draw[fill=black](1,3) circle(2pt);
		
		\end{tikzpicture}
 	 \end{center}
 	\caption{\small  The flow of Busemann measures follows the arrows.  The antidiagonal edge $(x+e_1, x+e_2)$  is identified with the dual point $x^*=x+\etstar$.   The Busemann measure  $\mu_{x+e_1,x+e_2}$ on this edge is composed of the mass flowing from the north and east, and it in turns divides its mass between the flows south and west.}
 \label{fig:flow}
 \end{figure}



The cocycle property also tells us that $\mu_{x+e_1, x+e_2}=\mu_{x+e_1, x+\et}+\mu_{x+\et,x+e_2}$.  This represents $\mu_{x+e_1, x+e_2}$ as the sum of the contributions it receives from the next level up: $\mu_{x+e_1, x+\et}$ comes from the east from dual vertex $x+e_1+\etstar$, while $\mu_{x+\et,x+e_2}$ comes from the north  from dual vertex $x+e_2+\etstar$. 

Now pick a pair of directions $\zeta\preceq\eta$ in $\ri\Uset$,  and consider the graph $\cB^*_{[\zeta, \eta]}$  on the dual lattice $\Z^{2*}$ obtained as follows.  Include vertex $x^*=x+\etstar$ if $[\zeta, \eta]\cap\supp\mu_{x+e_1, x+e_2}\ne\varnothing$.  For $i\in\{1,2\}$,  include dual edge $(x^*, x^*-e_i)$ if $[\zeta, \eta]$ intersects $\supp\mu_{x, x+e_{3-i}}$, or somewhat pictorially, if some of the support in $[\zeta, \eta]$ flows along the dual edge  $(x^*, x^*-e_i)$. \smallskip 

The results of this section hold $\P$-almost surely simultaneously for all $\zeta\preceq\eta$ in $\ri\Uset$, including for the case $\zeta=\eta=\xi$.

\begin{theorem}\label{th:flowS}
  The graphs $\cB^*_{[\zeta, \eta]}$ and $\shockG{[\zeta,\eta]}$ are the same.  
\end{theorem} 

Under  the jump condition \eqref{cond:jumpcond}, a closed set cannot intersect the support without actually having nonzero measure.  Thus under \eqref{cond:jumpcond},   Theorem \ref{th:flowS} tells us that $\shockG{[\zeta,\eta]}$ is precisely the graph along which positive Busemann measure in the interval $[\zeta, \eta]$  flows. 

 \medskip
 
 Next we describe the ``islands'' on $\Z^2$ carved out by the paths of the graph $\shockG{[\zeta, \eta]}$  (islands surrounded by red paths in Figures \ref{fig:shocks2a} and \ref{fig:shocks2b}).   These islands are trees, they are the connected components of an intersection of geodesic graphs, and they are the equivalence classes of an equivalence  relation defined in terms of the supports of Busemann measures. 
 
Define the graph $\G{\cap[\zeta, \eta]}=\bigcap_{\xi\in[\zeta, \eta]} (\G{\xi-}\cap\G{\xi+})$ on the  vertex set  $\Z^2$ by keeping only those edges that lie in each geodesic graph $\G{\xi\sig}$ as $\xi$ varies over $[\zeta, \eta]$ and $\sigg$ over $\{-,+\}$.  
%Equivalently,  $\G{\cap[\zeta, \eta]}=\G{\zeta-}\cap\G{\eta+}$ in terms of the two extreme ones. 
Also, directly from the definitions  follows that an edge of $\Z^2$ lies in $\G{\cap[\zeta, \eta]}$ if and only if the dual edge it crosses does not lie in the graph $\dS{[\zeta, \eta]}$ introduced in Section \ref{sec:web}.   Since each $\G{\xi\sig}$ is a forest, $\G{\cap[\zeta, \eta]}$ is a forest, that is, a union of disjoint trees.  
%  A priori these trees can be finite or infinite.  


Define an equivalence relation $\zesim$ on $\Z^2$  by   $x\zesim y$ if and only if  $\supp{\mu_{x,y}}\cap[\zeta, \eta]=\varnothing$. It is an equivalence relation because $\mu_{x,x}$ is the identically zero measure, and  $\B{\xi\sig}_{x,z}= \B{\xi\sig}_{x,y}+\B{\xi\sig}_{y,z}$  implies that $\abs{\mu_{x,z}} \le \abs{\mu_{x,y}} + \abs{\mu_{y,z}}$.     In terms of coalescence,  $x\zesim y$ if and only if the coalescence points  $\coal{\xi\sig}(x,y)$ remain  constant in $\Z^2$ as  $\xi$ varies across $[\zeta, \eta]$ and $\sigg$ over $\{-,+\}$.  (This follows from   Propositions \ref{pr:supp1}  and  \ref{pr:supp2} proved below.)    As usual, replace $\zesim$ with $\xisim$ when $[\zeta, \eta]=[\xi, \xi]$. 

\begin{proposition}\label{lm:K9} 
The equivalence classes of the relation $\zesim$ are exactly the connected components {\rm(}subtrees{\rm)} of $\G{\cap[\zeta, \eta]}$. 
\end{proposition} 

Lemma \ref{lm:cross} proved below shows that nearest-neighbor points of $\Z^2$ are in distinct $\zesim$ equivalence classes if and only if the edge between them is bisected by an edge of the instability graph $\shockG{[\zeta,\eta]}$.   Together with Proposition \ref{lm:K9} this tells us that the paths of $\shockG{[\zeta, \eta]}$ are precisely the boundaries that separate distinct connected components of $\G{\cap[\zeta, \eta]}$ and the equivalence classes of $\zesim$. 


The next two lemmas indicate how 
the structure of the   subtrees  of $\G{\cap[\zeta, \eta]}$ is constrained by the fact that they are  intersections of geodesic trees.     These properties are clearly visible in  the bottom pictures of Figure \ref{fig:shocks2b} where these  subtrees     are the blue/green trees in  the  islands separated by red paths.

\begin{lemma}\label{lm:K10}   Let  $\cK$ be a subtree of  $\G{\cap[\zeta, \eta]}$ and let  $x$ and  $y$ be two distinct vertices of $\cK$.   Assume that  neither strictly dominates the other in the coordinatewise ordering, that is, both coordinatewise strict  inequalities $x<y$ and $y<x$ fail.  Then    the  entire rectangle  $\lzb x\wedge y, x\vee y\rzb$  is a subset of the vertex set of $\cK$.  
\end{lemma} 

In particular, if for some integers $\{t,k,\ell\}$, level-$t$ lattice points $(k, t-k)$ and $(\ell, t-\ell)$ are vertices of a subtree $\cK$, the entire discrete interval $\{(i, t-i): i\in\lzb k,\ell\rzb\}$ is a subset of the vertex set of $\cK$.  Similarly, points on horizontal and vertical line segments between vertices of a subtree $\cK$ are again vertices of $\cK$.  

  
\begin{lemma} \label{lm:K12}   Let  $\cK$ be a subtree of  $\G{\cap[\zeta, \eta]}$.  
There is at most one vertex  $x$ in $\cK$ such that $\{x- e_1, x- e_2\}\cap\cK=\varnothing$.  Such a point $x$ exists if and only if $\inf\{ t\in\Z: \cK\cap\level_t\ne\varnothing\}>-\infty$.  In that case   $\cK$ lies in $\{y: y\ge x\}$. 
%$\{y:  y\cdot( e_1+ e_2)> x\cdot( e_1+ e_2)\}$ 
\end{lemma} 

Note that Lemma \ref{lm:K12} does not say that a subtree has a single leaf.  Both $x$ and $x-e_i$ can be leaves of a subtree when the edge $(x-e_i, x)$ is not present in $\G{\cap[\zeta, \eta]}$.


\medskip

%Under the jump condition \eqref{cond:jumpcond} we can 
For the remainder of this section assume the jump condition \eqref{cond:jumpcond},   in order to 
give a sharper description of the subtrees of $\G{\cap[\zeta, \eta]}$.  
 Let $\cifset_{[\zeta, \eta]}=\{z\in\Z^2: \cid(T_z\w)\in{[\zeta, \eta]}\}$.  By Theorem \ref{thm:shocks}\eqref{thm:shocks.c}, $z\in\cifset_{[\zeta, \eta]}$ if and only if $z+\etstar$ is a branch point of the instability graph $\shockG{[\zeta,\eta]}$.    It follows then that both $z\pm\exstar$ are also  $[\zeta,\eta]$-instability points.  
 
   Assume for the moment that $\cifset_{[\zeta, \eta]}\ne\varnothing$.  By Theorem \ref{th:V1}, under the jump condition \eqref{cond:jumpcond} this is equivalent to $[\zeta, \eta]\cap\,\aUset\ne\varnothing$. 
 
The graph $\G{\cap[\zeta, \eta]}$ has no outgoing up or right edges from a point  $z\in\cifset_{[\zeta, \eta]}$ because geodesics split: 
 $\geo{}{z}{\cid(T_z\w)-}$ and   $\{\geo{}{z}{\xi\pm}:\zeta\preceq \xi\prec\cid(T_z\w)\}$ take the $ e_2$-step at $z$, while  $\geo{}{z}{\cid(T_z\w)+}$ and  $\{\geo{}{z}{\xi\pm}:  \cid(T_z\w)\prec \xi\preceq\eta\}$ take the $ e_1$-step at $z$.   For each $z\in\cifset_{[\zeta, \eta]}$, let  the tree $\cK(z)$ consist of all directed  paths in $\G{\cap[\zeta, \eta]}$ that terminate at $z$. $\cK(z)$ can consist of $z$ alone.  
 
These  properties come  from previously established facts: 
 \begin{itemize} 
\item   Each $x\in\Z^2\setminus\cifset_{[\zeta, \eta]}$ lies in a unique $\cK(z)$ determined by  following  the common path  of the geodesics $\{\geo{}{x}{\xi\sig}:\xi\in[\zeta,\eta], \,\sigg\in\{-,+\}\}$ until  the first point $z$ at which a split happens.  A split must happen eventually  because for any $u\in\cifset_{[\zeta,\eta]}$ the two geodesics  $\geo{}{u}{\cid(T_u\w)\pm}$ separate immediately at $u$, while by Theorem  \ref{thm:+-coal}    the geodesic $\geo{}{x}{\cid(T_u\w)\sig}$  
 coalesces with $\geo{}{u}{\cid(T_u\w)\sig}$  for both $\sigg\in\{-,+\}$. 
 
 \item If $\zeta\prec\eta$ then each tree $\cK(z)$ is finite.  Same  holds also  for the case $\zeta=\eta=\xi$ under the no bi-infinite geodesics condition \eqref{cond:biinf}.   This follows from Theorem \ref{thm:shocks}\eqref{thm:shocks.d} because the $[\zeta,\eta]$-instability points   $z\pm\exstar$  that flank $z$ have a common descendant $u^*$  in the graph $\shockG{[\zeta,\eta]}$. The two directed paths  of $\shockG{[\zeta,\eta]}$ that connect $z+\etstar$ to $u^*$ surround $\cK(z)$.  
 
 \end{itemize}  
 
 The final theorem of this section decomposes $\G{\cap[\zeta, \eta]}$ into its connected components. 

\begin{theorem}\label{thm:jumpG}  Assume the jump condition \eqref{cond:jumpcond}. 
\begin{enumerate}[label={\rm(\alph*)}, ref={\rm\alph*}] \itemsep=3pt 
\item\label{thm:jumpG.a} $\G{\cap[\zeta, \eta]}$ is a single tree if and only if $[\zeta, \eta]\cap\,\aUset=\varnothing$. 
\item\label{thm:jumpG.b} If $[\zeta, \eta]\cap\,\aUset\ne\varnothing$, 
the  connected components of $\G{\cap[\zeta, \eta]}$ are the trees  
$\{\cK(z):  z\in\cifset_{[\zeta, \eta]}\}$. 
\end{enumerate}
\end{theorem} %\medskip

We finish by reminding the reader that all the hypotheses and hence all the conclusions hold in  the case of i.i.d.\ exponential weights. 
The results of Section \ref{sec:Busflow}  are proved in Section  \ref{sec:Busflowpf}.
%Section \ref{sec:LPPDS}  are proved in Section  \ref{sec:webpf}.



==> JEMS Post-Accept Revision/GeoWebPaper-Sec5.tex <==
% !TEX root = GeoWebPaper.tex

\section{Statistics of instability points in the exponential model}\label{sec:exp}  
Under condition \eqref{exp-assump}, i.e.~when the weights are exponentially distributed, we derive explicit statistics of the instability graphs. 
For $\xi\in\ri\Uset$, $k\in\Z$, and $\sigg\in\{-,+\}$, abbreviate $\depa^{\xi\sig}_k=\B{\xi\sig}\bigl(ke_1,(k+1)e_1\bigr)$ and write $\depa^\xi_k$ when there is no $\pm$ distinction.
For  $\zeta\preceq\eta$ in $\ri\Uset$ 
let 
\[ \dotsm<\tau^{\zeta, \eta}(-1)<0\le \tau^{\zeta, \eta}(0)<\tau^{\zeta, \eta}(1)<\dotsm\]  be the ordered  indices such that 
\be\label{78-45} 
\depa^{\zeta-}_k>\depa^{\eta+}_k\quad\text{if and only if}\quad k\in\{\tau^{\zeta, \eta}(i):i\in\Z\}.   
\ee
If $\depa^{\zeta-}_k>\depa^{\eta+}_k$ happens for only finitely many indices $k$, then some $\tau^{\zeta, \eta}(i)$ are set equal to $-\infty$ or $\infty$. 

By Theorem \ref{th:exp1}, under condition \eqref{exp-assump}, \eqref{78-45}  is equivalent to 
\[\coal{\zeta-}(k e_1, (k+1) e_1) \neq \coal{\eta+}(k e_1,(k+1)e_1).\] 
It is worth keeping this geometric implication of \eqref{78-45} in mind in this section to provide some context for the results that follow. 

It will be convenient in what follows to parametrize directions in $\ri\Uset$ through the increasing  bijection
 \be\label{u-a}    \zeta=\zeta(\alpha)=\biggl(    \frac{\alpha^2}{(1-\alpha)^2+\alpha^2}\,,  \frac{(1-\alpha)^2}{(1-\alpha)^2+\alpha^2}\biggr)
 \ \Longleftrightarrow \ 
 \alpha= \alpha(\zeta)= \frac{\sqrt{\zeta\cdot e_1}}{\sqrt{\zeta\cdot e_1}+ \sqrt{1-\zeta\cdot e_1}}
  \ee
 between $\zeta\in\ri\Uset$ and $\alpha\in(0,1)$. Recall   the {\it Catalan numbers}   $C_n=\frac{1}{n+1}{2n\choose n}$ for $n\geq 0$.  By \eqref{B4} from Appendix \ref{a:bus},  the conditioning event  in the theorem below has probability $\P(\depa^\zeta_0>\depa^\eta_0)= \frac{\alpha(\eta)-\alpha(\zeta)}{\alpha(\eta)}$. 
Since $\zeta\prec\eta$ are fixed, with probability one no $\pm$ distinction appears   in  the Busemann functions. 
 
 \begin{theorem}\label{th:palm1} 
Assume \eqref{exp-assump}.
Fix $\zeta\prec\eta$ in $\ri\Uset$. 
Conditional on $\depa^\zeta_0>\depa^\eta_0$,  \[\bigl\{\tau^{\zeta, \eta}(i+1)-\tau^{\zeta, \eta}(i), \depa^\zeta_{\tau^{\zeta, \eta}(i)}-\depa^\eta_{\tau^{\zeta, \eta}(i)}: i\in\Z\bigr\}\]
is an  i.i.d.\ sequence with marginal distribution 
\be\label{78-90} \begin{aligned} 
&\P\bigl(\tau^{\zeta, \eta}(i+1)-\tau^{\zeta, \eta}(i)=n, \, \depa^\zeta_{\tau^{\zeta, \eta}(i)}-\depa^\eta_{\tau^{\zeta, \eta}(i)}>r\,\big\vert\,\depa^\zeta_0>\depa^\eta_0\,\bigr) \\
&\qquad \qquad 
= C_{n-1}\,  \frac{\alpha(\zeta)^{n-1}\alpha(\eta)^n}{\bigl(\alpha(\zeta)+\alpha(\eta)\bigr)^{2n-1}}\,e^{-\alpha(\zeta) r}
% \\  &\qquad\qquad = \frac1n\binom{2n-2}{n-1}\,  \frac{\alpha^{n-1}\beta^n}{(\beta+\alpha)^{2n-1}}e^{-\alpha r}
\,,\quad \forall \, i\in\Z, \, n\in\N,\, r\in\R_+. 
\end{aligned} \ee
\end{theorem}

Abbreviate $\tau^\xi(i)=\tau^{\xi, \xi}(i)$. Our next goal is to describe the joint distribution of processes $(\{\tau^\xi(i):i\in\Z\}, \, \depa^{\xi-}_{\tau^{\xi}(i)}-\depa^{\xi+}_{\tau^{\xi}(i)})$ of locations and sizes of jumps in direction $\xi$, conditional on $\{\B{\xi-}_0 > \B{\xi+}_0\}$.   However, for a fixed $\xi$,    $\B{\xi+}=\B{\xi-}$ almost surely and so this conditioning has to be understood in the Palm sense.  This is natural for conditioning on a jump of a point process at a particular location. 

In the theorem below, Lebesgue measure on $\Uset$ refers to one-dimensional Lebesgue measure (length of a line segment). 
The Lebesgue-almost every qualifier is in the theorem because the Palm kernel is defined only up to Lebesgue-null sets of the points $\xi$.  We denote Palm conditioning with two vertical lines $||$ to distinguish it from ordinary conditioning.  The  definition of the Palm conditioning used in \eqref{rw113} below  appears in equation \eqref{eq:palmdef} at the end of Section \ref{sub:palm}. For references, see \cite{Kal-83, Kal-17}. 


\begin{theorem}\label{th:B-palm1}  
Assume \eqref{exp-assump}.
For Lebesgue-almost every $\xi\in\ri\Uset$,  under the Palm kernel, conditional on $\B{\xi-}_0 > \B{\xi+}_0$,
 $\{\tau^\xi(i+1)-\tau^\xi(i), \depa^{\xi-}_{\tau^{\xi}(i)}-\depa^{\xi+}_{\tau^{\xi}(i)} : i\in\Z\}$ is an  i.i.d.\ sequence with marginal distribution 
\be\label{rw113} \begin{aligned} 
&\bbP\bigl\{\tau^\xi(i+1)-\tau^\xi(i) =n, \depa^{\xi-}_{\tau^{\xi}(i)}-\depa^{\xi+}_{\tau^{\xi}(i)}>r\,||\, \B{\xi-}_0 > \B{\xi+}_0\bigr\} \\
&\qquad\qquad\qquad
= C_{n-1}\,  \frac1{2^{2n-1}}\, e^{-\alpha(\xi)r},\qquad \forall\, i\in\Z, \, n\in\N,\, r\in\R_+.  
\end{aligned} \ee
\end{theorem}

%\smallskip

Equation \eqref{rw113}  connects the Palm distribution of the locations of jumps of the Busemann process with the zero set of simple symmetric random  walk (SSRW). 
 Let $\RW_n$ denote a two-sided SSRW, that is, $\RW_0=0$ and $\RW_n-\RW_m=\sum_{i=m+1}^n \ZRW_i$ for all $m<n$ in $\Z$ where $\{\ZRW_i\}_{i\in\Z}$ are  i.i.d.\ with $P(\ZRW_i=\pm1) =1/2$.
Set $\rho_n = \one_{\{S_{2n} = 0\}}$ and let $\bfP$ be the  distribution of $\rho = \{\rho_n\}_{n\in\Z}$  on the sequence  space  $\{0,1\}^\Z$.  That is, $\bfP$ is the law of the zero set of simple symmetric random walk  sampled at even times.  The classical  inter-arrival distribution of this renewal process is (eqn.~III.3(3.7) on p.~78 of Feller \cite{Fel-68})
\be\label{rw117}  
\bfP( \rho_1=0, \dotsc, \rho_{n-1}=0, \rho_n=1) 
= C_{n-1}\,  \frac1{2^{2n-1}}.  \ee
Comparison of \eqref{rw113} and \eqref{rw117} reveals that for Lebesgue-almost every $\xi$, the Palm distribution of the locations of $\xi$-instability points on a line is the same as the law of the zero set of SSRW sampled at even times. 
(We record this fact precisely as Lemma \ref{lem:palmrw}.) The next result applies this to show that any translation invariant event which holds with probability one for the zero set of SSRW holds for all of the instability graphs simultaneously almost surely.


 \begin{theorem} \label{thm:ladder-xi}  
 Assume \eqref{exp-assump}.
 Suppose $A$ is a translation-invariant Borel subset of $\{0,1\}^\Z$ that  satisfies  $\bfP(A)=1$. 
Then 
\be\label{rw125}
\P\bigl\{ \forall\xi\in\aUset: \bigl( \one\{\B{\xi-}_\ell > \B{\xi+}_\ell\} : \ell \in \bbZ\bigr)\in A\bigr\}=1.
\ee
 \end{theorem} 
 
From \eqref{rw125} and known facts about random walk, we can derive corollaries. 
From \cite[equation (10.8)]{Rev-05}, we deduce that 
	\begin{align}
	\P\Bigl\{\forall\xi\in\aUset:\varlimsup_{n\to\infty}\frac{\sum_{i=0}^{n} \one\{\B{\xi-}_i > \B{\xi+}_i\}}{\sqrt{8n\log\log n}}=1\Bigr\}=1.
	\end{align}
From \cite[Theorem 11.1]{Rev-05} we also find that for a nonincreasing $\delta_n$,
	\begin{align}\label{red-LB}
	\P\Bigl\{\forall\xi\in\aUset:n^{-1/2}\sum_{i=0}^{n}\one\{\B{\xi-}_i > \B{\xi+}_i\}\ge\delta_n\quad\text{for all sufficiently large $n$}\Bigr\}=1 
	\end{align}
if $\sum_n\delta_n/n<\infty$ and 
	\begin{align}
	\P\Bigl\{\forall\xi\in\aUset:n^{-1/2}\sum_{i=0}^{n}\one\{\B{\xi-}_i > \B{\xi+}_i\}\le\delta_n\quad\text{infinitely often}\Bigr\}=1
	\end{align}
otherwise. 
Similar statements hold for the sums $\sum_{i=-n}^0$. This implies that for $\P$-almost every $\w$ and any $\xi\in\aUset$, the number of horizontal edges $(ke_1,(k+1)e_1)$ with $\xi\in\supp\mu_{ke_1,(k+1)e_1}$ and $-n\le k\le n$ is of order $n^{1/2}$. It suggests the number of such horizontal edges (and thus also vertical edges and $\xi$-instability points) in an $n\times n$ box should be of order $n^{3/2}$.  The next theorem gives an  upper bound.  The lower bound is left  for future work.



\begin{theorem}\label{thm:density-UB}
Assume \eqref{exp-assump} and fix $i\in\{1,2\}$.
Then for any $\zeta\in\ri\Uset$
		\begin{align*}%\label{claim2-UB}
		\P\Bigl\{\exists n_0:\forall \xi\in[\zeta,e_2[\,,\forall n\ge n_0:\sum_{x\in\lzb 0,n\rzb^2}\one\bigl\{\xi \in \supp\mu_{x,x+e_i}\bigr\}\le2n^{3/2}\sqrt{\log n}\Bigr\}=1.
		\end{align*}
The same holds when $\lzb0,n\rzb^2$ is replaced by any of $\lzb-n,0\rzb^2$, $\lzb0,n\rzb\times\lzb-n,0\rzb$, or $\lzb-n,0\rzb\times\lzb0,n\rzb$.
\end{theorem}
\medskip

This completes the presentation of the main results.   After a list of open problems, the remaining sections cover   the proofs.
The results of Section \ref{sec:exp}  are proved in Section  \ref{sec:exp-pf}.


==> JEMS Post-Accept Revision/GeoWebPaper-Sec6.tex <==
% !TEX root = GeoWebPaper.tex

\section{Busemann measures: proofs} \label{sec:bus}
The rest of the paper relies  on Appendix \ref{app:busgeo} where prior results from the literature are collected. The reader may wish to look through that appendix before proceeding; 
in particular, we will work on the $T$-invariant full-measure event $\Omega_0$ constructed in  \eqref{Om0}.\smallskip
%Throughout this section, we pick and fix $\w$ from the $T$-invariant full-measure event $\Omega_0$ which is constructed in equation \eqref{Om0} of Appendix \ref{app:busgeo}.\smallskip
%, although we will impose further conditions on $\w$ in results which are contingent on hypotheses stronger than Assumption \ref{main-assump}. \smallskip

%Recall %the forests $\G{\xi\pm}$  defined in Section \ref{sec:web} and
Fix a countable dense set $\Udense\subset\Diff$ of points of differentiability of the shape function $\gpp$ (recall \eqref{sh-th}).   These  play a role in the definition of the event $\Omega_0$ in \eqref{Om0}. 
Recall the definition \eqref{df:coal-z} of the %coalescence level $\ell^{\xi\sig}(x,y)$  and 
coalescence point $\coal{\xi\sig}(x,y)$.  %\eqref{df:coal-l} and  
%We also define 
%the {\it coalescence level}  of the $\geo{}{x}{\xi\sig}$ and $\geo{}{y}{\xi\sig}$ geodesics as 
%	\[\ell^{\xi\sig}(x,y)=\inf\{x\cdot\et: x \in \geo{}{x}{\xi\sig}\cap \geo{}{y}{\xi\sig}\}\]
%	 for each   $\xi \in \ri \Uset$ and sign $\sigg\in\{-,+\}$,  
%with the convention that the infimum of an empty set is $\infty$. 
When $\coal{\xi\sig}(x,y) \in \bbZ^2$, equation \eqref{eq:buspass} leads to the following identity, which is fundamental to the analysis that follows:
\begin{align} \label{eq:busdiff}
\B{\xi\sig}(x,y) &= G\bigl(x,\coal{\xi\sig}(x,y)\bigr) - G\bigl(y,\coal{\xi\sig}(x,y)\bigr) = \sum_{i=k}^{n-1} \w_{\geo{i}{x}{\xi\sig}} - \sum_{i=\ell}^{n-1} \w_{\geo{i}{y}{\xi\sig}},
\end{align}
where $k=x\cdot\et$, $\ell=y\cdot\et$, and $n=\coal{\xi\sig}(x,y)\cdot\et$. By Theorem \ref{thm1}\eqref{thm1:coal}, for all $\w \in \Omega_0$, all $\xi\in\Udense$,  and all $x,y \in \bbZ^2$,  both $\coal{\xi+}(x,y)$ and $\coal{\xi-}(x,y)$ are in $\bbZ^2$.
%\textcolor{red}{Should we include Lemma 2.7 from the notes file? It seems like just an observation at this point. We haven't used it anywhere... Maybe if we include it, it should be in a section about the properties of the dual graphs [along with mass transport, equivalence classes, etc]}


We begin with  results linking analytic properties of the Busemann process and coalescence points.% Recall the full measure event $\Omega_0$ defined in \eqref{Om0}.

\begin{proposition} \label{pr:supp1}
%Let $\Omega_0$ be the full measure event from Theorem \ref{thm1}.
%There exists a $T$-invariant event $\Omega_0 \subset \Omega$ with $\bbP(\Omega_0) = 1$ and such that 
For all $\w \in \Omega_0$, for any $\zeta \prec \eta$ in $\ri\Uset$, and any $x,y \in \bbZ^2$, the following statements are equivalent. 
\begin{enumerate}  [label={\rm(\roman*)}, ref={\rm\roman*}]   \itemsep=3pt 
\item\label{eq100} $\abs{\mu_{x,y}}(\,]\zeta,\eta[\,) = 0 $.
\item\label{eq101} $\B{\zeta+}(x,y) = \B{\eta-}(x,y)$ and $\coal{\zeta+}(x,y),\coal{\eta-}(x,y) \in \bbZ^2$.
\item\label{eq102} $\coal{\zeta+}(x,y) = \coal{\eta-}(x,y) \in \bbZ^2$.
%\item\label{eq103} For any $\xi\in\,]\zeta,\eta[$, any $\pi \in \{\geo{}{x}{\xi+},\geo{}{x}{\xi-} : \xi \in \, ]\zeta,\eta[\,\}$, and any $\geod{}' \in \{\geo{}{y}{\xi+},\geo{}{y}{\xi-} : \xi \in \, ]\zeta,\eta[\, \}$, %$\geod{}\cap \geod{}' \neq \varnothing$ and 
%$\geod{}$ and $\geod{}'$ coalesce. %\textcolor{red}{(the $\pm$ also match until that coalescence point)}
\item\label{eq103} There exists  $z \in \bbZ^2$ such that the following holds. For any $\pi \in \{\geo{}{x}{\xi\sig} : \xi \in \, ]\zeta,\eta[\,, \sigg\in\{-,+\}\}$ and any $\geod{}' \in \{\geo{}{y}{\xi\sig} : \xi \in \, ]\zeta,\eta[\,, \sigg\in\{-,+\} \}$, $\geod{}\cap \geod{}' \neq \varnothing$ and $z$ is the first point where $\pi$ and $\pi'$ intersect: $z\cdot\et=\min\{z'\cdot\et:z'\in\geod{}\cap\geod{}'\}$.
% = \argmin\{x \cdot \et: x \in  \geod{} \cap \geod{}'\}$.
\end{enumerate}
\end{proposition}

\begin{proof}  
%Take $\Omega_0$ as in Theorem \ref{thm1} and fix $\w\in\Omega_0$.
\eqref{eq100}$\implies$\eqref{eq101}. 
Under \eqref{eq100}   the functions $\xi \mapsto \B{\xi\sig}_{x,y}$ match for $\sigg\in\{-,+\}$ and are constant on the open interval $]\zeta,\eta[$.   $\B{\zeta+}(x,y) = \B{\eta-}(x,y)$ follows by taking limits $\xi \searrow \zeta$ and $\xi \nearrow \eta$. 

Since on $]\zeta,\eta[\,\cap\,\Udense$, $\xi \mapsto \B{\xi}_{x,y}$ is  constant  and  $\coal{\xi}(x,y)\in\Z^2$  (Theorem \ref{thm1}\eqref{thm1:coal}),   \eqref{eq:busdiff} and condition  \eqref{paths.2}  imply 
that $\coal{\xi}(x,y)$ is constant in $\Z^2$   for all  $\xi\in\,]\zeta,\eta[\,\cap\,\Udense$. 
Since $\Udense$ is dense in $]\zeta,\eta[\,$,  limits   
 \eqref{coal-lim} as $\xi \searrow \zeta$ and $\xi \nearrow \eta$ imply
%that $\coal{\xi\sig}(x,y)$ is constant for all $\xi\in\,]\zeta,\eta[$ and $\sigg\in\{-,+\}$.  Limits  $\xi \searrow \zeta$ and $\xi \nearrow \eta$ imply
 that $\coal{\zeta+}(x,y),\coal{\eta-}(x,y) \in \bbZ^2$.

% the fact that $\Udense$ is dense in $\ri\Uset$,  imply that $\coal{\xi\pm}(x,y)\in\Z^2$ for all $\xi\in\,]\zeta,\eta[$.
%\timonote{Should we add that the function on the left in \eqref{eq:busdiff} cannot be constant across $\xi\in \,]\zeta,\eta[$ unless $\coal{\xi\sig}(x,y)$ is constant. Otherwise how do we know that $\coal{\zeta+}(x,y),\coal{\eta-}(x,y) \in \bbZ^2$? It's a little weird that then we already get also \eqref{eq100}$\implies$\eqref{eq102}.} 
%Claim \eqref{eq101} follows by taking $\xi \searrow \zeta$ and $\xi \nearrow \eta$.

\smallskip

 \eqref{eq101}$\implies$\eqref{eq102}. 
Set $k=x \cdot \et $, $\ell=y \cdot \et $.   With  both $\coal{\zeta+}(x,y)$ and $\coal{\eta-}(x,y)$ in $\bbZ^2$, we also set  $m=\coal{\zeta+}(x,y)\cdot\et$, and $n=\coal{\eta-}(x,y)\cdot\et$. 
By \eqref{eq:busdiff}, 
\begin{align*}
\B{\zeta+}_{x,y} &= G\bigl(x,\coal{\zeta+}(x,y)\bigr) - G\bigl(y,\coal{\zeta+}(x,y)\bigr) = \sum_{i=k}^{m-1} \w_{\geo{i}{x}{\zeta+}} - \sum_{i=\ell}^{m-1} \w_{\geo{i}{y}{\zeta+}} 
\\
\text{and}\quad 
\B{\eta-}_{x,y} &=  G\bigl(x,\coal{\eta-}(x,y)\bigr) - G\bigl(y,\coal{\eta-}(x,y)\bigr) = \sum_{i=k}^{n-1} \w_{\geo{i}{x}{\eta-}} - \sum_{i=\ell}^{n-1} \w_{\geo{i}{y}{\eta-}}.
\end{align*}
By condition  \eqref{paths.2},  the vanishing of   $\B{\zeta+}_{x,y} - \B{\eta-}_{x,y}$    forces $m=n$, $\geo{k,m}{x}{\zeta+} = \geo{k,m}{x}{\eta-}$, and $\geo{\ell,m}{y}{\zeta+} = \geo{\ell,m}{y}{\eta-}$, and hence in particular $\coal{\zeta+}(x,y)=\coal{\eta-}(x,y)$.  

%Timo-proof:  From $\B{\zeta+}_{x,y}-\B{\eta-}_{x,y}=0$ cancel all weights that can be cancelled.  Then we can assume that the two paths from $x$ separate immediately, and so do the two paths from $y$.   

\smallskip 
 
\eqref{eq102}$\implies$\eqref{eq103}.
%Suppose that $\coal{\zeta+}(x,y) = \coal{\eta-}(x,y) \in \bbZ^2
With $m=\coal{\zeta+}(x,y)\cdot\et=\coal{\eta-}(x,y)\cdot\et$, 
  uniqueness of finite geodesics implies  $\geo{k,m}{x}{\zeta+} = \geo{k,m}{x}{\eta-}$ and $\geo{\ell,m}{y}{\zeta+} = \geo{\ell,m}{y}{\eta-}$. Then monotonicity  \eqref{path-ordering} gives   $\geo{k,m}{x}{\zeta+} = \geo{k,m}{x}{\xi\sig} = \geo{k,m}{x}{\eta-}$ and  $\geo{\ell,m}{y}{\zeta+} = \geo{\ell,m}{y}{\xi\sig} = \geo{\ell,m}{y}{\eta-}$ for all $\xi \in\, ]\zeta,\eta[$ and $\sigg\in\{-,+\}$. 
The point $z$ is  $\geo{m}{x}{\zeta+}=\geo{m}{y}{\zeta+}=\geo{m}{x}{\eta-}=\geo{m}{y}{\eta-}$.   

\smallskip
 
 \eqref{eq103}$\implies$\eqref{eq100}.
Let $m=z \cdot \et$. It follows from uniqueness of finite geodesics that all of the paths $\geo{k,m}{x}{\xi\pm}$ must be the same, for all $\xi\in\,]\zeta,\eta[$, and similarly all of the paths $\geo{\ell,m}{y}{\xi\pm}$ must be the same. Sending $\xi \searrow \zeta$ and $\xi \nearrow \eta$, we obtain that for all $\xi \in \, ]\zeta,\eta[$, $\geo{k,m}{x}{\zeta+} = \geo{k,m}{x}{\xi \pm} = \geo{k,m}{x}{\eta-}$ and $\geo{\ell,m}{y}{\zeta+} = \geo{\ell,m}{y}{\xi \pm} = \geo{\ell,m}{y}{\eta-}$.  
Recall that \eqref{eq:busdiff} applies for any $\xi\in\Udense$.
Thus, the functions  $\xi \mapsto \B{\xi\pm}_{x,y}$ match and are constant, when restricted to the dense set $\Udense\, \cap\, ]\zeta,\eta[$. Combining this with the left-continuity of $\xi \mapsto \B{\xi-}_{x,y}$ and the right-continuity of $\xi \mapsto \B{\xi+}_{x,y}$, we see that the functions $\xi \mapsto \B{\xi\pm}_{x,y}$ match and are constant on $]\zeta,\eta[$. 
This implies \eqref{eq100}.
%This implies that $|\mu_{x,y}|(\,]\zeta,\eta[)=0.$
\end{proof}

Proposition \ref{pr:supp1} has a counterpart in terms of fixed directions lying in the support of $\mu_{x,y}$.
\begin{proposition} \label{pr:supp2}
%There is a $T$-invariant event $\Omega_0$ with $\bbP(\Omega_0)=1$ and such that 
%Let $\Omega_0$ be the full measure event from Proposition \ref{pr:supp1}.
For all $\w \in \Omega_0$ and all $x,y \in \bbZ^2$, the following are equivalent:
\begin{enumerate} [label={\rm(\roman*)}, ref={\rm\roman*}]   \itemsep=3pt 
\item\label{eq110}  $\xi \not\in \supp{\mu_{x,y}}$.
\item\label{eq111} $\coal{\xi-}(x,y) = \coal{\xi+}(x,y) \in \bbZ^2$.
\item\label{eq112} $\B{\xi-}(x,y) = \B{\xi+}(x,y)$ and $\coal{\xi-}(x,y), \coal{\xi+}(x,y) \in \bbZ^2$. 
\end{enumerate}
\end{proposition}

\begin{proof}
Let $x \cdot \et = k$ and $y \cdot \et = \ell$. Take sequences $ \zeta_n, \eta_n \in \Udense$ with $\zeta_n \nearrow \xi$ and $\eta_n \searrow \xi$. Since $\zeta_n, \eta_n \in \Udense$ we have $\coal{\zeta_n}(x,y),\coal{\eta_n}(x,y) \in \bbZ^2$ for all $n$.   Furthermore,   $\B{\zeta_n}(x,y) \to  \B{\xi-}(x,y)$ and $\B{\eta_n}(x,y) \to  \B{\xi+}(x,y)$ as $n\to\infty$. 
 
 \smallskip 
 
 \eqref{eq110}$\implies$\eqref{eq111}.
  If $\xi \notin \supp{\mu_{x,y}}$, then  $\zeta \mapsto \B{\zeta\pm}(x,y)$ is constant on some neighborhood of $\xi$.   Then   \eqref{eq100}$\implies$\eqref{eq102} from  Proposition \ref{pr:supp1} gives \eqref{eq111}.  

\smallskip
   
\eqref{eq111}$\implies$\eqref{eq112}.
% Assume \eqref{eq111}. 
 Let $m=\coal{\xi-}(x,y)\cdot\et=\coal{\xi+}(x,y)\cdot\et$. Then  uniqueness of finite geodesics implies that  $\geo{k,m}{x}{\xi-} = \geo{k,m}{x}{\xi+}$ and $\geo{\ell,m}{y}{\xi-} = \geo{\ell,m}{y}{\xi+}$.
 %$m$ be such  that   
% $\geo{m}{x}{\xi-} = \geo{m}{y}{\xi-}=\coal{\xi-}(x,y) = \coal{\xi+}(x,y)= \geo{m}{x}{\xi+} =\geo{m}{y}{\xi+}$.
 % Now suppose that $\coal{\xi+}(x,y) = \coal{\xi-}(x,y) \in \bbZ^2$.  
  \eqref{pmgeolim} implies that for sufficiently large $n$,  $\geo{k,m}{x}{\xi-} = \geo{k,m}{x}{\zeta_n}$, $\geo{k,m}{x}{\xi+} = \geo{k,m}{x}{\eta_n}$, $\geo{\ell,m}{y}{\xi-} = \geo{\ell,m}{y}{\zeta_n}$, and $\geo{\ell,m}{y}{\xi+} = \geo{\ell,m}{y}{\eta_n}$.  For these large $n$, 
\begin{align*}
\B{\zeta_n}(x,y) &= G\bigl(x,\coal{\zeta_n}(x,y)\bigr) - G\bigl(y,\coal{\zeta_n}(x,y)\bigr) \\
&= \sum_{i=k}^{m-1} \w_{\geo{i}{x}{\zeta_n}} - \sum_{i=\ell}^{m-1} \w_{\geo{i}{y}{\zeta_n}} 
=\sum_{i=k}^{m-1} \w_{\geo{i}{x}{\xi-}} - \sum_{i=\ell}^{m-1} \w_{\geo{i}{y}{\xi-}}\\
&= \sum_{i=k}^{m-1} \w_{\geo{i}{x}{\xi+}} - \sum_{i=\ell}^{m-1} \w_{\geo{i}{y}{\xi+}}
= \sum_{i=k}^{m-1} \w_{\geo{i}{x}{\eta_n}} - \sum_{i=\ell}^{m-1} \w_{x_i^{y,\eta_n}}\\
&=  G\bigl(x,\coal{\eta_n}(x,y)\bigr) - G\bigl(y,\coal{\eta_n}(x,y)\bigr) =\B{\eta_n}(x,y).
\end{align*}
%The sums in the middle, along $\geo{}{x}{\xi\pm}$, do not depend on $n$. 
Taking $n\to\infty$ gives
$\B{\xi+}(x,y)=\B{\xi-}(x,y)$. Claim \eqref{eq112} is proved.
 
 \smallskip 
 
 \eqref{eq112}$\implies$\eqref{eq110}.
 The assumption $\coal{\xi-}(x,y), \coal{\xi+}(x,y) \in \bbZ^2$ allows us to use \eqref{eq:busdiff}.  This  
  and convergence of geodesics \eqref{pmgeolim} implies that  $\B{\zeta_n}(x,y) = \B{\xi-}(x,y)= \B{\xi+}(x,y)=\B{\eta_n}(x,y)$ for sufficiently large $n$.  The equivalence between \eqref{eq101} and \eqref{eq100} in Proposition \ref{pr:supp1} implies that for such $n$, both processes are constant on the interval $]\zeta_n,\eta_n[\,$. Therefore $\xi \notin \supp{\mu_{x,y}}$.
\end{proof}


With these results in hand, we next turn to the proofs of our main results.
%tool in what follows, Theorem \ref{thm:nonint}.

\begin{proof}[Proof of Theorem \ref{thm:nonint}]
%Take $\Omega_0$ to be the event in Proposition \ref{pr:supp2} 
Fix $\w\in\Omega_0$, $x,y\in\Z^2$, and $\xi\in\ri\Uset$.
Suppose that \eqref{thm:nonint.a} does not hold, i.e.\ $\xi \notin \supp{\mu_{x,y}}$. 
By Proposition \ref{pr:supp2}, we have $\coal{\xi-}(x,y) = \coal{\xi+}(x,y)\in\Z^2$, in which case both $\geo{}{x}{\xi-} \cap \geo{}{y}{\xi+}$ and $\geo{}{x}{\xi+} \cap \geo{}{y}{\xi-}$ include this common point and thus
\eqref{thm:nonint.b} is false.
This proves that \eqref{thm:nonint.b} implies \eqref{thm:nonint.a}.

Now, suppose that $\xi \in \supp{\mu_{x,y}}$ and that $\geo{}{x}{\xi-} \cap \geo{}{y}{\xi+} \neq \varnothing$ and $\geo{}{x}{\xi+} \cap \geo{}{y}{\xi-} \neq \varnothing$.   Without loss of generality assume that $x \cdot \et = k \leq m=y \cdot \et $. Let $z_1$ denote the first point at which $\geo{}{x}{\xi-}$ and $\geo{}{y}{\xi+}$ meet and call $z_2$ the first point at which $\geo{}{x}{\xi+}$ and $\geo{}{y}{\xi-}$ meet. Let $\ell_1 = z_1 \cdot \et$ and $\ell_2 = z_2 \cdot \et$. We denote by $u$ the leftmost (i.e.\ smallest $e_1$ coordinates) of the three points $\geo{m}{x}{\xi+},y,\geo{m}{x}{\xi-}$ and by $v$ the rightmost of these three points. Note that if $u=v$, then $\coal{\xi+}(x,y) = \coal{\xi-}(x,y)=y$, which would imply that  $\xi \notin \supp{\mu_{x,y}}$.  Thus   $u\ne v$ and there are  two cases: either $y \in \{u,v\}$ or not. We show a contradiction in both cases.

First, we work out the case $y=v$, with the case of $y=u$ being similar. See the left picture in Figure \ref{fig:nonint} for an illustration. 
In this case we have, for all $n \geq m$, $\geo{n}{x}{\xi-} \preceq \geo{n}{x}{\xi+}\preceq \geo{n}{y}{\xi+}$ and $\geo{n}{x}{\xi-} \preceq \geo{n}{y}{\xi-}\preceq \geo{n}{y}{\xi+}$. In words, $\geo{}{y}{\xi+}$ is the rightmost geodesic and $\geo{}{x}{\xi-}$ is the leftmost geodesic among the four geodesics $\geo{}{x}{\xi\pm}$, $\geo{}{y}{\xi\pm}$. By the path ordering \eqref{path-ordering} and planarity,  $z_1$ must lie on all four geodesics. Then by the uniqueness of finite geodesics  $\geo{k,\ell_1}{x}{\xi+} = \geo{k,\ell_1}{x}{\xi-}$ and   $\geo{m,\ell_1}{y}{\xi+} = \geo{m,\ell_1}{y}{\xi-}$. It follows that $z_1 =\coal{\xi+}(x,y) = \coal{\xi-}(x,y)$, contradicting $\xi \in \supp{\mu_{x,y}}$.

 \begin{figure}[h]
 	\begin{center}
 		 \begin{tikzpicture}[scale=1,shorten >=1pt,>={Latex[length=3.5mm,width=2mm]}]
	 		\begin{scope}
			\draw[color=sussexg, line width=1pt]plot[smooth] coordinates{(0,0)(0.2,0.5)(0.2,1)(.3,1.3)(0.4,1.5)(0.4,1.8)(0.7,2)(0.8,2.5)(0.9,2.7)(1.3,3)(1.6,3.1)(1.7,3.3)(2.3,3.5)(2.8,3.6)(3,3.7)(3.8,3.7)};
			\draw[color=sussexp, line width=2pt]plot[smooth] coordinates{(0.07,0)(0.3,0.5)(0.7,.7)(1.3,1.1)(1.6,1.2)(2,1.8)(2.3,1.9)(2.4,2)(2.65,2.35)(3,3.1)(3.3,3.2)(3.5,3.4)(3.8,3.7)};
			\draw[color=sussexg, line width=1pt]plot[smooth] coordinates{(1.5,0.5)(1.7,0.9)(1.8,1.2)(1.9,1.7)};%(2,2.5)(2.2,2.7)(2.3,3.5)};
			\draw[color=sussexg, line width=1pt]plot[smooth] coordinates{(1.9,1.7)(2.1,1.808)(2.3,1.9-0.05)(2.4,2-0.05)(2.65,2.35-0.05)(3,3.1-0.05)(3.3,3.2-0.05)(3.5,3.4-0.05)(3.8,3.7-0.05)};
			\draw[color=sussexp, line width=2pt]plot[smooth] coordinates{(1.55,0.5)(1.75,0.9)(2,1.1)(2.3,1.2)(2.4,1.7)%(2.7,1.8)(2.8,2.6)};
			(2.9,1.9)(3.1,2.5)(3.4,2.75)(3.8,3.7)};

			\draw[black,dashed,line width=0.5pt]plot(2,0)--(0,2);
			\draw[black,fill=white](0.03,0) circle(2.5pt);
			\draw[black,fill=white](1.53,0.5) circle(2.5pt);
			%\draw[black,fill=white](2.3,3.5) circle(2.5pt);
			\draw[black,fill=white](3.8,3.7) circle(2.5pt);
			%\draw[black,fill=white](2.77,2.6) circle(2.5pt);
			\draw[black,fill=white](1.93,1.7) circle(2.5pt);
			\draw[black,fill=white](0.4,1.6) circle(2.5pt);

			\draw(0,-.03)node[below]{$x$};
			\draw(1.6,0.5)node[right]{$y=v$};
			\draw(0.35,1.6)node[left]{$u$};
			%\draw(2.8,2.6)node[right]{$z^{\xi+}(x,y)$};
			%\draw(2.25,3.7)node[left]{$z^{\xi-}(x,y)$};
			\draw(4,3.7)node[above]{$z_1$};
			\draw(1.9,1.7)node[left]{$z_2$};
			\end{scope}
			
	 		\begin{scope}[shift={(6,0)}]
			\draw[color=sussexg, line width=1pt]plot[smooth] coordinates{(0,0)(0.2,0.5)(0.2,1)(.3,1.3)(0.4,1.5)(0.4,1.8)(0.7,2)(0.8,2.5)(0.9,2.7)(1.3,3)}; %(1.6,3.4)(1.7,3.5)(1.9,3.7)};
			\draw[color=sussexp, line width=2pt]plot[smooth] coordinates{(0.07,0)(0.3,0.5)(0.7,.7)(1.3,1.1)(1.6,1.2)(2,1.8)(2.3,1.9)(2.4,2)(2.65,2.35)(3.05,3.2)};%(3.3,3.2)(3.5,3.4)(3.8,3.7)};
			%\draw[color=sussexg, line width=1pt]plot[smooth] coordinates{(0.5,0.9)(0.7,1.4)(.7,1.9)(0.75,2.15)};
			\draw[color=sussexp, line width=2pt]plot[smooth] coordinates{(0.55,0.9)(0.75,1.4)(.9,2)(1.2,2.5)(1.3,2.94)(2,3)(2.3,3.1)(3.05,3.15)};%(3.26,3.19)};
			\draw[color=sussexg, line width=1pt]plot[smooth] coordinates{(0.53,0.9+.05)(0.75,1.4+.1)(.9,2+.1)(1.18,2.5)(1.2,2.75)(1.25,2.94+0.01)};
			\draw[color=sussexg, line width=1pt]plot[smooth] coordinates{(1.3,2.94+.05)(2,3+.05)(2.3,3.1+.05)(3.05,3.2)};

			\draw[black,dashed,line width=0.5pt]plot(0,1.4)--(1.4,0);
			\draw[black,fill=white](0.03,0) circle(2pt);
			%\draw[black,fill=white](0.7,2) circle(2pt);
			\draw[black,fill=white](0.53,0.9) circle(2pt);
			\draw[black,fill=white](1.28,2.95) circle(2pt);
			\draw[black,fill=white](3.05,3.17) circle(2pt);
			\draw[black,fill=white](0.25,1.15) circle(2pt);
			\draw[black,fill=white](0.7,0.7) circle(2pt);

			\draw(0,0)node[below]{$x$};
			\draw(0.5+0.05,0.9)node[left]{$y$};
			\draw(0.25,1.15)node[left]{$u$};
			\draw(0.75,0.68)node[right]{$v$};
			%\draw(3.05,2.9)node[right]{$z^{\xi+}(x,y)$};
			\draw(3.05,3.2)node[above]{$z_2$};
			%\draw(0.6,2.1)node[left]{$z^{\xi-}(x,y)$};
			\draw(1.3,3.1)node[left]{$z_1$};
			\end{scope}
		\end{tikzpicture}
	\end{center}
 	\caption{\small Proof of Theorem \ref{thm:nonint}. $\xi+$ geodesics are in purple with medium thickness. $\xi-$ geodesics are in green and thin.}
 \label{fig:nonint}
 \end{figure}

If $y \notin \{u,v\}$, then  $u = \geo{m}{x}{\xi-}\prec y\prec  v = \geo{m}{x}{\xi+}$ (right picture in Figure \ref{fig:nonint}). The geodesics  $\geo{}{x}{\xi+}$ and $\geo{}{x}{\xi-}$ have already split and so cannot meet again by the uniqueness of finite geodesics.   For all $n \geq m$, $\geo{n}{x}{\xi-}\preceq \geo{n}{y}{\xi-}\preceq \geo{n}{y}{\xi+} \preceq \geo{n}{x}{\xi+}$.   Due to this ordering, the meeting of  $\geo{n}{x}{\xi-}$ and  $\geo{n}{y}{\xi+}$   at $z_1$ implies that  $\geo{n}{x}{\xi-}$ and  $\geo{n}{y}{\xi-}$ coalesce at or before $z_1$.   By the uniqueness of finite geodesics again,  $\geo{}{y}{\xi-}$ and $ \geo{}{y}{\xi+}$ agree from $y$ to $z_1$.    The same reasoning applies to $z_2$ and gives that   $\geo{}{y}{\xi-}$ and $ \geo{}{y}{\xi+}$ agree from $y$ to $z_2$ and that  $\geo{}{y}{\xi+}$ and $\geo{}{x}{\xi+}$  coalesce at $z_2$.  Thus now    $\geo{}{y}{\xi-}$ and $ \geo{}{y}{\xi+}$ agree from $y$ through both $z_1$ and $z_2$.     The coalescence of $\geo{}{x}{\xi-}$ with $\geo{}{y}{\xi-}$ and the coalescence of $\geo{}{y}{\xi+}$ with $\geo{}{x}{\xi+}$ then  force $\geo{}{x}{\xi-}$ and $\geo{}{x}{\xi+}$ to  meet again, contradicting what was said above.
 We have now shown that \eqref{thm:nonint.a} implies \eqref{thm:nonint.b}.\smallskip


%%%%%%   earlier version %%%%%%%%
%If $y \notin \{u,v\}$, then we have $u = \geo{m}{x}{\xi-}, v = \geo{m}{x}{\xi+}$ (right picture in Figure \ref{fig:nonint}). In this case, $\geo{}{x}{\xi+}$ and $\geo{}{x}{\xi-}$ have already split and so cannot meet again by uniqueness of finite geodesics.  Similarly, once $\geo{}{y}{\xi-}$ and $\geo{}{y}{\xi+}$ split, they cannot meet again. But we also know that once $\geo{}{y}{\xi-}$ meets with $\geo{}{x}{\xi-}$, they coalesce, which would shield $\geo{}{y}{\xi+}$ from meeting $\geo{}{x}{\xi-}$ if the geodesics rooted at $y$ had already split. Therefore in order for it to be possible that $\geo{}{x}{\xi-}$ meets with $\geo{}{y}{\xi+}$, it must be the case that $z_1$ occurs before any such split happens. The same argument says that $z_2$ must occur before the geodesics rooted at $y$ split. We cannot have $\ell_1=\ell_2$ because this would imply $z_1=z_2$ and we said $\geo{}{x}{\xi+}$ and $\geo{}{x}{\xi-}$ cannot meet again after splitting. Suppose that $\ell_1 < \ell_2$, with the case of $\ell_1 > \ell_2$ being similar. In this case, since a split of the $y$ geodesics cannot occur before $z_2$, the geodesics $\geo{}{x}{\xi-}$ and $\geo{}{y}{\xi-}$ meet at $z_1$. At this point, they coalesce. On the other hand, the two geodesics rooted at $y$ must also meet with the geodesic $\geo{}{x}{\xi+}$ at $z_2$. This forces $z_2$ to lie on both $\geo{}{x}{\xi+}$ and $\geo{}{x}{\xi-}$, which contradicts uniqueness of finite geodesics. We have now shown that \eqref{thm:nonint.a} implies \eqref{thm:nonint.b}.\smallskip
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\eqref{thm:nonint.b} implies \eqref{thm:nonint.c} by the directedness in Theorem \ref{thm1}\eqref{thm1:exist}.
It remains to prove the reverse implication under the regularity condition \eqref{g-reg}.  
Without loss of generality we can assume that $x\cdot\et\le y\cdot\et=k$. If $\geod{k}^x\prec y$, then the extremality of the geodesics $\geo{}{\abullet}{\xi\pm}$ in Theorem \ref{thm:extreme}  and the fact that
$\geod{}^x\cap\geod{}^y=\varnothing$ imply that $\geo{}{x}{\xi-} \cap \geo{}{y}{\xi+} = \varnothing$. Similarly, if $\geod{k}^x\succ y$, then we get $\geo{}{x}{\xi+} \cap \geo{}{y}{\xi-} = \varnothing$. 
%Theorem \ref{thm:nonint} then implies that $\xi\in\supp{\mu_{x,y}}$.
\end{proof}



\begin{proof}[Proof of Theorem \ref{thm:1path}] 
The equivalence  \eqref{eq100}$\iff$\eqref{eq103} of Proposition \ref{pr:supp1}, together with the uniqueness of finite geodesics, gives Theorem \ref{thm:1path}. 
\end{proof} 

%We now turn to the proof of Lemma \ref{lm:isolated}, which says that the support of $\mu_{x,y}$ is nowhere dense.

\begin{proof}[Proof of Lemma \ref{lm:isolated}]
For $\xi \in \Udense$, almost surely 
$\coal{\xi+}(x,y)=\coal{\xi-}(x,y)=\coal{\xi}(x,y)\in\Z^2$.  Proposition \ref{pr:supp2} implies that $\xi$   lies in the complement of the closed set $\supp{\mu_{x,y}}$.  
%
%
%Theorem \ref{thm1}\eqref{thm1:coal} says that for any $\xi\in\ri\Uset$, any $\w\in\Omega_\xi^3$, and any $x,y\in\Z^2$ we have 
%$\coal{\xi\pm}(x,y)\in\Z^2$. Together with \eqref{B+=B-:temp} we get that 
%%Theorem \ref{thm:Bus}\eqref{thm:cocyexist:g} implies that if $\xi\in\Diff$, then for any $\w\in\Omega_\xi$ there is in fact 
%%no $\pm$ distinction.
%%Together, these two facts imply that 
%for any $\w\in\Omega_0$,  $\xi\in\Udense$, and $x,y\in\Z^2$, 
%$\coal{\xi+}(x,y) = \coal{\xi-}(x,y)\in \bbZ^2$. 
%%Proposition \ref{pr:supp2} implies that $\xi \notin \supp{\mu_{x,y}}$.  
%Now, let $x \cdot \et = k$, $y \cdot \et = \ell$, and $\coal{\xi}(x,y) \cdot \et = m$. Take sequences $\zeta_n,\eta_n \in \Udense$ with $\zeta_n \nearrow \xi$ and $\eta_n \searrow \xi$.  By \eqref{pmgeolim}, for $n$ sufficiently large, we have $\geo{k,m}{x}{\zeta_n\pm} = \geo{k,m}{x}{\xi-}$ and $\geo{\ell,m}{y}{\eta_n} = \geo{\ell,m}{y}{\xi+}$. Proposition \ref{pr:supp1} then says that for such an $n$, $]\zeta_n,\xi[$ and $]\xi,\eta_n[$ do not intersect $\supp{\mu_{x,y}}$.
\end{proof}


Next, we prove Theorem \ref{thm:supp-tri} about the relation between the coalescence points and properties of the support of Busemann measures.

%\begin{theorem}\label{th:isopt}
%%Let $\Omega_0$ be the full measure event in Proposition \ref{pr:supp2}.
%%There exists a $T$-invariant Borel set $\Omega_0 \subset \Omega$ with $\bbP(\Omega_0) = 1$ so that 
%For all $\w \in \Omega_0$, all $x,y \in \bbZ^2$, and $\xi \in \ri \Uset$, the following are equivalent.
%\begin{enumerate} [label={\rm(\alph*)}, ref={\rm\alph*}]   \itemsep=3pt 
%\item\label{prop:isopt:1} $\coal{\xi+}(x,y), \coal{\xi-}(x,y) \in \bbZ^2$ and $\coal{\xi+}(x,y) \neq \coal{\xi-}(x,y)$.
%\item\label{prop:isopt:2} $\xi$ is an isolated point of $\supp{\mu_{x,y}}$.
% \end{enumerate}
%\end{theorem}
%



\begin{proof}[Proof of Theorem \ref{thm:supp-tri}]
Take $\w\in\Omega_0$.
Equivalence \eqref{thm:supp-tri:1} follows from Proposition \ref{pr:supp2}. 
Equivalence \eqref{thm:supp-tri:2} follows from the  equivalences in \eqref{thm:supp-tri:1} and \eqref{thm:supp-tri:3}.
%isolated implies not left nor right limit which implies both coalescence points are on the lattice. but then being in the support implies the points have to be different.   for other direction, different coalescence points implies \xi is in the spport and and both on the lattice implies isolated on both sides. 

The two equivalences of   \eqref{thm:supp-tri:3}  are proved the same way. 
We prove the first equivalence  in this form:  $\exists \eta\succ\xi$ such that $\abs{\mu_{x,y}}(\,]\xi, \eta[\,)=0$    $\iff$ $\coal{\xi+}(x,y)\in \bbZ^2$. 

 The implication $\implies$  is contained  in \eqref{eq100}$\implies$\eqref{eq101} of Proposition \ref{pr:supp1}.    

To prove $\rimplies$, let $k=x \cdot \et $ and $\ell=y \cdot \et$,  suppose $\coal{\xi+}(x,y)\in \bbZ^2$, and let $m = \coal{\xi+}(x,y) \cdot \et$.   Take a sequence $\eta_n \in \Udense$ with $\eta_n \searrow \xi$ as $n\to\infty$.   For sufficiently large $n$,   $\geo{k,m}{x}{\xi+} = \geo{k,m}{x}{\eta_n}$ and  $\geo{\ell,m}{y}{\xi+} = \geo{\ell,m}{y}{\eta_n}$, and hence $\coal{\eta_n}(x,y)=\coal{\xi+}(x,y)$.
Implication  \eqref{eq102}$\implies$\eqref{eq100} of Proposition \ref{pr:supp1} gives 
$\abs{\mu_{x,y}}(\,]\xi, \eta_n[\,)=0$.  
%%%%%%    OLD PROOF.  DELETE IF NOT NEEDED?  %%%%%%%
%Since $\zeta_n,\eta_n \in \Udense$, we know that $\coal{\zeta_n}(x,y),\coal{\eta_n}(x,y) \in \bbZ^2$. Let $\coal{\zeta_n}(x,y) \cdot \et = m_n$ and let $\coal{\eta_n}(x,y) \cdot \et = r_n$.  It follows from Proposition \ref{pr:supp1} and the convergence of geodesics that for $n$ sufficiently large, $\geo{k,m_n}{x}{\zeta_n} = \geo{k,m_n}{x}{\xi-}$, $\geo{\ell,m_n}{y}{\zeta_n} = \geo{\ell,m_n}{y}{\xi-}$, $\geo{k,m_n}{x}{\eta_n} = \geo{k,m_n}{x}{\xi+}$, and $\geo{\ell,m_n}{y}{\eta_n} = \geo{\ell,m_n}{y}{\xi+}$. 
%But then since $\xi \in \supp{\mu_{x,y}}$, the equivalence of \eqref{eq110} and \eqref{eq111} in Proposition \ref{pr:supp2}, and the just proved fact that $\coal{\xi+}(x,y) \in \bbZ^2$ imply $\coal{\xi+}(x,y) \neq \coal{\xi-}(x,y)$.
\end{proof}

%PROOF OF AN OLDER VERSION:
%\begin{proof}[Proof of Theorem \ref{thm:supp-tri}]
%Equivalence \eqref{thm:supp-tri:1} follows from Proposition \ref{pr:supp2}. We prove equivalence \eqref{thm:supp-tri:2}, \eqref{thm:supp-tri:3} being similar.
%
%Take sequences $\zeta_n, \eta_n \in \Udense$ with $\zeta_n \nearrow \xi$ and $\eta_n \searrow \xi$ as $n\to\infty$. Let $x \cdot \et = k$ and $y \cdot \et = \ell$.
%
%Suppose first that \eqref{prop:isopt:1} holds.
%It follows from Proposition \ref{pr:supp2} that $\xi \in \supp{\mu_{x,y}}$. Let $m = \coal{\xi+}(x,y) \cdot \et$ and $r = \coal{\xi-}(x,y) \cdot \et$. For sufficiently large $n$, we have $\geo{k,m}{x}{\xi+} = \geo{k,m}{x}{\eta_n}$, $\geo{k,r}{x}{\xi-} = \geo{k,r}{x}{\zeta_n}$, $\geo{\ell,m}{y}{\xi+} = \geo{\ell,m}{y}{\eta_n}$, and $\geo{\ell,r}{y}{\xi-} = \geo{\ell,r}{y}{\zeta_n}$. In particular, $\coal{\eta_n}(x,y)=\coal{\xi+}(x,y)$ and $\coal{\zeta_n}(x,y)=\coal{\xi-}(x,y)$.
%It follows from this and \eqref{eq:busdiff} that for sufficiently large $n$, $\B{\eta_n}_{x,y}=\B{\xi+}_{x,y}$ and $\B{\zeta_n}_{x,y}=\B{\xi-}_{x,y}$. By Proposition \ref{pr:supp1}, both processes $\zeta \mapsto \B{\zeta\pm}_{x,y}$ match and are constant on each of $]\zeta_n,\xi[$ and $]\xi,\eta_n[$ and so it follows that $\xi$ is isolated in $\supp{\mu_{x,y}}$.
%
%Conversely, suppose that $\xi$ is an isolated point of $\supp{\mu_{x,y}}$. Then for $n$ sufficiently large, both processes $\zeta \mapsto \B{\zeta\pm}_{x,y}$ match and are constant on each of $]\zeta_n,\xi[$ and $]\xi,\eta_n[$. %and thus $\B{\eta_n}(x,y)=\B{\xi+}(x,y)$ and $\B{\zeta_n}(x,y)=\B{\xi-}(x,y)$. 
%The equivalence between \eqref{eq100} and \eqref{eq101} in Proposition \ref{pr:supp1} implies that 
%$\coal{\xi-}(x,y)$ and $\coal{\xi+}(x,y)$ are both in $\Z^2$.
%%Since $\zeta_n,\eta_n \in \Udense$, we know that $\coal{\zeta_n}(x,y),\coal{\eta_n}(x,y) \in \bbZ^2$. Let $\coal{\zeta_n}(x,y) \cdot \et = m_n$ and let $\coal{\eta_n}(x,y) \cdot \et = r_n$.  It follows from Proposition \ref{pr:supp1} and the convergence of geodesics that for $n$ sufficiently large, $\geo{k,m_n}{x}{\zeta_n} = \geo{k,m_n}{x}{\xi-}$, $\geo{\ell,m_n}{y}{\zeta_n} = \geo{\ell,m_n}{y}{\xi-}$, $\geo{k,m_n}{x}{\eta_n} = \geo{k,m_n}{x}{\xi+}$, and $\geo{\ell,m_n}{y}{\eta_n} = \geo{\ell,m_n}{y}{\xi+}$. 
%But then since $\xi \in \supp{\mu_{x,y}}$, the equivalence of \eqref{eq110} and \eqref{eq111} in Proposition \ref{pr:supp2}, and the just proved fact that $\coal{\xi+}(x,y), \coal{\xi-}(x,y) \in \bbZ^2$ imply $\coal{\xi+}(x,y) \neq \coal{\xi-}(x,y)$.
%\end{proof}

When the jump process condition \eqref{cond:jumpcond} holds,  call the event in the statement of that condition $\Omega_0^5$. 
As noted when it was introduced, Theorem \ref{thm:+-coal}, which gives the equivalence between  \eqref{cond:jumpcond} and coalescence of $\xi\sigg$ geodesics, is essentially an immediate consequence of Theorem \ref{thm:supp-tri}. 


\begin{proof}[Proof of Theorem \ref{thm:+-coal}]
Assume the jump process condition \eqref{cond:jumpcond}. Fix $\w\in\Omega_0\cap\Omega_0^5$, $x,y\in\Z^2$, and $\xi\in\ri\Uset$. 
If $\xi\not\in\supp{\mu_{x,y}}$, then Proposition \ref{pr:supp2} says that $\coal{\xi-}(x,y)=\coal{\xi+}(x,y)\in\Z^2$. In particular, $\geo{}{x}{\xi+}$ coalesces with $\geo{}{y}{\xi+}$ and $\geo{}{x}{\xi-}$ coalesces with $\geo{}{y}{\xi-}$. If, on the other hand, $\xi\in\supp{\mu_{x,y}}$, then it is an isolated point and now Theorem \ref{thm:supp-tri} says that $\coal{\xi\pm}(x,y)\in\Z^2$ (although now the two points are not equal). 
Again, $\geo{}{x}{\xi\pm}$ coalesces with $\geo{}{y}{\xi\pm}$, respectively. 
Statement  \eqref{thm:+-coal.b} is proved.

Now, assume \eqref{thm:+-coal.b} holds and let $\Omega_0^6$ be a full measure event on which the statement \eqref{thm:+-coal.b} holds. Let $\w\in\Omega_0\cap\Omega_0^6$, 
$x,y\in\Z^2$, and $\xi\in\supp{\mu_{x,y}}$. The fact that $\geo{}{x}{\xi\pm}$ and $\geo{}{y}{\xi\pm}$ coalesce, respectively, says that $\coal{\xi\pm}(x,y)\in\Z^2$. Since we assumed  $\xi\in\supp{\mu_{x,y}}$, Proposition \ref{pr:supp2} implies that the two coalescence  points $\coal{\xi\pm}(x,y)$  are not equal.
   Theorem \ref{thm:supp-tri} implies that $\xi$ is isolated.
\end{proof}

The proof of Lemma \ref{lm:downright} is delayed to the end of Section \ref{shockgraphs:pfs}.
When  the jump process condition  \eqref{cond:jumpcond} holds, define 
	\begin{align}\label{Omjump}
	\Omjump=\Omega_0\cap\Omega_0^5.  %\bigcap_{x\in\Z^2} T_x(\Omega_0^5\cap\Omega_0^6)$.
	\end{align}
	
	
\begin{proof}[Proof of Theorem \ref{thm:Vcid}]
Part \eqref{thm:Vcid.1}.  Take $\w\in\Omega_0$.
Let $x \cdot \et = k$ and   $\xi = \cid(T_x\w)$. Take  $T_x\w$ in place of $\w$ in \eqref{cid},  let  $\zeta\to\cid(T_x\w)$, and use \eqref{cov-prop}, \eqref{coc-prop}, and \eqref{Busemann-limits},   to get $\B{\xi-}(x,x+e_2)\le\B{\xi-}(x,x+e_1)$ and $\B{\xi+}(x,x+e_1)\le\B{\xi+}(x,x+e_2)$. 
Then by definition $\geo{k}{x}{\xi+}  = \geo{k}{x}{\xi-} =x$,  $\geo{k+1}{x}{\xi+} = x+  e_1$, and $\geo{k+1}{x}{\xi-} =  x + e_2$.  Therefore we cannot have $\coal{\xi+}(x,x+e_i) = \coal{\xi-}(x,x+e_i) \in \bbZ^2$ for either $i \in \{1,2\}$ by uniqueness of finite geodesics. By Proposition \ref{pr:supp2},   $\xi \in \supp \mu_{x,x+e_1}\cap \supp \mu_{x,x+e_2}$.  

For the converse, for $\zeta\prec\cid(T_x\w)\prec\eta $ we have  $\B{\zeta\pm}(x,x+e_2)=\w_x=\B{\eta\pm}(x,x+e_1) $.  Thus 
\[  
  \supp\mu_{x,x+e_1} \subset \,] e_2\,, \cid(T_x\w)] \quad\text{and}\quad
\supp \mu_{x,x+e_2} \subset [\cid(T_x\w), e_1[ .  \] 
Consequently,  $\supp \mu_{x,x+e_1} \cap \supp\mu_{x,x+e_2} \subset \{\cid(T_x\w)\}$.
 
\medskip 

Part \eqref{thm:Vcid.2}.   
 It remains to show  $\aUset\subset\{\cid(T_x\w):x\in\Z^2\}$. 
Assume the jump process condition \eqref{cond:jumpcond}
and that $\w\in\Omjump$.
Suppose $\zeta\in\supp\mu_{x,y}$. 
%\addmath{is it clear what is being said here?}
By Theorem \ref{thm:supp-tri}\eqref{thm:supp-tri:2} the coalescence points  $\coal{\zeta\pm}(x,y)$ are distinct lattice points.    Hence the  geodesics $\geo{}{x}{\zeta+}$ and $\geo{}{x}{\zeta-}$  separate at some  point $z$ where then  $\cid(T_z\w)=\zeta$.  
%Same is true for the  geodesics $\geo{}{y}{\zeta+}$ and $\geo{}{y}{\zeta-}$. 
%%%%%%%%%     OLDER VERSION OF PROOF  %%%%%%
%If it happens that $\geo{}{x}{\xi+}=\geo{}{x}{\xi-}$ for all $x\in\Z^2$, then Theorem \ref{thm:+-coal} would imply that all these geodesics coalesce and thus for any $x,y\in\Z^2$, $\coal{\xi+}(x,y)=\coal{\xi-}(x,y)\in\Z^2$. Proposition \ref{pr:supp2} then says that $\xi\not\in\supp{\mu_{x,y}}$. We thus see that if $\xi\in\aUset$, then
%there must exist an $x\in\Z^2$ such that $\geo{}{x}{\xi\pm}$ eventually separate, say at a point $z\in\Z^2$. 
%Then Theorem \ref{thm:cif}\eqref{thm:cif:(ii)} gives $\xi=\cid(T_z\w)$ and thus $\aUset\subset\{\cid(T_x\w):x\in\Z^2\}$
%and part \eqref{th:V1.1} is proved. 
%%%%%%%%%%%%%%%%%%%%%%%%%%  OLD  %%%%%%%%
\end{proof} 	

The next results relate   $\aUset$ to regularity properties of the shape function $\gpp$.  

% The event $\Omreg$ is defined in Lemma \ref{lm:B+>B-} in Appendix \ref{a:aux}.  

%We turn to the proof of Theorem \ref{th:V1}, which identifies some properties of $\aUset$ and in particular shows that under the jump process condition \eqref{cond:jumpcond}, these exceptional directions are all directions of competition interfaces.

\begin{lemma}\label{lm:V1}
The following holds for   all $\w\in\Omega_0$:  
for all  $\zeta\prec\eta$ in $\ri\Uset$,    $\,]\zeta,\eta[\,\cap\,\aUset\ne\varnothing$ if and only if $\nabla\gpp(\zeta+)\ne\nabla\gpp(\eta-)$. 
\end{lemma} 

%%%%%%%%   Old version %%%%%%%
%\begin{lemma}\label{lm:V1}
%The following hold for   all $\w\in\Omega_0$. %$\P$-almost every $\w$.
%\begin{enumerate}[label={\rm(\alph*)}, ref={\rm\alph*}] \itemsep=3pt 
%\item\label{lm:V1.0} 
%Let $\zeta\prec\eta$ in $\ri\Uset$.  Then $\,]\zeta,\eta[\,\cap\,\aUset\ne\varnothing$ if and only if $\nabla\gpp(\zeta+)\ne\nabla\gpp(\eta-)$. 
%  \item\label{lm:V1.0'} 
%Let $\zeta\prec\eta$ in $\ri\Uset$.  If $\nabla\gpp(\zeta-)=\nabla\gpp(\eta-)$, then $[\zeta,\eta[\,\cap\,\aUset=\varnothing$. Similarly, if 
%$\nabla\gpp(\zeta+)=\nabla\gpp(\eta+)$, then $]\zeta,\eta]\cap\,\aUset=\varnothing$. 
%Under  the regularity condition \eqref{g-reg}  these implications are  equivalences on the full-probability event   $\Omreg\subset\Omega_0$.
% \end{enumerate}
%\end{lemma} 

\begin{proof} 

%Part \eqref{lm:V1.0}.
If $\nabla\gpp(\zeta+)\ne\nabla\gpp(\eta-)$,  Theorem \ref{thm:cif}\eqref{thm:cif.c} says   that $]\zeta,\eta[$ contains some $\cid(T_x\w)$, which  by Theorem \ref{thm:Vcid}\eqref{thm:Vcid.1}  is a member of $\aUset$. 

%Assume first that $\nabla\gpp(\zeta+)\ne\nabla\gpp(\eta-)$. Note that Theorems \ref{thm:cif}\eqref{thm:cif:(ii)} and \ref{thm:nonint} imply that  $\{\cid(T_x\w):x\in\Z^2\}\subset\aUset$. This and Theorem \ref{thm:cif}\eqref{thm:cif.c} imply that $]\zeta,\eta[\,\subset\aUset$.

If $\nabla\gpp(\zeta+)=\nabla\gpp(\eta-)$, then by concavity,   $\nabla\gpp(\zeta+)=\nabla\gpp(\eta-)=\nabla\gpp(\xi\sig)$ for all $\xi\in\,]\zeta,\eta[$ and $\sigg\in\{-,+\}$.  By  Theorem \ref{thm:Bus}\eqref{thm:cocyexist:foo},    $\B{\xi\sig}(x,y,\w)$ is constant over $\xi\in\,]\zeta,\eta[$ and  $\sigg\in\{-,+\}$, for any $x,y\in\Z^2$ and $\w\in\Omega$.  Consequently,  for  any given $x$,  the geodesics  $\geo{}{x}{\xi\sig}$ match.    By Theorem \ref{thm1}\eqref{thm1:coal}, all these geodesics  coalesce on the event $\Omega_0$.   Hence  the coalescence points $\coal{\xi\sig}(x,y)$ also match.  By Theorem \ref{thm:supp-tri}\eqref{thm:supp-tri:1}, no point $\xi\in\,]\zeta,\eta[$ is a member of $\aUset$. 
%
%
%Conversely, suppose $\nabla\gpp(\zeta+)=\nabla\gpp(\eta-)$. By concavity, these two are equal 
%to $\nabla\gpp(\xi\pm)$ for all $\xi\in\,]\zeta,\eta[$. Theorem \ref{thm:Bus}\eqref{thm:cocyexist:foo} implies then that for any $x,y\in\Z^2$ and $\sigg\in\{-,+\}$, $\B{\xi\sig}(x,y,\w)$ is constant over $\xi\in\,]\zeta,\eta[$. 
%%Now take $\w\in\Omega_0$. Then 
%Taking $\xi'\in\,]\zeta,\eta[\,\cap\Diff$ we have by \eqref{B+=B-:temp} that $\B{\xi'\pm}(x,y,\w)$ match and hence 
%$\B{\xi\pm}(x,y,\w)$ match for all $\xi\in\,]\zeta,\eta[$.
%Hence, $\geo{}{x}{\xi\pm}$ match and equal $\geo{}{x}{\xi'}$ for all $x\in\Z^2$ and $\xi\in\,]\zeta,\eta[$. 
%By Theorem \ref{thm1}\eqref{thm1:coal}, all these geodesics  coalesce. By Theorem \ref{th:V2}\eqref{th:V2.a}, $\xi\not\in\aUset$ for any $\xi\in\,]\zeta,\eta[$. Claim \eqref{th:V1.0} is proved.
%
%\medskip
%
%Part \eqref{lm:V1.0'}.  In the first case  $\nabla\gpp(\zeta-)=\nabla\gpp(\zeta+)=\nabla\gpp(\eta-)$ so the Busemann functions $\B{\xi\sig}(x,y,\w)$ coincide for $\xi\in[\zeta,\eta[\,$. 
%The   argument of part \eqref{lm:V1.0} works again. The case $\nabla\gpp(\zeta+)=\nabla\gpp(\eta+)$ is similar.
%
%By Lemma \ref{lm:B+>B-},   
% $(\ri\Uset)\setminus\Diff\subset\aUset$ for  $\w\in\Omreg\subset\Omega_0$. 
% %In other words, $\aUset$ contains all points of non-differentiability of $\gpp$  almost surely. 
% Together with part \eqref{lm:V1.0},  this turns the implications in part \eqref{lm:V1.0'} into equivalences.
%%%%%%%%% OLD 
%Now  $\nabla\gpp(\zeta-)=\nabla\gpp(\zeta+)=\nabla\gpp(\eta-)$.
%Part \eqref{th:V1.0} implies that $]\zeta,\eta[\,\cap\aUset=\varnothing$. We also
%have $\zeta\in\Diff$. But then  $\nabla\gpp(\zeta\pm)$ match and equal $\nabla\gpp(\xi')$, from the proof of \eqref{th:V1.0}. The same argument as above implies that $\geo{}{x}{\zeta\pm}$ match and equal $\geo{}{x}{\xi'}$ and all these geodesics coalesce. Again, we conclude that $\zeta\not\in\aUset$. The same works for the case $\nabla\gpp(\zeta+)=\nabla\gpp(\eta+)$.
%\medskip
\end{proof}
 
 
\begin{proof}[Proof of Theorem \ref{th:V1}]
Part \eqref{th:V1.a}. Let $\xi \in \Diff$.
Theorem \ref{thm1}\eqref{thm1:coal} says that almost surely $\coal{\xi\pm}(x,x+e_i)\in\Z^2$   for    $x\in\Z^2$ and $i\in\{1,2\}$. 
Theorem \ref{thm:Bus}\eqref{thm:cocyexist:g} says that there is  no $\pm$ distinction.
Hence $\mathbb{P}(\coal{\xi-}(x,x+e_i)=\coal{\xi+}(x,x+e_i)\in\Z^2)=1$ and therefore $\bbP(\xi \in \supp \mu_{x,x+e_i})=0$ by Proposition \ref{pr:supp2}.  A union bound implies that $\bbP(\exists x\in\Z^2,i\in\{1,2\}:\xi \in \supp \mu_{x,x+e_i})=0$. 
%\addmath{do we want to spell this out?  it's commented out for now}
%If $\xi\not\in\supp\mu_{x,x+e_i}$ for all $x$ and all $i$, then $\xi\not\in\supp{\mu_{x,y}}$ for any $x,y$ because $\abs{\mu_{x,y}}$ is a sum of measures of the form $\abs{\mu_{z,z+e_i}}$.
The cocycle property \eqref{coc-prop} implies then that $\bbP(\xi \in \aUset)=0$.

Let $\xi \in\ri\Uset\setminus\Diff$.  Theorem \ref{thm:cif}\eqref{thm:cif.c1} implies that $\xi$ is among $\{\cid(T_x\w): x\in\Z^2\}$, and these lie in $\aUset$ by   Theorem \ref{thm:Vcid}\eqref{thm:Vcid.1}. 

%Conversely, suppose that $\xi \notin \Diff$.
%By homogeneity $\gpp(\xi)=\xi\cdot\nabla\gpp(\xi\pm)$. This  forces  $\nabla\gpp(\xi-)\cdot e_i\ne\nabla\gpp(\xi+)\cdot e_i$ for both $i\in\{1,2\}$. 
%By \eqref{E[h(B)]}, $\bbE[\B{\xi+}(x,x+e_i)] \neq \bbE[\B{\xi-}(x,x+e_i)]$ and
%	\[\bbP(\xi\in\aUset)\ge\bbP(\xi \in \supp \mu_{x,x+e_i})\ge\bbP\bigl(\B{\xi+}(x,x+e_i) \neq \B{\xi-}(x,x+e_i)\bigr) > 0.\]

\medskip 

Part \eqref{th:V1.b}. 
 By definition,  the complement of $\fUset$ is the   union of the (at most countably many)  maximal open intervals $\,]\zeta,\eta[\,$ such that $\nabla\gpp(\zeta+)=\nabla\gpp(\eta-)$ and their differentiable endpoints.  Lemma \ref{lm:V1} together with  part \eqref{th:V1.a} proved above imply that 
$\P(\aUset\cap\fUset^c\ne\varnothing)=0$.  Hence almost surely, $\{\cid(T_x\w): x\in\Z^2\}\subset\aUset\subset\fUset$. 

% By definition,  $\fUset$ is the complement in $\ri\Uset$ of the union 
%\begin{align*}
%\{ \, ]\zeta,\eta[\,:  \nabla\gpp(\zeta+)=\nabla\gpp(\eta-)\} 
%\cup  \{  [\zeta,\eta[\,:  \nabla\gpp(\zeta-)=\nabla\gpp(\eta-)\}
%\cup  \{  \,]\zeta,\eta]:  \nabla\gpp(\zeta+)=\nabla\gpp(\eta+)\}  
%\end{align*} 
%that can be expressed in terms   of  an at most countable family of   nonempty  intervals.   
%Lemma \ref{lm:V1} implies $\P(\aUset\subset\fUset)=1$.
 
For the density claim it is enough to prove that  $\{\cid(T_x\w): x\in\Z^2\}$ is dense in $\fUset$. 
Suppose first that   $\xi\in\fUset\cap\Diff$.  Then $\xi$ is not on a closed linear segment of $\gpp$, and hence for any $\zeta\prec\xi\prec\eta$ we have $\nabla\gpp(\zeta+)\ne\nabla\gpp(\eta-)$.  By Theorem \ref{thm:cif}\eqref{thm:cif.c} the open interval $\,]\zeta,\eta[\,$ contains a value $\cid(T_x\w)$.  
 The other case is $\xi\in\fUset\setminus\Diff$. Then  $\xi\in\{\cid(T_x\w): x\in\Z^2\}$  by Theorem \ref{thm:cif}\eqref{thm:cif.c1}. 
\end{proof}



The next proof, of Theorem \ref{th:V2},  identifies $\Uset \backslash \aUset$ in terms of directions in which (Busemann) geodesic uniqueness holds.

\begin{proof}[Proof of Theorem \ref{th:V2}]
Part \eqref{th:V2.a}. 
Fix $\w\in\Omega_0$ and $\xi\in\ri\Uset$.
Suppose first that there exists an $x \in \bbZ^2$ with the property that $\geo{}{x}{\xi+} \neq \geo{}{x}{\xi-}$.  These geodesics separate at some point $z$  where then $\xi=\cid(T_z\w)\in\aUset$. 
%  Since the two geodesics cannot meet after having split,  Theorem \ref{thm:nonint} implies $\xi\in\supp\mu_{z+e_1,z+e_2}\subset\aUset$.
%Then 
%	\[\w_z=\B{\xi+}(z,z+e_1)\le\B{\xi+}(z,z+e_2)\quad\text{and}\quad\w_z=\B{\xi-}(z,z+e_2)\le\B{\xi+}(z,z+e_1).\]
%%if \xi\prec\cid\circ T_z, we woud have \B{\xi\pm}(z,z+e_1)>\B{\xi\pm}(z,z+e_2)
%%so \xi\suceq\cid\circ T_z.  similarly, \xi\preceq\cid\circ T_z
%This and \eqref{cid} imply that $\xi = \cid(T_z \w)$.
%Theorems \ref{thm1}\eqref{thm1:exist}, \ref{thm:cif}\eqref{thm:cif:(ii)}, and \ref{thm:nonint} imply that $\cid(T_x\w)\in\supp{\mu_{x+e_1,x+e_2}}\subset\aUset$.  
%Thus, $\xi \in \aUset$. 
If, on the other hand, $\geo{}{x}{\xi+} = \geo{}{x}{\xi-}$ for all $x \in \bbZ^2$, but there exist $x$ and $y$ for which $\geo{}{x}{\xi}$ and $\geo{}{y}{\xi}$ do not coalesce, then   Proposition \ref{pr:supp2}  implies that $\xi \in \supp{\mu_{x,y}} \subset \aUset$.  

Conversely, suppose $\xi \in \aUset$ and let $x,y$ be such that $\xi \in \supp{\mu_{x,y}}$. Then by Theorem \ref{thm:nonint}, possibly after interchanging the roles of $x$ and $y$, we have $\geo{}{x}{\xi+} \cap \geo{}{y}{\xi-} = \varnothing$. In particular, these two geodesics do not coalesce. Part \eqref{th:V2.a} is proved.

%\smallskip 

Part \eqref{th:V2.c}.  Assume the jump process condition \eqref{cond:jumpcond} and let $\w\in\Omjump$. Suppose that 
$\geo{}{x}{\xi+}=\geo{}{x}{\xi-}=\geo{}{x}{\xi}$.   By Theorem \ref{thm:+-coal},  
  $\geo{}{y}{\xi\sig}$ coalesces with $\geo{}{x}{\xi}$ for all   $y\in\Z^2$ and both signs $\sigg\in\{-,+\}$.    By the uniqueness of finite geodesics $\geo{}{y}{\xi+}=\geo{}{y}{\xi-}$.  Now  all these geodesics coalesce.  Part \eqref{th:V2.a} implies  $\xi\notin\aUset$.  
% That $\xi\notin\aUset$ implies  $\geo{}{x}{\xi+}=\geo{}{x}{\xi-}$ follows from the already proved part \eqref{th:V2.a}. 
% \eqref{th:V2.c} holds.

Parts \eqref{th:V2.b} and \eqref{th:V2.d}  follow  from  \eqref{th:V2.a} and \eqref{th:V2.c}, respectively, because  under the regularity condition \eqref{g-reg}, Theorem \ref{thm:extreme} implies that the uniqueness of a $\Uset_\xi$-directed geodesic out of $x$ is equivalent to  $\geo{}{x}{\xi+}=\geo{}{x}{\xi-}$. 
\end{proof}

The next lemma completes the proof of Theorem \ref{th:capst}.  Recall the event $\Omega_0$ defined in \eqref{Om0}.

\begin{lemma}\label{lm:capst-aux}
Assume  the regularity condition \eqref{g-reg}. If $\w\in\Omega_0$ and $\xi \in \aUset$, then $\Uset_\xi = \{\xi\}$.
\end{lemma}

\begin{proof}
%Suppose that $\Uset_\xi \neq \{\xi\}$. Recall the dense set of differentiability directions $\Udense$ introduced just before \eqref{Om0} and the definition of $\Omega_0$ in that equation. Because $\Uset_\xi$ is a line segment in $\Uset$, the intersection $\Udense \cap \Uset_\xi$ is not empty. Theorem \ref{thm:Bus}\eqref{thm:cocyexist:foo} implies that for all $x,y \in \bbZ^2$ and all directions $\zeta,\eta \in \Uset_\xi, \B{\zeta+}(x,y) = \B{\eta-}(x,y)$. For $\zeta \in \Udense \cap \Uset_\xi$, we have $\Omega_\zeta^3 \subset \Omega_0$, where $\Omega_\zeta^3$ is the event introduced in Theorem \ref{thm1}.  Theorem \ref{thm1}\eqref{thm1:cont} then implies that $\coal{\xi+}(x,y) = \coal{\xi-}(x,y)\in\Z^2$ for each pair $x,y$. Theorem \ref{thm:supp-tri}\eqref{thm:supp-tri:1} now shows that $\xi \notin \aUset$.
Take $\w\in\Omega_0$ and
suppose  $\Uset_\xi \neq \{\xi\}$. Recall the dense set of differentiability directions $\Udense$ introduced just before \eqref{Om0}. Because $\Uset_\xi$ is a line segment in $\Uset$, there exists a $\zeta\in\Udense \cap \Uset_\xi$.
By its definition, $\Omega_0\subset\Omega_\zeta^3$, where $\Omega_\zeta^3$ was introduced in Theorem \ref{thm1}. 
Theorem \ref{thm1}\eqref{thm1:cont} then implies that $\coal{\zeta-}(x,y) = \coal{\zeta+}(x,y)\in\Z^2$ for each pair $x,y$. 
Since $\zeta,\xi\in\Uset_\xi$ and we assumed \eqref{g-reg}, Theorem \ref{thm:Bus}\eqref{thm:cocyexist:foo} implies that for all $x,y \in \bbZ^2$, $\B{\zeta-}(x,y) = \B{\zeta+}(x,y)=\B{\xi-}(x,y)=\B{\xi+}(x,y)$. 
Consequently, $\coal{\xi-}(x,y) = \coal{\xi+}(x,y)\in\Z^2$ for all $x,y\in\Z^2$ and Theorem \ref{thm:supp-tri}\eqref{thm:supp-tri:1} shows that $\xi \notin \aUset$.
\end{proof}

\begin{proof}[Proof of Theorem \ref{th:exp1}]
Part  \eqref{th:exp1.a}. Theorem \ref{thm-Coupier} implies  that for $\xi\in\aUset$, $\geo{}{x}{\xi-}$ and $\geo{}{x}{\xi+}$  are the only $\xi$-directed geodesics out of $x$.  

Part  \eqref{th:exp1.b}.  Consider any  three  geodesics with the same asymptotic direction $\xi\in\ri\Uset$.  If $\xi\in(\ri\Uset)\setminus\aUset$ then by Theorem \ref{th:capst}\eqref{th:capst.c} all three coalesce.   If $\xi\in\aUset$ then by part  \eqref{th:exp1.a} 
  at least  two of these three geodesics must have the same sign $+$ or $-$.  By Theorem \ref{th:capst}\eqref{th:capst.d}  these two coalesce.   
  
Part \eqref{th:exp1.c}. Consider a sequence $v_n$ as in the first part of the statement and call $k = x \cdot \ehat$. From an arbitrary subsequence, extract a further subsequence $n_\ell$ so that $\geo{k,\infty}{x}{v_{n_\ell}}$ converges to a semi-infinite geodesic $\pi_{k,\infty}$  vertex-by-vertex. Let $\zeta \prec \xi \prec \eta$. Using the fact that $v_n/n \to \xi$ and directedness of $\geo{}{x}{\zeta+}$ and $\geo{}{x}{\eta-}$, for all sufficiently large $n$, we must have $\geo{n}{x}{\zeta+} \prec v_n \prec \geo{n}{x}{\eta-}$.  By uniqueness of finite geodesics, we must then have  $\geo{m}{x}{\zeta+} \prec \geo{m}{x}{v_n} \prec \geo{m}{x}{\eta-}$ for all $m \geq x \cdot \ehat$ and all such $n$. It then follows by sending $\zeta,\eta \to \xi$ that $\pi$ must be $\xi$-directed. Therefore, by part \eqref{th:exp1.a}, $\pi \in \{\geo{}{x}{\xi+}, \geo{}{x}{\xi-}\}$. Let $r = \spt{\xi}{x} \cdot \ehat$ and let $n_\ell$ be sufficiently large that $\geo{k,r+1}{x}{v_{n_\ell}} = \pi_{k,r+1}$. By definition of the competition interface, since $v_{n_\ell} \prec \varphi_{n_\ell}^{\spt{\xi}{x}}$ we must have $\pi_{r+1} =\spt{\xi}{x} + e_2$, which identifies $\pi$ as $\geo{}{x}{\xi-}$.  As the subsequence was arbitrary,  the result follows. The second claim is similar.

Part \eqref{th:exp1:d}. By Theorem \ref{thm1}\eqref{thm1:direct}, any semi-infinite geodesic emanating from $x$ is $\xi$-directed for some $\xi \in \Uset$. Combining part \eqref{th:exp1.a} and Theorem \ref{th:capst}\eqref{th:capst.c}, the only claim which remains to be shown is that $\geo{}{x}{e_i}$ is the only $e_i$-directed geodesic. This comes from Lemma \ref{lem:notriv}.   %CHANGED HERE
\end{proof}  


%%%%%%%     OLD PROOF OF EXPONENTIAL THM  %%%%%%
%\begin{proof}[Proof of Theorem \ref{th:exp1}] Recall that when the weights are exponentially distributed, the jump process condition \eqref{cond:jumpcond} holds. Recall also the full measure event $\OmCou$ from Theorem \ref{thm-Coupier}.
%Fix $\w\in\Omjump\cap\OmCou$.
%
%Part \eqref{th:exp1.a} holds because $\xi\in\aUset$ if and only if $\xi\in\supp\mu_{x,y}$ for some $x,y\in\Z^2$, which due to \eqref{cond:jumpcond} holds if and only if $\B{\xi+}(x,y)\ne\B{\xi-}(x,y)$.
%Part \eqref{th:exp1.b} follows from Theorem \ref{th:V1}\eqref{th:V1.1}.
%
%%Lemma \ref{lm:alt-char} implies that for $\w\in\Omega_0$, $\{\cid(T_x\w):x\in\Z^2\}\subset\aUset$. 
%%On the other hand, if $\xi\in\aUset$, then parts \eqref{thm:shocks.c} and \eqref{thm:shocks.f} of Theorem \ref{thm:shocks} imply that there exist infinitely many lattice points $x$ with $\cid(T_x\w)=\xi$. 
%%This shows that $\aUset\subset\{\cid(T_x\w):x\in\Z^2\}$ and part \eqref{th:exp1.b} is proved. 
%
%Part \eqref{th:exp1.c} is a consequence of Theorem \ref{th:V2}\eqref{th:V2.b} because  % in the  case of exponentially distributed weights  
%the regularity condition \eqref{g-reg} holds and  $\gpp$ is strictly concave   so that    $\Uset_\xi=\{\xi\}$ for every $\xi\in\Uset$.
%
%Part \eqref{th:exp1.d}. Since  \eqref{cond:jumpcond} holds and $\w\in\Omjump\subset\Omega_0^6$, Theorem \ref{thm:+-coal} says that for any $\xi\in\ri\Uset$, $\{\geo{}{x}{\xi+}:x\in\Z^2\}$ all coalesce and  $\{\geo{}{x}{\xi-}:x\in\Z^2\}$ all coalesce.  Since $\Uset_\xi=\{\xi\}$, by Theorem \ref{thm1}\eqref{thm1:exist}   these geodesics are all $\xi$-directed. 
%
%If $\xi\in\aUset$, then by Theorem \ref{thm:nonint} there exist points $u,v\in\Z^2$ such that $\geo{}{u}{\xi-}\cap\geo{}{v}{\xi+}=\varnothing$. But we just argued that for any $x\in\Z^2$, $\geo{}{x}{\xi-}$ must coalesce with $\geo{}{u}{\xi-}$ and $\geo{}{x}{\xi+}$ must coalesce with $\geo{}{v}{\xi+}$. Hence, $\geo{}{x}{\xi\pm}$ must eventually separate. Now, since we are also assuming $\w\in\OmCou$ and we just showed that $\geo{}{x}{\xi\pm}$ are two different $\xi$-directed geodesics, Theorem \ref{thm-Coupier} says that they are the only two $\xi$-directed geodesics out of $x$. Part \eqref{th:exp1.d} is proved.
%\end{proof}
%%%%%%%    END OF OLD PROOF OF EXPONENTIAL THM  %%%%%%
 


==> JEMS Post-Accept Revision/GeoWebPaper-Sec7.tex <==
% !TEX root = GeoWebPaper.tex

\section{Webs of instability: proofs} \label{sec:webpf}

Recall again event $\Omega_0$ constructed in  \eqref{Om0} and fix $\w\in\Omega_0$ throughout this section.  Unless otherwise indicated, an assumption of the form  $\zeta\preceq\eta$ includes the case $\zeta=\eta=\xi$. 

\subsection{Instability points and graphs}\label{shockgraphs:pfs}
%Fix $\w\in\Omega_0$ throughout the whole section.


\begin{proof}[Proof of Lemma \ref{lem:shockequiv}]
Suppose  $x^*$ is a  $[\zeta,\eta]$-instability point. Then there exists a direction $\xi\in[\zeta,\eta]\cap\supp\mu_{x+e_1,x+e_2}$, which by Theorem \ref{thm:nonint} implies $\geo{}{x+e_1}{\xi-}\cap\geo{}{x+e_2}{\xi+}=\varnothing$.  Then the ordering of geodesics implies $\geo{}{x+e_1}{\zeta-}\cap\geo{}{x+e_2}{\eta+}=\varnothing$.  %The case of a $]\zeta,\eta[$-instability point is similar.

%For the other direction suppose $x^*$ is not a $]\zeta,\eta[$-instability point. Then $\mu_{x+e_1,x+e_2}(\,]\zeta,\eta[\,)=0$ and by  the equivalence of \eqref{eq100} and \eqref{eq102} in Proposition \ref{pr:supp1} this implies that $\geo{}{x+e_1}{\zeta+}\cap\geo{}{x+e_2}{\eta-}\ne\varnothing$. 


If $x^*$ is not a $[\zeta,\eta]$-instability point, then combining Propositions \ref{pr:supp1} and \ref{pr:supp2} 
we have that 
	\[z=\coal{\zeta-}(x+e_1,x+e_2)=\coal{\zeta+}(x+e_1,x+e_2)=\coal{\eta-}(x+e_1,x+e_2)=\coal{\eta+}(x+e_1,x+e_2)\in\Z^2,\]
$\geo{}{x+e_1}{\zeta\pm}$ and $\geo{}{x+e_1}{\eta\pm}$ all match until $z$ is reached, and $\geo{}{x+e_2}{\zeta\pm}$ $\geo{}{x+e_2}{\eta\pm}$ also all match until $z$ is reached. 
In particular, $z\in\geo{}{x+e_1}{\zeta-}\cap\geo{}{x+e_2}{\eta+}$.
\end{proof}


The following is immediate from the definitions and monotonicity.

\begin{lemma}\label{no-cross}
Let $\zeta\preceq\eta$ in $\ri\Uset$. A directed path  in $\dS{[\zeta,\eta]}$ can never cross a directed path in $\G{\eta+}$ from right to left {\rm (}i.e.~along a dual edge in the $-e_1$ direction{\rm )} nor a directed path in $\G{\zeta-}$ from above to below {\rm (}i.e.~along a dual edge in the $-e_2$ direction{\rm )}. 
\end{lemma}




The next lemma  characterizes the ancestors of an instability point in the graph $\dG{\cup[\zeta,\eta]}$.  

\begin{lemma}\label{lm:an1}
Let $\zeta\preceq\eta$ in $\ri\Uset$ and $x^*\in\shock{[\zeta,\eta]}$.  The following statements \eqref{an110} and \eqref{an111} are equivalent for any point $y^*\in\Z^{2*}$. 
\begin{enumerate} [label={\rm(\roman*)}, ref={\rm\roman*}]   \itemsep=3pt 
\item\label{an110}    There is a directed path from $y^*$ to $x^*$ in the graph $\dG{\cup[\zeta,\eta]}$. 
\item\label{an111}    $y^*\ge x^*$ and $y^*$ is between the two geodesics $\geo{}{x^*+\exstar}{\zeta-}$ and $\geo{}{x^*-\exstar}{\eta+}$, embedded as paths on $\R^2$.
%\item\label{an112}  
\end{enumerate}
 \end{lemma}

\begin{proof} \eqref{an110}$\implies$\eqref{an111}.   By  Lemma \ref{no-cross} no directed path in $\dS{[\zeta,\eta]}$ can go from $y^*$ to $x^*$ unless
$y^*$ lies between $\geo{}{x^*+\exstar}{\zeta-}$ and $\geo{}{x^*-\exstar}{\eta+}$.

\medskip 

\eqref{an111}$\implies$\eqref{an110}.   We prove this by induction on $\abs{y^*-x^*}_1$.  The claim is trivial if $y^*=x^*$. Suppose $y^*\ge x^*$ is such that $y^*\neq x^*$  and $y^*$  is between $\geo{}{x^*+\exstar}{\zeta-}$ and $\geo{}{x^*-\exstar}{\eta+}$. If $y^*$ points to  both $y^*-e_1$ and $y^*-e_2$ in $\dS{[\zeta,\eta]}$, then since $y^*-e_i$ is between the two geodesics for at least one $i\in\{1,2\}$, the induction hypothesis implies that there is a directed path from $y^*$ to $x^*$ through this $y^*-e_i$. 

   Suppose next that  $y^*$ points to $y^*-e_1$ in $\dS{[\zeta,\eta]}$ but $y^*-e_1$  is not between the two geodesics. Then, on the one hand, $y^*-e_2$ must be between the geodesics and the induction hypothesis implies that there is a path from $y^*-e_2$ to $x^*$.
 On the other hand, $y^*-\etstar$ must point to $y^*+\exstar$ in $\G{\zeta-}$ to prevent $y^*-e_1$ from falling between the two geodesics.   
This implies that $y^*$ points to $y^*-e_2$ in $\dS{[\zeta,\eta]}$. Now we have a path from $y^*$ to $x^*$ through $y^*-e_2$.
  See the left plot in Figure \ref{fig:lineage}. The case when $y^*$ points to $y^*-e_2$ and the latter is not between the two geodesics is similar.
\end{proof} 

%%%%%%%%    OLD ANCESTRY LEMMA  %%%%%%%%%
%\begin{lemma}\label{ancestry}
%Let $\zeta\preceq\eta$ in $\ri\Uset$.
%The following holds for all $x^*\in\shock{[\zeta,\eta]}$.
%The set $\ans{[\zeta,\eta]}{x^*}$  of the ancestors  of $x^*$  is exactly the set of vertices  $y^*\in\shock{[\zeta,\eta]}$ such 
%that $y^*\ge x^*$ and $y^*$ is between the two geodesics $\geo{}{x^*+\exstar}{\zeta-}$ and $\geo{}{x^*-\exstar}{\eta+}$ {\rm(}embedded as paths on $\R^2${\rm)}.
%\end{lemma}
%
%\begin{proof}
%First, suppose $y^*$ is an ancestor of $x^*$. 
%By  Lemma \ref{no-cross} no directed path in $\dS{[\zeta,\eta]}$ can go from $y^*$ to $x^*$ unless
%$y^*$ lies between $\geo{}{x^*+\exstar}{\zeta-}$ and $\geo{}{x^*-\exstar}{\eta+}$
%
%We prove the converse by induction on $\abs{y^*-x^*}_1$.  The claim is trivial if $y^*=x^*$. Suppose $y^*\ge x^*$ is such that $y^*\neq x^*$, $y^*\in\shock{[\zeta,\eta]}$, and $y^*$  is between $\geo{}{x^*+\exstar}{\zeta-}$ and $\geo{}{x^*-\exstar}{\eta+}$. If $y^*$ points to  both $y^*-e_1$ and $y^*-e_2$ in $\dS{[\zeta,\eta]}$, then since $y^*-e_i$ is between the two geodesics for at least one $i\in\{1,2\}$, the induction hypothesis implies that this $y^*-e_i\in\ans{[\zeta,\eta]}{x^*}$
%and thus $y^*\in\ans{[\zeta,\eta]}{x^*}$.    Suppose next that  $y^*$ points to $y^*-e_1$ in $\dS{[\zeta,\eta]}$ but that the latter is not between the two geodesics. Then, on the one hand, $y^*-e_2$ must be between the geodesics and the induction hypothesis implies $y^*-e_2\in\ans{[\zeta,\eta]}{x^*}$.
% On the other hand, $y^*-\etstar$ must point to $y^*+\exstar$ in $\G{\zeta-}$ (to prevent $y^*-e_1$ from falling between the two geodesics), 
% which implies that $y^*$ points to $y^*-e_2$ in $\dS{[\zeta,\eta]}$. But now we have $y^*\in\ans{[\zeta,\eta]}{x^*}$.
%  See the left plot in Figure \ref{fig:lineage}. The case when $y^*$ points to $y^*-e_2$ and the latter is not between the two geodesics is similar.
% \end{proof}
%%%%%%%%%%%%%%    END OLD ANCESTRY LEMMA   %%%%%%

%\textcolor{red}{Note: Lemma \ref{ancestry} has a connection to the way Yura defines ancestry, using the set absorbed by $x^*$. But in our setting, it does not seem like a good name to use, since red edges can get out of that set!}

The next lemma characterizes  $[\zeta,\eta]$-instability points as the {\it endpoints} of semi-infinite directed paths in $\dG{\cup[\zeta,\eta]}$.  Furthermore, such paths consist entirely of instability points.  

\begin{lemma} \label{lm:ans}  Let $\zeta\preceq\eta$ in $\ri\Uset$.
\begin{enumerate}   [label={\rm(\alph*)}, ref={\rm\alph*}]   \itemsep=3pt 
\item\label{ans110}   Let $\{x^*_k\}_{k\ge m}$ be any semi-infinite path on $\Z^{2*}$ such that  $x^*_{k+1}$ points to $x^*_k$ in $\dG{\cup[\zeta,\eta]}$  for each $k\ge m$.  
Then 
 $\{x^*_k\}_{k\ge m}\subset\shock{[\zeta,\eta]}$ and  as $k\to\infty$,   the limit points of $x^*_k/k$    lie in the interval $[\zetamin,\etamax]$. 
\item\label{ans111}  
Let  $x^*\in\Z^{2*}$ and $m=x^*\cdot\et$.  Then $x^*\in\shock{[\zeta,\eta]}$ if and only if there is a path $\{x^*_k\}_{k\ge m}$ on $\Z^{2*}$ such that $x^*_m=x^*$ and  for each $k\ge m$, $x^*_k\cdot\et=k$ and   $x^*_{k+1}$ points to $x^*_k$ in $\dG{\cup[\zeta,\eta]}$.   When this happens, the path $\{x^*_k\}_{k\ge m}$ satisfies part \eqref{ans110} above.  
 \end{enumerate} 
\end{lemma} 


\begin{proof} Part \eqref{ans110}.  For each $k$, Lemma \ref{no-cross} implies that the geodesics 
$\geo{}{x^*_k+\exstar}{\zeta-}$ and $\geo{}{x^*_k-\exstar}{\eta+}$ are disjoint because they remain forever separated by the path $\{x^*_k\}_{k\ge m}$. 
Since the backward path $\{x^*_k\}_{k\ge m}$   is sandwiched between the geodesics $\geo{}{x^*_m+\exstar}{\zeta-}$ and $\geo{}{x^*_m-\exstar}{\eta+}$, Theorem \ref{thm1}\eqref{thm1:exist} implies that as $k\to\infty$ the limit points of $x^*_k/k$   
lie in the interval $[\zetamin,\etamax]$. 
\medskip 

Part \eqref{ans111}.   The {\it if} claim follows from part \eqref{ans110} of the lemma.  To prove the {\it only if} claim, suppose  $x^*\in\shock{[\zeta,\eta]}$.  Then the geodesics 
$\geo{}{x^*+\exstar}{\zeta-}$ and $\geo{}{x^*-\exstar}{\eta+}$ are disjoint. At every level $k>x^*\cdot\et$ we can choose a  point $y^*_k$ between the geodesics 
$\geo{}{x^*+\exstar}{\zeta-}$ and $\geo{}{x^*-\exstar}{\eta+}$, that is, a point $y^*_k\in\Z^{2*}$ such that $y^*\cdot\et=k$ and $\geo{k}{x^*+\exstar}{\zeta-}\prec y^*_k\prec\geo{k}{x^*-\exstar}{\eta+}$.  By Lemma \ref{lm:an1} there is a directed path in $\dG{\cup[\zeta,\eta]}$ from  each  $y^*_k$ to $x^*$.  Along some subsequence these directed paths converge to a semi-infinite directed path to $x^*$. 
\end{proof} 


\begin{proof}[Proof of Theorem \ref{thm:shock1}] 
%Since $\shockG{\xi}\subset\shockG{[\zeta,\eta]}$ if $\xi\in[\zeta,\eta]$, it is enough to prove statements (\ref{thm:shocks.0}-\ref{thm:shocks.c}) and \eqref{thm:shocks.e} for the case of $\xi\in[\zeta,\eta]\cap\,\aUset$. For the other two statements one has to distinguish the two cases $\zeta\prec\eta$ and $\zeta=\eta$.\medskip

%{\it Part \eqref{thm:shocks.0}.} 
{\bf Step 1.}  
We show that $\shock{\xi}\neq\varnothing$ for 
any  $\xi\in\aUset$.  Since   $\xi\in\supp{\mu_{z,y}}$  for some $z,y\in\Z^2$,  the cocycle property \eqref{coc-prop} implies that  
  $\xi\in\supp{\mu_{x,x+e_i}}$ for some nearest-neighbor edge $(x,x+e_i)$.   Since $\mu_{x+e_1, x+e_2}=\mu_{x+e_1, x}+\mu_{x,x+e_2}$ is a sum of two positive measures there can be no cancellation, and hence    $\xi\in\supp{\mu_{x+e_1,x+e_2}}$ and thereby $x+\etstar\in\shock{\xi}$.  
 
 %%%%  OLD  %%%%%
% By the cocycle property \eqref{coc-prop}, 
%	\[\B{\xi\pm}(x,y)=\sum_{i=0}^{n-1}\B{\xi\pm}(x_i,x_{i+1})\]
%for any nearest-neighbor path $x_{0,n}$ from $x_0=x$ to $x_n=y$. Then  
%$\xi\in\supp\mu_{x_i,x_{i+1}}$ for some $i$. 
%By the monotonicity \eqref{mono} and the cocycle property \eqref{coc-prop}, 
%	\begin{align}\label{mu=|mu|}
%	\supp{\mu_{u+e_1,u+e_2}} =\supp\mu_{u,u+e_1}\cup\supp\mu_{u,u+e_2}\quad\text{for any }u\in\Z^2.
%	\end{align} 
%	The orientation of the edge  $(x_i,x_{i+1})$ gives two cases: either $x_{i+1}\in\{x_i+e_1,x_i+e_2\}$ and then 
%  $x_i+\etstar\in\shock{\xi}$,  or    $x_{i}\in\{x_{i+1}+e_1,x_{i+1}+e_2\}$ and then  $x_{i+1}+\etstar\in\shock{\xi}$ otherwise. Since $\shockG{\xi}\subset\shockG{[\zeta,\eta]}$. 
%%part \eqref{thm:shocks.0} is proved.

\medskip
	
%{\it Part \eqref{thm:shocks.a}.} 
{\bf Step 2.}   We show that every  edge of $\dS{[\zeta,\eta]}$ that emanates from a point of $\shock{[\zeta,\eta]}$ is an edge of  $\shockG{[\zeta,\eta]}$.
Take $x^*\in\shock{[\zeta,\eta]}$.
Then $\geo{}{x^*+\exstar}{\zeta-}$ and $\geo{}{x^*-\exstar}{\eta+}$ are disjoint.
Suppose $x^*$ points to  $x^*-e_1$ in $\dS{[\zeta,\eta]}$. Then $x^*-\etstar$ points to  $x^*-\exstar$ in $\G{\eta+}$.  The geodesic 
$\geo{}{x^*-\etstar}{\eta+}$ takes first  an $e_1$ step and then follows $\geo{}{x^*-\exstar}{\eta+}$. Since $\geo{}{x^*-e_1+\exstar}{\zeta-}$ must 
always stay to the left of $\geo{}{x^*+\exstar}{\zeta-}$, it is prevented from touching $\geo{}{x^*-\etstar}{\eta+}=\geo{}{x^*-e_1-\exstar}{\eta+}$ and we see that $x^*-e_1\in\shock{[\zeta,\eta]}$. See the right plot in Figure \ref{fig:lineage}. The case when $x^*$ points to  $x^*-e_2$ in $\dS{[\zeta,\eta]}$ is similar.
%This proves part \eqref{thm:shocks.a}.



\medskip  

%{\it Part \eqref{thm:shocks.b}.} 
{\bf Step 3.}  We conclude the proof.  Combining Lemma \ref{lm:ans}\eqref{ans110} with Step 2 implies that every bi-infinite directed path of the graph $\dG{\cup[\zeta,\eta]}$ is in fact a directed path of the graph $\shockG{[\zeta,\eta]}$.   

Conversely, let $x^*\in\shock{[\zeta,\eta]}$.   Lemma \ref{lm:ans} together with Step 2  implies that $x^*$ is the endpoint of a semi-infinite directed path in  $\shockG{[\zeta,\eta]}$ which is inherited from $\dG{\cup[\zeta,\eta]}$.    Step 2 implies that by following the edges of $\dG{\cup[\zeta,\eta]}$  from $x^*$ creates  an infinite down-left directed path   in the graph $\dG{\cup[\zeta,\eta]}$, and this path is a directed path also in $\shockG{[\zeta,\eta]}$.   In other words, every instability point $x^*\in\shock{[\zeta,\eta]}$ lies on a bi-infinite directed path of the graph $\shockG{[\zeta,\eta]}$ that was inherited from $\dG{\cup[\zeta,\eta]}$. 

The  $[\zetamin,\etamax]$-directedness of these paths comes from Lemma \ref{lm:ans}\eqref{ans110}. 
%
%%%%%%%   OLD LAST PART OF THE PROOF  
%We  prove the existence of an up-right backward-directed path   in $\shockG{[\zeta,\eta]}$ from any given $[\zeta,\eta]$-shock point.  
%%  it is enough to show that   for any $x^*\in\shock{[\zeta,\eta]}$, one of the points $x^*+e_i$, $i\in\{1,2\}$,  points to $x^*$.
%By Lemma \ref{ancestry},  it suffices to show that for any $x^*\in\shock{[\zeta,\eta]}$ there are points of $\shock{[\zeta,\eta]}$   at a level above $x^*$  between the geodesics $\geo{}{x^*+\exstar}{\zeta-}$ and $\geo{}{x^*-\exstar}{\eta+}$. 
%
%Consider an antidiagonal $\{z_0, z_1, \dotsc, z_k\}$ on $\Z^2$ between the two geodesics.  That is, for some integer $k>x^*\cdot\et$, $z_i\cdot\et=k$ for each $i$, $z_0\in\geo{}{x^*+\exstar}{\zeta-}$, $z_k\in\geo{}{x^*-\exstar}{\eta+}$, and $z_i=z_{i-1}-\ex$.  Suppose there are no points of $\shock{[\zeta,\eta]}$  between the two geodesics at any level at or above $k$.  Then, since $z_i+\exstar\notin\shock{[\zeta,\eta]}$ for each $i=1,\dotsc,k$, the geodesics $\geo{}{z_{i-1}}{\zeta-}$ and $\geo{}{z_i}{\eta+}$ must intersect. But then they must coalesce because if they separate at $y$, the dual point $y+\etstar$ lies in $\shock{[\zeta,\eta]}$.  Consequently also  $\geo{}{z_{i}}{\zeta-}$ coalesces with  $\geo{}{z_{i-1}}{\zeta-}$ and $\geo{}{z_i}{\eta+}$ because it lies between the two. 
%Thus  for all $i=1,\dotsc,k$, $\geo{}{z_{i-1}}{\zeta-}$, $\geo{}{z_{i}}{\zeta-}$  and $\geo{}{z_i}{\eta+}$ coalesce.  Thereby   $\geo{}{z_0}{\zeta-}$ and $\geo{}{z_k}{\eta+}$ coalesce and  contradict the assumption   $x^*\in\shock{[\zeta,\eta]}$. 
%
%We have proved that out of any $x^*\in\shock{[\zeta,\eta]}$, there exists an up-right path $x^*_{n,\infty}$ such that for any $i\ge n$, $x^*_{i+1}$ points to $x^*_i$ in $\shockG{[\zeta,\eta]}$.
%Since the backward path $x^*_{n,\infty}$ is sandwiched between $\geo{}{x^*_n+\exstar}{\zeta-}$ and $\geo{}{x^*_n-\exstar}{\eta+}$ (for any $n\in\Z$), Theorem \ref{thm1}\eqref{thm1:exist} implies that as $n\to\infty$ the limit points of $x^*_n/n$   
%lie in the interval $[\zetamin,\etamax]$. 
%%Part \eqref{thm:shocks.b} is proved.
\end{proof} 

\begin{figure}%[h]
 	\begin{center}
 		 \begin{tikzpicture}[scale=1,shorten >=1pt,>={Latex[length=3.5mm,width=2mm]}]
		\begin{scope}
			\draw[->,>={Latex[length=3.5mm,width=3mm]},line width=3pt, color=nicosred](4.5,2.5)--(3.4,2.5);
			\draw[line width=3pt, color=nicosred](4,2.5)--(3.5,2.5);
			\draw[->,>={Latex[length=3.5mm,width=3mm]},line width=3pt, color=nicosred](4.5,2.5)--(4.5,1.6);
			\draw[line width=3pt, color=nicosred](4.5,2)--(4.5,1.5);
			\draw[nicosred,fill=nicosred](4.5,2.5) circle(3pt);
			\draw[nicosred,fill=nicosred](3.5,2.5) circle(3pt);
			\draw[nicosred,fill=nicosred](4.5,1.5) circle(3pt);
			\draw[nicosred,fill=nicosred](1/2,1/2) circle(3pt);
		 	\draw[->,line width=1pt, color=sussexg](4.1,2)--(4.1,3.1);
		 	\draw[line width=1pt, color=sussexg](4.1,2.5)--(4.1,3.2);
			\draw[color=sussexg, line width=1pt,->]plot[smooth] coordinates{(0,1)(0.5,1.3)(1.1,1.55)};
			\draw[color=sussexg, line width=1pt]plot[smooth] coordinates{(0.95,1.5)(1.5,1.6)(1.8,1.9)(4.1,2)};
			\draw[color=sussexp, line width=2pt,->]plot[smooth] coordinates{(1,0)(1.5,0)(2,0.3)(2.5,0.5)(4.5,0.6)(5.1,0.8)(5.7,1.2)};			
			
			\draw[black,fill=white](4.1,2) circle(3pt);
			\draw[black,fill=white](4.1,3.1) circle(3pt);
			\draw[black,fill=white](1,0) circle(3pt);
			\draw[black,fill=white](0,1) circle(3pt);

			\draw(4.5+.1,2.5)node[right]{$y^*$};
			\draw(0.5,0.5)node[left]{$x^*$};
			\draw(3.5,2.5)node[left]{$y^*-e_1$};
			\draw(4.6,1.5)node[right]{$y^*-e_2$};
			\draw(4,3.1)node[above]{$y^*+\exstar$};
			\draw(3.3,2)node[below]{$y^*-\etstar$};
		\end{scope}

		\begin{scope}[scale=0.8,shift={(12,0)}]
			\draw[nicosred,fill=nicosred](1/2,1/2) circle(3pt);
			\draw[nicosred,fill=nicosred](-1/2,1/2) circle(3pt);
			\draw[->,>={Latex[length=3.5mm,width=3mm]},line width=3pt, color=nicosred](1/2,1/2)--(-.3,1/2);
			\draw[line width=3pt, color=nicosred](0,1/2)--(-1/2,1/2);
			\draw(1/2+0.05,1/2+0.1)node[right]{$x^*$};
			%\draw(-1/2,1/2+0.1)node[above]{$x^*-e_1$};
		 	\draw[->,line width=2pt, color=sussexp](0,0)--(0.85,0);
		 	\draw[line width=2pt, color=sussexp](0.5,0)--(1,0);
			\draw[color=sussexp, line width=2pt,->]plot[smooth] coordinates{(1,0)(1.5,0)(2,0.5)(2.5,0.75)};			
			\draw[color=sussexg, line width=1pt,->]plot[smooth] coordinates{(0,1)(0.5,1.4)(1.1,1.5)(1.5,1.9)(2,2.1)};
			\draw[color=sussexg, line width=1pt,->]plot[smooth] coordinates{(-1,1)(-0.5,1.1)(0.1,1.7)(0.7,1.8)(1,2)(1.5,2.3)};			
			\draw[black,fill=white](0,0) circle(3pt);
			\draw[black,fill=white](1,0) circle(3pt);
			\draw[black,fill=white](0,1) circle(3pt);
			\draw[black,fill=white](-1,1) circle(3pt);
			\draw(-1-0.05,1+0.1)node[left]{$x^*-e_1+\exstar$};
			\draw(-1/2-0.05,1/2)node[left]{$x^*-e_1$};
			\draw(1.5+0.05,0)node[below]{$x^*-\exstar$};
			\draw(-1/2,0)node[below]{$x^*-\etstar$};
			\draw(0.1,1)node[right]{$x^*+\exstar$};
		\end{scope}


		\end{tikzpicture}
 	 \end{center}
 	\caption{\small  The proofs of Lemma \ref{lm:an1} (left) and  Theorem \ref{thm:shock1}  (right). $\zeta-$ geodesics are in green and thin. $\eta+$ geodesics are in purple with medium thickness. Directed edges in $\dS{[\zeta,\eta]}$ are in red/thick.  White circles are points in $\Z^2$ while points in $\Z^{2*}$ are filled in (red).}
 \label{fig:lineage}
 \end{figure}
 
\begin{proof}[Proof of Theorem \ref{thm:shocks}] 
%Since $\shockG{\xi}\subset\shockG{[\zeta,\eta]}$ if $\xi\in[\zeta,\eta]$, it is enough to prove statements (\ref{thm:shocks.0}-\ref{thm:shocks.c}) and \eqref{thm:shocks.e} for the case of $\xi\in[\zeta,\eta]\cap\,\aUset$. For the other two statements one has to distinguish the two cases $\zeta\prec\eta$ and $\zeta=\eta$.\medskip

%%%%%%%%   The parts commented out below were moved to a separate theorem 2019-11-23  (Timo) %%%%%%%%%%%%%%
%{\it Part \eqref{thm:shocks.0}.} 
%Take $\xi\in[\zeta,\eta]\cap\,\aUset$. There exist points $x,y\in\Z^2$ with $\xi\in\supp{\mu_{x,y}}$.
%By the cocycle property \eqref{coc-prop} we can write 
%	\[\B{\xi\pm}(x,y)=\sum_{i=0}^{n-1}\B{\xi\pm}(x_i,x_{i+1})\]
%for any nearest-neighbor path $x_{0,n}$ from $x_0=x$ to $x_n=y$. But then it must be the case that 
%$\xi\in\supp\mu_{x_i,x_{i+1}}$ for at least one $i$. 
%By the monotonicity \eqref{mono} and the cocycle property \eqref{coc-prop} 
%	\begin{align}\label{mu=|mu|}
%	\supp{\mu_{u+e_1,u+e_2}} =\supp\mu_{u,u+e_1}\cup\supp\mu_{u,u+e_2}\quad\text{for any }u\in\Z^2.
%	\end{align} 
%Therefore, $x_i+\etstar\in\shock{\xi}$ if $x_{i+1}\in\{x_i+e_1,x_i+e_2\}$ and $x_{i+1}+\etstar\in\shock{\xi}$ otherwise. Since $\shockG{\xi}\subset\shockG{[\zeta,\eta]}$, 
%part \eqref{thm:shocks.0} is proved.\medskip
%	
%{\it Part \eqref{thm:shocks.a}.} Take $x^*\in\shock{[\zeta,\eta]}$.
%Then $\geo{}{x^*+\exstar}{\zeta-}$ and $\geo{}{x^*-\exstar}{\eta+}$ are disjoint.
%Suppose $x^*$ points to $x^*-e_1$ in $\dS{[\zeta,\eta]}$. Then $x^*-\etstar$ points to $x^*-\exstar$ in $\G{\eta+}$ and 
%$\geo{}{x^*-\etstar}{\eta+}$ first takes an $e_1$ step then follows $\geo{}{x^*-\exstar}{\eta+}$. Since $\geo{}{x^*-e_1+\exstar}{\zeta-}$ must 
%always stay to the left of $\geo{}{x^*+\exstar}{\zeta-}$, it is prevented from touching $\geo{}{x^*-\etstar}{\eta+}=\geo{}{x^*-e_1-\exstar}{\eta+}$ and we see that $x^*-e_1\in\shock{[\zeta,\eta]}$. See the right plot in Figure \ref{fig:lineage}. The case when $x^*$ points to $x^*-e_2$ in $\dS{[\zeta,\eta]}$ is similar.
%This proves part \eqref{thm:shocks.a}.\medskip  
%
%{\it Part \eqref{thm:shocks.b}.} To prove the existence of the up-right path of points in $\shock{[\zeta,\eta]}$ it is enough to show that 
%for any $x^*\in\shock{[\zeta,\eta]}$, $x^*+e_i$ points to $x^*$ for at least one $i\in\{1,2\}$.
%Lemma \ref{ancestry} says that for this it suffices to show that there exist points of $\shock{[\zeta,\eta]}$ other than $x^*$ between the geodesics $\geo{}{x^*+\exstar}{\zeta-}$ and $\geo{}{x^*-\exstar}{\eta+}$.  We will show that such points exist at all levels above $x^*$. 
%
%Consider an antidiagonal $\{z_0, z_1, \dotsc, z_k\}$ between the two geodesics.  That is, for some integer $m>x^*\cdot\et$, $z_i\cdot\et=m$ for each $i$, $z_0\in\geo{}{x^*+\exstar}{\zeta-}$, $z_k\in\geo{}{x^*-\exstar}{\eta+}$, and $z_i=z_{i-1}-\ex$.  Suppose there are no points of $\shock{[\zeta,\eta]}$  between the two geodesics at any level at or above $m$.  Then, since $z_i+\exstar\notin\shock{[\zeta,\eta]}$ for each $i=1,\dotsc,k$, the geodesics $\geo{}{z_{i-1}}{\zeta-}$ and $\geo{}{z_i}{\eta+}$ must intersect. But then they must coalesce because if they separate at $y$, the dual point $y+\etstar$ lies in $\shock{[\zeta,\eta]}$.  Consequently also  $\geo{}{z_{i}}{\zeta-}$ coalesces with  $\geo{}{z_{i-1}}{\zeta-}$ and $\geo{}{z_i}{\eta+}$ because it lies between the two. 
%
%To summarize, for $i=1,\dotsc,k$, $\geo{}{z_{i-1}}{\zeta-}$, $\geo{}{z_{i}}{\zeta-}$  and $\geo{}{z_i}{\eta+}$ coalesce.  This implies that  $\geo{}{z_0}{\zeta-}$ and $\geo{}{z_k}{\eta+}$ coalesce and thereby contradicts the assumption that $x^*\in\shock{[\zeta,\eta]}$. We have thus proved that out of any $x^*\in\shock{[\zeta,\eta]}$, there exists an up-right path $x^*_{n,\infty}$ such that for any $i\ge n$, $x^*_{i+1}$ points to $x^*_i$.
%
%Since the backward path $x^*_{n,\infty}$ is sandwiched between $\geo{}{x^*_n+\exstar}{\zeta-}$ and $\geo{}{x^*_n-\exstar}{\eta+}$ (for any $n\in\Z$), Theorem \ref{thm1}\eqref{thm1:exist} implies that the limit points of $x^*_n/n$, as $n\to\infty$, 
%are all in the interval $[\zetamin,\etamax]$. 
%Part \eqref{thm:shocks.b} is proved.\medskip
%%%%%%%%%    The parts above were moved to a separate theorem %%%%%

{\it Part \eqref{thm:shocks.c}.}  Let $x=x^*-\etstar$. If $x^*$ is a branch point in $\shockG{[\zeta,\eta]}$, then $\geo{}{x}{\zeta-}$ goes from $x$ to $x+e_2$ and $\geo{}{x}{\eta+}$ goes from $x$ to $x+e_1$, which is equivalent to 
$\B{\zeta-}(x+e_1,x+e_2)\le0\le\B{\eta+}(x+e_1,x+e_2)$, which in turn is equivalent to $\cid(T_x\w)\in[\zeta,\eta]$. 

Conversely, suppose $\cid(T_x\w)\in[\zeta,\eta]$. Reversing the above equivalences we see that 
$x^*\in\shock{[\zeta,\eta]}$ and points to both $x^*-e_1$ and $x^*-e_2$ in $\dS{[\zeta,\eta]}$. 
By Step 2 of the proof of Theorem  \ref{thm:shock1} above these edges are in  $\shockG{[\zeta,\eta]}$,  and hence $x^*$ is a branch point. 
\medskip


{\it Part \eqref{thm:shocks.d}}. Start with the case $\zeta\prec\eta$.
Let $\xi\in[\zeta,\eta]\cap\,\Udense$. 
 Then $\Omega_{\xi}^3\subset\Omega_0$ and parts \eqref{thm1:coal} and \eqref{thm1:biinf} of Theorem \ref{thm1} imply that $\G{\xi}$ is a tree that does not contain any bi-infinite up-right paths. 
 (Recall that for $\xi\in\Udense$ there is no $\pm$ distinction.)
This implies that $\dG{\xi}$ is a tree as well, i.e.\ all down-left paths of $\dG{\xi}$ coalesce.
 %If $\dG{\zeta-}$ were made of multiple trees, then we can consider two distinct subtrees and there would be a path $x_{-\infty,n}$ in $\G{\zeta-}$ that separates the two.
%But then one can continue the path in $\G{\zeta-}$ to form a bi-infinite path, which then would be a bi-infinite geodesic. 
%However, in the exponential case we now know there are no bi-infinite geodesics \cite{Bas-Hof-Sly-18-}. 
%\addmath{should we alert the reader to the fact that $x^*$ and $y^*$ may not be in $\shockG{\xi}$, but that this does not matter? T: Maybe OK.}
Since $\dG{\xi}\subset\dG{\cup[\zeta,\eta]}$, one can follow the edges e.g.\ in $\dG{\xi}$ starting from $x^*$ and from $y^*$ to get to a coalescence point $z^*$ that will then be a descendant of both points in $\shockG{[\zeta,\eta]}$. 
The same argument can be repeated if $\zeta=\eta=\xi\in\aUset$ when condition \eqref{cond:biinf} holds, since then both $\dG{\xi\pm}$ are trees.
Claim \eqref{thm:shocks.d} is proved.\medskip

{\it Part \eqref{thm:shocks.e}}. Observe that for any $x^*,y^*\in\shock{[\zeta,\eta]}$, Theorem \ref{thm:+-coal} says that 
under the jump process condition \eqref{cond:jumpcond}, if $\w\in\Omjump$ (defined in \eqref{Omjump}), 
then the geodesics $\geo{}{x^*+\exstar}{\zeta-}$ and $\geo{}{y^*+\exstar}{\zeta-}$ coalesce, as do  $\geo{}{x^*-\exstar}{\eta+}$ and $\geo{}{y^*-\exstar}{\eta+}$.  
By Lemma \ref{lm:an1}, any point in $\shock{[\zeta,\eta]}$ that is between the two $+$ and $-$ coalesced geodesics is an ancestor to both $x^*$ and $y^*$. Such a point exists. For example, 
take a point $z$ on $\geo{}{x^*+\exstar}{\zeta-}$ above the coalescence levels, in other words, such that  $z\cdot\et\ge(\coal{\zeta-}(x^*+\exstar,y^*+\exstar)\cdot\et)\vee(\coal{\eta+}(x^*-\exstar,y^*-\exstar)\cdot\et)$.  
Since $\geo{}{z}{\eta+}$ coalesces with 
$\geo{}{x^*-\exstar}{\eta+}$, which does not touch $\geo{}{z}{\zeta-}$ (because this latter  is part of $\geo{}{x^*+\exstar}{\zeta-}$), $\geo{}{z}{\eta+}$ must separate from $\geo{}{z}{\zeta-}$ at some point $z'$.
The dual point $z'+\etstar$ is then in $\shock{[\zeta,\eta]}$ and is an ancestor to both $x^*$ and $y^*$. 
Part \eqref{thm:shocks.e} is proved.\medskip

{\it Part \eqref{thm:shocks.f}}.   The assumption is that $\zeta\prec\eta$ and $]\zeta,\eta[\,\cap\aUset\ne\varnothing$.   By Lemma \ref{lm:V1},  $\nabla\gpp(\zeta+)\ne\nabla\gpp(\eta-)$.   For any $z\in\Z^2$,  Theorem \ref{thm:cif}\eqref{thm:cif.c} gives a strictly increasing sequence $z<z_1<z_2<\dotsm$     such that 
  $\cid(T_{z_k}\w)\in\,]\zeta,\eta[$ for each $k$.   Then by \eqref{cid}, $\B{\zeta+}(z_k+e_1,z_k+e_2)<0<\B{\eta-}(z_k+e_1,z_k+e_2)$, which implies that $z^*_k=z_k+\etstar$ is a $[\zeta,\eta]$-instability point.
 Each such point is a branch point in $\shockG{[\zeta,\eta]}$ because $z_k$ points to $z_k+e_2$ in $\G{\zeta+}$, and hence also in $\G{\zeta-}$, and to $z_k+e_1$ in $\G{\eta-}$, and hence also in $\G{\eta+}$. 
 
 %Thus, there are infinitely many branch points in $\shockG{[\zeta,\eta]}$. 
%
%Now, assume $\nabla\gpp(\zeta+)=\nabla\gpp(\eta-)$.  The fact that $[\zeta,\eta]\cap\aUset\ne\varnothing$ and Theorem \ref{th:V1}\eqref{th:V1.0'}  imply that $\{\zeta,\eta\}\cap\aUset\setminus\Diff\ne\varnothing$. Suppose $\zeta$ is in this intersection.
%\textcolor{red}{TBC}
%

The proof of the existence of infinitely many coalescence points in $\shockG{[\zeta,\eta]}$ follows from this and the first claim in part \eqref{thm:shocks.d} in a way similar to the proof below for the case of $\shockG{\xi}$ (but without the need for any extra conditions) and is therefore omitted.\medskip


%\addmath{The proof of \eqref{thm:shocks.g} needs streamlining! maybe can use the flow of measure results...}
{\it Part \eqref{thm:shocks.g}.}    Fix $\xi\in\aUset$ for the duration of the proof. 
Assume the jump process condition \eqref{cond:jumpcond}.
% and take $\w\in\Omjump$ and $\xi\in\aUset$. Then 
By Theorem \ref{thm:nonint} there exist $x,y\in\Z^2$ such that $\geo{}{x}{\xi-}\cap\geo{}{y}{\xi+}=\varnothing$ and then Theorem \ref{thm:+-coal} says that for any $z\in\Z^2$, the two geodesics $\geo{}{z}{\xi\pm}$ must separate at some point $z_1$ (in order to coalesce with $\geo{}{x}{\xi-}$ and $\geo{}{y}{\xi+}$, respectively). Uniqueness of finite geodesics implies that $\geo{}{z_1+e_i}{\xi\pm}$, $i\in\{1,2\}$, cannot touch. Thus, $z_1+\etstar\in\shock{\xi}$. 
Now define inductively $z_{n+1}$ to be the point where the geodesics $\geo{}{z_n+\et}{\xi\pm}$ separate.    Then for each $n$,  $z_{n+1}>z_n$ coordinatewise and  $z^*_n=z_n+\etstar$ is a point in $\shock{\xi}$.

Next, assume both  the jump process condition \eqref{cond:jumpcond} and the no bi-infinite geodesic condition \eqref{cond:biinf}. 
We prove the second claim of  part \eqref{thm:shocks.g} about infinitely many  coalescence points by mapping branch points injectively  into coalescence points as follows.

Given a branch point $x^*$,  let $\pi^*$ and $\bar\pi^*$ be the two innermost down-left paths out of $x^*$ along the directed graph $\shockG{\xi}$, defined by these rules: 
\be\label{aux783} \begin{aligned} 
 &\text{(i) $\pi^*$ starts with edge $(x^*, x^*-e_1)$,  follows the arrows of $\shockG{\xi}$, 
 and at vertices}\\ 
 &\text{where both $-e_1$ and $-e_2$ steps are allowed, it takes the  $-e_2$ step; }\\
   &\text{(ii) $\bar\pi^*$ starts with edge $(x^*, x^*-e_2)$,  follows the arrows of $\shockG{\xi}$,  and whenever}\\  
   &\text{both steps are available takes the  $-e_1$ step. }
  \end{aligned}\ee 
% Any  other two paths in this graph that emanate from $x^*$ and start with steps $-e_1$ and $-e_2$ must sandwich $\pi^*$ and $\bar\pi^*$.  

By part \eqref{thm:shocks.d}, $x^*-e_1$ and $x^*-e_2$ have a common descendant (this is where assumption \eqref{cond:biinf} is used).  By planarity,  the   paths $\pi^*$ and $\bar\pi^*$ must then meet at some point after $x^*$.    Let $z^*$  be their first common point after $x^*$, that is, the  point   $z^*\in(\pi^*\cap\bar\pi^*)\setminus\{x^*\}$  that maximizes $z^*\cdot\et$. This $z^*$ is the coalescence point that branch point $x^*$ is mapped to.  

We argue that the map $x^*\mapsto z^*$ thus defined  is one-to-one.   Two observations that help:  
\begin{itemize} 
\item   There cannot be any $\shock{\xi}$-points strictly inside the region bounded by $\pi^*$ and $\bar\pi^*$ between $x^*$ and  $z^*$.  By Theorem \ref{thm:shock1} such a point would lie on an  $\shockG{\xi}$ path that contradicts the choice of $\pi^*$ and $\bar\pi^*$ as the innermost paths between $x^*$ to $z^*$. 
\item  The last step that $\pi^*$ takes to reach $z^*$ is $-e_2$ and the last step of $\bar\pi^*$   is $-e_1$.   Otherwise $\pi^*$ and $\bar\pi^*$ would have met before $z^*$.  
\end{itemize} 

 Suppose another branch point $y^*\in\shock{\xi}$ distinct from $x^*$  maps to the same coalescence point $z^*$. Let the innermost paths  from $y^*$ to $z^*$ be $\gamma^*$ and $\bar\gamma^*$, defined by the same rules \eqref{aux783} but with $x^*$ replaced by $y^*$.      As observed, $\gamma^*$ and $\bar\gamma^*$  cannot  enter the region strictly between $\pi^*$ and $\bar\pi^*$.  
 
 
\begin{figure}[h]
 	\begin{center}
 		 \begin{tikzpicture}[scale=0.7]
		 
		 \begin{scope}
		 	\draw[line width=1pt](0,0)--(1,0)--(1,1)--(3,1)--(3,2)--(4,2);
			\draw[middlearrow={stealth},line width=1pt](4,4)--(4,2);
			\draw[middlearrow={stealth},line width=1pt] (0,2) -- (0,0);			
		 	\draw[line width=1pt](0,2)--(1,2)--(1,3);
			\draw[middlearrow={stealth},line width=1pt] (3,3) -- (1,3);			
		 	\draw[line width=1pt](3,3)--(3,4);
			\draw[middlearrow={stealth},line width=1pt](4,4)--(3,4);
			\draw[fill=black](0,0) circle(4pt);
			\draw[fill=black](3,3) circle(4pt);
			\draw[fill=black](4,4) circle(4pt);
			\draw(0.3,2)node[above]{$\pi^*$};
			\draw(1,.3)node[right]{$\bar\pi^*$};
			\draw(2.7,3)node[above]{$x^*$};
			\draw(4.1,4)node[right]{$y^*$};
			\draw(-0.2,-0.1)node[below]{$z^*$};
			\draw(3.5,4)node[above]{$\gamma^*$};
			\draw(2.95,2.5)node[right]{$\gamma^*$};
			\draw(4,3)node[right]{$\bar\gamma^*$};
			\draw[middlearrow={stealth},line width=1pt] (3,3) -- (3,2);	
		\end{scope}
		
		\begin{scope}[shift={(7,0)}]
		 	\draw[line width=1pt](0,0)--(1,0)--(1,1)--(3,1)--(3,2)--(4,2);
			\draw[middlearrow={stealth},line width=1pt](4,4)--(4,2);
			\draw[middlearrow={stealth},line width=1pt] (0,2) -- (0,0);			
		 	\draw[line width=1pt](0,2)--(1,2)--(1,3)--(3,3);
			\draw[middlearrow={stealth},line width=1pt](4,4)--(2,4);
			\draw[middlearrow={stealth},line width=1pt](2,4)--(2,3);
			\draw[fill=black](0,0) circle(4pt);
			\draw[fill=black](3,3) circle(4pt);
			\draw[fill=black](4,4) circle(4pt);
			\draw(0.3,2)node[above]{$\pi^*$};
			\draw(1,.3)node[right]{$\bar\pi^*$};
			\draw(2.9,3)node[above]{$x^*$};
			\draw(4.1,4)node[right]{$y^*$};
			\draw(-0.2,-0.1)node[below]{$z^*$};
			\draw(2.8,4)node[above]{$\gamma^*$};
			\draw(4,3)node[right]{$\bar\gamma^*$};
			\draw[line width=1pt](3,3) -- (3,2);	
		\end{scope}
		
		
		\end{tikzpicture}
 	 \end{center}
 	\caption{\small  Illustration of the proof that the map $x^*\mapsto z^*$ is one-to-one.}
 \label{fig:thm:shocks.g}
 \end{figure}

  Since   $\gamma^*$ uses the edge $(z^*+e_2, z^*)$, it must coalesce at some point with $\pi^*$.
 Point  $x^*$ itself cannot  lie on $\gamma^*$ because otherwise   \eqref{aux783} forces   $\gamma^*$ to take the edge $(x^*, x^*-e_2)$ and $\gamma^*$ cannot   follow $\pi^*$ to $z^*$.  This scenario is depicted by the left drawing in Figure \ref{fig:thm:shocks.g}.
 Thus $\gamma^*$ meets $\pi^*$ after $x^*$, at which point rule \eqref{aux783} forces them to  coalesce (right drawing in Figure \ref{fig:thm:shocks.g}).  
 
  Similarly,  $x^*$ cannot lie on $\bar\gamma^*$, and  $\bar\gamma^*$ meets $\bar\pi^*$ after $x^*$ at which point these coalesce (right drawing in Figure \ref{fig:thm:shocks.g}).
  
 Paths from $y^*$ cannot meet both $\pi^*$ and $\bar\pi^*$ while avoiding $x^*$ unless   $y^*>x^*$   holds coordinatewise.    
  It follows now  that $x^*$ must lie strictly inside the region bounded by $\gamma^*$ and $\bar\gamma^*$ between $y^*$ and  $z^*$, as illustrated by 
  the right drawing in Figure \ref{fig:thm:shocks.g}.
  But we already ruled out such a possibility.  These contradictions show that the map is one-to-one. 



%%%%%%   old version of 1-1 proof  %%%%%%%
%This and planarity imply that if there were another point $y^*\in\shock{\xi}$ that mapped to the same coalescence point $z^*$, then there must exist a point $u^*\in\shock{\xi}$ strictly inside the region between the segments of the paths $\pi^*$ and $\bar\pi^*$ that start at $x^*$ and end at $z^*$. 
%Theorem \ref{thm:shock1} implies then the existence of a semi-infinite path that follows the directed edges of $\shockG{\xi}$ and ends at $u^*$. But planarity forces such a path to  cross $\pi^*$  
%or $\bar\pi^*$ at some point $v^*\ne x^*$.  But this would contradict the construction of the paths $\pi^*$ and $\bar\pi^*$. For example, if $v^*\in\pi^*$ then we would get that $v^*$ is a parent to both $v^*-e_1$ and $v^*-e_2$ (because $v^*$ is a point where two paths in $\shockG{\xi}$ crossed) and yet $\pi^*$ to a $-e_1$ step out of $v^*$ (because the path from $v^*$ to $u^*$ had to take a $-e_2$ step since $u^*$ is between $\pi^*$ and $\bar\pi^*$). This is contrary to the construction of $\pi^*$, which said that since both steps are available, it should take a $-e_2$ step.  
%%%%%%  end old version %%%%%%%%
%The upshot of the above paragraph is that our mapping assigns a distinct coalescence point to each branch point.  

Since we already proved that under the jump process condition \eqref{cond:jumpcond} there are infinitely many branch points
in $\shockG{\xi}$, it now follows that there are also infinitely many coalescence points and part \eqref{thm:shocks.g} is proved.
%
%Under the assumption that the weights are exponentially distributed, the last claim in part \eqref{thm:shocks.f} follows from 
%Lemma \ref{LIL}, which we prove in Section \ref{sec:exp-pf}.  Indeed, applying \eqref{red-LB} with $\delta_n=n^{-1/4}$ gives us that for $\P$-almost every $\w$, for any $\xi\in\aUset$ and $\ell\in\Z$, there exist infinitely many $\xi$-shock points $x$ with $x\cdot e_2=\ell$. By part \eqref{thm:shocks.d}, any two such points have a common descendant. Consequently, there is a coalescence point below every horizontal level. Part \eqref{thm:shocks.f} is proved.
\end{proof}

\begin{proof}[Proof of the claim in Remark \ref{rk:erg2}] 
%Only parts \eqref{thm:shocks.0}, \eqref{thm:shocks.d}, and  \eqref{thm:shocks.f}  need extra arguments, under the assumptions that $\w\in\Omreg$, $\zeta\preceq\eta$, and at least one of the two, say $\zeta$, is not in $\Diff$.\smallskip
%
%Lemma \ref{lm:B+>B-} implies the existence of an $x\in\Z^2$ such that $x^*\in\shock{\zeta}\subset\shock{[\zeta,\eta]}$,
%finishing the proof of part \eqref{thm:shocks.0}.
%For part \eqref{thm:shocks.d} take $\xi'=\zeta\not\in\Diff$.  Then we still have $\Omega_{\xi'}^3\subset\Omega_0$ and the existing argument works word for word.
%Lastly, Lemma \ref{lm:B+>B-} implies the existence of infinitely many points $x$ with $\cid(T_x\w)=\zeta$, each of which is a branch point in $\shockG{\zeta}$ and hence in $\shockG{[\zeta,\eta]}$.
%This finishes the proof of part \eqref{thm:shocks.f}.
It suffices to consider the case where $]\zeta,\eta[\,\cap\aUset=\varnothing$ but $\{\zeta,\eta\}\cap\aUset\ne\varnothing$. 
%Parts \eqref{lm:V1.0} and \eqref{lm:V1.0'} of Lemma \ref{lm:V1} imply then that 
By Theorem \ref{th:V1}\eqref{th:V1.a}, the differentiable endpoints of the (countably many) linear segments of $\gpp$ are all outside $\aUset$.
By Theorem \ref{th:V1}\eqref{th:V1.b} we know $]\zeta,\eta[$ must be inside a linear segment. 
Thus, it must be the case that $\{\zeta,\eta\}\cap\aUset\setminus\Diff\ne\varnothing$. 
Suppose, without loss of generality, that $\zeta$ is in this intersection. 
Then Theorem \ref{thm:cif}\eqref{thm:cif.c1} 
%Lemma \ref{lm:B+>B-} 
implies the existence of infinitely many $x\in\Z^2$ with $\cid(T_x\w)=\zeta\in\aUset$ and part Theorem \ref{thm:shocks}\eqref{thm:shocks.c} says that the corresponding dual points $x^*$ are all branch points in $\shockG{\zeta}\subset\shockG{[\zeta,\eta]}$. The claim about coalescence points follows from the just proved infinite number of branch points, combined with the first claim in part \eqref{thm:shocks.d}, similarly to the way the claim is proved in Theorem \ref{thm:shocks}\eqref{thm:shocks.g}.
\end{proof}

In words, the next result says that there are no semi-infinite horizontal or vertical paths in any of the instability graphs $\shock{[\zeta,\eta]}$. The idea behind the proof is that the existence of such a path would force the existence of a semi-infinite horizontal or vertical path in one of the geodesic graphs $\G{\xi \sig}$ for some $\sig \in  \{+,-\}$ and $\xi \in \ri \Uset$. This is ruled out by the law of large numbers behavior of the Busemann functions.

\begin{lemma}\label{hor-red}
For any $\w\in\Omega_0$, $\zeta\preceq\eta$, and $i\in\{1,2\}$, there does not exist an $x^*\in\shock{[\zeta,\eta]}$ such that $x^*-ne_i\in\ans{[\zeta,\eta]}{x^*-(n+1)e_i}$ for all $n\in\Z_+$ and nor does there exist an $x^*\in\shock{[\zeta,\eta]}$ such that $x^*+(n+1)e_i\in \ans{[\zeta,\eta]}{x^*+ne_i}$ for all $n\in\Z_+$.
\end{lemma}

\begin{proof}
We prove the result for $i=1$, $i=2$ being similar. We also only work with paths of the first type. The other type can be treated similarly.

The existence of a path of the first type, with $i=1$, implies that $x^*-ne_1-\etstar$ points to  $x^*-(n-1)e_1-\etstar$ in $\G{\eta+}$ 
for all $n\in\Z_+$. But this implies that $\B{\eta+}(x^*-ne_1-\etstar,x^*-(n-1)e_1-\etstar)=\w_{x^*-ne_1-\etstar}$, for all $n\in\Z_+$. Take any sequence $\eta_m\in\Udense$ such that $\eta_m\searrow\eta$.
Then \eqref{mono} and \eqref{coc-prop} imply that
	\[\sum_{k=1}^n\w_{x^*-ke_1-\etstar}=\B{\eta+}(x^*-ne_1-\etstar,x^*-\etstar)\ge\B{\eta_m}(x^*-ne_1-\etstar,x^*-\etstar).\]
Divide by $n$ and apply the ergodic theorem on the left-hand side and \eqref{eq:erg-coc} on the right-hand side to get $\E[\w_0]\ge e_1\cdot\nabla\gpp(\eta_m)$ for all $m$.
Take $m\to\infty$ to get $\E[\w_0]\ge e_1\cdot\nabla\gpp(\eta+)$. It follows from Martin's estimate of the asymptotic behavior of the shape function near the boundary of $\Uset$, \cite[Theorem 2.4]{Mar-04}, along with concavity that this cannot happen.
\end{proof}

\begin{proof}[Proof of Lemma \ref{lm:downright}]
A general step of the path can be decomposed as 
$x_{i+1}-x_i=\sum_k (y_{k+1}-y_k)$ where each $y_{k+1}-y_k\in\{e_1, -e_2\}$.  Then each $\mu_{y_k, y_{k+1}}$ is a negative measure, and consequently $\supp\mu_{x_i, x_{i+1}}=\bigcup_k \supp\mu_{y_k, y_{k+1}}$.  Thus we may assume   that the path satisfies $x_{i+1}-x_i\in\{e_1, -e_2\}$ for all $i$.  

One direction is clear:
	$\bigcup_{i\in\Z} \supp\mu_{x_i,x_{i+1}}\subset\aUset$. 
	
For the other direction, take $\xi\in\aUset$.  By  Theorem \ref{thm:shock1},   there is a bi-infinite up-right reverse-directed  path $x^*_{-\infty,\infty}$   through $x^*$ in $\shockG{\xi}$ with  increments in $\{e_1,e_2\}$. By Lemma \ref{hor-red} this path must cross any down-right lattice path $x_{-\infty,\infty}$. This means that there exists an $i\in\Z$ such that either $x_{i+1}-x_i=e_1$ and $x_i+\etstar$ points to  $x_i-\exstar$ in $\shockG{\xi}$, i.e.\ $x_i$ points to $x_i+e_2$ in $\G{\xi-}$, or $x_{i+1}-x_i=-e_2$ and $x_i-\exstar$ points to  $x_i-\etstar$ in $\shockG{\xi}$, i.e.\ $x_i$ points to $x_i+e_1$ in $\G{\xi+}$. 
In the former case, $\geo{}{x_i}{\xi-}$ goes from $x_i$ to $x_i+e_2$ and from there 
it never touches $\geo{}{x_{i+1}}{\xi+}=\geo{}{x_i+e_1}{\xi+}$, since $x_i+\etstar\in\shock{xi}$. Consequently, in this case Theorem \ref{thm:nonint} says that $\xi\in\supp\mu_{x_i,x_{i+1}}$. The other case is similar and again gives $\xi\in\supp\mu_{x_i,x_{i+1}}$.  This proves Lemma \ref{lm:downright}.
\end{proof}

\subsection{Density of instability points on the lattice}
For $\zeta\preceq\eta$ in $\ri\Uset$, $x\in\Z^2$, and $i\in\{1,2\}$ %\note{C: We should move all of this down to the proofs section.}
let 
\be\label{df:rho5} \rho_x^i(\zeta,\eta)=\one\bigl\{[\zeta,\eta]\cap\supp{\mu_{x,x+e_i}}\neq\varnothing\bigr\}.\ee 
We write $\rho_x^i(\xi)$ for $\rho_x^i(\xi,\xi)$. 
By definition, $x+\etstar\in\shock{[\zeta,\eta]}$ if and only if $\rho_x^1(\zeta,\eta)$ and $\rho_x^2(\zeta,\eta)$ are not both $0$.
By Lemma \ref{lm:cross} below,  $\rho_x^i(\zeta,\eta)=1$ is equivalent to $x+\etstar$ pointing to $x+\etstar-e_{3-i}$ in $\shockG{[\zeta,\eta]}$. 
Also, $\rho_x^1(\xi)=\rho_x^2(\xi)=1$ if and only if $\cid(T_x\w)=\xi$.
Let
	\[\kappa_i(\zeta,\eta)=\P\{\rho_0^i(\zeta,\eta)=1\}.\]
Since $\supp{\mu_{x,x+e_i}}$ is by definition closed,  $\kappa_i$ is left-continuous in $\zeta$ and right-continuous in $\eta$. 
Furthermore, by Theorem \ref{th:V1} $\kappa_i$ is continuous in each argument at points of differentiability of $\gpp$. 
%F: we just said that the thing is left-continuous in $\zeta$ and right-continuous in $\eta$. For continuity we need the other two statements: right-continuous in $\zeta$ and left-continuous in $\eta$.  The thing is monotone in both variables and thus continuity just follows from not assigning mass points, i.e.\ from Theorem \ref{th:V1}.}  
Again, we write $\kappa_i(\xi)$ for $\kappa_i(\xi,\xi)$.
%A fact that is needed to see this is that the support is a closed set. So any accumulation point stays in the support.
We thus have
	\[\kappa_i(\xi)=\lim_{\zeta\nearrow\xi,\eta\searrow\xi}\kappa_i(\zeta,\eta).\]
By Theorem \ref{th:V1}, $\xi \in \Diff$ if and only if $\kappa_i(\xi)=0$ for any (and hence both) $i\in\{1,2\}$.
Let 
	\[\kappa_{12}(\zeta,\eta)=\P\{\rho_0^1(\zeta,\eta)=\rho_0^2(\zeta,\eta)=1\}=\P\{\cid\in[\zeta,\eta]\}\]
and write $\kappa_{12}(\xi)$ for $\kappa_{12}(\xi,\xi)$. The last equality above follows because if $\cid\notin[\zeta,\eta]$, then by recovery \eqref{rec-prop2} and by the Busemann characterization \eqref{cid} of $\cid$, one of the processes $\xi\mapsto\B{\xi\pm}(0,e_i)$ for $i\in\{1,2\}$ is constant for $\xi\in[\zeta,\eta]$. 

% the Busemann process is constant on $[\zeta,\eta]$ for one of the two edges.

The next result essentially follows from the ergodic theorem and 
gives the density of horizontal and vertical edges, instability points, branch points, and coalescence points. 

%Recall the full measure event $\Omreg$ introduced in Lemma \ref{lm:B+>B-}.

\begin{lemma}\label{lm:den}
Assume the regularity condition \eqref{g-reg}.
There exists a $T$-invariant event $\Omega_0'\subset\Omega_0$ with $\P(\Omega_0')=1$ and 
such that for all $\w\in\Omega+0'$, $i,j\in\{1,2\}$, $a,b,a',b'\in\{0,1\}$ with $(b-a)(b'-a')\ne0$, and for all $\zeta\preceq\eta$ in $\ri\Uset$, we have
	\begin{align}
		\begin{split}
		\label{den:edge}
		&\lim_{n\to\infty}\frac1{\abs{b-a}n}\sum_{k=-an}^{bn}\rho_{ke_i}^j(\zeta,\eta)\\
		&\qquad\qquad=\lim_{n\to\infty}\frac1{\abs{(b-a)(b'-a')}n^2}\sum_{x\in[-an,bn]\times[-a'n,b'n]}\!\!\!\!\!\!\!\!\!\!\!\!\!\rho_x^j(\zeta,\eta)=\kappa_j(\zeta,\eta),
		\end{split}\\
		\begin{split}
		\label{den:red}
		&\lim_{n\to\infty}\frac1{\abs{b-a}n}\sum_{k=-an}^{bn}\one\{ke_i+\etstar\in\shock{[\zeta,\eta]}\}\\
		&\qquad\qquad=\lim_{n\to\infty}\frac1{(b-a)(b'-a')n^2}\sum_{x\in[-an,bn]\times[-a'n,b'n]}\!\!\!\!\!\!\!\!\!\!\!\!\!\one\{x+\etstar\in\shock{[\zeta,\eta]}\}\\
		&\qquad\qquad=\kappa_1(\zeta,\eta)+\kappa_2(\zeta,\eta)-\kappa_{12}(\zeta,\eta),
		\end{split}\\
		\begin{split}
		\label{den:cid}
		&\lim_{n\to\infty}\frac1{\abs{b-a}n}\sum_{k=-an}^{bn}\rho_{ke_i}^1(\zeta,\eta)\rho_{ke_i}^2(\zeta,\eta)\\
		&\qquad\qquad=\lim_{n\to\infty}\frac1{\abs{(b-a)(b'-a')}n^2}\sum_{x\in[-an,bn]\times[-a'n,b'n]}\!\!\!\!\!\!\!\!\!\!\!\!\!\rho_x^1(\zeta,\eta)\rho_x^2(\zeta,\eta)=\kappa_{12}(\zeta,\eta),	
		\end{split}\\
		&\text{and}\notag\\
		\begin{split}
		\label{den:coal}
		&\lim_{n\to\infty}\frac1{\abs{b-a}n}\sum_{k=-an}^{bn}\rho_{ke_i}^1(\zeta,\eta)\rho_{(k+1)e_i-e_{3-i}}^2(\zeta,\eta)\\
		&\qquad\qquad=\lim_{n\to\infty}\frac1{\abs{(b-a)(b'-a')}n^2}\sum_{x\in[-an,bn]\times[-a'n,b'n]}\!\!\!\!\!\!\!\!\!\!\!\!\!\rho_{x-e_1}^1(\zeta,\eta)\rho_{x-e_2}^2(\zeta,\eta)=\kappa_{12}(\zeta,\eta).
		\end{split}
%		&\lim_{n\to\infty}\frac1{(b-a)n}\sum_{k=-an}^{bn}\one\{ke_i+\etstar\in\shock{[\zeta,\eta]}\}
%		=\lim_{n\to\infty}\frac1{[(b-a)n]^2}\sum_{x\in[-an,bn]^2}\one\{x+\etstar\in\shock{\zeta,\eta}\}
%		=\kappa_1(\zeta,\eta)+\kappa_2(\zeta,\eta)-\kappa_{12}(\zeta,\eta),\label{den:red}\\
%		&\lim_{n\to\infty}\frac1{(b-a)n}\sum_{k=-an}^{bn}\rho_{ke_i}^j(\xi)=\lim_{n\to\infty}\frac1{[(b-a)n]^2}\sum_{x\in[-an,bn]^2}\rho_x^j(\xi)=\kappa^j(\xi).\label{den:zero}
               	\end{align}
All of the above limits are positive if and only if $\nabla\gpp(\zeta+)\ne\nabla\gpp(\eta-)$.
\end{lemma}

%We compute these quantities explicitly in the case of exponential weights in Corollary \ref{cor:explicit} below.

 \begin{proof}%[Proof of Lemma \ref{lm:den}] 
As explained in Remark \ref{rk:ergodicity}, under the regularity condition \eqref{g-reg}, the Busemann process is a measurable function of $\{\w_x:x\in\Z^2\}$. Thus, by the ergodic theorem,  there exists a $T$-invariant event 
$\Omega_0'\subset\Omega_0$ with $\P(\Omega_0')=1$ and such that for $\w\in\Omega_0'$ the limits (\ref{den:edge}-\ref{den:coal}) hold for
 all $\zeta,\eta\in\Udense\cup\bigl((\ri\Uset)\setminus\Diff\bigr)$.
 
 To justify the equality of the limit in \eqref{den:coal} with the one in \eqref{den:cid} observe that since every instability point must have at least one descendant and at least one ancestor, we have
	\[\P\{-\etstar\in\shock{[\zeta,\eta]}\}=\P\{\rho_{-e_1}^1(\zeta,\eta)=1\}+\P\{\rho_{-e_2}^2(\zeta,\eta)=1\}-\P\{\rho_{-e_1}^1(\zeta,\eta)=\rho_{-e_2}^2(\zeta,\eta)=1\}\]
and
	\[\P\{\etstar\in\shock{[\zeta,\eta]}\}=\P\{\rho_0^1(\zeta,\eta)=1\}+\P\{\rho_0^2(\zeta,\eta)=1\}-\P\{\rho_0^1(\zeta,\eta)=\rho_0^2(\zeta,\eta)=1\}.\]
By shift invariance, the first three probabilities in the first display match the corresponding three probabilities in the second display.  Thus, 
	\[\P\{\rho_{-e_1}^1(\zeta,\eta)=\rho_{-e_2}^2(\zeta,\eta)=1\}=\kappa_{12}(\zeta,\eta).\]


%Let $\cA$ be a dense countable subset of $\ri\Uset$ that contains 
%the (countably many) points $\xi\in\ri\Uset$ where $\gpp$ is not differentiable.
%Let $\Omega_0$ be the full-measure event on which these claims hold for all $\zeta\preceq\eta$ in $\cA$. 
We now prove the first limit in \eqref{den:edge}, the rest of the limits in the statement of the lemma being similar.
Take $\w\in\Omega_0'$ and any $\zeta\prec\eta$ in $\ri\Uset$. Suppose first $\gpp$ is differentiable at both $\zeta$ and $\eta$.
Take sequences $\zeta_m'\prec\zeta\prec\zeta_m\prec\eta_m\prec\eta\prec\eta_m'$ with $\zeta_m', \zeta_m, \eta_m, \eta_m' \in \Udense$ and use monotonicity and the continuity of $\kappa_j$ to get
	\begin{align*}
%	\kappa_j(\zeta,\eta)=\kappa_j(\zeta-,\eta+)
	\kappa_j(\zeta_m,\eta_m)
	&=\lim_{n\to\infty}\frac1{(b-a)n}\sum_{k=-an}^{bn}\rho_{ke_i}^j(\zeta_m,\eta_m)\\
	&\le\varliminf_{n\to\infty}\frac1{(b-a)n}\sum_{k=-an}^{bn}\rho_{ke_i}^j(\zeta,\eta)
	\le \varlimsup_{n\to\infty}\frac1{(b-a)n}\sum_{k=-an}^{bn}\rho_{ke_i}^j(\zeta,\eta)\\
	&\le \lim_{n\to\infty}\frac1{(b-a)n}\sum_{k=-an}^{bn}\rho_{ke_i}^j(\zeta_m',\eta_m')
	=\kappa_j(\zeta_m',\eta_m').
	\end{align*}
Taking $m\to\infty$ and using continuity of $\kappa_j$ at $\zeta$ and $\eta$ 
gives that the above liminf and limsup are equal to $\kappa_j(\zeta,\eta)$.
The same proof works if $\zeta=\eta$ is a point of differentiability of $\gpp$. In this case, we can use $0$ as a lower bound and for the upper bound we have $\kappa_j(\zeta)=\kappa_j(\eta)=0$. 	

Next, suppose $\zeta$ is a point of non-differentiability of $\gpp$, but $\eta$ is still a point of differentiability.
We can repeat the same argument as above, but this time only using the sequences $\eta_m$ and $\eta'_m$ and the intervals $[\zeta,\eta_m]$ and $[\zeta,\eta_m']$ for the upper and lower bounds, 
because $\zeta$ has been included in the set $\Udense\cup\bigl((\ri\Uset)\setminus\Diff\bigr)$. 
A similar argument works if $\zeta$ is a point of differentiability but $\eta$ is not. When $\gpp$ is not differentiable at both $\zeta$ and $\eta$, the claimed limits follow from the choice of $\Omega_0'$.
\end{proof}

\begin{proof}[Proof of Proposition \ref{prop:trichotomy}]
The claim follows from Lemma \ref{lm:den} 
%(a) follows from the definition of $\aUset$. (b) and (c) follow from $\kappa(\xi)=0$ iff $\xi\in\Diff$.
\end{proof}

\subsection{Flow of Busemann measures}\label{sec:Busflowpf}

\begin{proof}[Proof of Theorem \ref{th:flowS}]
The vertex set of $\cB^*_{[\zeta, \eta]}$ is by definition the same as that of $\shockG{[\zeta,\eta]}$. That the edges also agree follows from Lemma \ref{lm:cross} below. 
\end{proof} 

 
\begin{lemma}\label{lm:cross}
For $i\in\{1,2\}$, $[\zeta,\eta]\cap\supp{\mu_{x,x+e_i}}\neq\varnothing$  if and only if 
$(x+\etstar, x+\etstar-e_{3-i})$ is a directed  edge in the graph $\shockG{[\zeta,\eta]}$.  
%$x+\etstar\in\shock{[\zeta,\eta]}$ and $x+\etstar\in\shock{[\zeta,\eta]}$ points to $x+\etstar-e_{3-i}$ in $\dS{[\zeta,\eta]}$. 
\end{lemma}

\begin{proof}
We argue the case of $i=1$.
Assume first that $[\zeta,\eta]\cap\supp{\mu_{x,x+e_1}}\neq\varnothing$. 
From $\mu_{x+e_1, x+e_2}=\mu_{x+e_1, x}+\mu_{x,x+e_2}$ and $\mu_{x-\ex, x}=\mu_{x-\ex, x+e_1}+\mu_{x+e_1, x}$ (sums of positive measures) we see that both $x+\etstar, x+\etstar-e_{2}\in\shock{[\zeta, \eta]}$. 

Suppose $\xi\in[\zeta,\eta]\cap\supp{\mu_{x,x+e_1}}$.  By Theorem \ref{thm:nonint}, $x$ must point to $x+e_2$ in $\G{\xi-}$,   which forces the same   in $\G{\zeta-}$.  
Thus    $x+\etstar$ points to $x+\etstar-e_2$ in $\dG{\zeta-}$ and hence also in $\dS{[\zeta,\eta]}$. 


Conversely, if $x+\etstar\in\shock{[\zeta,\eta]}$ then $\geo{}{x+e_2}{\zeta-}$ and $\geo{}{x+e_1}{\eta+}$ do not intersect. If furthermore $x+\etstar$ points to $x+\etstar-e_2$ in $\dS{[\zeta,\eta]}$, then $x$ points to $x+e_2$ in $\G{\zeta-}$ and hence $\geo{}{x}{\zeta-}$ joins $\geo{}{x+e_2}{\zeta-}$ and does not intersect $\geo{}{x+e_1}{\eta+}$.   
 
 Let $\zeta'\prec\zeta$ and $\eta'\succ\eta$.  By geodesic ordering \eqref{path-ordering}, $\geo{}{x}{\zeta'+}$ and $\geo{}{x+e_1}{\eta'-}$ are disjoint.  In particular, the coalescence points $\coal{\zeta'+}(x,x+e_1)$ and $\coal{\eta'-}(x,x+e_1)$ cannot coincide on $\Z^2$.  By Proposition \ref{pr:supp1}, $]\zeta', \eta'[$  intersects  $\supp{\mu_{x,x+e_1}}$. Since this holds  for every choice of $]\zeta', \eta'[\,\supset [\zeta,\eta]$, it follows that also 
  $[\zeta,\eta]$ intersects $\supp{\mu_{x,x+e_1}}$.
\end{proof}

\begin{proof}[Proof of Proposition \ref{lm:K9}]
Suppose $x\zesim y$.    Since  $\supp\mu_{x,y}$ is a closed subset of $\ri\Uset$  and $[\zeta, \eta]$  a compact set,   we can find $\zeta'\prec\zeta$ and $\eta'\succ\eta$ such that  $\abs{\mu_{x,y}}(\,]\zeta', \eta'[\,)=0$.   Then by Proposition \ref{pr:supp1}, there exists $z\in\Z^2$ such that all geodesics $\geo{}{x}{\xi\sig}$ and $\geo{}{y}{\xi\sig}$ for $\xi\in[\zeta, \eta]$ and $\sigg\in\{-,+\}$ meet at $z$.  Thus  $x$ and $y$ are in the same subtree of the graph $\G{\cap[\zeta, \eta]}$. 

Conversely, suppose $x$ and $y$ are two distinct points  in the same subtree $\cK$ of the graph $\G{\cap[\zeta, \eta]}$.   In this tree the following holds. 
\be\label{aux775} \begin{aligned} 
&\text{In $\cK$ there is a point $z$ and a path $\pi$ from $x$ to $z$  and a path $\pi'$ from $y$ to $z$ }\\[-2pt] 
&\text{such that $z$ is the first common point of $\pi$ and $\pi'$. For each $\xi\in[\zeta, \eta]$ and }\\[-2pt]
&\text{both signs  $\sigg\in\{-,+\}$, all the geodesics $\geo{}{x}{\xi\sig}$ follow $\pi$  from $x$ to $z$,  }\\[-2pt]
&\text{and all the geodesics $\geo{}{y}{\xi\sig}$  follow $\pi'$  from $y$ to $z$.} 
\end{aligned}\ee
 % For each $\xi\in[\zeta, \eta]$ and both signs  $\sig\in\{-,+\}$,  all the geodesics $\geo{}{x}{\xi\sig}$ follow $\pi$  from $x$ to $z$,  and all the geodesics $\geo{}{y}{\xi\sig}$  follow $\pi'$  from $y$ to $z$.  
  Consequently each  $\xi\in[\zeta, \eta]$ satisfies $\coal{\xi-}(x,y)=\coal{\xi+}(x,y)=z$.  By Proposition \ref{pr:supp2} each  $\xi\in[\zeta, \eta]$ lies outside $\supp\mu_{x,y}$. 
\end{proof}

\begin{figure}[h]
 	\begin{center}
 		 \begin{tikzpicture}[scale=1]
		 
		 	\draw(0,0)--(1.5,0)--(1.5,1.5)--(0,1.5)--(0,0);
		 	\draw[line width=1.5pt](0,1.5)--(0.5,1.5)--(0.5,1.7)--(0.9,1.7)--(0.9,1.9)--(1.4,1.9)--(1.4,2.1)--(1.8,2.1)--(1.8,2.3)--(2.2,2.3)--(2.2,2.5)--(2.7,2.5);
			\draw[fill=black](0,1.5) circle(2pt);
			\draw(0,1.5)node[left]{$x$};
			\draw(0.9,1.9)node[above]{$\pi$};
			\draw[line width=1.5pt](1.5,0)--(1.5,0.6)--(1.8,0.6)--(1.8,1)--(2.1,1)--(2.1,1.6)--(2.4,1.6)--(2.4,2.1)--(2.7,2.1)--(2.7,2.5);
			\draw[fill=black](1.5,0) circle(2pt);
			\draw(1.5,0)node[right]{$y$};
			\draw(2.1,1.3)node[right]{$\pi'$};
			\draw[line width=1.5pt](0.4,0.8)--(0.8,0.8)--(0.8,1.2)--(1.2,1.2)--(1.2,1.7)--(1.6,1.7)--(1.6,2.1);
			\draw[fill=black](0.4,0.8) circle(2pt);
			\draw(0.38,0.8)node[below]{$u$};
			\draw(1.2,1.25)node[below]{$\pi''$};
			\draw[fill=black](2.7,2.5) circle(2pt);
			\draw(2.85,2.5)node[above]{$z$};
		
		\end{tikzpicture}
 	 \end{center}
 	\caption{\small  Proof of Lemma \ref{lm:K10}.}
 \label{fig:K10}
 \end{figure}


\begin{proof}[Proof of Lemma \ref{lm:K10}]
The hypotheses imply that, by switching $x$ and $y$ around if necessary, $x\cdot e_1\le y\cdot e_1$ and $x\cdot e_2\ge y\cdot e_2$.    Let $z, \pi, \pi'$ be as in \eqref{aux775}.  
 %Let  $\pi$ be the path from $x$ to $z$ followed by all the geodesics $\{\geo{}{x}{\xi\pm}: \xi\in[\zeta, \eta]\}$, and similarly let  $\pi'$ be the path from $y$ to $z$ followed by all the geodesics  $\{\geo{}{y}{\xi\pm}: \xi\in[\zeta, \eta]\}$.  
Let $u$ be any point of  $\lzb x\wedge y, x\vee y\rzb$.    By planarity, 
%\timonote{Picture? Better words? Something like: since $u_2\le x_2$ and $u_1\ge x_1$, the geodesic from $u$ stays weakly below the one from $x$?}  
 each geodesic $\geo{}{u}{\xi\sig}$ for $ \xi\in[\zeta, \eta]$ and  $\sigg\in\{-,+\}$  must eventually intersect $\pi$ or $\pi'$ and then follow this to $z$.   See Figure \ref{fig:K10}.
 By  uniqueness of finite geodesics,  all  these geodesics  $\geo{}{u}{\xi\sig}$  follow the same path $\pi''$ from $u$ to $z$.     Thus $\pi''$ is part of the graph $\G{\cap[\zeta, \eta]}$, and since it comes together  with $\pi$ and $\pi'$ at $z$,  $\pi''$ is part of the same  subtree $\cK$.  
\end{proof}


\begin{proof} [Proof of Lemma \ref{lm:K12}] 
Suppose $x$ is such a vertex but  $\cK\subset\{y: y\ge x\}$ fails. 
We claim that then there necessarily exists a vertex $y\in\cK$ such that $x$ and $y$ satisfy the hypotheses of Lemma \ref{lm:K10} and one of $\{x- e_1, x- e_2\}$ lies in  $\lzb x\wedge y, x\vee y\rzb$. This leads to a contradiction. 

To verify the claim,  
pick $y\in\cK$ such that $y\ge x$ fails.  If $y<x$ also fails,  there are two possible cases: 
\begin{enumerate}     [label={\rm(\roman*)}, ref={\rm(\roman*)}]   \itemsep=3pt  
\item    $y\cdot e_1< x\cdot e_1$ and $y\cdot e_2\ge  x\cdot e_2$, in which case  $x- e_1\in\lzb x\wedge y, x\vee y\rzb\subset\cK$;
\item  $y\cdot e_1\ge x\cdot e_1$ and $y\cdot e_2< x\cdot e_2$, in which case  $x- e_2\in\lzb x\wedge y, x\vee y\rzb\subset\cK$.  
\end{enumerate} 

If $y<x$ does not fail, follow the geodesics $\{\geo{}{y}{\xi\pm}: \xi\in[\zeta, \eta]\}$ until they hit the level  $\level_{x\cdot\et}$ at some point $y'$.    The assumption that neither $x- e_1$ nor $x- e_2$ lies in $\cK$ implies that $y'\ne x$.  Thus $y'$ is a point of  $\cK$ that fails both   $y'\ge x$ and  $y'<x$.  Replace $y$ with $y'$ and apply the previous argument. 

We have shown that the existence of $x\in\cK$ such that $\{x- e_1, x- e_2\}\cap\cK=\varnothing$ implies that $\cK\subset\{y: y\ge x\}$.     That such $x$ must be unique follows since $x$ lies outside $\{y: y\ge x'\}$ for any $x'\ne x$ that satisfies $x'\ge x$. 
 
Assuming that $\inf\{ t\in\Z: \cK\cap\level_t\ne\varnothing\}>-\infty$,  pick $x \in\cK$ to minimize the level $x\cdot\et$.  
\end{proof}

\begin{proof}[Proof of Theorem \ref{thm:jumpG}] 
{\it Part \eqref{thm:jumpG.a}.}  If $[\zeta, \eta]\cap\,\aUset=\varnothing$ then the interval  $[\zeta, \eta]$  is  strictly on one    side of $\cid(T_x\w)$ at every $x$.   Hence the graphs  $\{ \G{\xi\sig}: \xi\in[\zeta, \eta], \sigg\in\{-,+\}\}$ are all identical.  This common graph is a tree by Theorem \ref{thm:+-coal}. 

Conversely, if   $\xi\in[\zeta, \eta]\cap\,\aUset$,  then there exist $x,y$ such that $\xi\in\supp{\mu_{x,y}}$ and by Theorem \ref{thm:nonint} there are disjoint geodesics in $\G{\cap[\zeta, \eta]}$. 
\medskip

{\it Part \eqref{thm:jumpG.b}.}
It follows from what was already said that $\{\cK(z):  z\in\cifset^{[\zeta, \eta]}\}$ are disjoint subtrees  of $\G{\cap[\zeta, \eta]}$ and their vertex sets cover $\Z^2$.   Suppose  $(x,x+ e_i)$ is an edge in $\G{\cap[\zeta, \eta]}$.  Then all geodesics $\{\geo{}{x}{\xi\sig}: \xi\in[\zeta, \eta], \sigg\in\{-,+\}\}$ go through this edge.  Thus this edge must be an edge of the tree $\cK(z)$ that contains both $x$ and $x+ e_i$.    Hence each edge of $\G{\cap[\zeta, \eta]}$ is an edge of one of the trees $\cK(z)$, and no such edge can connect two  trees $\cK(z)$ and $\cK(z')$ for distinct $z$ and $z'$. 
\end{proof} 


==> JEMS Post-Accept Revision/GeoWebPaper-Sec8.tex <==
% !TEX root = GeoWebPaper.tex

\section{Instability points in the exponential model: proofs}\label{sec:exp-pf}
%In the exponential case the densities in Lemma \ref{lm:den} can  be computed explicitly in terms of the parametrization \eqref{u-a}. 
%
%\addmath{this should just be a remark and maybe we can even get rid of it if Lemma \ref{lm:den} is removed}
%\begin{corollary} \label{cor:explicit}
%Assume \eqref{exp-assump}.  For  $\zeta\prec\eta$ in $\ri\Uset$ we have the following:
%	\begin{align*}%\label{kappas}
%	&\kappa_1(\zeta,\eta)=\frac{\alpha(\eta)-\alpha(\zeta)}{\alpha(\eta)},\quad
%	\kappa_2(\zeta,\eta)=\frac{\alpha(\eta)-\alpha(\zeta)}{1-\alpha(\zeta)},\quad
%	\kappa_{12}(\zeta,\eta)=\alpha(\eta)-\alpha(\zeta)\\
%	&\text{and}\quad\kappa_1(\zeta,\eta)+\kappa_2(\zeta,\eta)-\kappa_{12}(\zeta,\eta)=\bigl(\alpha(\eta)-\alpha(\zeta)\bigr)\bigl(\alpha(\eta)^{-1}+\alpha(\zeta)^{-1}-1\bigr).
%	\end{align*}
%\end{corollary}
%\begin{proof}%[Proof of Corollary \ref{cor:explicit}]
%\textcolor{red}{This is a direct  simple computation, once Timo's part is in.}
%\timonote{Do we want this here?} 
%\end{proof}


%\begin{proof}[Proof of Corollary \ref{cor:ladder}]
%This too is a consequence of a direct computation.  On the one hand, \eqref{78-90} implies that given $\tau(0)=0$, $\{\tau(i+1)-\tau(i):i\in\Z\}$ is an i.i.d.\ sequence under $\P$, with a marginal distribution having the mass function
%	\[f_\tau(n)=C_{n-1}\,  \frac{\alpha(\zeta)^{n-1}\alpha(\eta)^n}{\bigl(\alpha(\zeta)+\alpha(\eta)\bigr)^{2n-1}},\quad n\in\N.\]
%On the other hand, the sequence $\{\sigma_{i+1}-\sigma_i:i\in\Z\}$ is also an i.i.d.\ sequence and its marginal distribution has the 
%\addmath{reference? does Feller have this?}
%mass function $f(2n)=0$ and
%	\[f_\sigma(2n-1)=\frac1{2n-1}{2n-1\choose n}\Bigl(\frac{\alpha(\eta)}{\alpha(\zeta)+\alpha(\eta)}\Bigr)^n\Bigl(\frac{\alpha(\zeta)}{\alpha(\zeta)+\alpha(\eta)}\Bigr)^{n-1}=f_\tau(n),\quad n\in\N.\]
	%C_{n-1}=\frac1n{2n-2\choose n-1}=\frac1n (2n-2)!/[(n-1)!]^2
	%\frac1{2n-1}{2n-1\choose n}=\frac1{2n-1}(2n-1)!/[(n-1)!n!]=\frac1n (2n-2)!/[(n-1)!]^2 = C_{n-1}
%The claim follows.
%\end{proof}

We turn  to the proof of the results in Section \ref{sec:exp}, beginning with a discussion of Palm kernels, which are needed in order to prove Theorems \ref{th:B-palm1} and \ref{thm:ladder-xi}.
\subsection{Palm kernels} \label{sub:palm}

Let $\cM_{\Z\times\ri\Uset}$ denote the space of locally bounded positive  Borel measures  on the locally compact space  $\Z\times\ri\Uset$.   Consider  $\Z\times\ri\Uset$  as the disjoint union of copies of $\ri\Uset$, one copy for each horizontal edge $(ke_1, (k+1)e_1)$ on the $x$-axis. Recall that $\B{\xi\sig}_k=\B{\xi\sig}(ke_1,(k+1)e_1)$.
We define  two random measures $\Bppa$ and $\Bpp$  on  $\Z\times\ri\Uset$ in terms of the Busemann functions $\xi\mapsto\B{\xi\pm}_k$ attached to   these  edges.  


%\addmath{maybe we can go lighter on the notation? e.g.\ no need for the $\{k\}\times$ and just consider $\nu_k$ as a measure on $\ri\Uset$ directly?}
On each subset $\{k\}\times\ri\Uset$ of $\Z\times\ri\Uset$ we (slightly abuse notation and) define the measure $\Bppa_k$ by 
 \[  \Bppa_k\bigl(\{k\}\times ]\zeta, \eta]\,\bigr) = \Bppa_k\bigl(\,]\zeta,\eta]\, \bigr)=\B{\zeta+}_k-\B{\eta+}_k\] 
 for $\zeta\prec\eta$ in $\ri\Uset$. 
In terms of definition \eqref{Bmeas},   $\Bppa_k=\mu_{(k+1)e_1, ke_1}$ is  a positive measure due to monotonicity \eqref{mono}. 
 %Since the particular copy of $\ri\Uset$ is uniquely specified by the subscript of $\Bppa_k$, we can  also consider $\Bppa_k$ as a measure on $\ri\Uset$:  $\Bppa_k\,]\zeta, \eta]=\Bppa_k(\{k\}\times ]\zeta, \eta])$.  
 On $\Z\times\ri\Uset$, define the measure   $\Bppa=\sum_k\Bppa_k$.  In other words, for Borel sets $A_k\subset\ri\Uset$,  
$\Bppa\bigl( \,\bigcup_k \{k\}\times A_k\bigr)=\sum_k \Bppa_k(A_k)$. 


Let $\Bpp_k$ denote the simple point process on  $\{k\}\times\ri\Uset$ that records   the locations of the jumps of the Busemann function $\xi\mapsto\B{\xi\pm}_k$:  for Borel $A\subset\ri\Uset$,
 \[  \Bpp_k(\{k\}\times A) = \Bpp_k(A) = \sum_{\xi\in A} \ind\{\B{\xi-}_k>  \B{\xi+}_k\}.  \]

We describe the probability distributions of the component measures $\Bppa_k$ and $\Bpp_k$, given in Theorem 3.4 of \cite{Fan-Sep-20}. 
%In terms of the variable $\alpha$ on the open unit interval $(0,1)$ given in \eqref{u-a}, 
Marginally, for each $k$, $\Bpp_k$ is a Poisson point process on $\ri\Uset$  with intensity measure
\be\label{Bmm}
  \Bmm\bigl(\,]\zeta, \eta]\,\bigr) = \Bmm_k\bigl(\,]\zeta, \eta]\,\bigr)= \E\bigl[ \Bpp_k(\,]\zeta, \eta]\,)\bigr]= \int_{\alpha(\zeta)}^{\alpha(\eta)}  \frac{ds}s = \log \frac{\alpha(\eta)}{\alpha(\zeta)}. 
  \ee
  In particular,  almost every realization of $\Bpp_k$ satisfies  $\Bpp_k[\zeta, \eta]<\infty$
for all $\zeta\prec\eta$ in $\ri\Uset$. 

 Create a marked Poisson process by attaching an independent Exp$(\alpha(\xi))$-distributed weight $Y_{\xi}$ to each point $\xi$ in the support of $\Bpp_k$.  Then   the distribution of $\Bppa_k$ is that of the purely atomic measure defined by 
\be\label{Bppa4}   \Bppa_k\bigl(\,]\zeta, \eta]\,\bigr) = \sum_{\xi\in\ri\Uset:\,\Bpp_k(\xi)=1}  Y_{\xi} \,\ind_{]\zeta, \eta]}(\xi) \quad \text{for }  \zeta\prec\eta\text{ in } \ri\Uset. \ee
The random variable $\Bppa_k(\,]\zeta, \eta]\,)$ has distribution $\text{Ber}(1-\frac{\alpha(\zeta)}{\alpha(\eta)})\otimes\text{Exp}(\alpha(\zeta))$ (product of a Bernoulli and an independent exponential) and 
expectation 
\be\label{Bmma}
%  \Bmm(\zeta, \eta] = \Bmm_k(\zeta,\eta]= 
  \E\bigl[ \Bppa_k\bigl(\,]\zeta, \eta]\,\bigr)\bigr]=  \frac1{\alpha(\zeta)} - \frac1{\alpha(\eta)}\,. 
  \ee


 
Note the following technical point.  The jumps of $\B{\xi\pm}_k$ concentrate at $e_2$ and $\B{e_2-}_k=\infty$.  To define $\Bppa$ and $\Bpp$ as locally finite measures, the standard Euclidean topology of  $\ri\Uset$ has to be metrized so that $]e_2, \eta]$ is an unbounded set for any $\eta\succ e_2$.   This point makes no difference to our calculations and we already encountered this same issue around  definition \eqref{Bmeas} of the Busemann measures.  
%since in any case we consider these measures only on compact subsets of $\ri\Uset$. 
With this convention we can regard   $\Bpp=\sum_k\Bpp_k$ as a simple point process on $\Z\times\ri\Uset$ with mean measure $\widetilde{\Bmm}= (\text{counting  measure on $\bbZ$})\otimes \lambda$.  

For $(k,\xi)\in \Z \times \ri \Uset$, let $Q_{(k,\xi)}$ be the Palm kernel of $\Bppa$ with respect to $\Bpp$.  That is, $Q_{(k,\xi)}$ is the stochastic kernel from $ \Z \times \ri \Uset$ into $\cM_{\Z \times \ri \Uset}$  that gives the  distribution of $\Bppa$,  conditional on $\Bpp$ having a point at $(k,\xi)$, understood in the Palm sense.   Rigorously, the kernel is defined by disintegrating the Campbell measure of the pair $(\Bpp,\Bppa)$ with respect to the mean measure $\widetilde{\Bmm}$ of $\Bpp$ (this is developed in Section 6.1 in \cite{Kal-17}):
%for any compact $A\subset\ri\Uset$ and a Borel set   $M\subset\cM_\cX$, 
%\be\label{79-50} 
%\E [ \Bpp(\{k\}\times A)\,\ind_M(\Bppa)]   = \int_{\ri\Uset}\!\!\!\ind_A(\xi) \, Q_{(k,\xi)}(M)\,\Bmm_k(d\xi).   
%\ee
%Standard approximation arguments give then that 
for any nonnegative  Borel  function $f:(\Z \times \ri \Uset) \times\cM_{\Z \times \ri \Uset}\to\R_+$,
\begin{align}\label{79-50-50} 
\E\Bigl[ \int_{\Z \times \ri \Uset} \!\!\!f(k,\xi,\Bppa)\, \Bpp(dk \otimes d\xi)\Bigr] &= \int_{\Z\times\ri\Uset}  \int_{\cM_{\Z\times\ri\Uset}} f(k,\xi,\Bppavar) \,Q_{(k,\xi)}(d\Bppavar)\, \widetilde{\Bmm}(dk \otimes d\xi).
%&= \sum_{k\in \bbZ} \int_{\ri\Uset}\int_{\cM_\cX}\!\!\!f((k,\xi),\Bppavar)\,Q_{(k,\xi)}(d\Bppavar) \,\Bmm_k(d\xi). \notag
\end{align}
%For  $\xi\in\ri\Uset$,  denote the jump at $\xi$  of the  Busemann function attached to  interval $(ke_1, (k+1)e_1)$ by 
%\[  \Delta^\xi_k= \B{\xi-}_{ke_1, (k+1)e_1} -\B{\xi+}_{ke_1, (k+1)e_1}\]

Now we consider the indices $\tau^\xi(i)=\tau^{\xi,\xi}(i)$ of jumps at $\xi$,  defined in \eqref{78-45}.  
%  let $\dotsm<\tau^\xi(-1)<\tau^\xi(0)=0<\tau^\xi(1)<\dotsm$ be the indices such that $\Bpp(k, \xi)=1$ if and only if $k\in\{\tau^\xi(i):i\in\Z\}$.  Equivalently, 
%$\Delta^\xi_k>0$ 
In terms of the random measures introduced above, for $(k,\xi)\in \Z \times \ri \Uset$, 
% and the functions $\rho_k^1$  introduced in \eqref{df:rho5}, 
\[   
%\Bppa_k\{\xi\}>0 \; \iff \; \Bpp_k\{\xi\}=1 \; \iff \; 
\Bppa\{(k,\xi)\}>0 \; \iff \; \Bpp\{(k,\xi)\}=1 \; \iff \; 
\B{\xi-}_k> \B{\xi+}_k   %\;\iff \; \rho_k^1(\xi)=1
\;\iff \;k\in\{\tau^\xi(i):i\in\Z\}. \] 


%$\Bppa_k\{\xi\}>0$ $\iff$  $\Bpp_k\{\xi\}=1$ $\iff$  $\B{\xi-}_k> \B{\xi+}_k$ $\iff$ $\rho_k^1(\xi)=1$  $\iff$ $k\in\{\tau^\xi(i):i\in\Z\}$. 
 We condition on the event $\{\Bpp(0,\xi)=1\}$, in other words, consider the distribution of 
  $\{\tau^\xi(i)\}$ under $Q_{(0, \xi)}$. For this  to be well-defined, we  define these functions also on the space $\cM_{\Z \times \ri \Uset}$ in the obvious way:  for  $\nu\in\cM_{\Z \times \ri \Uset}$, the $\Z\cup\{\pm\infty\}$-valued functions $\tau^\xi(i)=\tau^\xi(i,\nu)$ are defined by the order requirement  
\[ \dotsm<\tau^\xi(-1,\nu)<0\le \tau^\xi(0,\nu)<\tau^\xi(1,\nu)<\dotsm\]  and the condition 
%$\depa^\zeta_k>\depa^\eta_k$ if and only if $k\in\{\tau^{\zeta, \eta}(i):i\in\Z\}$.   
\[ %\be\label{78-45-nu} 
\text{for $k\in\Z$,} \quad  \nu\{(k,\xi)\}>0\quad\text{if and only if}\quad k\in\{\tau^\xi(i,\nu):i\in\Z\}.   
\] %\ee
Since $\Bppa$ is $\P$-almost surely a purely atomic measure, it follows from general theory that  $Q_{(0, \xi)}$ is also supported on such measures. Furthermore, the conditioning itself forces   $Q_{(0, \xi)}\{\nu: \tau^\xi(0,\nu)=0\}=1$.   Thus   the random integer points $\tau^\xi(i,\nu)$ are not all trivially $\pm\infty$ under  $Q_{(0, \xi)}$. Connecting back to the notation of Section \ref{sec:exp}, for each $k \in \bbZ$, $\xi \in \ri \Uset$, each finite $A \subset \bbZ$  and $n_i \in \bbZ_+, r_i \in \bbR_+$ with $i \in A$, the Palm kernel introduced in that section is defined  by
\begin{align}
&\bbP\bigl\{ \tau^\xi(i+1)-\tau^\xi(i) =n_i, \depa^{\xi-}_{\tau^{\xi}(i)}-\depa^{\xi+}_{\tau^{\xi}(i)}>r_i  \; \forall   i \in A \,||\, \B{\xi-}_k > \B{\xi+}_k\bigr\} \label{eq:palmdef} \\
&\qquad=Q_{(k, \xi)}\bigl\{ \nu: \tau^\xi(i+1,\nu)-\tau^\xi(i,\nu)=n_i, \,\nu\{(\tau^\xi(i,\nu),\xi)\}> r_i   \; \forall   i \in A\bigr\}. \notag
\end{align}

\subsection{Statistics of instability points}
We   turn to the proofs of the theorems of Section \ref{sec:exp}. These proofs make use of results from  Appendices \ref{a:bus} and \ref{a:RW}.

\begin{proof}[Proof of Theorem \ref{th:palm1}]
 By Corollary \ref{cor:B-q2},   the process $\{ \depa^\zeta_k-\depa^\eta_k\}_{k\in\Z}$ has the same distribution as $\{W^+_k\}_{k\in\Z}$ defined in \eqref{Wk}.   An application of the appropriate  mapping to these sequences produces the sequence 
 $\bigl\{\depa^\zeta_0-\depa^\eta_0, \, \tau^{\zeta, \eta}(i+1)-\tau^{\zeta, \eta}(i), \depa^\zeta_{\tau^{\zeta, \eta}(i)}-\depa^\eta_{\tau^{\zeta, \eta}(i)}: i\in\Z\bigr\}$ 
 that appears in  Theorem \ref{th:palm1} 
 and the sequence 
 $\{W^+_0, \, \sigma_{i+1}-\sigma_i, \, W^+_{\sigma_i}: i\in\Z\}$ that appears in  Theorem \ref{th:78-70}.  Hence these sequences also have identical distribution.   ($W^+_{\sigma_i}=W_{\sigma_i}$ by \eqref{78-65}.) 
The distributions remain equal when these sequences are conditioned on the positive probability events $ \depa^\zeta_0-\depa^\eta_0>0$ and $W^+_0>0$.  
 \end{proof}

It will be convenient to have notation for the conditional joint distribution that appears in \eqref{78-90} in Theorem \ref{th:palm1}. 
For $0<\alpha\le\beta\le 1$ define   probability distributions  $q^{\alpha, \beta}$   on the product space   $\Z^\Z\times[0,\infty)^\Z$ as follows.  Denote the  generic variables on this product space  by $(\{\tau_i\}_{i\in\Z},  \{\Delta_k\}_{k\in\Z})$ with $\tau_i\in\Z$ and $0\le\Delta_k<\infty$.     Given an integer $L>0$, integers 
$n_{-L}<\dotsm < n_{-2}< n_{-1}<n_0=0<n_1<n_2< \dotsm<n_L$,  
%$n_{-L}<n_{-L+1}<\dotsm<n_0=0<n_1<\dotsm<n_L$ 
and positive reals $r_{-L}, \dotsc, r_L$,  abbreviate $b_i=n_{i+1}-n_i$.  The measure  $q^{\alpha, \beta}$ is defined by 
\be\label{qab4}\begin{aligned}  
&q^{\alpha, \beta}\bigl\{\tau_{i}=n_i \text{ and }  \Delta_{n_i}> r_i \text{ for } i\in\lzb-L,L\rzb, \,  \Delta_k=0 
\text{ for } k\in\lzb n_{-L},n_L\rzb\setminus\{ n_j\}_{j\in\lzb-L,L\rzb}  \bigr\}\\
&=\biggl( \; \prod_{i=-L}^{L-1} C_{b_i-1}\,  \frac{\alpha^{b_i-1}\beta^{b_i}}{(\alpha+\beta)^{2b_i-1}}\biggr) \cdot 
 \biggl( \; \prod_{i=-L}^{L} e^{-\alpha r_i}\biggr).  
\end{aligned} \ee
To paraphrase the definition,  the following holds under  $q^{\alpha, \beta}$:  $\tau_0=0$,   $\Delta_k=0$ for $k\notin\{\tau_i\}_{i\in\Z}$, and  the variables   $\{\tau_{i+1}-\tau_{i}, \Delta_{\tau_i}\}_{i\in\Z}$   are mutually independent with marginal distribution 
\be\label{qab6} 
q^{\alpha, \beta}\{\tau_{i+1}-\tau_{i}=n, \Delta_{\tau_i}>r\}=C_{n-1}\,  \frac{\alpha^{n-1}\beta^n}{(\alpha+\beta)^{2n-1}} e^{-\alpha r}\quad \text{ for } i\in\Z, \,n\ge 1,\, r\ge0. 
\ee
 Abbreviate   $q^\alpha=q^{\alpha,\alpha}$   which has marginal  $q^\alpha\{\tau_{i+1}-\tau_{i}=n, \Delta_{\tau_i}>r\}=C_{n-1}(\tfrac12)^{2n-1} e^{-\alpha r}$.   As 
$\beta\to\alpha$,  $q^{\alpha, \beta}$ converges weakly to $q^\alpha$. 

%We derive a simple  tail bound for $q^{\alpha, \beta}$.  There exists an absolute  constant $c_0$ such that  the following bound holds for all $\alpha, \beta\in(0,\infty)$ and all $n\ge 2$:  
%\be\label{qab9} \begin{aligned}
%q^{\alpha, \beta}\{\tau_{i+1}-\tau_{i}\ge n\}  &= \sum_{k=n}^\infty C_{k-1}\,  \frac{\alpha^{k-1}\beta^k}{(\alpha+\beta)^{2k-1}}
%\le  \sum_{k=n}^\infty C_{k-1}\,  \frac{(1-\frac1k)^{k-1}}{(1-\frac1{2k})^{2k-1}} \cdot \biggl(\frac12\biggr)^{2k-1}\\
%&\le c_0 \sum_{k=n}^\infty C_{k-1}\,   \biggl(\frac12\biggr)^{2k-1}. 
%\end{aligned}\ee 
%The first inequality  above came from  \eqref{a:t498} in Appendix \ref{a:aux}. 
%\timonote{The need for this seems to have disappeared? Don't remember what it was in the first place...} 

Theorem \ref{th:palm1} can now be restated by saying that,  conditional on
$\depa^\zeta_0>\depa^\eta_0$,    the variables   \[\bigl(\{\tau^{\zeta, \eta}(i)\}_{i\in\Z}, \,  \{\depa^\zeta_k-\depa^\eta_{k}\}_{k\in\Z}\bigr)\]
  have joint   distribution $q^{\alpha(\zeta), \alpha(\eta)}$. 
Consequently, for a measurable set $A\subset\Z^\Z\times[0,\infty)^\Z$, 
\be\label{78-92} \begin{aligned}
&\P\bigl[  \depa^\zeta_0>\depa^\eta_0, \, \bigl(\{\tau^{\zeta, \eta}(i)\}_{i\in\Z}, \,  \{\depa^\zeta_k-\depa^\eta_{k}\}_{k\in\Z}\bigr) \in A  \bigr]\\[4pt] 
&=\P\bigl(  \depa^\zeta_0>\depa^\eta_0\bigr) \, \P\bigl[ \bigl(\{\tau^{\zeta, \eta}(i)\}_{i\in\Z}, \,  \{\depa^\zeta_k-\depa^\eta_{k}\}_{k\in\Z}\bigr) \in A  \,\big\vert\, \depa^\zeta_0>\depa^\eta_0\,\bigr] 
 \\
&=  \frac{\alpha(\eta)-\alpha(\zeta)}{\alpha(\eta)} \cdot   q^{\alpha(\zeta), \alpha(\eta)}(A). 
%
%&\P\bigl\{  \depa^2_0>\depa^1_0, \, \tau(i)-\tau(i-1)=k_i\ \text{ for } i\in\lzb -L+1, L\rzb  \bigr\}\\[4pt] 
%&=\P\bigl\{  \depa^2_0>\depa^1_0\bigr\} \, \P\bigl\{  \tau(i)-\tau(i-1)=k_i\ \text{ for } i\in\lzb -L+1, L\rzb  \,\big\vert\, \depa^2_0>\depa^1_0\bigr \}
% \\
%&=  \frac{\beta-\alpha}{\beta} \cdot  \prod_{i=-L+1}^L q^{\alpha, \beta}\{\tau(i)-\tau(i-1)=k_i\}. 
\end{aligned} \ee
The first probability on the last line came from \eqref{B4} and the second from Theorem \ref{th:palm1}. 



\begin{proof}[Proof of Theorem \ref{th:B-palm1}]
 
Define $\Z\cup\{\pm\infty\}$-valued ordered indices 
   $\dotsm<\tau^{\zeta, \eta}_{-1}<0\le \tau^{\zeta, \eta}_0<\tau^{\zeta, \eta}_1<\dotsm$   as measurable  functions of a locally finite measure  $\nu\in\cM_{\Z \times \ri \Uset}$ by  the rule  
\be\label{78-105}   \nu(\{k\}\times[\zeta,\eta])>0
\ \iff  \ k\in\{\tau^{\zeta, \eta}_i:i\in\Z\}. \ee
If  $\nu(\{k\}\times[\zeta,\eta])>0$ does not hold for infinitely many $k>0$ then  $\tau^{\zeta, \eta}_i=\infty$ for large enough $i$, and analogously  for 
$k<0$.    Definition \eqref{78-105}  applied  to the random measure   $\Bppa=\sum_k\Bppa_k$  reproduces  \eqref{78-45}.  

Fix integers   $K, N\in\N$ and  $ \ell_{-N}\le \dotsm \le  \ell_{-1}\le \ell_0=0 \le \ell_1\le \dotsm\le \ell_N$   and strictly positive reals $r_{-K}, \dotsc, r_K$. 
  Define the event 
\be\label{Bze8} \begin{aligned} 
  H^{\zeta, \eta}=H(\zeta, \eta) = % \{\nu: \tau^{\zeta, \eta}_0=0\,\} &\cap
   &\bigcap_{1\le i\le N}\bigl\{ \nu:  \tau^{\zeta, \eta}_{-i}\le \ell_{-i} \text{ and }  \tau^{\zeta, \eta}_{i}\ge\ell_i \bigr\}
   \\
   %%%%  Finite needed? 
 %\bigl\{ \nu: \,-\infty<\tau^{\zeta, \eta}_{-i}\le \ell_{-i} \text{ and } \ell_i\le \tau^{\zeta, \eta}_{i}<\infty \bigr\}\\  
   &\qquad 
   \cap
   \bigcap_{-K\le k\le K}\bigl\{ \nu:  \nu(\{k\}\times]\zeta, \eta]) < r_k\bigr\} 
\end{aligned}  \ee 
 on the space $\cM_{\Z \times \ri \Uset}$. %  of locally finite  measures $\nu$ on ${\Z \times \ri \Uset}$.   
  Note the monotonicity 
 \be\label{Bze-mon}
 H^{\zeta, \eta}\subset H^{\zeta', \eta'}\quad\text{ for } \ [\zeta', \eta']\subset [\zeta, \eta].
 \ee 
 Abbreviate $H^\xi=H^{\xi, \xi}$.     Recall the measures $q^{\alpha, \beta}$ defined in \eqref{qab4}. 
The analogous event under the measures $q^{\alpha, \beta}$ on the space $\Z^\Z\times[0,\infty)^\Z$  is denoted  by 
\be\label{Bze18} \begin{aligned} 
 H_q =\bigl\{ (\{\tau_i\}_{i\in\Z}, \{\Delta_k\}_{k\in\Z})\in \Z^\Z\times[0,\infty)^\Z :   \ &\tau_{-i}\le \ell_{-i} \text{ and } \tau_{i}\ge\ell_i \text{ for } i\in\lzb 1,N\rzb, \,  \\
    &\quad   \Delta_k< r_k\text{ for } k\in\lzb-K,K\rzb\bigr\}. 
 \end{aligned}\ee
 
 Fix $\zeta\prec\eta$ in $\ri\Uset$. % with   parameters   $\alpha(\zeta)<\alpha(\eta)$. 
  We prove the theorem by showing that  
 \be\label{Bze4} \begin{aligned} 
 Q_{(0,\xi)}(H^\xi)  =q^{\alpha(\xi)}(H_q) 
%\\ &=q^{\alpha(\xi)}\bigl\{\tau_{-i}\le \ell_{-i} \text{ and } \tau_{i}\ge\ell_i \text{ for } i\in[N], \,  \Delta_k< r_k\text{ for } i\in\lzb-K,K\rzb\bigr\} \\[4pt] 
 \qquad\text{for Lebesgue-almost every $\xi\in\,]\zeta, \eta]$.} 
% \qquad\text{for Lebesgue-almost every $\xi\in\ri\Uset$.}  
\end{aligned}  \ee
This equality comes from separate arguments for upper and lower bounds.  

\bigskip 

{\it Upper bound proof.}  
Define a sequence of nested partitions $\zeta=\zeta^n_0\prec\zeta^n_1\prec\dotsm\prec \zeta^n_n=\eta$.  For each $n$ and $\xi\in\,]\zeta, \eta]$,  let $]\zeta^n(\xi), \eta^n(\xi)]$ denote the unique interval $]\zeta^n_i, \zeta^n_{i+1}]$ that contains $\xi$.  Assume that, as $n\nearrow\infty$,   the mesh size $\max_i\abs{\zeta^n_{i+1}-\zeta^n_i} \to 0$. Consequently, for each $\xi\in\,]\zeta, \eta]$,  the intervals $]\zeta^n(\xi), \eta^n(\xi)]$ decrease to the singleton $\{\xi\}$. 

 

%stated as Theorem \ref{th:palm100}  in Appendix \ref{a:palm},  
The key step of this upper bound proof is that  for all $m$ and $i$ and Lebesgue-a.e.\ $\xi\in\,]\zeta, \eta]$, 
\be\label{79-43}\begin{aligned}  &Q_{(0, \xi)}(H^{\zeta^m_i, \zeta^m_{i+1}}) 
=  \lim_{n\to\infty}     \P\bigl\{ \Bppa \in H^{\zeta^m_i, \zeta^m_{i+1}} \,\big\vert\, \Bpp_{0}(\,]\zeta^n(\xi), \eta^n(\xi)]\,)\ge 1 \bigr\} .  
\end{aligned} \ee 
This limit is a special case of Theorem 6.32(iii) in Kallenberg \cite{Kal-17}, for the simple point process $\Bpp$ and  the sets $B_n=\{0\}\times(\zeta^n(\xi), \eta^n(\xi)]\searrow\{(0,\xi)\}$. 
  The proof given for  Theorem 12.8  in \cite{Kal-83} can also be used to establish this limit.    Theorem 12.8  of  \cite{Kal-83}  by itself is not quite adequate because we use the Palm kernel for the measure $\Bppa$ which is not the same as $\Bpp$.

 If we take $\xi\in \,]\zeta^m_i, \zeta^m_{i+1}]$, then for   $n\ge m$,   
 $]\zeta^n(\xi), \eta^n(\xi)]\subset \,]\zeta^m(\xi), \eta^m(\xi)]=\,]\zeta^m_i, \zeta^m_{i+1}]$.  Considering all $\xi$ in the union $]\zeta, \eta]=\bigcup_i \,]\zeta^m_i, \zeta^m_{i+1}]$, we have that  for any fixed $m$ and Lebesgue-a.e.\ $\xi\in\,]\zeta, \eta]$, 
 \begin{align*}
 Q_{(0, \xi)}(H^{\zeta^m(\xi), \eta^m(\xi)}) &=
  \lim_{n\to\infty} \P\bigl\{  \Bppa \in H^{\zeta^m(\xi), \eta^m(\xi)} \,\big\vert\, \Bpp_{0}(\,]\zeta^n(\xi), \eta^n(\xi)]\,)\ge 1 \bigr\}  \\[3pt] 
% & \lim_{n\to\infty} \P\bigl\{  \Bpp \in H^{\zeta^m_i, \zeta^m_{i+1}} \,\big\vert\, \Bpp_{0}(\zeta^n(\xi), \eta^n(\xi)]\ge 1 \bigr\}  \\[3pt] 
&  \le  
   \varliminf_{n\to\infty} \P\bigl\{  \Bppa \in H^{\zeta^n(\xi), \eta^n(\xi)} \,\big\vert\, \Bpp_{0}(\,]\zeta^n(\xi), \eta^n(\xi)]\,)\ge 1 \bigr\} .
   \end{align*} 
The inequality is due to \eqref{Bze-mon}.    
   
 Interpreting    \eqref{78-92}  in terms of the random measures $\Bppa$ and $\Bpp$ and referring to \eqref{Bze8} and  \eqref{Bze18} gives the identity 
\[ \P\bigl\{  \Bppa \in H^{\zeta^n(\xi), \eta^n(\xi)} \,\big\vert\, \Bpp_{0}(\,]\zeta^n(\xi), \eta^n(\xi)]\,)\ge 1 \bigr\}
=  q^{\alpha(\zeta^n(\xi)), \alpha(\eta^n(\xi))}(H_q).  \]
   %Equation  \eqref{78-92}  shows that  under the conditioned distribution   $\P\{\,\Bppa\in\bbullet\, \vert\, \Bpp_0(\zeta^n(\xi),\eta^n(\xi)] \ge 1\}$   the joint law  of $\{\tau^{\zeta^n(\xi), \eta^n(\xi)}_i\}_{i\in\Z}$ and  $\{\Bppa(\{k\}\times[\zeta^n(\xi), \eta^n(\xi)])\}_{k\in\Z}$ is  $q^{\alpha(\zeta^n(\xi)), \alpha(\eta^n(\xi))}$.  
%\timonote{Some caveats needed about open versus closed intervals?} 
 As $(\zeta^n(\xi), \eta^n(\xi)]\searrow\{\xi\}$, the   parameters converge:  $\alpha(\zeta^n(\xi)), \alpha(\eta^n(\xi))\to\alpha(\xi)$. 
Consequently the distribution $q^{\alpha(\zeta^n(\xi)), \,\alpha(\eta^n(\xi))}$
 converges to   $q^{\alpha(\xi)}$. 
Hence
 \begin{align*}
  \lim_{n\to\infty} \P\bigl\{  \Bppa \in H^{\zeta^n(\xi), \eta^n(\xi)} \,\big\vert\, \Bpp_{0}(\,]\zeta^n(\xi), \eta^n(\xi)]\,)\ge 1 \bigr\} 
  =q^{\alpha(\xi)}(H_q). 
%   \\  &\qquad 
%= q^{\alpha(\xi)}\bigl\{\tau_{-i}\le \ell_{-i} \text{ and } \tau_{i}\ge\ell_i \text{ for } i\in[N], \,  \Delta_i\le r_i\text{ for } i\in\lzb-N,N\rzb\bigr\}. 
\end{align*}  
 In summary, we have for all $m$   and Lebesgue-a.e.\ $\xi\in \,]\zeta, \eta]$, 
\be\label{79-46} \nn \begin{aligned} 
&Q_{(0, \xi)}(H^{\zeta^m(\xi), \eta^m(\xi)})  \le q^{\alpha(\xi)}(H_q). 
%\\ &\quad 
%\le  q^{\alpha(\xi)}\bigl\{\tau_{-i}\le \ell_{-i} \text{ and } \tau_{i}\ge\ell_i \text{ for } i\in[N],\,  \Delta_i\le r_i\text{ for } i\in\lzb-N,N\rzb\bigr\}. 
\end{aligned} \ee
Let $m\nearrow\infty$ so that $H^{\zeta^m(\xi), \eta^m(\xi)}\nearrow H^\xi$, to obtain the upper  bound  
\be\label{79-47} \begin{aligned} 
&Q_{(0, \xi)}(H^\xi)   \le q^{\alpha(\xi)}(H_q) 
%\\
%%&=Q_{(0, \xi)}(H^{\zeta^m_i, \zeta^m_{i+1}})\\[3pt] 
%%&
%&\quad
%\le  q^{\alpha(\xi)}\bigl\{\tau_{-i}\le \ell_{-i} \text{ and } \tau_{i}\ge\ell_i \text{ for } i\in[N],  \,  \Delta_i\le r_i\text{ for } i\in\lzb-N,N\rzb\bigr\}. 
\end{aligned} \ee
for Lebesgue-a.e.\ $\xi\in \,]\zeta, \eta]$.  
 
\bigskip 

{\it Lower bound proof.} 
%Fix $\zeta\prec\eta$ in $(e_2, e_1)$  with  parameters   $\underline\alpha=\alpha(\zeta)<\alpha(\eta)=\wb\alpha$.  
Let  $\zeta=\zeta_0\prec\zeta_1\prec\dotsm\prec \zeta_\ell=\eta$ be a  partition of the interval $[\zeta, \eta]$ and set  $\alpha_j=\alpha(\zeta_j)$. 

 In order to get an estimate below,  let $\mvec=(m_i)_{1\le\abs i\le N}$ be a $2N$-vector of 
  integers such that  $m_i<\ell_i$ for $-N\le i\le -1$ and $m_i>\ell_i$ for $1\le i\le N$. Define the  subset  $H^{\mvec}_q$ of $H_q$ from \eqref{Bze18} by truncating the coordinates $\tau_i$: 
\be\label{Bze20} \begin{aligned} 
 H^{\mvec}_q =\bigl\{ (\{\tau_i\}_{i\in\Z}, \{\Delta_k\}_{k\in\Z})\in \Z^\Z\times[0,\infty)^\Z :   \ &m_{-i}\le \tau_{-i}\le \ell_{-i} \text{ and }  \ell_i \le \tau_{i}\le m_i   \\
    &  \text{ for } i\in\lzb 1,N\rzb, \, \Delta_k< r_k\text{ for } k\in\lzb-K,K\rzb\bigr\}. 
 \end{aligned}\ee
%Let $\xi\in (\zeta, \eta)$. 

On the last line in the following computation, $c_1$ is a constant that depends on the parameters $\alpha(\zeta)$ and $\alpha(\eta)$ and on the quantities in \eqref{Bze20}:
\begin{align*}
&\int_{]\zeta,\eta]}  Q_{(0,\xi)}(H^\xi)\,\Bmm_0(d\xi)  = \sum_{j=0}^{\ell-1} \int_{]\zeta_j,\zeta_{j+1}]}  Q_{(0,\xi)}(H^\xi)\,\Bmm_0(d\xi) \\[4pt] 
&\ge \sum_{j=0}^{\ell-1} \int_{]\zeta_j,\zeta_{j+1}]}  Q_{(0,\xi)}(H^{\zeta_j,\zeta_{j+1}})\,\Bmm_0(d\xi)
%\\ &
=  \sum_{j=0}^{\ell-1} \E\bigl[  \Bpp_0(\,]\zeta_j,\zeta_{j+1}]\,)  \cdot \ind_{H^{\zeta_j,\zeta_{j+1}}}(\Bppa)  \bigr]  
 \\[4pt] 
 &\ge \sum_{j=0}^{\ell-1} 
 \P\bigl\{   \Bpp_0(\,]\zeta_j,\zeta_{j+1}]\,) \ge 1,\,   \Bppa\in H^{\zeta_j,\zeta_{j+1}}  \bigr\} \\
 &= \sum_{j=0}^{\ell-1}  \frac{\alpha_{j+1}-\alpha_j}{\alpha_{j+1}} \,q^{\alpha_j, \alpha_{j+1}}(H_q) 
 %\{ \tau_{-i}\le \ell_{-i} \text{ and } \tau_{i}\ge\ell_i \; \forall i\in\lzb1,N\rzb\}   \\&
\; \ge \; \sum_{j=0}^{\ell-1}  \frac{\alpha_{j+1}-\alpha_j}{\alpha_{j+1}} \,q^{\alpha_j, \alpha_{j+1}}(H^{\mvec}_q) 
 %\{ m_i\le \tau_{-i}\le \ell_{-i} \text{ and } \ell_i\le \tau_{i}\le m_i \; \forall i\in\lzb1,N\rzb\}   
 \\ &
 \ge \sum_{j=0}^{\ell-1}  \frac{\alpha_{j+1}-\alpha_j}{\alpha_{j+1}} \, q^{\alpha_{j+1}} (H^{\mvec}_q) \cdot \bigl(1-c_1(\alpha_{j+1}-\alpha_j)\bigr) .  
 %\{ m_i\le \tau_{-i}\le \ell_{-i} \text{ and } \ell_i\le \tau_{i}\le m_i \; \forall i\in\lzb1,N\rzb\}.
\end{align*} 
The steps above come as follows.  The second equality uses the characterization \eqref{79-50-50}  of  the kernel $Q_{(0,\xi)}$. 
The third equality is from \eqref{78-92}.    The second last inequality  is from $H^{\mvec}_q\subset H_q$.    The last inequality is from Lemma \ref{lm:palm10} below, which is valid once the mesh size $\max(\alpha_{j+1}-\alpha_j)$ is small enough relative to the numbers $\{m_i, \ell_i\}$.  

The function $\alpha\mapsto q^\alpha (H^{\mvec}_q)$ is continuous in the Riemann sum approximation on the last line of the calculation above. 
Let $\max(\alpha_{j+1}-\alpha_j)\to 0$ to obtain the inequality
 \begin{align*}
&\int_{]\zeta,\eta]}  Q_{(0,\xi)}(H^\xi) \,\Bmm_0(d\xi)
\ge   \int_{\alpha(\zeta)}^{\alpha(\eta)}  q^\alpha (H^{\mvec}_q) \,\frac{d\alpha}\alpha 
= \int_{]\zeta,\eta]}   q^{\alpha(\xi)}  (H^{\mvec}_q)\,\Bmm_0(d\xi). 
\end{align*} 
Let $m_i\searrow-\infty$ for $-N\le i\le -1$ and $m_i\nearrow\infty$ for $1\le i\le N$.  
The above turns into 
\be\label{79-104} \begin{aligned}
\int_{]\zeta,\eta]}  Q_{(0,\xi)}(H^\xi)\,\Bmm_0(d\xi) 
\ge 
 \int_{]\zeta,\eta]}   q^{\alpha(\xi)}  (H_q)\,\Bmm_0(d\xi). 
\end{aligned}  \ee

\medskip

The upper bound \eqref{79-47} and the lower bound \eqref{79-104} together imply the conclusion \eqref{Bze4}. 
 \end{proof} 
 
 The proof of Theorem \ref{th:B-palm1} is complete once we verify the auxiliary lemma used in the calculation above. 
 
\begin{lemma} \label{lm:palm10} 
Let the event $H^{\mvec}_q$ be as defined in  \eqref{Bze20}. 
% Fix a positive integer $N$ and integers $m_i<\ell_i<0$ for $-N\le i\le 1$ and $m_i>\ell_i>0$ for $1\le i\le N$.  
 Fix $0<\underline\alpha<\wb\alpha<1$.  Then there exist constants  $\e, c_1\in(0,\infty)$    such that 
\begin{align*}
q^{\alpha, \beta}(H^{\mvec}_q) \ge q^{\beta}(H^{\mvec}_q) \cdot \bigl(1-c_1(\beta-\alpha)\bigr) 
%&q^{\alpha, \beta}\{ m_i\le \tau_{-i}\le \ell_{-i} \text{ and } \ell_i\le \tau_{i}\le m_i \; \forall i\in\lzb1,N\rzb\} \\
%&\ge \bar q \{ m_i\le \tau_{-i}\le \ell_{-i} \text{ and } \ell_i\le \tau_{i}\le m_i \; \forall i\in\lzb1,N\rzb\}
\end{align*}
for  all $\alpha,\beta\in[\underline\alpha,\wb\alpha]$ such that $\alpha\le\beta\le\alpha+\e$.    The constants  $\e, c_1\in(0,\infty)$   depend on $\underline\alpha$,  $\wb\alpha$, and  the parameters $\ell_i, m_i$ and $r_k$  in \eqref{Bze20}. 
\end{lemma} 

\begin{proof} Let 
\begin{align*} 
\cA=  \bigl\{ &\pvec=(p_i)_{-N\le i\le N} \in\Z^{2N+1} :   p_0=0, \, p_i<p_j \text{ for } i<j, \\
&\qquad \qquad\qquad
m_{-i}\le p_{-i} \le \ell_{-i} \text{ and } \ell_i\le p_{i}\le m_i \; \forall i\in\lzb1,N\rzb\bigr\}
\end{align*}
be the relevant  finite set of    integer-valued $(2N+1)$-vectors for  the decomposition below.   For each  $\pvec\in\cA$ let  $\cK(\pvec)=\{p_i: i\in\lzb-N,N\rzb,  p_i\in \lzb-K,K\rzb\}$ be the set of coordinates of $\pvec$  in $\lzb-K,K\rzb$.  Abbreviate  $b_i=p_{i+1}-p_i$. 
Recall that, under $q^{\alpha, \beta}$, $\tau_0=0$, that $\Delta_k<r_k$ holds with probability one if $k\notin\{\tau_i\}$,  and the independence in \eqref{qab6}.    The factors $d_k>0$ below that satisfy  $ 1-e^{-\alpha r_k} \ge (1-e^{-\beta r_k}) (1- d_k(\beta-\alpha))$ can be chosen uniformly for $\alpha\le\beta$ in $[\underline\alpha,\wb\alpha]$, as functions of $\underline\alpha$, $\wb\alpha$, and $\{r_k\}$. Now compute: 
%come from applying the mean value theorem to the function  $f_k(x)=\frac{1-e^{x r_k}}{1-e^{\beta r_k}}$ that satisfies $f_k(\beta)=1$. 
\begin{align*}
&q^{\alpha, \beta}(H^{\mvec}_q)
=q^{\alpha, \beta}\bigl\{ m_i\le \tau_{-i}\le \ell_{-i} \text{ and } \ell_i\le \tau_{i}\le m_i \; \forall i\in\lzb1,N\rzb, \,   \Delta_k< r_k\text{ for } k\in\lzb-K,K\rzb\bigr\} \\[4pt] 
&\qquad=\sum_{\pvec\,\in\,\cA}  q^{\alpha, \beta}\bigl\{   \tau_{i}=p_i \text{ for }  i\in\lzb-N,N\rzb, \,   \Delta_k< r_k\text{ for } k\in\lzb-K,K\rzb\bigr\}
\\[4pt] 
&\qquad=\sum_{\pvec\,\in\,\cA}  q^{\alpha, \beta}\bigl\{   \tau_{i+1}-\tau_{i}=b_i \ \forall i\in\lzb-N,N-1\rzb\bigr\}  \cdot \prod_{k\,\in\,\cK(\pvec)}  (1-e^{-\alpha r_k})  \\
&\qquad\ge\sum_{\pvec\,\in\,\cA} \; \biggl( \; \prod_{i=-N}^{N-1}  C_{b_i-1}\,  \frac{\alpha^{b_i-1}\beta^{b_i}}{(\alpha+\beta)^{2b_i-1}}  \biggr)  
 \cdot \prod_{k\,\in\,\cK(\pvec)}  (1-e^{-\beta r_k}) \bigl(1- d_k(\beta-\alpha)\bigr)  \\
&\qquad\ge \sum_{\pvec\,\in\,\cA} \;  \biggl( \; \prod_{i=-N}^{N-1}  C_{b_i-1}\,  \biggl(\frac12\biggr)^{2b_i-1} \biggr) \biggl(\; \prod_{k\,\in\,\cK(\pvec)}  (1-e^{-\beta r_k}) \biggr) \cdot \bigl(1-c_1(\beta-\alpha)\bigr)   \\
&\qquad=\sum_{\pvec\,\in\,\cA}  q^\beta\bigl\{   \tau_{i+1}-\tau_{i}=b_i \ \forall i\in\lzb-N,N-1\rzb, \,   \Delta_k< r_k\text{ for } k\in\lzb-K,K\rzb\bigr\} 
% \biggl(\; \prod_{k\,\in\,\cK(\pvec)} (1-e^{-\beta r_k}) \biggr) \cdot \bigl(1-c_1(\beta-\alpha)\bigr) 
 \cdot \bigl(1-c_1(\beta-\alpha)\bigr) \\
%&= q^\beta \bigl\{ m_i\le \tau_{-i}\le \ell_{-i} \text{ and } \ell_i\le \tau_{i}\le m_i \; \forall i\in\lzb1,N\rzb \,   \Delta_i< r_i\text{ for } i\in\lzb-N,N\rzb\bigr\} \cdot \bigl(1-c_1(\beta-\alpha)\bigr)\\
&\qquad= q^\beta(H^{\mvec}_q) \cdot \bigl(1-c_1(\beta-\alpha)\bigr). 
\end{align*}
To get  the  inequality above, (i)  apply   Lemma \ref{a:lm:t500} to the first factor in parentheses with  $\e$ chosen    so that $0<\e<\underline\alpha/b_i$ for all $\pvec\in\cA$, and (ii)   set $c_1= \sum_{k=-K}^K  d_k$. 
%=\max_{\pvec\in\cA}\sum_{k\,\in\,\cK(\pvec)}  d_k$
\end{proof} 

%
%Homogeneity of the law of $\Bppa$ implies the following result.
%
%\begin{corollary} \label{cor:shift}
%For any integer $k \in \Z$ and Lebesgue-almost every $\xi \in \ri \Uset$ and for any Borel set $A \subset \{0,1\}^{\Z}$,
%\begin{align*}
%Q_{(k,\xi)}\left( (\Bpp_{k+\ell}\{\xi\}: \ell \in \bbZ) \in A \right) &= Q_{0,\xi}\left((\Bpp_{\ell}\{\xi\}: \ell \in \Z) \in A \right).
%\end{align*}
%\end{corollary}
% 

In the proofs that follow, we denote the indicators of the locations of the positive atoms of a measure $\nu\in\cM_{\Z\times\ri\Uset}$ by 
$u_k(\nu,\xi) = u_k(\xi)=\ind[\nu\{(k,\xi)\}>0]$ for $(k,\xi)\in\Z\times\ri\Uset$.  Applied to the random measure $\Bppa$ this gives $u_k(\Bppa, \xi)=\Bpp_k(\xi)$.

\begin{lemma} \label{lem:palmrw}
For Lebesgue-almost every $\xi\in\ri\Uset$   and all $m\in\Z$, 
 \be\label{rw123}  Q_{(m,\xi)}\bigl[ \nu :  \{\umeas_{m+k}(\nu,\xi)\}_{k\in\Z} \in A\bigr]  
 = \bfP(A)
 \ee
 for all Borel sets $A\subset\{0,1\}^\Z$. \end{lemma}
\begin{proof}
For $m=0$, \eqref{rw123} comes from a comparison of \eqref{rw113} and \eqref{rw117}.   For general $m$ it then  follows from the shift-invariance of the weights $\w$. 
\end{proof}

\begin{proof}[Proof of Theorem \ref{thm:ladder-xi}]


%%%%%  Below attempt to explain more -- perhaps not needed? 
%To generalize to arbitrary $m$, observe that, 
%as a function of the weights $\w$, the random measure $\Bppa$ satisfies  
%$ \Bppa^{T_{j,0}\w} =  \Bppa^\w\circ\theta_j^{-1}$ for  the shift $\theta_j(k, \zeta)=(k+j, \zeta)$ on the space   $\Z\times\ri\Uset$.  Similarly for $\Bpp$. This gives 
%\eqref{rw123}.   Through \eqref{79-5--50} this leads to 
%This gives 
%\be\label{37-02}     Q_{(k,\xi)} =  Q_{(k+j,\xi)}\circ(\theta_j^*)^{-1}\qquad \text{for Lebesgue-a.e. } \xi \ee
%where the mapping $theta_j^*$ on $\cM_{\Z\times\ri\Uset}$ is 

%This comes from a direct computation. By corollary \ref{cor:shift} it suffices to consider the case of $k=0$. Theorem \ref{th:B-palm1} says that under $Q_{(0,\xi)}$, $\{\tau^\xi(i+1)-\tau^\xi(i):i\in\Z\}$ is an i.i.d.\ sequence with marginal probability  mass function
%	\begin{align}\label{Catalan-pmf}
%	f_{\tau^\xi}(n)=C_{n-1}\,\frac1{2^{2n-1}},\quad n\in\N.
%	\end{align}
% The distances between the locations of the zeros of a simple symmetric random walk $S_n$ is an i.i.d.\ sequence with marginal  probability  mass function $f(2n-1)=0$ and
%	\[f(2n)=P(S_1\ne0,\dotsc,S_{2n-1}\ne0,S_{2n}=0)
%	%={2n\choose n}\frac1{2^{2n}}=f_{\tau^\xi}(n).\]
%%=2\cdot\frac12\cdot f_\sigma(2n-1) (with \zeta=\eta=\xi)
%	=\frac1{2n-1}{2n-1\choose n}\frac1{2^{2n-1}}=f_{\tau^\xi}(n),\quad n\in\N.\]
%(See for example equation III.3(3.7)  in Feller \cite{Fel-68}.) The claim follows.
 
Take $A\subset\{0,1\}^\Z$ as in the statement of Theorem \ref{thm:ladder-xi}.  Fix   $\zeta \prec \eta $ in  $\ri \Uset$ and let $N \in \bbN$.   %Recall the notation $u_k(\xi)=u_k(\nu, \xi)=\ind[\nu\{(k,\xi)\}>0]$. 
We restrict the integrals below to the compact set $[-N,N] \times [\zeta,\eta]$ with the indicator 
\[  g(k,\xi,\Bppavar) = \one_{[-N,N]\times [\zeta,\eta]}(k,\xi) \] 
  and then define on  $\Z \times \ri \Uset \times \sM_{\Z \times \ri \Uset} $
\begin{align*}
%g(k,\xi,\Bppavar) = \one_{[-N,N]\times [\zeta,\eta]}(k,\xi)
%\quad \text{and}\quad
f(k,\xi,\Bppavar) &= g(k,\xi,\Bppavar) \cdot \one_{\{(u_\ell\{\xi\} : \ell \in \Z) \,\in\, A\}}(\xi,\Bppavar).
%f(k,\xi,\Bppavar) &= \one_{[-N,N]\times [\zeta,\eta]}(k,\xi) \one_{\{(\Bppavar_\ell\{\xi\} : \ell \in \Z) \in A\}}(\xi,\Bppavar), \quad \text{and}\quad g(k,\xi,\Bppavar) = \one_{[-N,N]\times [\zeta,\eta]}(k,\xi).
\end{align*}
  By the definition  \eqref{79-50-50} of the Palm kernel,  
\begin{align*}
&\E\left[\;\int_{\Z \times \ri \Uset} f(k,\xi,\Bppa) \,\Bpp(dk \otimes d\xi )\right] %&= \int_{\Z \times \ri \Uset} \int_{\sM_{\Z \times \ri \Uset}} \one_{[-N,N]\times [\zeta,\eta]}(k,\xi) \one_{\{(\Bppavar_\ell\{\xi\} : \ell \in \Z) \in A\}}(\xi,\Bppavar) Q_{(k,\xi)}(d\Bppavar) \widetilde{\Bmm}(dk \otimes d\xi) \\
= \int_{[-N,N] \times [\zeta,\eta]} Q_{(k,\xi)}\{(u_\ell\{\xi\} : \ell \in \Z) \in A\} \,\widetilde{\Bmm}( dk \otimes d\xi) \\
&\qquad\qquad\qquad=\int_{[-N,N] \times [\zeta,\eta]} Q_{(k,\xi)}\{(u_{k+\ell}\{\xi\} : \ell \in \Z) \in A\} \,\widetilde{\Bmm}(dk \otimes d\xi) \\
&\qquad\qquad\qquad
= \int_{[-N,N] \times [\zeta,\eta]} \widetilde{\Bmm}(dk \otimes d\xi) = \E\left[\;\int_{\Z \times \ri \Uset} g(k,\xi,\Bppa) \Bpp(dk \otimes d\xi )\right].
\end{align*}
The second equality used shift-invariance of $A$ and  the third equality used \eqref{rw123} and $\bfP(A)=1$. %and in both we have taken the notational convention $\Bppavar_\ell\{\xi\} = \Bppavar(\{\ell\}\times \{\xi\})$ for $\Bppavar \in \sM_{\Z\times \ri \Uset}$. 
The left-hand side and the right-hand side are both finite because the integrals are restricted to the compact set $[-N,N] \times [\zeta,\eta]$. Since $\Bpp$ is a positive random measure, it follows that
\begin{align*}
\bbP\left(\;\int_{\Z \times \ri \Uset} f(k,\xi,\Bppa) \,\Bpp(dk \otimes d\xi ) = \int_{\Z \times \ri \Uset} g(k,\xi,\Bppa) \,\Bpp(dk \otimes d\xi )\right)=1.
\end{align*}
As $\zeta,\eta,$ and $N$ were arbitrary, we conclude that $\P$-almost surely   $(\Bpp_\ell\{\xi\} : \ell \in \Z) \in A$ for all $(k,\xi)\in\Z\times\ri\Uset$ such that $\Bpp\{(k,\xi)\}=1$.  Lemma \ref{lm:downright} applied to the $x$-axis ($x_i=ie_1$) then shows that $\xi\in\aUset$ if and only if   $\Bpp\{(k,\xi)\}=1$ for some $k$. 
%\begin{align*}
%\bbP\left(\forall (k,\xi) \in \Bpp, (\Bpp_\ell\{\xi\} : \ell \in \Z) \in A \right) &=1. \qedhere
%\end{align*}
\end{proof}


%\begin{proof}[Proof of Lemma \ref{LIL}]
%For $\xi\in\ri\Uset$ and a realization of $\Bpp$ let $f(\xi,\Bpp)=\one\{\Zerobar^{(0)}\in A\}$.
%The shift-invariance of $A$ says that we also have $f(\xi,\Bpp)=\one\{\Zerobar^{(k)}\in A\}$.
%	\[f(\xi,\Bpp)=\one\Bigl\{\varliminf_{n\to\infty}\frac{\sum_{i=0}^{n-1}\one\{(i,\xi)\in\Bpp\}}{\sqrt{2n/\log\log n}}=\varlimsup_{n\to\infty}\frac{\sum_{i=0}^{n-1}\one\{(i,\xi)\in\Bpp\}}{\sqrt{2n\log\log n}}=1\Bigr\}.\]
%Fix $k\in\Z$ and $\zeta\prec\eta$ in $\ri\Uset$. Given $\xi\in\ri\Uset$ and $\Bppavar\in\cM_{\Z \times \ri \Uset}$ define
%	\[\Zerobar^{(k)}_n(\xi,\Bppavar)=\begin{cases}  
%	-\sum_{i=k+n+1}^k \one\bigl\{\Bppavar\{(i,\xi)\}>0\bigr\}, &n<0, \\[3pt]  0, &n=0,\\[3pt] 
%	\sum_{i=k+1}^{k+n}\one\bigl\{\Bppavar\{(i,\xi)\}>0\bigr\}, &n>0.  \end{cases}\] 
%For a set $A\subset\Z_+^\Z$ define the function $f$ on $\ri\Uset\times\cM_{\Z \times \ri \Uset}$ by
%	\[f(\xi,\Bppavar)=\one_{[\zeta,\eta]}(\xi)\one\{\Zerobar^{(0)}(\xi,\Bppavar)\in A\}.\]
%Apply \eqref{79-50-50} to get
%	\[\E\Bigl[\int\one_{[\zeta,\eta]}(\xi)f(\xi,\Bpp)\,\Bpp_k(d\xi)\Bigr]=\int\one_{[\zeta,\eta]}(\xi)\int f(\xi,\Bpp)\,Q_{(k,\xi)}(d\Bpp)\,\Bmm_k(d\xi).\]
%	\[\E\Bigl[\int\one_{[\zeta,\eta]}(\xi)\one\{\Zerobar^{(0)}(\xi,\Bppa)\in A\}\,\Bpp_k(d\xi)\Bigr]=\int\one_{[\zeta,\eta]}(\xi)\,Q_{(k,\xi)}\bigl\{\Bppavar:\Zerobar^{(0)}(\xi,\Bppavar)\in A\bigr\}\,\Bmm_k(d\xi).\]
%By the invariance \eqref{Ainv} of $A$ we have $\{\Zerobar^{(0)}\in A\}=\{\Zerobar^{(k)}\in A\}$.
%Thus $Q_{(k,\xi)}\{\Zerobar^{(0)}\in A\}=Q_{(k,\xi)}\{\Zerobar^{(k)}\in A\}$, which by Corollary \ref{cor:ladder-xi} equals $\bfP(A)=1$. Hence, we have
%	\[\E\Bigl[\int\one_{[\zeta,\eta]}(\xi)\one\{\Zerobar^{(0)}(\xi,\Bppa)\in A\}\,\Bpp_k(d\xi)\Bigr]=\E\Bigl[\int\one_{[\zeta,\eta]}(\xi)\,\Bpp_k(d\xi)\Bigr].\]
%But since the integral on the left-hand side is bounded above by the integral on the right-hand side, we get that $\P$-almost surely
%	\[\int\one_{[\zeta,\eta]}(\xi)\one\{\Zerobar^{(0)}(\xi,\Bppa)\in A\}\,\Bpp_k(d\xi)=\int\one_{[\zeta,\eta]}(\xi)\,\Bpp_k(d\xi),\]
%for any $k\in\Z$ and $\zeta\prec\eta$ in $\bbQ^2\cap\ri\Uset$. This implies that $\P$-almost surely, $\one\{\Zerobar^{(0)}(\xi,\Bppa)\in A\}=1$, for $\Bpp$-almost every $\xi$.
%But $\Bpp$ is supported exactly on $\aUset$. The lemma is proved.
%\end{proof}

%\begin{lemma}
%Suppose that $\Delta$ is a random variable with probability mass function given by 
%\[P(\Delta  = n) &= C_{n-1} \,\frac{1}{2^{2n-1}}, \quad n\in\N.\]
%Then for $\lambda \geq 0$,
%\[E[e^{-\lambda\Delta}] = 1 - \sqrt{1- e^{-\lambda}}.\]
%\end{lemma}
%
%\begin{proof}
%Using the generating function for the Catalan numbers, we see that
%\[E[e^{-\lambda \Delta}] = 2 \sum_{n=1}^\infty C_{n-1} \,(e^{-\lambda}/4)^n = \frac{e^{-\lambda}}{2} \sum_{k=0}^\infty C_k ]\,(e^{-\lambda}/4)^k =  1-\sqrt{1-e^{-\lambda}}.\]
%\end{proof}


\begin{lemma}\label{lm:UB-aux}
Assume \eqref{exp-assump}.
Then for any $\delta\in(0,1)$, $n\in\N$, and $\zeta\in\ri\Uset$ we have
	\[\P\Bigl\{\exists\xi\in[\zeta,e_1[\,: \Bpp( \lzb0,n\rzb\times\{\xi\}) 
	%\sum_{i=0}^n\one\{(i,\xi)\in\Bpp\}	
	>2\delta n+1\Bigr\}\le 2(n+1)\Bigl(\frac{(1-\delta/2)^{2-\delta}}{(1-\delta)^{1-\delta}}\Bigr)^{n}\log\alpha(\zeta)^{-1}.\]
\end{lemma}

\begin{proof}
Let $\{\Delta_j\}_{j\in\N}$ be i.i.d.\ random variables with probability mass function 
$p(n)=C_{n-1}{2^{1-2n}}$  for $n\in\N$.  
%\eqref{Catalan-pmf}.
For $k\in\lzb 0,n\rzb$ and $\xi\in\ri\Uset$ use a union bound, translation, and  \eqref{rw113} %and Corollary \ref{cor:ladder-xi} 
to write
	\begin{align*}
	&Q_{(k,\xi)}\Bigl\{\,\sum_{i=0}^n u_i(\xi)>2\delta n+1\Bigr\}
	\le Q_{(k,\xi)}\Bigl\{\,\sum_{i=k-n}^{k+n} u_i(\xi)>2\delta n+1\Bigr\}\\
	&\quad= Q_{(0,\xi)}\Bigl\{\,\sum_{i=-n}^n u_i(\xi)>2\delta n+1\Bigr\}\\
	&\quad\le Q_{(0,\xi)}\Bigl\{\,\sum_{i=1}^n u_i(\xi)>\delta n\Bigr\}
	+ Q_{(0,\xi)}\Bigl\{\,\sum_{i=-n}^{-1} u_i(\xi)>\delta n\Bigr\}
	%\\&\quad
	\le 2P\Bigl\{\,\sum_{j=1}^{\ce{\delta n}}\Delta_j\le n\Bigr\}.
	\end{align*}
Using 
%\addmath{reference?}
the generating function $f(s)=\sum_{n\ge 0} C_ns^n=\tfrac12(1-\sqrt{1-4s}\,)$   of Catalan numbers we obtain for $0<s<1$, 
	\begin{align*}
	P\Bigl\{\,\sum_{j=1}^{\ce{\delta n}}\Delta_j\le n\Bigr\}
	&\le s^{-n}E[s^{\Delta}]^{\delta n}
	= s^{-n} \Bigl(2\sum_{n=1}^\infty C_{n-1} \,(s/4)^n\Bigr)^{\delta n}\\ 
	&= s^{-n}\Bigl(\,\frac{s}{2} \sum_{k=0}^\infty C_k \,(s/4)^k\Bigr)^{\delta n} 
	=  s^{-n}\bigl(1-\sqrt{1-s}\bigr)^{\delta n}.
	\end{align*}
%4(1-\delta)<4-4\delta+\delta^2
Take  $s=\frac{4(1-\delta)}{(2-\delta)^2}<1$  in the upper bound above to get
	\[Q_{(k,\xi)}\Bigl\{\,\sum_{i=0}^n u_i(\xi)>2\delta n+1\Bigr\}\le 2\Bigl(\frac{(1-\delta/2)^{2-\delta}}{(1-\delta)^{1-\delta}}\Bigr)^{n}.\]
	%(1-\sqrt{1-s})^\delta/s=(1-\delta/(2-\delta))^\delta \cdot (2-\delta)^2/(4(1-\delta)) 
	%=2^{\delta-2}(1-\delta)^{\delta-1}(2-\delta)^{2-\delta}
Apply \eqref{79-50-50} to write
	\begin{align*}
	&\E\Bigl[\,\int_{\ri\Uset}\one\{\xi\in[\zeta,e_1[\,\}\cdot\one\bigl\{
	\Bpp( \lzb0,n\rzb\times\{\xi\})
	%\,\sum_{i=0}^n\one\{(i,\xi)\in\Bpp\}
	>2\delta n+1\bigr\}\,\Bpp_k(d\xi)\Bigr]\\
	&\qquad=\int_{\ri\Uset} \one\{\xi\in[\zeta,e_1[\,\}\,Q_{(k,\xi)}\Bigl\{\,\sum_{i=0}^n u_i(\xi) >2\delta n+1\Bigr\}\,\Bmm_k(d\xi)\\
	&\qquad\le 2\Bigl(\frac{(1-\delta/2)^{2-\delta}}{(1-\delta)^{1-\delta}}\Bigr)^{n}\int_{\ri\Uset}\one\{\xi\in[\zeta,e_1[\,\}\Bmm_k(d\xi)
	%\\&\qquad
	\overset{\eqref{Bmm}}= 2\Bigl(\frac{(1-\delta/2)^{2-\delta}}{(1-\delta)^{1-\delta}}\Bigr)^{n}\log\alpha(\zeta)^{-1}.
	\end{align*}
To complete the proof, add over $k\in\lzb0,n\rzb$ and observe that
	\begin{align*}
	&\int_{\ri\Uset}\one\{\xi\in[\zeta,e_1[\,\}\one\bigl\{
	\Bpp( \lzb0,n\rzb\times\{\xi\})
	%\,\sum_{i=0}^n\one\{(i,\xi)\in\Bpp\}
	>2\delta n+1\bigr\}\sum_{k=0}^n\Bpp_k(d\xi)\\
	&\qquad\qquad\ge\one\Bigl\{\exists\xi\in[\zeta,e_1[\,:\Bpp( \lzb0,n\rzb\times\{\xi\})
	%\,\sum_{i=0}^n\one\{(i,\xi)\in\Bpp\}
	>2\delta n+1\Bigr\}.\qedhere
	\end{align*}
\end{proof}

\begin{proof}[Proof of Theorem \ref{thm:density-UB}]
The result follows from Theorem \ref{thm:density-UB2} below and the observation that 
for any $\e>0$, $\delta_n=2\sqrt{n^{-1}\log n}$
%$\delta_n=\sqrt{3n^{-1}\log n+(1+\e)n^{-1}\log\log n}$ 
satisfies the summability condition in that theorem. 
\end{proof}

\begin{theorem}\label{thm:density-UB2}
Assume \eqref{exp-assump} and fix $i\in\{1,2\}$. 
Consider a sequence $\delta_n\in(0,1)$ with $\sum n^2 e^{-n\delta_n^2}<\infty$. Then for any $\zeta\in\ri\Uset$
		\begin{align}\label{claim2-UB}
		\P\Bigl\{\exists n_0:\forall \xi\in[\zeta,e_2[,\forall n\ge n_0:\sum_{x\in\lzb0,n\rzb^2}\one\bigl\{\xi \in \supp\mu_{x,x+e_i}\bigr\}\le n^2\delta_n\Bigr\}=1.
		\end{align}
The same result holds when $\lzb0,n\rzb^2$ is replaced by any one of $\lzb-n,0\rzb^2$, $\lzb0,n\rzb\times\lzb-n,0\rzb$, or $\lzb-n,0\rzb\times\lzb0,n\rzb$.
\end{theorem}

\begin{proof}
Apply Lemma \ref{lm:UB-aux} and a union bound to get that for any $j\in\{1,2\}$, $\delta\in(0,1)$, $n\in\N$, and $\zeta\in\ri\Uset$,
	\[\P\Bigl\{\exists\xi\in[\zeta,e_1[\,:\sum_{x\in\lzb0,n\rzb^2}\rho^j_x(\xi) \ge(2\delta n+1)(n+1)\Bigr\}\le 2(n+1)^2\Bigl(\frac{(1-\delta/2)^{2-\delta}}{(1-\delta)^{1-\delta}}\Bigr)^{n}\log\alpha(\zeta)^{-1}.\]
A Taylor expansion gives 
	\[\log\Bigl(\frac{(1-\delta/2)^{2-\delta}}{(1-\delta)^{1-\delta}}\Bigr)
	=-\delta^2/4+\cO(\delta^3).\]
Thus, we see that for any $\zeta\in\ri\Uset$, for any sequence $\delta_n\in(0,1)$ such that $\sum n^2 e^{-n\delta_n^2}<\infty$, we have
	\[\P\Bigl\{\exists n_0\in\N:\forall \xi\in[\zeta,e_1[\,,\forall n\ge n_0:\sum_{x\in\lzb0,n\rzb^2}\rho^j_x(\xi)\le n^2\delta_n\Bigr\}=1.\]
The result for the other three sums comes similarly.
\end{proof}


==> JEMS Post-Accept Revision/GeoWebPaper-SecProblems.tex <==
% !TEX root = GeoWebPaper.tex

\section{Open problems}\label{sec:prob}  


%Equivalence of jump condition and V is cids. 

The list below contains some immediate open questions raised by the results of this paper. 
\begin{enumerate} %[label={\rm(\alph*)}, ref={\rm\alph*}] 
\itemsep=3pt 

\item Find tail estimates for the coalescence points $\coal{\xi}(x,y)$. 

\item
Theorem \ref{thm:Vcid}\eqref{thm:Vcid.2} showed that the jump process condition \eqref{cond:jumpcond} implies that $\aUset=\{\cid(T_x\w): x\in\Z^2\}$.  Is this implication an equivalence?  

\item 
Prove the jump process condition \eqref{cond:jumpcond}  for any  model other than the exactly solvable exponential and geometric cases.  

\item 
Does the web of instability have a scaling limit?  

\item 
Does the web of instability, with branching and coalescing  in exceptional directions, have any analogue in stochastic equations in continuous space and/or continuous time?    

 \item 
 Extend the statistics of instability points in the exponential model beyond a single line on the lattice. 
 
 \end{enumerate}  
